Safe asynchronous mixed-choice for timed interactions

Mixed-choice has long been barred from models of asynchronous communication since it compromises key properties of communicating finite-state machines. Session types inherit this restriction, which precludes them from fully modelling timeouts -- a key programming feature to handle failures. To address this deficiency, we present (binary) TimeOut Asynchronous Session Types ({TOAST}) as an extension to (binary) asynchronous timed session types to permit mixed-choice. {TOAST} deploy timing constraints to regulate the use of mixed-choice so as to preserve communication safety. We provide a new behavioural semantics for {TOAST} which guarantees progress in the presence of mixed-choice. Building upon {TOAST}, we provide a calculus featuring process timers which is capable of modelling timeouts using a $\mathtt{receive\text{-}after}$ pattern, much like Erlang, and informally illustrate the correspondence with TOAST specifications.

==> _abstract_only.tex <==

\title{Safe asynchronous mixed-choice for timed interactions
    % \thanks{EPSRC phd scholarship?}
}

\author{% ? cant get orcidID to compile
    Jonah Pears\inst{1} %\orcidID{0000-0003-4492-4072}%
    \and Laura Bocchi\inst{1} %\orcidID{0000-0002-7177-9395} %
    \and Andy King\inst{1} %\orcidID{0000-0001-5806-4822} %
}

\institute{%
    University of Kent, Canterbury, UK
    \\ \email{jjp38@kent.ac.uk}
    \\ \email{l.bocchi@kent.ac.uk}
    \\ \email{a.m.king@kent.ac.uk}
}

\maketitle
% ! can't use \and in \keywords{}, it just breaks
% https://tex.stackexchange.com/questions/351778/springers-middot-character
\def\middot{\textperiodcentered~}
\input{tex/main/abstract.tex}


==> _backups/_old_processes_listeners.tex <==
This section introduces an extension of the asynchronous calculus for timed processes~\cite{Bocchi2019}, catered for the new Timeout Session Types.

In definition that follows
\begin{inline}
   \item \epointp\ and \epointq\ are two endpoints
   %
   \item \pchan\ is a channel between two endpoints
   %
   \item \pchan\ is a channel between two endpoints
   %
   \item \bool\ is a boolean condition
   %
\end{inline}
\pbuffer\ is an ordered sequence of messages, functioning either as: a channel buffer; or, a list of messages to discard.
\prequeue\ is a sequence of messages waiting to be received, with branches added dynamically at run-time, and facilitates a process recalling to an earlier point and taking a different branch.
\precallcache\ is each an ordered list of the messages sent corresponding to each of the receiving branches able to trigger a recall; this is used to ensure that there are no messages left in the queue that are unable to be received.

The process variable \prcvar\ contains the following ordered sequences
\begin{inline}
   \item \setLabel\ of message labels
   %
   \item \setChan\ of session channels
   %
\end{inline}
\begin{equation*}
   \mproccescalc%
\end{equation*}
The following sections provide an in-depth description on the possible forms a process can take, with a focus on the new additions. Specific details and design decisions become clear when considered in the context of the reduction steps, shown later in~\cref{ssec:prc_reduction_rules}.

\subsubsection*{Sending Messages}\hfill\mbox{$\mpsendalways$}\mbox{ }\par%
As standard, a process \prc\ can send a message \msglabel\ on channel \pchan\ and continue as \qrc.
Sending actions such as these can now be accompanied by a set of branching receiving actions.

\paragraph*{Listening for Timeouts}\hfill\mbox{$\mpsendlisten$}\mbox{ }\par%
In additional to performing standard sending actions, a process can provide a set of messages that can potentially be received after this sending action, within $n$ time units, and pertain to a different viable branch.

These potential receptions are moved to a \emph{listener} process private to the sending individual, and is able to continue listen for, and receive, those messages arriving in the queue once the main thread has progressed onwards.

\subsubsection*{Listeners}\hfill\mbox{$\mprcrecall$}\mbox{ }\par%
A \emph{listener process} is a private to an individual, and runs in parallel to the main thread.
Messages accumulated by the listener correspond to the entry points to other branches this process could have possibly taken, in the case that the other participant has unknowingly taken one of these branches.

\paragraph*{Tidying Messages}\hfill\mbox{$\mathtt{tidy}:\mpbuffer$}\mbox{ }\par%
A listener process is always able to receive a special \texttt{tidy} message, which contains an ordered sequence of messages to be ignored from their queue.

\paragraph*{Message Logs}\hfill\mbox{$\mkset{\mprecallcache}$}\mbox{ }\par%
Each timeout message branch of the listener process is assigned a log that accumulates the messages sent by a participant since it was added to the listener.
\begin{note}
   Messages held in the listening process are referred to as \emph{timeout messages} (excluding the \texttt{tidy} message).
\end{note}

\subsubsection*{Receiving Messages}\hfill\mbox{$\mprecvuntil$}\mbox{ }\par%
As with the previous work, a message $\of{a}{i}$ can be received from a channel \pchan\ within $n$ time units, and continue as the corresponding $\of{\mprc}{i}$. However, in the case that a message isn't received on time, this not result in a run-time failure, as instead the process continues as \qrc.

Whenever the main thread of a process successfully receives a message, it is known that both participants are in compatible states.
Therefore any timeout message branches of the listener process are removed, and the log against them is cleared as well.

When a message is instead received by the listening process, corresponding to a timeout message branch, the process is required to make a recall; receiving the message and continuing as the relevant branch.
It is at this point that a special \texttt{tidy} message is sent to the other participant, detailing any messages sent pertaining to the other branch.
\begin{note}
   When $n=\infty$ the process can instead be written, omitting the $\mathtt{after}\;\mqrc$: $\mprecvalways$; yielding the same meaning as \qrc\ will have been reached.
\end{note}

% \subsubsection*{Timers}\hfill\mbox{$\mprctimer$}\mbox{ }\par%
% A process can utilise simple timers, and accumulate them in a separate thread $\mprctimers$. Individual timers can be reset to 0 via $\mprctimerreset$.

% \paragraph*{Evaluating Timers}\hfill\mbox{$\mprctimereval{n}$}\mbox{ }\par%
% The value of a timer can be evaluated against an integer $n\in\msetR_{\geq0}$, and a boolean is returned if it holds. The evaluations available are as standard
% \begin{inline}
%    \item $=$
%    \item $\neq$
%    \item $>$
%    \item $<$
%    \item $\geq$
%    \item $\leq$
% \end{inline}
% These can be utilised by the condition of an \texttt{if} statement.
% \begin{note}
%    These timers are distinct from the ones shown in the types, and represent simple timer implementations in languages such as \texttt{go} or \texttt{erlang}.
% \end{note}

% \subsubsection*{Unchanged}
The remaining cases are unchanged from~\cite{Bocchi2019}, briefly summarised:
$\mpscope$ is a scope restriction of process \prc\ between endpoints \epointp\ and \epointq.
%
$\mprcpar$ are parallel processes.
%
$\mifthenelse$ continues as \prc\ if \mbool\ is \ttrue, and \qrc\ if \tfalse.
%
$\mdelayfunc$ represents a time-consuming process with an expected runtime somewhere within \constr.
%
$\mpsetrec$ establishes a recursion point, taking the current ordered sequences of message labels, channels, and timers (and their values) and associating them with the continuation process \prc.
%
$\mpcallrec$ triggers a recursive call, returning the to the processes corresponding to this process variable.
%
$\mepointp\mepointq:\mpbuffer$ is the channel between two endpoints (\epointp\ and \epointq), with $\mpbuffer$ containing an ordered sequence of messages.
%
$0$ is the termination point.

\subsection{Reduction Rules}\label{ssec:prc_reduction_rules}
The reduction rules for processes is shown in~\cref{fig:processes_reduction_rules_main,fig:processes_reduction_rules_other}, extending the work of~\cite{Bocchi2019}.
\begin{figure}[htb]
   \input{tex/figs/process_reduction_rules_comm.tex}
   %
   \caption{Reduction rules for processes.}
   \label{fig:processes_reduction_rules_main}
\end{figure}

\begin{description}[itemsep=1.25ex,labelsep=2ex]
   %
   \item[$\rulem{Det}$] Allows \tval\ amount of time to pass over all parts of a process \prc, by applying time passing function \ptimefunc, as defined in~\cref{fig:processes_time_func}. The definition is such that it can be applied any amount of times and will result in a process able to make progress.
      %
      %
   \item[$\rulem{Recv}$] Allows a branching process to receive a message from the channel buffer, and continue as the relevant process.
      Once a message is successfully received from a participant, all timeout branches are removed as it is known that the other party is in the corresponding state, and that the participants are compatible.

      Messages must be received within $n$ time units; by \ptimefunc, if this is exceeded the processes continues as \qrc.
      %
      %
   \item[$\rulem{Send}$] For sending actions without unattended timeout receptions; a message is sent on channel \pchan, added to the end of the buffer.

      The message is added to the list of messages sent since the last received correspondence with the other party, with a separate list for every message possibly going to be received.
      %
      %
   \item[$\rulem{Listen}$] Before sending a message, any receptions $\of{b}{i}$ that could be received from this state in the future are added to a parallel processes private to the sender.

      Recall points are established for each new branch being monitored, enabling the process to return to this state and take one of these branches if one of these messages is received. Additionally, the list of messages sent since passing a branch is initialised with an empty set, ready to have the sending action added to it by \rulet{Send} when the sending action is performed at the next reduction step \emph(although a message being received on a branch between this point and that would also be handled successfully).
      %
      %
   \item[$\rulem{Recall}$] A message from the buffer of channel \pchan\ is received by the processes private \emph{listener}, indicating that the other participant is at an earlier point in the processes, and has taken a different branch.

      The recall point corresponding to the message received is called, and the processes continues on the corresponding branch. Additionally, the processes sends a special message containing all of the messages sent since this recall point was established, so that the other participant can safely discard those messages and avoid unspecified reception.
      %
      %
   \item[$\rulem{Tidy}$] A processes can receive a special message at any time which contains a list of messages to discard from the channels buffer. This indicates that their co-party had at some point continued on a different branch, but has now recovered and re-established compatibility.
      %
      %
\end{description}

\subsection{Time-passing Functions}
The \rulet{Delay}\ step allows time to pass over all processes of a system, and is defined inductively in~\cref{fig:processes_time_func}.
\begin{figure}[htb]
   \input{tex/figs/process_time_func.tex}
   %
   \caption{Inductive definition of the time-passing function \ptimefunc. All other cases are undefined.}
   \label{fig:processes_time_func}
\end{figure}

The auxiliary functions it depends on are unchanged from~\cite{Bocchi2019}, and a brief description for them is given below:
\begin{description}[itemsep=1.25ex,labelsep=2ex]
   \item[$\mathtt{Wait(\mprc)}$] Recursively expands processes until able to return a message that is waiting to be received given the value of \tval\ in the \ptimefunc\ that calls this function.
      %
      %
   \item[$\mathtt{NEQueue(\mprc)}$] Recursively expands a process until reaching an endpoint with a \emph{Non-Empty Queue}, otherwise returning the emptyset.
      %
      %
\end{description}

\begin{figure}[hp]
   \input{tex/figs/process_reduction_rules_other.tex}
   %
   \caption{Standard reduction rules.}
   \label{fig:processes_reduction_rules_other}
\end{figure}

\subsection{Typing Processes}

\begin{equation*}
   \mprocessjudge%
\end{equation*}

\pagebreak
\subsection{Constructing Processes}
Using the producer and consumer example from~\cref{fig:motiv_example_producer_consumer_diagram}, shown again below:
\vspace{2ex}
\begin{minipage}{\textwidth}\centering
   \begin{minipage}{0.44\textwidth}\centering
      \input{tex/figs/example_producer_consumer_diagram_single.tex}
   \end{minipage}
   \begin{minipage}{0.54\textwidth}\centering
      \input{tex/figs/example_producer_consumer_type.tex}
   \end{minipage}
\end{minipage}

Below are some processes possible given the typing above. The first would send stop immediately and terminate.
\begin{equation}
   \begin{array}{l}
      \mathtt{def}\;{A}^{\alpha}=%
      \mpvar\left(\emptyset,\left\{\mpchan\right\}\right)%
      \mathtt{in}\;%
      %
      \mpchan\,\mpsend\,\mathtt{stop}\,\left\{\emptyset\right\}%
      \,.\,%
      0%
   \end{array}
\end{equation}

While the second encapsulates the full behaviour described by the types, relying on some internal function $\mathtt{close}()$ to determine which branch is chosen.
\begin{equation}
   \begin{array}{l}
      \mathtt{def}\;{A}^{\alpha}=%
      \mpvar\left(\emptyset,\left\{\mpchan\right\}\right)%
      \mathtt{in:}\;%
      \\[1ex]\mbox{\hspace{4ex}}%
      %
      \left(\begin{array}{l}
                  %
                  \mathtt{if}\;%
                  \left(\mathtt{bool:close}()==\mtrue\right)%
                  \;\mathtt{then:}\;%
                  \\\mbox{\hspace{2ex}}%
                  %
                  \left(\begin{array}{l}
                        %
                        \mpchan\,\mpsend\,\mathtt{stop}\,%
                        \left\{\emptyset\right\}%
                        \,.\,%
                        0%
                     \end{array}\right)
                  \\[2ex]%
                  %
                  \mathtt{else:}%
                  \\\mbox{\hspace{2ex}}%
                  %
                  \left(\begin{array}{l}
                        %
                        \mpchan^{5}\,\mprecv\,\mathtt{data}%
                        \,.\,%
                        \left({A}^{\alpha}\right)%
                        %
                        \\\mbox{\hspace{2ex}}%
                        \mathtt{after}\;%
                        (\mpchan\,\mpsend\,\mathtt{TO}%
                        \,.\,%
                        (\mpchan\,\mprecv\,\mathtt{retry}%
                        \,.\,%
                        \left({A}^{\alpha}\right)))%
                     \end{array}\right)
               \end{array}\right)
      %
   \end{array}
\end{equation}

\endinput


































































\paragraph*{Processes}
Let
\begin{inline}
   \item $\mprc,\mprc', \mqrc$ range over processes
   %
   \item \pvar\ range over process variables
   %
   \item \setA\ be an ordered set of message labels
   %
   \item \setC\ be an ordered set of session channels
   %
   \item \psetX\ be the set of local clocks (distinct to the set of clocks \setX\ used in the syntax of types)
   %
\end{inline}

In definition that follows
\begin{inline}
   \item \epointp\ and \epointq\ are two endpoints
   %
   \item \pchan\ is a channel between two endpoints
   %
   \item \bool\ is a boolean condition
   %
   \item \pbuffer\ points to the head of a channels buffer (ordered chronologically)
   %
\end{inline}
\begin{equation*}
   % \hspace{-5ex}%
   \mproccescalc%
\end{equation*}
The following sections discusses all of the changes from the previous work of~\cite{Bocchi2019}. \REDO[i am unsure if i have formulated \opt\ correctly, will need to discuss]
\TODO[still need single actions even though they can be represented here?]
\TODO[is it wrong to enforce active() on actions?]

\subsection{New\TODO}

\subsubsection*{Choices and Options}
A process $\mprc=\mpchan\;\mopt$ describes that the channel \pchan\ will be used by one of the options taken in \opt.

\opt\ is structured

\begin{example}[Constructing Processes]
   Below is a modification of the type shown in~\cref{fig:motiv_example_producer_consumer_diagram}:
   \begin{equation*}
      \resizebox{\textwidth}{!}{$
            \mrec\,{{\mreclabel}^{Z}}%
            \,.\,%
            \left\{\def\arraystretch{1.7}%
            \begin{array}{l}%
               \mrecv\mathtt{ready}\,\left(1\leq x\leq 2,\,x\right)%
               \,.\,%
               \left\{\def\arraystretch{1.7}%
               \begin{array}{l}%
                  \msend\mathtt{latency}\,\left(y-x=2,\right)%
                  \,.\,%
                  {{\mreclabel}^{Z}}%
                  \,, \\%
                  %
                  %
                  \msend\mathtt{start}\,\left(x=2,\right)%
                  \,.\,%
                  \mrec\,{{\mreclabel}^{A}}%
                  \,.\,%
                  \left\{\def\arraystretch{1.7}%
                  \begin{array}{l}%
                     \msend\mathtt{cancel}\,\left(x\leq 2\right)%
                     \,.\,%
                     \mend%
                     \,, \\%
                     %
                     %
                     \mrecv\mathtt{done}\,\left(2\leq x\leq 5\right)%
                     \,.\,%
                     \msend\mathtt{ok}%
                     \,.\,%
                     \mend%
                     \,, \\%
                     %
                     %
                     \mrecv\mathtt{data}\,\left(2\leq x\leq 5\right)%
                     \,.\,%
                     {{\mreclabel}^{A}}%
                     \,, \\%
                     %
                     %
                     \mrecv\mathtt{error}\,\left(2\leq x\leq 6\right)%
                     \,.\,%
                     \msend\mathtt{restart}%
                     \,.\,%
                     {{\mreclabel}^{Z}}%
                     \,, \\%
                     %
                     %
                     \msend\mathtt{timeout}\,\left(6<x\right)%
                     \,.\,%
                     {{\mreclabel}^{Z}}%
                     %
                     %
                  \end{array}%
                  \right\}%
                  %
                  %
               \end{array}%
               \right\}%
               \,, \\%
               %
               %
               \msend\mathtt{close}\,\left(x=2.5\right)%
               \,.\,%
               \mend%
               %
               %
            \end{array}%
            \right\}%
         $}
   \end{equation*}

   Against a global clock $g$ (which can only be reset when a recursive call is made), the following graph can be constructed to represent the possible traces of viable sequences and timings of interactions:\newline
   \resizebox{\textwidth}{!}{%
      \begin{tikzpicture}
         % grid
         \draw (0,0) -- (8,0);%
         \draw (0,0) -- (0,10);%
         % draw horizontal
         \foreach \y in {1,...,10}%
            {%
               \draw[gray] (0,\y) -- (8,\y);%
               \node[left] at (0,\y) {\y};
            }%
         % draw vertical
         \foreach \x in {1,...,8}%
            {%
               \draw[gray] (\x,0) -- (\x,10);%
               \node[below] at (\x,0) {\x};
            }%

         % complete trace
         \filldraw [gray, opacity = 0.25, line width = 2pt]%
         (0,0) -- (2.5,2.5);%
         \filldraw [blue, opacity = 1, line width = 2pt]% ready
         (2,2) -- (1,1);%
         \filldraw [yellow, opacity = 0.25, line width = 0pt]% reset
         (0,1) -- (0,2) -- (2,2) -- (1,1);%
         \filldraw [gray, opacity = 0.25, line width = 0pt]%
         (0,1) -- (0,2) -- (1,3) -- (2,3);%
         \filldraw [red, opacity = 1, line width = 2pt]% latency
         (0,2) -- (8,10);%

         \filldraw [yellow, opacity = 0.25, line width = 0pt]% reset
         (0,3) -- (0,4) -- (2,4) -- (2,3);%
         \filldraw [red, opacity = 0.25, line width = 0pt]% cancel
         (0,3) -- (0,4) -- (2,6) -- (2,5);%
         \filldraw [blue, opacity = 0.25, line width = 0pt]% done
         (2,5) -- (2,6) -- (5,9) -- (5,8);%
         \filldraw [blue, opacity = 0.25, line width = 0pt]% data
         (2,5) -- (2,6) -- (5,9) -- (5,8);%
         \filldraw [blue, opacity = 0.25, line width = 0pt]% error
         (2,5) -- (2,6) -- (6,10) -- (6,9);%
         \filldraw [red, opacity = 0.25, line width = 0pt]% timeout
         (6,9) -- (6,10) -- (7,10);%

         % def z
         \draw[fill, cyan] (0,0) circle (4pt);
         \node[right] at (0.2, 0.5) {\Large $\mrec\,{{\mreclabel}^{Z}}$};

         % def a
         \draw[fill, cyan] (2,3) circle (4pt);
         \draw[fill, cyan] (2,4) circle (4pt);
         \filldraw [cyan, line width = 8pt] (2,3) -- (2,4);
         \node[right] at (2.2,3.5) {\Large $\mrec\,{{\mreclabel}^{A}}$};

         % send start
         \filldraw [red, opacity = 1, line width = 2pt]% start
         (2,4) -- (2,3);%

         % send close
         \filldraw [red, opacity = 1, line width = 2pt]%
         (2.5,2.5) circle (4pt);

         % axis labels
         \node[below] at (7.5,-0.5) {\Large $x,y,z\in\msetX$};
         \node[left] at (-0.5, 9.5) {\Large $g$};

         % % table of clock values: g
         % \node at (9, 10.5) {\Large $g$};
         % \node at (9, 10) {$10$};
         % \node at (9, 9) {$9$};
         % \node at (9, 8) {$8$};
         % \node at (9, 7) {$7$};
         % \node at (9, 6) {$6$};
         % \node at (9, 5) {$5$};
         % \node at (9, 4) {$4$};
         % \node at (9, 3) {$3$};
         % \node at (9, 2) {$2$};
         % \node at (9, 1) {$1$};
         % \node at (9, 0) {$0$};
         % % table of clock values: x
         % \node at (10, 10.5) {\Large $x$};
         % \node at (10, 10) {$(6,7)$};
         % \node at (10, 9) {$(5,6)$};
         % \node at (10, 8) {$(4,5)$};
         % \node at (10, 7) {$(3,4)$};
         % \node at (10, 6) {$(2,3)$};
         % \node at (10, 5) {$(1,2)$};
         % \node at (10, 4) {$2\mapsto 0$};
         % \node at (10, 3) {$\begin{array}{c}(1,2)\\2\mapsto 0\end{array}$};
         % \node at (10, 2) {$\begin{array}{c}(1,2)\\2\mapsto 0\end{array}$};
         % \node at (10, 1) {$1\mapsto 0$};
         % \node at (10, 0) {$0$};
         % % table of clock values: y
         % \node at (11, 10.5) {\Large $y$};
         % \node at (11, 10) {$10$};
         % \node at (11, 9) {$9$};
         % \node at (11, 8) {$8$};
         % \node at (11, 7) {$7$};
         % \node at (11, 6) {$6$};
         % \node at (11, 5) {$5$};
         % \node at (11, 4) {$4$};
         % \node at (11, 3) {$3$};
         % \node at (11, 2) {$2$};
         % \node at (11, 1) {$1$};
         % \node at (11, 0) {$0$};
      \end{tikzpicture}
   }

   Using the above graph, the following decision diagram can be extracted\TODO[work in progress]:\newline
   % \resizebox{\textwidth}{!}{%
   \resizebox{!}{20cm}{%
      \begin{tikzpicture}[
            every node/.style={xshift=0mm,yshift=0mm,draw,rectangle,rounded corners,fill=gray!20},
            %
            edge from parent/.style={
                  draw,->,
                  nodes={fill=blue!20,rectangle}
               },
            %
            end/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=black,text=white,circle},
                  level distance=20mm
               },
            %
            Zdef/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=green!40,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=green!30,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=30mm
               },
            %
            Zrec/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=green!60,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=green!50,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=35mm
               },
            %
            Adef/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=orange!40,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=orange!30,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=30mm
               },
            %
            Arec/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=orange!60,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=orange!50,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=35mm
               },
            % general actions
            act/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=white,rectangle,rounded corners},
                  edge from parent/.style={
                        draw,->,
                        nodes={fill=cyan!20,rectangle,xshift=0mm,yshift=2mm}
                     },
                  level distance=40mm
               },
            % middle actions in options
            optact/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=white,rectangle,rounded corners},
                  edge from parent/.style={
                        draw,->,
                        nodes={fill=cyan!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=45mm
               },
            % always actions
            allact/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=white,rectangle,rounded corners},
                  edge from parent/.style={
                        draw,->,
                        nodes={fill=cyan!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=35mm
               },
            % options
            opt/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=magenta!40,diamond},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=magenta!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=48mm
               },
            % nested options
            subopt/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=magenta!40,diamond},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=magenta!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=40mm
               }
         ]
         % root
         \node[act] {$
               \begin{array}{c}
                  g=0 \\% g
                  x=0 \\% x
                  y=0 % y
               \end{array}
            $}
         % def z
         child[Zdef] {
               node {$
                        \begin{array}{c}
                           g=0 \\% g
                           x=0 \\% x
                           y=0 % y
                        \end{array}
                     $}
               % recv ready
               child[act,grow=south west] {
                     node {$
                              \begin{array}{c}
                                 1\leq g\leq 2 \\% g
                                 x=0           \\% x
                                 1\leq y\leq 2 % y
                              \end{array}
                           $}
                     % send latency
                     child[act,grow=south west] {
                           node {$
                                    \begin{array}{c}
                                       2\leq g< 3 \\% g
                                       0\leq x< 2 \\% x
                                       2\leq y< 3 % y
                                    \end{array}
                                 $}
                           % rec z
                           child[Zrec] {
                                 node {$
                                          \begin{array}{c}
                                             g=0 \\% g
                                             x=0 \\% x
                                             y=0 % y
                                          \end{array}
                                       $}
                                 %
                                 edge from parent
                                 node {$
                                          {{\mreclabel}^{Z}}
                                       $}
                              }
                           %
                           edge from parent
                           node[left] {$
                                    \begin{array}{c}
                                       \msend\mathtt{latency}
                                       \\
                                       y-x=2
                                    \end{array}
                                 $}
                        }
                     % send latency or start
                     child[opt,grow=south] {
                           node {$
                                    \begin{array}{c}
                                       3\leq g\leq 4 \\% g
                                       x=2           \\% x
                                       3\leq y\leq 4 % y
                                    \end{array}
                                 $}
                           % send latency
                           child[act,grow=south west]  {
                                 node {$
                                          \begin{array}{c}
                                             3\leq g\leq 4 \\% g
                                             x=2           \\% x
                                             3\leq y\leq 4 % y
                                          \end{array}
                                       $}
                                 % rec z
                                 child[Zrec] {
                                       node {$
                                                \begin{array}{c}
                                                   g=0 \\% g
                                                   x=0 \\% x
                                                   y=0 % y
                                                \end{array}
                                             $}
                                       %
                                       edge from parent
                                       node {$
                                                {{\mreclabel}^{Z}}
                                             $}
                                    }
                                 % label
                                 edge from parent
                                 node[left] {$
                                          \begin{array}{c}
                                             \msend\mathtt{latency}
                                             \\
                                             y-x=2
                                          \end{array}
                                       $}
                              }
                           % send start
                           child[act,grow=south east]  {
                                 node {$
                                          \begin{array}{c}
                                             3\leq g\leq 4 \\% g
                                             x=0           \\% x
                                             3\leq y\leq 4 % y
                                          \end{array}
                                       $}
                                 % def a
                                 child[Adef,grow=south] {
                                       node {$
                                                \begin{array}{c}
                                                   3\leq g\leq 4 \\% g
                                                   x=0           \\% x
                                                   3\leq y\leq 4 % y
                                                \end{array}
                                             $}
                                       % send cancel
                                       child[act,grow=south west] {
                                             node {$
                                                      \begin{array}{c}
                                                         3\leq g\leq 6 \\% g
                                                         0\leq x\leq 2 \\% x
                                                         3\leq y\leq 6 % y
                                                      \end{array}
                                                   $}
                                             % end
                                             child[end] {
                                                   node {$\mend$}
                                                }
                                             %
                                             edge from parent
                                             node[left] {$
                                                      \begin{array}{c}
                                                         \msend\mathtt{cancel}
                                                         \\
                                                         x\leq 2
                                                      \end{array}
                                                   $}
                                          }
                                       % recv done, data or error
                                       child[opt,grow=south] {
                                             node {$
                                                      \begin{array}{c}
                                                         5< g\leq 9 \\% g
                                                         2< x\leq 5 \\% x
                                                         5< g\leq 9 % y
                                                      \end{array}
                                                   $}
                                             % recv done, data or error
                                             child[subopt,grow=south west] {
                                                   node {$
                                                            \begin{array}{c}
                                                               5< g\leq 9 \\% g
                                                               2< x\leq 5 \\% x
                                                               5< g\leq 9 % y
                                                            \end{array}
                                                         $}
                                                   % recv done
                                                   child[optact,grow=south west] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     5< g\leq 9 \\% g
                                                                     2< x\leq 5 \\% x
                                                                     5< g\leq 9 % y
                                                                  \end{array}
                                                               $}
                                                         % send ok
                                                         child[allact] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           5< g\leq 9 \\% g
                                                                           2< x\leq 5 \\% x
                                                                           5< g\leq 9 % y
                                                                        \end{array}
                                                                     $}
                                                               % end
                                                               child[end] {
                                                                     node {$\mend$}
                                                                  }
                                                               %
                                                               edge from parent
                                                               node[right] {$\msend\mathtt{ok}$}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[left] {$
                                                                  \begin{array}{c}
                                                                     \mrecv\mathtt{done},
                                                                     \\
                                                                     2<x\leq 5
                                                                  \end{array}$}
                                                      }
                                                   % recv data
                                                   child[optact,grow=south,level distance=45mm] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     5< g\leq 9 \\% g
                                                                     2< x\leq 5 \\% x
                                                                     5< g\leq 9 % y
                                                                  \end{array}
                                                               $}
                                                         % rec a
                                                         child[Arec] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           3\leq g\leq 4 \\% g
                                                                           x=0           \\% x
                                                                           3\leq y\leq 4 % y
                                                                        \end{array}
                                                                     $}
                                                               %
                                                               edge from parent
                                                               node {$
                                                                        {{\mreclabel}^{A}}
                                                                     $}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[midway] {$
                                                                  \begin{array}{c}
                                                                     \mrecv\mathtt{data},
                                                                     \\
                                                                     2<x\leq 5
                                                                  \end{array}
                                                               $}
                                                      }
                                                   % recv error
                                                   child[optact,grow=south east] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     5< g\leq 9 \\% g
                                                                     2< x\leq 5 \\% x
                                                                     5< g\leq 9 % y
                                                                  \end{array}
                                                               $}
                                                         % send restart
                                                         child[allact] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           5< g\leq 9 \\% g
                                                                           2< x\leq 5 \\% x
                                                                           5< g\leq 9 % y
                                                                        \end{array}
                                                                     $}
                                                               % rec z
                                                               child[Zrec] {
                                                                     node {$
                                                                              \begin{array}{c}
                                                                                 g=0 \\% g
                                                                                 x=0 \\% x
                                                                                 y=0 % y
                                                                              \end{array}
                                                                           $}
                                                                     %
                                                                     edge from parent
                                                                     node {$
                                                                              {{\mreclabel}^{Z}}
                                                                           $}
                                                                  }
                                                               %
                                                               edge from parent
                                                               node[right] {$\msend\mathtt{restart}$}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[right] {$
                                                                  \begin{array}{c}
                                                                     \mrecv\mathtt{error},
                                                                     \\
                                                                     2<x\leq 6
                                                                  \end{array}$}
                                                      }
                                                   %
                                                   edge from parent
                                                   node {$\left\{\mrecv\right\}$}
                                                }
                                             % recv error
                                             child[act,grow=south east] {
                                                   node {$
                                                            \begin{array}{c}
                                                               8< g\leq 10 \\% g
                                                               5< x\leq 6  \\% x
                                                               8< y\leq 10 % y
                                                            \end{array}
                                                         $}
                                                   % send restart
                                                   child[allact] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     8< g\leq 10 \\% g
                                                                     5< x\leq 6  \\% x
                                                                     8< y\leq 10 % y
                                                                  \end{array}
                                                               $}
                                                         % rec z
                                                         child[Zrec] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           g=0 \\% g
                                                                           x=0 \\% x
                                                                           y=0 % y
                                                                        \end{array}
                                                                     $}
                                                               %
                                                               edge from parent
                                                               node {$
                                                                        {{\mreclabel}^{Z}}
                                                                     $}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[right] {$\msend\mathtt{restart}$}
                                                      }
                                                   %
                                                   edge from parent
                                                   node[right] {$
                                                            \begin{array}{c}
                                                               \msend\mathtt{error},
                                                               \\
                                                               2<x\leq 6
                                                            \end{array}$}
                                                }
                                             %
                                             edge from parent
                                             node {$\left\{\mrecv\right\}$}
                                          }
                                       % send timeout
                                       child[act,grow=south east] {
                                             node {$
                                                      \begin{array}{c}
                                                         9< g\leq \infty \\% g
                                                         6< x\leq \infty \\% x
                                                         9< y\leq \infty % y
                                                      \end{array}
                                                   $}
                                             % rec z
                                             child[Zrec] {
                                                   node {$
                                                            \begin{array}{c}
                                                               g=0 \\% g
                                                               x=0 \\% x
                                                               y=0 % y
                                                            \end{array}
                                                         $}
                                                   %
                                                   edge from parent
                                                   node {$
                                                            {{\mreclabel}^{Z}}
                                                         $}
                                                }
                                             %
                                             edge from parent
                                             node[right] {$
                                                      \begin{array}{c}
                                                         \msend\mathtt{timeout},
                                                         \\
                                                         6<x
                                                      \end{array}$}
                                          }
                                       %
                                       edge from parent
                                       node {$\mrec\,{{\mreclabel}^{A}}$}
                                    }
                                 edge from parent
                                 node[right] {$
                                          \begin{array}{c}
                                             \msend\mathtt{start},\,x\mapsto 0
                                             \\
                                             x=2
                                          \end{array}
                                       $}
                              }
                           %
                           edge from parent
                           node {$\left\{\msend\right\}$}
                        }
                     % send latency
                     child[act,grow=south east]  {
                           node {$
                                    \begin{array}{c}
                                       4<g\leq\infty \\% g
                                       2<x\leq\infty \\% x
                                       4<y\leq\infty % y
                                    \end{array}
                                 $}
                           % rec z
                           child[Zrec] {
                                 node {$
                                          \begin{array}{c}
                                             g=0 \\% g
                                             x=0 \\% x
                                             y=0 % y
                                          \end{array}
                                       $}
                                 %
                                 edge from parent
                                 node {$
                                          {{\mreclabel}^{Z}}
                                       $}
                              }
                           %
                           edge from parent
                           node[right] {$
                                    \begin{array}{c}
                                       \msend\mathtt{latency}
                                       \\
                                       y-x=2
                                    \end{array}
                                 $}
                        }
                     edge from parent
                     node[left] {$
                              \begin{array}{c}
                                 \mrecv\mathtt{ready},\,x\mapsto 0
                                 \\
                                 1\leq x\leq2
                              \end{array}
                           $}
                  }
               % send close
               child[act,grow=south east] {
                     node {$
                              \begin{array}{c}
                                 g=2.5 \\% g
                                 x=2.5 \\% x
                                 y=2.5 % y
                              \end{array}
                           $}
                     % end
                     child[end] {
                           node {$\mend$}
                        }
                     %
                     edge from parent
                     node[right] {$
                              \begin{array}{c}
                                 \msend\mathtt{close}
                                 \\
                                 x=2.5
                              \end{array}
                           $}
                  }
               %
               edge from parent
               node {$\mrec\,{{\mreclabel}^{Z}}$}
            };
      \end{tikzpicture}
   }
\end{example}


\subsubsection*{Recursion}
The major change is the addition of local clocks \psetX\ to process variables \pvar; allowing, and requiring, that there exists some implementation of local clocks which to be evaluated at run-time.

A subtle change to the definition is the removal of the redundant assignment of a process variable \pvar\ to a continuation process \prc, which is assumed.


\paragraph*{Other approaches}
\TODO[acknowledge other possible approach using affinity]~\cite{Lagaillardie2022}.
\REDO[however, this approach is more formally grounded with respects to the time constraints, ] \TODO

==> _backups/_processes_subtyping_tree.tex <==


\paragraph*{Processes}
Let
\begin{inline}
   \item $\mprc,\mprc', \mqrc$ range over processes
   %
   \item \pvar\ range over process variables
   %
   \item \setA\ be an ordered set of message labels
   %
   \item \setC\ be an ordered set of session channels
   %
   \item \psetX\ be the set of local clocks (distinct to the set of clocks \setX\ used in the syntax of types)
   %
\end{inline}

In definition that follows
\begin{inline}
   \item \epointp\ and \epointq\ are two endpoints
   %
   \item \pchan\ is a channel between two endpoints
   %
   \item \bool\ is a boolean condition
   %
   \item \pbuffer\ points to the head of a channels buffer (ordered chronologically)
   %
\end{inline}
\begin{equation*}
   % \hspace{-5ex}%
   \mproccescalc%
\end{equation*}
The following sections discusses all of the changes from the previous work of~\cite{Bocchi2019}. \REDO[i am unsure if i have formulated \opt\ correctly, will need to discuss]
\TODO[still need single actions even though they can be represented here?]
\TODO[is it wrong to enforce active() on actions?]

\subsection{New\TODO}

\subsubsection*{Choices and Options}
A process $\mprc=\mpchan\;\mopt$ describes that the channel \pchan\ will be used by one of the options taken in \opt.

\opt\ is structured

\begin{example}[Constructing Processes]
   Below is a modification of the type shown in~\cref{fig:motiv_example_producer_consumer_diagram}:
   \begin{equation*}
      \resizebox{\textwidth}{!}{$
            \mrec\,{{\mreclabel}^{Z}}%
            \,.\,%
            \left\{\def\arraystretch{1.7}%
            \begin{array}{l}%
               \mrecv\mathtt{ready}\,\left(1\leq x\leq 2,\,x\right)%
               \,.\,%
               \left\{\def\arraystretch{1.7}%
               \begin{array}{l}%
                  \msend\mathtt{latency}\,\left(y-x=2,\right)%
                  \,.\,%
                  {{\mreclabel}^{Z}}%
                  \,, \\%
                  %
                  %
                  \msend\mathtt{start}\,\left(x=2,\right)%
                  \,.\,%
                  \mrec\,{{\mreclabel}^{A}}%
                  \,.\,%
                  \left\{\def\arraystretch{1.7}%
                  \begin{array}{l}%
                     \msend\mathtt{cancel}\,\left(x\leq 2\right)%
                     \,.\,%
                     \mend%
                     \,, \\%
                     %
                     %
                     \mrecv\mathtt{done}\,\left(2\leq x\leq 5\right)%
                     \,.\,%
                     \msend\mathtt{ok}%
                     \,.\,%
                     \mend%
                     \,, \\%
                     %
                     %
                     \mrecv\mathtt{data}\,\left(2\leq x\leq 5\right)%
                     \,.\,%
                     {{\mreclabel}^{A}}%
                     \,, \\%
                     %
                     %
                     \mrecv\mathtt{error}\,\left(2\leq x\leq 6\right)%
                     \,.\,%
                     \msend\mathtt{restart}%
                     \,.\,%
                     {{\mreclabel}^{Z}}%
                     \,, \\%
                     %
                     %
                     \msend\mathtt{timeout}\,\left(6<x\right)%
                     \,.\,%
                     {{\mreclabel}^{Z}}%
                     %
                     %
                  \end{array}%
                  \right\}%
                  %
                  %
               \end{array}%
               \right\}%
               \,, \\%
               %
               %
               \msend\mathtt{close}\,\left(x=2.5\right)%
               \,.\,%
               \mend%
               %
               %
            \end{array}%
            \right\}%
         $}
   \end{equation*}

   Against a global clock $g$ (which can only be reset when a recursive call is made), the following graph can be constructed to represent the possible traces of viable sequences and timings of interactions:\newline
   \resizebox{\textwidth}{!}{%
      \begin{tikzpicture}
         % grid
         \draw (0,0) -- (8,0);%
         \draw (0,0) -- (0,10);%
         % draw horizontal
         \foreach \y in {1,...,10}%
            {%
               \draw[gray] (0,\y) -- (8,\y);%
               \node[left] at (0,\y) {\y};
            }%
         % draw vertical
         \foreach \x in {1,...,8}%
            {%
               \draw[gray] (\x,0) -- (\x,10);%
               \node[below] at (\x,0) {\x};
            }%

         % complete trace
         \filldraw [gray, opacity = 0.25, line width = 2pt]%
         (0,0) -- (2.5,2.5);%
         \filldraw [blue, opacity = 1, line width = 2pt]% ready
         (2,2) -- (1,1);%
         \filldraw [yellow, opacity = 0.25, line width = 0pt]% reset
         (0,1) -- (0,2) -- (2,2) -- (1,1);%
         \filldraw [gray, opacity = 0.25, line width = 0pt]%
         (0,1) -- (0,2) -- (1,3) -- (2,3);%
         \filldraw [red, opacity = 1, line width = 2pt]% latency
         (0,2) -- (8,10);%

         \filldraw [yellow, opacity = 0.25, line width = 0pt]% reset
         (0,3) -- (0,4) -- (2,4) -- (2,3);%
         \filldraw [red, opacity = 0.25, line width = 0pt]% cancel
         (0,3) -- (0,4) -- (2,6) -- (2,5);%
         \filldraw [blue, opacity = 0.25, line width = 0pt]% done
         (2,5) -- (2,6) -- (5,9) -- (5,8);%
         \filldraw [blue, opacity = 0.25, line width = 0pt]% data
         (2,5) -- (2,6) -- (5,9) -- (5,8);%
         \filldraw [blue, opacity = 0.25, line width = 0pt]% error
         (2,5) -- (2,6) -- (6,10) -- (6,9);%
         \filldraw [red, opacity = 0.25, line width = 0pt]% timeout
         (6,9) -- (6,10) -- (7,10);%

         % def z
         \draw[fill, cyan] (0,0) circle (4pt);
         \node[right] at (0.2, 0.5) {\Large $\mrec\,{{\mreclabel}^{Z}}$};

         % def a
         \draw[fill, cyan] (2,3) circle (4pt);
         \draw[fill, cyan] (2,4) circle (4pt);
         \filldraw [cyan, line width = 8pt] (2,3) -- (2,4);
         \node[right] at (2.2,3.5) {\Large $\mrec\,{{\mreclabel}^{A}}$};

         % send start
         \filldraw [red, opacity = 1, line width = 2pt]% start
         (2,4) -- (2,3);%

         % send close
         \filldraw [red, opacity = 1, line width = 2pt]%
         (2.5,2.5) circle (4pt);

         % axis labels
         \node[below] at (7.5,-0.5) {\Large $x,y,z\in\msetX$};
         \node[left] at (-0.5, 9.5) {\Large $g$};

         % % table of clock values: g
         % \node at (9, 10.5) {\Large $g$};
         % \node at (9, 10) {$10$};
         % \node at (9, 9) {$9$};
         % \node at (9, 8) {$8$};
         % \node at (9, 7) {$7$};
         % \node at (9, 6) {$6$};
         % \node at (9, 5) {$5$};
         % \node at (9, 4) {$4$};
         % \node at (9, 3) {$3$};
         % \node at (9, 2) {$2$};
         % \node at (9, 1) {$1$};
         % \node at (9, 0) {$0$};
         % % table of clock values: x
         % \node at (10, 10.5) {\Large $x$};
         % \node at (10, 10) {$(6,7)$};
         % \node at (10, 9) {$(5,6)$};
         % \node at (10, 8) {$(4,5)$};
         % \node at (10, 7) {$(3,4)$};
         % \node at (10, 6) {$(2,3)$};
         % \node at (10, 5) {$(1,2)$};
         % \node at (10, 4) {$2\mapsto 0$};
         % \node at (10, 3) {$\begin{array}{c}(1,2)\\2\mapsto 0\end{array}$};
         % \node at (10, 2) {$\begin{array}{c}(1,2)\\2\mapsto 0\end{array}$};
         % \node at (10, 1) {$1\mapsto 0$};
         % \node at (10, 0) {$0$};
         % % table of clock values: y
         % \node at (11, 10.5) {\Large $y$};
         % \node at (11, 10) {$10$};
         % \node at (11, 9) {$9$};
         % \node at (11, 8) {$8$};
         % \node at (11, 7) {$7$};
         % \node at (11, 6) {$6$};
         % \node at (11, 5) {$5$};
         % \node at (11, 4) {$4$};
         % \node at (11, 3) {$3$};
         % \node at (11, 2) {$2$};
         % \node at (11, 1) {$1$};
         % \node at (11, 0) {$0$};
      \end{tikzpicture}
   }

   Using the above graph, the following decision diagram can be extracted\TODO[work in progress]:\newline
   % \resizebox{\textwidth}{!}{%
   \resizebox{!}{20cm}{%
      \begin{tikzpicture}[
            every node/.style={xshift=0mm,yshift=0mm,draw,rectangle,rounded corners,fill=gray!20},
            %
            edge from parent/.style={
                  draw,->,
                  nodes={fill=blue!20,rectangle}
               },
            %
            end/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=black,text=white,circle},
                  level distance=20mm
               },
            %
            Zdef/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=green!40,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=green!30,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=30mm
               },
            %
            Zrec/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=green!60,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=green!50,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=35mm
               },
            %
            Adef/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=orange!40,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=orange!30,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=30mm
               },
            %
            Arec/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=orange!60,ellipse},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=orange!50,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=35mm
               },
            % general actions
            act/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=white,rectangle,rounded corners},
                  edge from parent/.style={
                        draw,->,
                        nodes={fill=cyan!20,rectangle,xshift=0mm,yshift=2mm}
                     },
                  level distance=40mm
               },
            % middle actions in options
            optact/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=white,rectangle,rounded corners},
                  edge from parent/.style={
                        draw,->,
                        nodes={fill=cyan!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=45mm
               },
            % always actions
            allact/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=white,rectangle,rounded corners},
                  edge from parent/.style={
                        draw,->,
                        nodes={fill=cyan!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=35mm
               },
            % options
            opt/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=magenta!40,diamond},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=magenta!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=48mm
               },
            % nested options
            subopt/.style={
                  nodes={xshift=0mm,yshift=0mm,fill=magenta!40,diamond},
                  edge from parent/.style={
                        midway,draw,->,
                        nodes={fill=magenta!20,rectangle,xshift=0mm,yshift=0mm}
                     },
                  level distance=40mm
               }
         ]
         % root
         \node[act] {$
               \begin{array}{c}
                  g=0 \\% g
                  x=0 \\% x
                  y=0 % y
               \end{array}
            $}
         % def z
         child[Zdef] {
               node {$
                        \begin{array}{c}
                           g=0 \\% g
                           x=0 \\% x
                           y=0 % y
                        \end{array}
                     $}
               % recv ready
               child[act,grow=south west] {
                     node {$
                              \begin{array}{c}
                                 1\leq g\leq 2 \\% g
                                 x=0           \\% x
                                 1\leq y\leq 2 % y
                              \end{array}
                           $}
                     % send latency
                     child[act,grow=south west] {
                           node {$
                                    \begin{array}{c}
                                       2\leq g< 3 \\% g
                                       0\leq x< 2 \\% x
                                       2\leq y< 3 % y
                                    \end{array}
                                 $}
                           % rec z
                           child[Zrec] {
                                 node {$
                                          \begin{array}{c}
                                             g=0 \\% g
                                             x=0 \\% x
                                             y=0 % y
                                          \end{array}
                                       $}
                                 %
                                 edge from parent
                                 node {$
                                          {{\mreclabel}^{Z}}
                                       $}
                              }
                           %
                           edge from parent
                           node[left] {$
                                    \begin{array}{c}
                                       \msend\mathtt{latency}
                                       \\
                                       y-x=2
                                    \end{array}
                                 $}
                        }
                     % send latency or start
                     child[opt,grow=south] {
                           node {$
                                    \begin{array}{c}
                                       3\leq g\leq 4 \\% g
                                       x=2           \\% x
                                       3\leq y\leq 4 % y
                                    \end{array}
                                 $}
                           % send latency
                           child[act,grow=south west]  {
                                 node {$
                                          \begin{array}{c}
                                             3\leq g\leq 4 \\% g
                                             x=2           \\% x
                                             3\leq y\leq 4 % y
                                          \end{array}
                                       $}
                                 % rec z
                                 child[Zrec] {
                                       node {$
                                                \begin{array}{c}
                                                   g=0 \\% g
                                                   x=0 \\% x
                                                   y=0 % y
                                                \end{array}
                                             $}
                                       %
                                       edge from parent
                                       node {$
                                                {{\mreclabel}^{Z}}
                                             $}
                                    }
                                 % label
                                 edge from parent
                                 node[left] {$
                                          \begin{array}{c}
                                             \msend\mathtt{latency}
                                             \\
                                             y-x=2
                                          \end{array}
                                       $}
                              }
                           % send start
                           child[act,grow=south east]  {
                                 node {$
                                          \begin{array}{c}
                                             3\leq g\leq 4 \\% g
                                             x=0           \\% x
                                             3\leq y\leq 4 % y
                                          \end{array}
                                       $}
                                 % def a
                                 child[Adef,grow=south] {
                                       node {$
                                                \begin{array}{c}
                                                   3\leq g\leq 4 \\% g
                                                   x=0           \\% x
                                                   3\leq y\leq 4 % y
                                                \end{array}
                                             $}
                                       % send cancel
                                       child[act,grow=south west] {
                                             node {$
                                                      \begin{array}{c}
                                                         3\leq g\leq 6 \\% g
                                                         0\leq x\leq 2 \\% x
                                                         3\leq y\leq 6 % y
                                                      \end{array}
                                                   $}
                                             % end
                                             child[end] {
                                                   node {$\mend$}
                                                }
                                             %
                                             edge from parent
                                             node[left] {$
                                                      \begin{array}{c}
                                                         \msend\mathtt{cancel}
                                                         \\
                                                         x\leq 2
                                                      \end{array}
                                                   $}
                                          }
                                       % recv done, data or error
                                       child[opt,grow=south] {
                                             node {$
                                                      \begin{array}{c}
                                                         5< g\leq 9 \\% g
                                                         2< x\leq 5 \\% x
                                                         5< g\leq 9 % y
                                                      \end{array}
                                                   $}
                                             % recv done, data or error
                                             child[subopt,grow=south west] {
                                                   node {$
                                                            \begin{array}{c}
                                                               5< g\leq 9 \\% g
                                                               2< x\leq 5 \\% x
                                                               5< g\leq 9 % y
                                                            \end{array}
                                                         $}
                                                   % recv done
                                                   child[optact,grow=south west] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     5< g\leq 9 \\% g
                                                                     2< x\leq 5 \\% x
                                                                     5< g\leq 9 % y
                                                                  \end{array}
                                                               $}
                                                         % send ok
                                                         child[allact] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           5< g\leq 9 \\% g
                                                                           2< x\leq 5 \\% x
                                                                           5< g\leq 9 % y
                                                                        \end{array}
                                                                     $}
                                                               % end
                                                               child[end] {
                                                                     node {$\mend$}
                                                                  }
                                                               %
                                                               edge from parent
                                                               node[right] {$\msend\mathtt{ok}$}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[left] {$
                                                                  \begin{array}{c}
                                                                     \mrecv\mathtt{done},
                                                                     \\
                                                                     2<x\leq 5
                                                                  \end{array}$}
                                                      }
                                                   % recv data
                                                   child[optact,grow=south,level distance=45mm] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     5< g\leq 9 \\% g
                                                                     2< x\leq 5 \\% x
                                                                     5< g\leq 9 % y
                                                                  \end{array}
                                                               $}
                                                         % rec a
                                                         child[Arec] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           3\leq g\leq 4 \\% g
                                                                           x=0           \\% x
                                                                           3\leq y\leq 4 % y
                                                                        \end{array}
                                                                     $}
                                                               %
                                                               edge from parent
                                                               node {$
                                                                        {{\mreclabel}^{A}}
                                                                     $}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[midway] {$
                                                                  \begin{array}{c}
                                                                     \mrecv\mathtt{data},
                                                                     \\
                                                                     2<x\leq 5
                                                                  \end{array}
                                                               $}
                                                      }
                                                   % recv error
                                                   child[optact,grow=south east] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     5< g\leq 9 \\% g
                                                                     2< x\leq 5 \\% x
                                                                     5< g\leq 9 % y
                                                                  \end{array}
                                                               $}
                                                         % send restart
                                                         child[allact] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           5< g\leq 9 \\% g
                                                                           2< x\leq 5 \\% x
                                                                           5< g\leq 9 % y
                                                                        \end{array}
                                                                     $}
                                                               % rec z
                                                               child[Zrec] {
                                                                     node {$
                                                                              \begin{array}{c}
                                                                                 g=0 \\% g
                                                                                 x=0 \\% x
                                                                                 y=0 % y
                                                                              \end{array}
                                                                           $}
                                                                     %
                                                                     edge from parent
                                                                     node {$
                                                                              {{\mreclabel}^{Z}}
                                                                           $}
                                                                  }
                                                               %
                                                               edge from parent
                                                               node[right] {$\msend\mathtt{restart}$}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[right] {$
                                                                  \begin{array}{c}
                                                                     \mrecv\mathtt{error},
                                                                     \\
                                                                     2<x\leq 6
                                                                  \end{array}$}
                                                      }
                                                   %
                                                   edge from parent
                                                   node {$\left\{\mrecv\right\}$}
                                                }
                                             % recv error
                                             child[act,grow=south east] {
                                                   node {$
                                                            \begin{array}{c}
                                                               8< g\leq 10 \\% g
                                                               5< x\leq 6  \\% x
                                                               8< y\leq 10 % y
                                                            \end{array}
                                                         $}
                                                   % send restart
                                                   child[allact] {
                                                         node {$
                                                                  \begin{array}{c}
                                                                     8< g\leq 10 \\% g
                                                                     5< x\leq 6  \\% x
                                                                     8< y\leq 10 % y
                                                                  \end{array}
                                                               $}
                                                         % rec z
                                                         child[Zrec] {
                                                               node {$
                                                                        \begin{array}{c}
                                                                           g=0 \\% g
                                                                           x=0 \\% x
                                                                           y=0 % y
                                                                        \end{array}
                                                                     $}
                                                               %
                                                               edge from parent
                                                               node {$
                                                                        {{\mreclabel}^{Z}}
                                                                     $}
                                                            }
                                                         %
                                                         edge from parent
                                                         node[right] {$\msend\mathtt{restart}$}
                                                      }
                                                   %
                                                   edge from parent
                                                   node[right] {$
                                                            \begin{array}{c}
                                                               \msend\mathtt{error},
                                                               \\
                                                               2<x\leq 6
                                                            \end{array}$}
                                                }
                                             %
                                             edge from parent
                                             node {$\left\{\mrecv\right\}$}
                                          }
                                       % send timeout
                                       child[act,grow=south east] {
                                             node {$
                                                      \begin{array}{c}
                                                         9< g\leq \infty \\% g
                                                         6< x\leq \infty \\% x
                                                         9< y\leq \infty % y
                                                      \end{array}
                                                   $}
                                             % rec z
                                             child[Zrec] {
                                                   node {$
                                                            \begin{array}{c}
                                                               g=0 \\% g
                                                               x=0 \\% x
                                                               y=0 % y
                                                            \end{array}
                                                         $}
                                                   %
                                                   edge from parent
                                                   node {$
                                                            {{\mreclabel}^{Z}}
                                                         $}
                                                }
                                             %
                                             edge from parent
                                             node[right] {$
                                                      \begin{array}{c}
                                                         \msend\mathtt{timeout},
                                                         \\
                                                         6<x
                                                      \end{array}$}
                                          }
                                       %
                                       edge from parent
                                       node {$\mrec\,{{\mreclabel}^{A}}$}
                                    }
                                 edge from parent
                                 node[right] {$
                                          \begin{array}{c}
                                             \msend\mathtt{start},\,x\mapsto 0
                                             \\
                                             x=2
                                          \end{array}
                                       $}
                              }
                           %
                           edge from parent
                           node {$\left\{\msend\right\}$}
                        }
                     % send latency
                     child[act,grow=south east]  {
                           node {$
                                    \begin{array}{c}
                                       4<g\leq\infty \\% g
                                       2<x\leq\infty \\% x
                                       4<y\leq\infty % y
                                    \end{array}
                                 $}
                           % rec z
                           child[Zrec] {
                                 node {$
                                          \begin{array}{c}
                                             g=0 \\% g
                                             x=0 \\% x
                                             y=0 % y
                                          \end{array}
                                       $}
                                 %
                                 edge from parent
                                 node {$
                                          {{\mreclabel}^{Z}}
                                       $}
                              }
                           %
                           edge from parent
                           node[right] {$
                                    \begin{array}{c}
                                       \msend\mathtt{latency}
                                       \\
                                       y-x=2
                                    \end{array}
                                 $}
                        }
                     edge from parent
                     node[left] {$
                              \begin{array}{c}
                                 \mrecv\mathtt{ready},\,x\mapsto 0
                                 \\
                                 1\leq x\leq2
                              \end{array}
                           $}
                  }
               % send close
               child[act,grow=south east] {
                     node {$
                              \begin{array}{c}
                                 g=2.5 \\% g
                                 x=2.5 \\% x
                                 y=2.5 % y
                              \end{array}
                           $}
                     % end
                     child[end] {
                           node {$\mend$}
                        }
                     %
                     edge from parent
                     node[right] {$
                              \begin{array}{c}
                                 \msend\mathtt{close}
                                 \\
                                 x=2.5
                              \end{array}
                           $}
                  }
               %
               edge from parent
               node {$\mrec\,{{\mreclabel}^{Z}}$}
            };
      \end{tikzpicture}
   }
\end{example}


\subsubsection*{Recursion}
The major change is the addition of local clocks \psetX\ to process variables \pvar; allowing, and requiring, that there exists some implementation of local clocks which to be evaluated at run-time.

A subtle change to the definition is the removal of the redundant assignment of a process variable \pvar\ to a continuation process \prc, which is assumed.


\paragraph*{Other approaches}
\TODO[acknowledge other possible approach using affinity]~\cite{Lagaillardie2022}.
\REDO[however, this approach is more formally grounded with respects to the time constraints, ] \TODO

==> _backups/process_calc_defs.tex <==

% processes
\newcommand{\mprc}[0]{P}
\newcommand{\prc}[0]{$\mprc$}
\newcommand{\mqrc}[0]{Q}
\newcommand{\qrc}[0]{$\mqrc$}

% recall process
\newcommand{\mprecall}[0]{R}
\newcommand{\precall}[0]{$\mprecall$}

% recall queue
\newcommand{\mprequeue}[0]{\mathbf{r}}
\newcommand{\prequeue}[0]{$\mprequeue$}

% recall queue cache
\newcommand{\mprecallcache}[0]{\mathbf{k}}
\newcommand{\precallcache}[0]{$\mprecallcache$}

% option in choice
\newcommand{\mopt}[0]{O}
\newcommand{\opt}[0]{$\mopt$}

\newcommand{\mpdef}[0]{D}
\newcommand{\pdef}[0]{$\mpdef$}

\newcommand{\mpvar}[0]{\set{x}}
\newcommand{\pvar}[0]{$\mpvar$}

\newcommand{\msetLabel}[0]{\bset{\textbf{\small a\normalsize}}}
\newcommand{\setLabel}[0]{$\msetLabel$}

\newcommand{\msetChan}[0]{\bset{\textbf{\small c\normalsize}}}
\newcommand{\setChan}[0]{$\msetChan$}

\newcommand{\mnum}[0]{n}
\newcommand{\num}[0]{$\mnum$}

\newcommand{\mbool}[0]{v}
\newcommand{\bool}[0]{$\mbool$}

\newcommand{\mpchan}[0]{c}
\newcommand{\pchan}[0]{$\mpchan$}

\newcommand{\mepointp}[0]{\elem{p}}
\newcommand{\epointp}[0]{$\mepointp$}

\newcommand{\mepointq}[0]{\elem{q}}
\newcommand{\epointq}[0]{$\mepointq$}

% arrows
\DeclareMathOperator{\mtreduce}{~~\rightsquigarrow~~}
\DeclareMathOperator{\mareduce}{~~\rightharpoonup~~}
\DeclareMathOperator{\mreduce}{~~\longrightarrow~~}

% chan direction
\DeclareMathOperator{\mprecv}{\vartriangleright}
\DeclareMathOperator{\mpsend}{\vartriangleleft}
\DeclareMathOperator{\mptyped}{\vartriangleright}

\newcommand{\precv}[0]{$\mprecv$}
\newcommand{\psend}[0]{$\mpsend$}
\newcommand{\ptyped}[0]{$\mptyped$}

% \DeclareMathOperator{\dia}{\mbox{\raisebox{\depth}{\rotatebox[origin=c]{45}{$\sq$}}}\!\,}

% \newcommand{\mpcomm}[0]{\dia}
% \newcommand{\pcomm}[0]{\mpcomm}

% channel buffer
\newcommand{\mpbuffer}[0]{h}
\newcommand{\pbuffer}[0]{$\mpbuffer$}

% func
\newcommand{\mdelayfunc}[1][\mconstr]{\mathtt{delay}\left(#1\right)}
\newcommand{\delayfunc}[1][\mconstr]{$\mdelayfunc[#1]$}

\newcommand{\mwaitfunc}[1][\mprc]{\mathtt{Wait}\left(#1\right)}
\newcommand{\waitfunc}[1][\mprc]{$\mwaitfunc[#1]$}

\newcommand{\mnequeuefunc}[1][\mprc]{\mathtt{NEQueue}\left(#1\right)}
\newcommand{\nequeuefunc}[1][\mprc]{$\mwaitfunc[#1]$}

\newcommand{\mprcfail}[0]{\mathtt{failed}}
\newcommand{\prcfail}[0]{$\mprcfail$}

\newcommand{\mprcvar}[1][\msetLabel;\msetChan]{\mpvar\left(#1\right)}
\newcommand{\prcvar}[1][\msetLabel;\msetChan]{$\mprcvar[#1]$}

% def rec
\newcommand{\mpsetrec}[1][\msetLabel;\msetChan]{\mathtt{def}\;\mprcvar[#1]=\mprc\;\mathtt{in}\;}
\newcommand{\psetrec}[1][\msetLabel;\msetChan]{$\mpsetrec[#1]$}

% call rec
\newcommand{\mpcallrec}[1][\msetLabel;\msetChan]{\mpvar\left\langle#1\right\rangle}
\newcommand{\pcallrec}[0]{$\mpcallrec$}

% send and listen
\newcommand{\mpsendlisten}[1][\mqrc]{\mpchan\,\mpsend\,a\;\mathtt{listen}\;\of{\left\{{\left(\of{b}{i}:\of{\mprc}{i}\right)}^{n}\right\}}{\elemofset{i}{i}}\,.\,#1}

\newcommand{\mpsendalways}[1][\mprc]{\mpchan\,\mpsend\,a\,.\,#1}

% recv until p
\newcommand{\mprecvuntil}[1][n]{{{\mpchan}^{#1}}\,\mprecv\,\of{\left\{\of{a}{i}:\of{\mprc}{i}\right\}}{\elemofset{i}{i}}\,\mathtt{after}\;\mqrc}

\newcommand{\mprecvalways}[0]{{{\mpchan}^{\infty}}\,\mprecv\,\of{\left\{\of{a}{i}:\of{\mprc}{i}\right\}}{\elemofset{i}{i}}}

% if then else
\newcommand{\mifthenelse}[0]{\mathtt{if}\;\mbool\;\mathtt{then}\;\mprc\;\mathtt{else}\;\mqrc}

% recall process
\newcommand{\mprcrecall}[0]{\mpchan\,\mprecv\,\mkset{\mprequeue}}

% scope
\newcommand{\mpscope}[1][\mepointp\mepointq]{\left(\nu#1\right)}

\newcommand{\mprcpar}[1][\mprc]{\of{#1}{1}\mid\of{#1}{2}}

% timers
\newcommand{\mprctimerset}[1][x]{\mathtt{set}\left(#1\right)}
\newcommand{\prctimerset}[1][x]{$\mprctimerset[#1]$}

\newcommand{\mprctimer}[1][x]{\left(\nu#1\right)}
\newcommand{\prctimer}[1][x]{$\mprctimer[#1]$}

\newcommand{\mprctimereval}[1][x]{#1\models\mconstr}

% calculus
\newcommand{\mproccescalc}[0]{%
   \begin{array}{r c l r c l}%
      \mprc,\mqrc & ::=\;                              %
                  & \mpsendalways                      %
                  & \mbox{ }                           %
                  & \quad \mid \quad\,                 %
                  & \mprecvuntil                       %    
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mpsendlisten                      %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & 0                                  %
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mpscope\,\mprc                    %
                  & \mbox{ }                           %   
                  & \mid \quad                         %
                  & \mepointp\mepointq:\mpbuffer       % 
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mifthenelse                       %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & \mdelayfunc.\mprc                  %
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mprcpar                           %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & \mprctimerset\,.\,\mprc            %
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mpsetrec\mprc                     %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & \mpcallrec                         %
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mprcrecall                        %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & \mkset{\mprecallcache}             %
      %
      %
      %
      %
      \\\rule{0pt}{3.5ex} %
      \mbool      & ::=                                %
                  & \mtrue                             %
                  & \mpbuffer                          %
                  & ::=                                %
                  & \emptyset                          %
      %
      \\\rule{0pt}{2ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mfalse                            %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & \mpbuffer\cdot\mlabel
      %
      \\\rule{0pt}{2ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mprctimereval                     %
                  & \mbox{ }                           %
      % & \mid                               %
      % & \mpbuffer\cdot\mlabel              %
      %
      %
      %
      %
      \\\rule{0pt}{3.5ex} %
      \mprequeue  & ::=                                %
                  & \mathtt{tidy}:\mpbuffer,\mprequeue %
                  & \mprecallcache                     %
                  & ::=                                %
                  & \emptyset                          %
      %
      \\\rule{0pt}{2ex} %
      \mbox{ }    & \mid \quad                         %
                  & \mprequeue,\,a:\mprc               %
                  & \mbox{ }                           %
                  & \mid \quad                         %
                  & a:\mpbuffer                        %
      %
      %
      %
   \end{array}}

\newcommand{\proccescalc}[0]{$\mproccescalc$}

% pass time function
\DeclareMathOperator{\mptime}{\of{\mathit{\Phi}}{\mathit{t}}}

\newcommand{\mptimefunc}[1][0]{\mptime\left(#1\right)}
\newcommand{\ptimefunc}[1][0]{$\mptimefunc$}

% process judgements
\DeclareMathOperator{\mpenv}{\mathit{\Gamma}}
\DeclareMathOperator{\msenv}{\mathit{\Delta}}
\DeclareMathOperator{\msset}{\mathit{\Theta}}

\newcommand{\penv}[0]{$\mpenv$}
\newcommand{\senv}[0]{$\msenv$}
\newcommand{\sset}[0]{$\msset$}

% vector of sorts T
\newcommand{\msetT}[0]{\boldsymbol{\mtype}}
\newcommand{\setT}[0]{$\msetT$}

% v = l mbox v = l
\newcommand{\mprocessjudge}[0]{\begin{array}{r c l r c l}
      \msenv   & ::=                                        %
               & \emptyset                                  %
               & \mbox{}\quad\mbox{}                        %
      %
      \mpenv   & ::=                                        %
               & \emptyset                                  %
      %
      %
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ } & \mid \quad                                 %
               & \msenv,\mpchan:\left(\mval,\,\mst\right)   %
               & \mbox{ }                                   %
               & \mid \quad                                 %
               & \mpenv,\mlabel:\mtype                      %
      %
      %
      %
      \\\rule{0pt}{2.25ex} %
      \mbox{ } & \mid \quad                                 %
               & \msenv,\mepointp\mepointq:\queue           %
               & \mbox{ }                                   %
               & \mid \quad                                 %
               & \mpenv,\mpvar:\left(\msetT;\,\msset\right)
      %
      %
      %
      \\\rule{0pt}{3.5ex} %
      \msset   & ::=                                        %
               & \mathrlap{                                 %
         \emptyset%
         \quad\mid\quad%
         \msset\cup\left\{\msenv\right\}%
      } %
      %
      %
   \end{array}}

\newcommand{\processjudge}[0]{$\mprocessjudge$}

==> _backups/process_calc_rules.tex <==
% process reduction rules

% timer
\newcommand{\mpreducttimer}[0]{%
   \mprctimerset[x].\,\left(\mprc\right)%
   \mid%
   \mqrc%
   %
   \mareduce%
   %
   \mprctimer[x:0]\left(\mprc\right)%
   \mid%
   \mqrc%
}

% reset
\newcommand{\mpreductreset}[0]{%
   \mprctimer[x]\left(\mprctimerset[x].\,\mprc\right)%
   \mid%
   \mqrc%
   %
   \mareduce%
   %
   \mprctimer[x:0]\left(\mprc\right)%
   \mid%
   \mqrc%
}

% reduce
\newcommand{\mpreductareduce}[0]{%
   \infer{%
      \mprc\mreduce\mqrc%
   }{%
      \mprc\mareduce\mqrc%
   }
}

% time reduce
\newcommand{\mpreducttreduce}[0]{%
   \infer{%
      \mprc\mreduce\mqrc%
   }{%
      \mprc\mtreduce\mqrc%
   }
}

% delay
\newcommand{\mpreductdelay}[0]{%
   \mprc%
   %
   \mtreduce%
   %
   \mptimefunc[\mprc]%
}

% scope
\newcommand{\mpreductscope}[0]{%
   \infer{%
      \left(\nu\mepointp\mepointq\right)\mprc%
      \mreduce%
      \left(\nu\mepointp\mepointq\right)\mprc'%
   }{%
      \mprc\mareduce\mprc'%
   }
}

% structural congruence
\newcommand{\mpreductastr}[0]{%
   \infer{%
      \mprc\mreduce\mqrc%
   }{%
      \mprc\equiv\mprc'%
      \quad%
      \mprc'\mareduce\mqrc'%
      \quad%
      \mqrc'\equiv\mqrc%}
   }
}

% timed structural congruence
\newcommand{\mpreducttstr}[0]{%
   \infer{%
      \mprc\mreduce\mqrc%
   }{%
      \mprc\equiv\mprc'%
      \quad%
      \mprc'\mtreduce\mqrc'%
      \quad%
      \mqrc'\equiv\mqrc%}
   }
}

% det
\newcommand{\mpreductdet}[0]{%
   \infer{%
      \mathtt{delay}(\mconstr).\mprc%
      \mareduce%
      \mathtt{delay}(\mtval).\mqrc%
   }{%
      \mtval\models\mconstr\left[\sfrac{\mtval}{x}\right]%
   }
}

% par
\newcommand{\mpreductpar}[0]{%
   \infer{%
      \mprc\mid\mqrc%
      \mareduce%
      \mprc'\mid\mqrc%
   }{%
      \mprc\mareduce\mprc'%
   }
}

% def
\newcommand{\mpreductdef}[0]{%
   \infer{%
      \mpsetrec\mprc%
      \mareduce%
      \mpsetrec\mprc'%
   }{%
      \mprc\mareduce\mprc'%
   }
}

% cont
\newcommand{\mpreductcont}[0]{%
   \infer{%
      \mpsetrec\mqrc%
      \mareduce%
      \mpsetrec\mqrc'%
   }{%
      \mqrc\mareduce\mqrc'%
   }
}

% rec
\newcommand{\mpreductrec}[0]{%
   \mpsetrec%
   \mpcallrec[\msetLabel';\msetChan']\mid\mqrc%
   \mareduce%
   \mpsetrec%
   \mprc\left[\sfrac{\msetLabel';\msetChan'}{\msetLabel;\msetChan}\right]\mid\mqrc%
}

% ift
\newcommand{\mpreductift}[0]{%
   \mifthenelse\mareduce\mprc%
}

% iff
\newcommand{\mpreductiff}[0]{%
   \mifthenelse\mareduce\mqrc%
}


% send
\newcommand{\mpreductsend}[0]{%
   \infer{%
      \mpsendalways%
      \mid%
      \mepointp\mepointq:\mpbuffer%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mprequeue\right\}%
      \mid%
      \left\{\mprecallcache\right\}%
      \right)%
      %
      \mareduce%
      %
      \mprc%
      \mid%
      \mepointp\mepointq:\mpbuffer\cdot a%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mprequeue\right\}%
      \mid%
      \left\{\mprecallcache'\right\}%
      \right)%
   }{%
      \forall \of{a}{k},\of{\mpbuffer}{k}\in%
      \left\{\mprecallcache\right\}:%
      \quad%
      \mprecallcache'=\of{a}{k}:\of{\mpbuffer}{k}\cdot a%
   }
}

% listen
\newcommand{\mpreductlisten}[0]{%
   \infer{%[\rulem{AddListen}]{%
      \mpsendlisten%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mprequeue\right\}%
      \mid%
      \left\{\mprecallcache\right\}%
      \right)%
      %
      \mareduce%
      %
      \mpsendalways[\mqrc]%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mprequeue'\right\}%
      \mid%
      \left\{\mprecallcache,\mprecallcache'\right\}%
      \right)%
   }{%
      \begin{array}{c}
         \forall\elemofset{i}{i}:%
         \quad%
         \mathtt{def}\;\mpvar\left(\msetLabel;\msetChan\right)=\of{\mprc}{i}\,\mathtt{in}\;\mqrc%
         %
         \qquad%
         %
         \mprecallcache'=\of{b}{i}:\emptyset%
         %
         \\%
         \mprequeue'=\mprequeue,\,\of{b}{1}:\of{\mprc}{1},\dots,\of{b}{i}:\of{\mprc}{i}%
         %
         %
      \end{array}
   }
}

% recv 
\newcommand{\mpreductrecv}[0]{%
   \mprecvuntil%
   \mid%
   \mepointp\mepointq:\mmsg\cdot\mpbuffer%
   \mid%
   \left(\nu\mepointp\right)%
   \left(%
   \mpchan\,\mprecv\,\left\{\mprequeue\right\}%
   \mid%
   \left\{\mprecallcache\right\}%
   \right)%
   %
   \mareduce%
   %
   \of{\mprc}{i}\left[\sfrac{\mmsg}{\of{a}{i}}\right]%
   \mid%
   \mepointp\mepointq:\mpbuffer%
   \mid%
   \left(\nu\mepointp\right)%
   \left(%
   \mpchan\,\mprecv\,\left\{\mathtt{tidy}:\mpbuffer\right\}%
   \mid%
   \left\{\emptyset\right\}%
   \right)%
}

% recall
\newcommand{\mpreductrecall}[0]{%
   \infer{%
      \mprc%
      \mid%
      \mepointp\mepointq:\mmsg\cdot\mpbuffer%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{e:\mqrc,\,\mprequeue\right\}%
      \mid%
      \left\{\mprecallcache\right\}%
      \right)%
      %
      \mareduce%
      %
      \mqrc\left[\sfrac{\mmsg}{e}\right]%
      \mid%
      \mepointp\mepointq:\mpbuffer\cdot(\mathtt{tidy}:\mpbuffer')%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mathtt{tidy}:\mpbuffer\right\}%
      \mid%
      \left\{\emptyset\right\}%
      \right)%
   }{%
      \forall \of{a}{k},\of{\mpbuffer}{k}\in%
      \left\{\mprecallcache\right\}:%
      \quad%
      \exists\of{a}{k}=e:\of{\mpbuffer}{k}=\mpbuffer'%
   }
}

% tidy
\newcommand{\mpreducttidy}[0]{%
   \infer{%
      \mpchan\,\mprecv\,(\mathtt{tidy}:\mpbuffer').\mprc%
      \mid%
      \mepointp\mepointq:(\mathtt{tidy}:\mpbuffer')\cdot\mpbuffer%
      \mid%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mprequeue\right\}%
      \mid%
      \left\{\mprecallcache\right\}%
      \right)%
      %
      \mareduce%
      %
      \mprc%
      \mid%
      \mepointp\mepointq:\mpbuffer''%
      \left(\nu\mepointp\right)%
      \left(%
      \mpchan\,\mprecv\,\left\{\mathtt{tidy}:\mpbuffer\right\}%
      \mid%
      \left\{\emptyset\right\}%
      \right)%
   }{%
      \forall a\in\mpbuffer:%
      \quad%
      a\notin\mpbuffer'\implies a\in\mpbuffer''%
   }
}

\newcommand{\prcredrules}[0]{$\mprcredrules$}

\newcommand{\mprctimefuncrecv}[0]{%
   \left\{\begin{array}{l} %
      %
      {\mpchan}^{n-t}\,\mprecv\,\of{\left\{\of{a}{i}:\of{\mprc}{i}\right\}}{\elemofset{i}{i}}\,.\,\mqrc %
      %
      \\[2ex]
      \mqrc %
      %
   \end{array}\right. %
}

\newcommand{\mprctimefuncpar}[0]{\mptimefunc[\of{\mprc}{1}]\mid\mptimefunc[\of{\mprc}{2}]}

\newcommand{\mprctimefuncparcondition}[0]{\text{if}\;\mwaitfunc{\of{\mprc}{i}}\cap\mnequeuefunc{\of{\mprc}{j}}=\emptyset,i\neq j\in\{1,2\}}

\newcommand{\mprctimefunctimer}[0]{\mprctimer[x+\mtval]\mptimefunc[\mprc]}

% time passing definition
\newcommand{\mprctimedef}[0]{%
   \resizebox{\textwidth}{!}{$%
         %
         %
         \begin{array}{rcl c rcl c l}
            %
            %
            \mptimefunc[0] %
             & =                              %
             & 0                              %
            %
             & \mbox{ }                     & %
            \mptimefunc[\mpsetrec\mprc] %
             & =                              %
             & \mpsetrec\mptimefunc[\mprc]    %
            %  
            %
            %
            \\[2ex] %
            \mptimefunc[\mepointp\mepointq:\mpbuffer] %
             & =                              %
             & \mepointp\mepointq:\mpbuffer   %
            %
             & \mbox{ }                     & %
            %
            \mptimefunc[\mdelayfunc[t'].\mprc] %
             & =                              %
             & \mdelayfunc[t'-t].\mprc        %
            %
             & \mbox{ }                     & %
            \text{if\;}t'\geq t                                      %
            %              
            %     
            %
            %
            \\[3ex] %
            \mptimefunc[\mpscope\mprc] %
             & =                              %
             & \mpscope\mptimefunc[\mprc]     %
            %     
             & \mbox{ }                     & %
            %
            \mptimefunc[\mprecvuntil] %
             & =                              %
             & \mprctimefuncrecv              %
            %
             & \mbox{ }                     & %
            \begin{array}{l}n\geq t \\[2ex] \text{otherwise}\end{array}   %
            %
            %
            \\[6ex] %
            \mptimefunc[\mprcfail] %
             & =                              %
             & \mprcfail                      %
            %
             & \mbox{ }                     & %
            %
            \mptimefunc[{\mprecvalways}] %
             & =                              %
             & \mprecvalways                  %
            %
            %
            %
            % par process
            \\[4ex] %
            \mptimefunc[\mprcpar] %
             & =                              %
             & \mprctimefuncpar               %
            % 
             & \mbox{ }                       %
            %
            \mathrlap{\mbox{\hspace{2ex}}\mprctimefuncparcondition}
            %
            %
            %
            % timer progress
            \\[4ex] %
            \mptimefunc[\mprctimer[x]\mprc] %
             & =                              %
             & \mprctimefunctimer             %
         \end{array}
         %
         %
      $}%
}

==> _backups/process_calc_tools.tex <==

\newcommand{\mpchoice}[3]{\left\{{#1}\right\}}

% mpoptslice if: #1 removes else; #2 delta; #3 bool; #4 comm; #5 opts
\newcommand{\mpoptslice}[5][\mathtt{else}\;]{{#1}\mathtt{if}\;\mathtt{active}({#2})\land\ {#3}\;\mathtt{then}\;\mathtt{wait}({#2})\;\mathtt{then}\; {#4}\;{#5}}

% all option actions at once, parts of slice: #1 options
\newcommand{\mpoptsliceparts}[1]{\left\{{#1}\right\}}

% single option action: #1 msg; #2 continuation
\newcommand{\mpoptaction}[2]{\left\{{#1}:{#2}\right\}}

==> _processes_only.tex <==

% \begin{document}\newgeometry{left=1cm,right=1cm,top=1cm,bottom=1cm}

\input{tex/figs/processes/calculus.tex}

\input{tex/figs/processes/reduction.tex}

\input{tex/figs/processes/func/time_passing.tex}
\input{tex/figs/processes/func/wait.tex}
\input{tex/figs/processes/func/nonempty.tex}

\input{tex/defs/processes/free_queues.tex}
\input{tex/defs/processes/well_formed.tex}
\input{tex/defs/processes/fail_free.tex}

\input{tex/figs/processes/typing.tex}
\input{tex/figs/processes/rule_typing.tex}

\input{tex/defs/processes/session/balanced.tex}
\input{tex/defs/processes/session/fully_balanced.tex}

\input{tex/defs/processes/session/free_queues.tex}
\input{tex/defs/processes/session/delayable.tex}
\input{tex/figs/processes/session_reduction.tex}

\input{tex/proofs/reduction/thm.tex}


% \bibliographystyle{IEEEtran.bst}
% \bibliography{bib_library.bib,time.bib}

% \end{document}

\endinput

==> _proof_only.tex <==

\begin{document}
%
\section{Proof of Type Progress}
%
\input{tex/figs/types/syntax.tex}
\input{tex/figs/types/rule_formation.tex}
%
\input{tex/figs/configs/rule_iso.tex}
%
\subsubsection*{Summary}
Types constructed using the syntax of~\cref{eq:types_syntax} are judged against the rules given in~\cref{fig:types_rule}.
Types are well-formed against a valuation \ValClocks*\ as in~\cref{def:types_wf}.

A simple/isolated configuration \CIso*\ is well-formed following~\cref{def:configs_wf}.
A social configuration \CSoc*\ extends an isolated configuration with a queue \Queue*\ that stores messages \Msg*.

Configurations may transition as specified in~\cref{fig:typesemantics} using any of the actions described in~\cref{eq:type_labels}.
\CIso*\ may be written as \VIso*, and \CSoc*\ as \VSoc*.
\begin{minieq}\label{eq:type_labels} \ProgAction::=\TypComm\Msg
    \mid\,\ValTime
    \mid\SiltAction
    %
    \qquad
    %
    \Msg::=\DefMsgType
    %
    \qquad \TypComm ::=!\mid?
    %
\end{minieq}
%
A configuration is said to be live if there is an amount of time that can be waited for an action to be viable to be taken.
A configuration that is live can be described by a future enabled action \FutureEn*, where \TypComm*\ can be used to specify which kind of actions are viable in the future.

Systems are composed of two social configurations in parallel \CSys*.
Two social configurations are compatible \Compat*\ if either
\begin{inline}*|
    \item one has a message in their queue that is able to be received at the current moment which results in a new compatible system configuration
    \item both configurations have matching clock valuations, empty queues, and dual types
\end{inline}

\input{tex/defs/types/duality.tex}
%
\input{tex/defs/types/well_formed.tex}
%
\input{tex/defs/configs/iso/future_en.tex}
%
\input{tex/defs/configs/iso/live.tex}
%
\input{tex/defs/configs/iso/well_formed.tex}
%
\input{tex/defs/configs/sys/compat.tex}
%
\input{tex/defs/types/progress.tex}
\input{tex/proofs/progress/thm.tex}

\subsubsection*{Overview of proof}
%
The proof culminates in~\cref{lem:configs_sys_progress} which states that the progress of a system in its initial state \Parl*{\CSoc[\ValClocks_0];:{\emptyset},\CSoc[\ValClocks_0];[\Dual]:{\emptyset}}\ is guaranteed to \emph{enjoy progress} (see~\cref{def:types_progress}).
%
The initial system configuration is well-formed by~\cref{def:types_wf} and compatible by~\cref{def:configs_compat}.



\Cref{lem:configs_trans_compat_wf_preserved} combines~\cref{lem:configs_trans_compat_preserved,lem:cfgs_trans_wf_preserved} proving that compatibility and well-formedness are preserved across an arbitrary number of transitions.
%
\Cref{lem:configs_compat_wf_fe} proves that system that is compatible and well-formed behaves as defined in~\cref{def:types_progress} (extending the notion of liveness of single configurations of~\cref{def:configs_live} proven in~\cref{lem:wf_then_live}).
%
\Cref{lem:wf_then_live} proves that a well-formed configuration is live, and~\cref{lem:init_wf_then_live} proves that initial configurations are well-formed and live inherently.



\Cref{lem:sys_compat_time_trans} proves that all queues must be empty when time passes over the whole system \Trans*{\VSys}:{\ValTime}\ (or $\ValTime=0$ when a queue is non-empty).
%
\Cref{lem:configs_iso_trans,lem:configs_soc_trans} are similar to the "inversion lemma" of~\cite[Lemma~30, Page~51]{Bocchi2019} and highlight how configurations relate before and after a transitions (useful when reasoning how a resulting configuration is live).

Currently omitted from the proof are~\cite[Lemmas~1~to~5, Pages~31~to~34]{Bocchi2019} which regard recursive types. They clarify the meaning of typing judgements, provide detail on how recursive types are evaluated, and defined "capture avoiding" for recursive variables (stating that all types within an unfolding are "capture avoiding" if they do not correspond to the recursive call).


\subsubsection*{Remaining work}
I need to finish the recursive cases of~\cref{lem:wf_then_live,lem:cfgs_trans_wf_preserved}.
I need to decide if I will include the current missing lemmas (\cite[Lemmas~1~to~5, Pages~31~to~34]{Bocchi2019}), or if it is enough to do a co-inductive proof ( i think ).

\input{tex/proofs/progress/progress.tex}

\newpage
\section{Proof of Subject Reduction}
%
\input{tex/figs/processes/calculus.tex}
\input{tex/figs/processes/typing.tex}
%
\input{tex/figs/processes/reduction.tex}
%
\input{tex/figs/processes/func/time_passing.tex}
%
\input{tex/figs/processes/rule_typing.tex}
%
% \subsubsection*{Summary}

\subsubsection*{Overview of proof}
In~\cite{Bocchi2019} the subject reduction proof has the following structure
\begin{enumerate}
    \item implications of a well-typed process
    \item typing processes
    \item typing environment variables
    \item typing messages received processes
    \item delaying processes
    \item delaying sessions
    \item typing delayed sessions against delayed sessions
    \item any reduction of a well-typed process is also well-typed
\end{enumerate}
The proof then continues by proving that well-typed processes never reduces to a failed state, and that fail-free processes are always well-typed.
Processes are proven to always be fully-reducible using the \emph{untimed calculus}. Processes without time are always able to perform their next action, and are live.

% %
% \input{tex/defs/processes/domain_clocks.tex}
% \input{tex/defs/processes/t_reading.tex}
% %
% \input{tex/defs/processes/free_queues.tex}
% \input{tex/defs/processes/well_formed.tex}
% \input{tex/proofs/reduction/thm.tex}
% %
% \input{tex/defs/processes/session/balanced.tex}
% \input{tex/defs/processes/session/fully_balanced.tex}
% \input{tex/defs/processes/session/free_queues.tex}
% \input{tex/defs/processes/session/delayable.tex}
% \input{tex/defs/processes/session/reduction.tex}

% \subsubsection{*Overview of proof}


% \input{tex/proofs/reduction/reduction.tex}

% \newpage
% \section*{Question/Feedback LIST}
% \begin{itemize}
%     %
%     \item updated~\cref{fig:prc_func_time} to not remove "after Q" from infinite receptions as then it cannot be typed, and added \PFuncTime*\ to set(x).P
%           %
%     \item is there anywhere "nice" to explain that \LblPrcRedDelay*\ applies \PFuncTime* ?
%           %
%     \item tweaked~\cref{lem:configs_wf_timestep_fe} to reflect mixed-choice and the new \LblCfgSocTime*
%           %
%     \item rule \LblPrcTypRes*\ depends on \emph{compatibility}, which has been moved to the appendix.
%     \item include \LblPrcRedIfT*\ in reduction rules? how do i write that true is dependant on a clock existing to satisfy a \Const*?
%           %
% \end{itemize}

% \section*{Todo LIST}
% \begin{itemize}
%     %
%     \item update proof of progress
%           \begin{itemize}
%               \item recursive cases
%               \item update for new \LblCfgSocTime*\ rule for social configuration transitions
%           \end{itemize}
%           %
%     \item proof of subject reduction
%           \begin{itemize}
%               \item avoid fail-free by proving if-then-else and recv-after always hold, similarly as proof of progress
%           \end{itemize}
%           %
%     \item make sure \LblTypChoice*\ is correct
%     \item change future-enabled definition \& symbol to be directionless
%     \item move live definition to appendix
%     \item change semantic rules to be symmetric (not $i\neq j\{1,2\}$)
%     \item change notes about configuration notations to be paragraph
%     \item define configuration transitions
%     \item move compatibility to proof
%     \item make Andy new packaged-proof-paper with fixes and updates
%     \item update \ITypeAct*\ used in examples to better reflect \IMsgType*
%           %
% \end{itemize}


% % \pagebreak
% \appendix
% \section{Auxiliary Functions}
% % \FigPrcFuncTime*
% \input{tex/figs/processes/func/wait.tex}
% \input{tex/figs/processes/func/nonempty.tex}

\bibliographystyle{IEEEtran.bst}
\bibliography{bib_library.bib,time.bib}

\end{document}

\endinput

==> _types_and_processes_only.tex <==

% \begin{document}\newgeometry{left=1cm,right=1cm,top=1cm,bottom=1cm}

\input{tex/figs/types/syntax.tex}
\input{tex/figs/types/rule_formation.tex}

\input{tex/figs/configs/rule_iso.tex}
\begin{minieq}\label{eq:type_labels} \ProgAction::=\TypComm\Msg
    \mid\,\ValTime
    \mid\SiltAction
    %
    \qquad
    %
    \Msg::=\DefMsgType
    %
    \qquad \TypComm ::=!\mid?
    %
\end{minieq}

\input{tex/defs/types/duality.tex}

\input{tex/defs/types/well_formed.tex}

\input{tex/defs/configs/iso/future_en.tex}
\input{tex/defs/configs/iso/latest_en.tex}

\input{tex/defs/configs/iso/live.tex}

\input{tex/defs/configs/iso/well_formed.tex}

\input{tex/defs/configs/sys/compat.tex}
\input{tex/defs/types/progress.tex}
\input{tex/proofs/progress/thm.tex}

\input{tex/figs/processes/calculus.tex}

\input{tex/figs/processes/reduction.tex}

\input{tex/figs/processes/func/time_passing.tex}
\input{tex/figs/processes/func/wait.tex}
\input{tex/figs/processes/func/nonempty.tex}

\input{tex/defs/processes/free_queues.tex}
\input{tex/defs/processes/well_formed.tex}
\input{tex/defs/processes/fail_free.tex}

\input{tex/figs/processes/typing.tex}
\input{tex/figs/processes/rule_typing.tex}

\input{tex/defs/processes/session/balanced.tex}
\input{tex/defs/processes/session/fully_balanced.tex}

\input{tex/defs/processes/session/free_queues.tex}
\input{tex/defs/processes/session/delayable.tex}
\input{tex/figs/processes/session_reduction.tex}

\input{tex/proofs/reduction/thm.tex}


% \bibliographystyle{IEEEtran.bst}
% \bibliography{bib_library.bib,time.bib}

% \end{document}

\endinput

==> _types_only.tex <==

% \begin{document}%\newgeometry{left=1cm,right=1cm,top=1cm,bottom=1cm}

\input{tex/figs/types/syntax.tex}
\begin{minieq}\label{eq:types_constraints}
    %
    \Const ::= \TypeTrue%
    \mid \Clx>\ValTime%
    \mid \Clx=\ValTime%
    \mid \Clx-\Cly>\ValTime%
    \mid \Clx-\Cly=\ValTime%
    \mid \neg\Const%
    \mid \Const_1\land\Const_2%
    %
\end{minieq}
\input{tex/figs/types/rule_formation.tex}
%
\input{tex/figs/configs/rule_iso.tex}
\begin{minieq}\label{eq:type_labels}
    \ProgAction::=\TypComm\Msg
    ~\mid~\ValTime
    ~\mid~\SiltAction
    %
    \qquad
    \Msg::=\DefMsgType
    %
    \qquad
    \TypComm ::= \TypSend~\mid~\TypRecv
    %
    % \qquad
    % \Queue ::= \emptyset~\mid~\Msg;\Queue
    %
  \end{minieq}

\input{tex/defs/types/duality.tex}

\input{tex/defs/types/well_formed.tex}

\input{tex/defs/configs/iso/future_en.tex}
\input{tex/defs/configs/iso/latest_en.tex}

\input{tex/defs/configs/iso/live.tex}

\input{tex/defs/configs/iso/well_formed.tex}

\input{tex/defs/configs/sys/compat.tex}
\input{tex/defs/types/progress.tex}
\input{tex/proofs/progress/thm.tex}

% \end{document}

\endinput

==> library.tex <==
%\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}
\newcommand{\pvar}{X}
\newcommand{\zo}[1]{[#1]}
\newcommand{\subst}[2]{[#1/#2]}
\newcommand{\judg}[3]{#1   \proves  #3  \has  #2}

\newcommand{\ch}{a}
\newcommand{\chh}{b}
\newcommand{\chhh}{c}
\newcommand{\dclock}{x}
\newcommand{\aclock}{x_0}
\newcommand{\chvar}{a}
\newcommand{\chvarr}{b}
\newcommand{\chvarrr}{c}
\newcommand{\tmap}[2]{(#1 , \ #2)}
\newcommand{\proves}{\ \vdash \ }
\newcommand{\dom}[1]{\mathrm{dom}(#1)}

\newcommand{\preals}{\mathbf{R}_{\geq 0}}

%SEMANTICS
\newcommand{\reduce}{~~\longrightarrow~~}
%\newcommand{\timereduce}{~~\stackrel{ \blacktriangleright}{\longrightarrow}~~}
%\newcommand{\nowreduce}{~~\stackrel{\blacktriangledown}{\longrightarrow}~~}
\newcommand{\timereduce}{~~\rightsquigarrow~~}
\newcommand{\nowreduce}{~~\rightharpoonup~~}

\newcommand{\infer}[2]{\frac{\displaystyle{#1}%
{\vspace{3mm}}%
}{
{\vspace{3mm}}%
\displaystyle{#2}
}}
\newcommand{\unf}[1]{\textit{unfold}(#1)}
\newcommand{\Sorts}{T}
\newcommand{\ty}{\tva}

%NOTATIONS AND SETS
\newcommand{\guards}{\mathcal{G}}
\newcommand{\clocks}{\mathbb{X}}
\newcommand{\rel}{\mathcal{R}}
\newcommand{\Types}{\mathcal{S}}
\newcommand{\clock}{x}
\newcommand{\const}{n}
\newcommand{\rconst}{t}
\newcommand{\iconst}{i}

\newcommand{\resets}{\lambda}
\newcommand{\guard}{\delta}
\newcommand{\guardi}{\delta'}
\newcommand{\guardii}{\delta''}
\newcommand{\guardd}{\gamma}
\newcommand{\guarddi}{\gamma'}
\newcommand{\guarddii}{\gamma''}

\newcommand{\vc}{\nu}

\newcommand{\typevars}{\mathbb{A}}
\newcommand{\tva}{\alpha}
\newcommand{\tvai}{\alpha'}
\newcommand{\tvb}{\beta}
\newcommand{\tvbi}{\beta'}

\newcommand{\ocint}{]\hspace{-3pt}[}
\newcommand{\ve}[1]{\stackrel{~}{#1}}
\newcommand{\subs}[2]{[#1/#2]}
\newcommand{\recnull}{\_}
\newcommand{\subt}{<\,:}

\newcommand{\setcomp}[2]{\left\{{#1} \,\middle|\, {#2}\right\}}

%PROCESSES
\newcommand{\Pacc}[3]{\mathtt{accept} \ #1(#2) \ \mathtt{in} \ #3}
\newcommand{\Preq}[3]{\mathtt{request } \ #1(#2) \ \mathtt{in} \ #3}
\newcommand{\exception}{\mathtt{failed}}
\newcommand{\Frule}[1]{\small(\mathtt{#1})\normalsize}
\newcommand{\Prule}[1]{\small[\mathtt{#1}]\normalsize}
\newcommand{\Srule}[1]{{\footnotesize{\{\mathtt{#1}\}}\normalsize}}
\newcommand{\rdy}[1]{\mathtt{rdy}(#1)}
\newcommand{\wait}[1]{\mathtt{Wait}(#1)}
\newcommand{\queues}[1]{\mathtt{NEQueue}(#1)}

\newcommand{\Pend}{0}
%
\newcommand{\Psendc}[3]{\overline{#1}  \, #2   . \, #3}
\newcommand{\Psend}[2]{\overline{#1} \, #2 }
%
\newcommand{\Prcvc}[4]{#1^{#4}(#2).\, #3}
\newcommand{\Prcv}[3]{#1^{#3}(#2)}
%
\newcommand{\Pselc}[3]{{#1}\triangleleft\mathtt{#2}.\, #3}
\newcommand{\Psel}[2]{{#1}\triangleleft\mathtt{#2}}
%
\newcommand{\Pbra}[3]{{#1}^{#3}\triangleright \{\mathtt{#2}_{i}:P_{i}\}_{i\in I}}
%
\newcommand{\delay}[2]{\mathtt{delay}(#1).\, #2}
\newcommand{\delayp}[2]{\mathtt{delay}(\stackrel{#1}{\alap}).\, #2}
\newcommand{\grec}[3]{#1*(#2).\, #3}
\newcommand{\rep}[3]{!^{#2}_{#3}#1}
\newcommand{\now}{\mathtt{now}()}
%
\newcommand{\coda}{\mathit{h}}
\newcommand{\inter}[2]{\ocint #1 \ .. \ #2 \ocint}
\newcommand{\alap}{\leftrightarrow}
\newcommand{\has}{\triangleright}
\newcommand{\Pif}[3]{\mathtt{if}~#1~\mathtt{then}~#2~\mathtt{else}~#3}
\newcommand{\sacc}[3]{\overline{#1}(#2).#3}
\newcommand{\srec}[3]{#1(#2).#3}
%\newcommand{\sel}[4]{\oplus\{ \lab{#1} \ \ass{#2} \ : #3 \}_{#4}}
%\newcommand{\selnew}[4]{\oplus\{ \lab{#1} \  : #3 \}_{#4}}
%\newcommand{\selna}[3]{\oplus\{ \lab{#1}: \ass{#2} \}_{#3}}
%\newcommand{\seldiy}[1]{\oplus\{ {#1} \}}
%%
%\newcommand{\lab}[1]{\color{blue}\mathrm{#1}\color{black}}
%\newcommand{\sort}[1]{\mathtt{#1}}
%\newcommand{\ass}[1]{\color{red} { #1}\color{black}}
%%
%\newcommand{\bra}[4]{\& \{ \lab{#1} : #3 \}_{#4}}
%\newcommand{\brana}[3]{\&\{ \lab{#1}:  \}_{#3}}
%\newcommand{\bradiy}[1]{\& \{ #1 \}}

\newcommand{\MND}[2]{MND(#1,  #2 )}

\newcommand{\asym}{ \ \small \square \ }
%TYPES
\newcommand{\ST}{S}
\newcommand{\STi}{S'}
\newcommand{\STii}{S''}
\newcommand{\STiii}{S'''}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mSs}{\mathcal{S}^*}
%
\newcommand{\tend}{\mathtt{end}}
%
\newcommand{\jollyc}[3]{\asym   \sort{#1} \, {\ass{#3}} \, . #2}
\newcommand{\sendc}[3]{!   \sort{#1} \, {\ass{#3}} \, . #2}
\newcommand{\send}[2]{!  {#2}  \, \sort{#1} }
\newcommand{\rcvc}[3]{?  \sort{#1}\, {\ass{#3}} \, . #2}
\newcommand{\rcv}[2]{?  {#2} \, \sort{#1}}
\newcommand{\fn}[1]{\mathit{fn}(#1)}

\newcommand{\sep}{; \ }
%
%\newcommand{\sel}[4]{\oplus^\ass{#2}\{ \lab{#1} \  \ : #3 \}_{#4}}
\newcommand{\jollymc}[4]{\asym \{ \lab{#1}{\ass{#3}}  : {#2} \}_{#4}}
\newcommand{\selnew}[4]{\oplus \{ \lab{#1}{\ass{#3}}  : {#2} \}_{#4}}
%\newcommand{\selna}[3]{\oplus\{ \lab{#1}: \ass{#2} \}_{#3}}
%\newcommand{\seldiy}[1]{\oplus\{ {#1} \}}
%
\newcommand{\lab}[1]{\color{blue}\mathrm{#1}\color{black}}
\newcommand{\sort}[1]{{#1}}
\newcommand{\ass}[1]{\color{red} \small{ #1}\color{black}}
%
\newcommand{\branew}[4]{\&  \{ \lab{#1}   {\ass{#3}} : {#2} \}_{#4}}
%\newcommand{\brana}[3]{\&^\ass{#2}\{ \lab{#1}:  \}_{#3}}
%\newcommand{\bradiy}[1]{\&^ \{ #1 \}}

%
\newcommand{\dualdash}{\vdash_{\dual}}
\newcommand{\dual}[1]{\overline{#1}}
%Annotations
\newcommand{\fesend}[1]{#1 \stackrel{!}{\Rightarrow}}

\newcommand{\atrue}{\_}
\newcommand{\assert}[1]{\mathtt{assert}(#1)}
\newcommand{\assume}[1]{\mathtt{assume}(#1)}
\newcommand{\consume}[1]{\mathtt{consume}(#1)}
\newcommand{\reject}[1]{\mathtt{reject}(#1)}
\newcommand{\may}[1]{\mathtt{can}(#1)}
%Mixed
\newcommand{\mt}{\mathtt{true}}
\newcommand{\mf}{\mathtt{false}}
\newcommand{\mycite}[1]{(\ref{#1})}
\newcommand{\myeq}{:: =}
\newcommand{\env}{\mathcal{C}}
\newcommand{\myplus}{\ \underline{\uplus} \ }
\newcommand{\entails}{\Rightarrow }
\newcommand{\merge}[3]{ #2 \  \stackrel{#1}{\LEFTcircle}\  #3}
\newcommand{\unmerge}[3]{ #2  \ \stackrel{#1}{\LEFTCIRCLE} \ #3}
\newcommand{\direction}{\updownarrow}
\newcommand{\repeatable}[1]{\circlearrowright (#1)}
\newcommand{\trans}[1]{\stackrel{#1}{\rightarrow}}
\newcommand{\ntrans}[1]{\stackrel{#1}{\not \rightarrow}}
%Zones
\newcommand{\zones}{\mathcal{Z}}
\newcommand{\zone}{z}
\newcommand{\past}[1]{\mathbin{\downarrow {#1}}}
\newcommand{\future}[1]{\mathbin{\uparrow {#1}}}
\newcommand{\zoneReset}[2]{{#1}[{#2}\mapsto 0]}
\newcommand{\invReset}[2]{[{#2}\mapsto 0]^{-1}{#1}}
\newcommand{\rectangle}{\fboxsep0pt\fbox{\rule{1em}{0pt}\rule{0pt}{1ex}}}
\newcommand{\semenv}[3]{(#1, {#3},   #2) }
\newcommand{\ssemenv}[2]{(#1, \  #2 ) }
\newcommand{\mq}{\mathtt{M}}
\newcommand{\stype}[1]{\langle #1 \rangle}
\newcommand{\system}{\mathbf{S}}

\newcommand{\runR}[1][]{\rho_{#1}}
\newcommand{\runRi}[1][]{\rho'_{#1}}

\newcommand{\runconf}[2]{\mathit{conf}_{#1}{(#2)}}
\newcommand{\rundelay}[2]{\mathit{delay}_{#1}{(#2)}}
\newcommand{\runact}[2]{\mathit{act}_{#1}{(#2)}}
\newcommand{\runTime}[2]{\mathit{time}_{#1}{(#2)}}
%\newcommand{\ptp}[1]{\mathtt{\color{blue}#1}}
%\newcommand{\function}[2]{\mathbf{\mathit{\color{red}#1(}}#2\mathbf{\mathit{\color{red})}}}
%\newcommand{\GT}[4]{\ptp{#1}\rightarrow \ptp{#2} : \langle #3 \rangle . \mathit{#4}}
%\newcommand{\GTt}[5]{\ptp{#1}\rightarrow \ptp{#2} : \color{red}\{#5\}\color{black} \langle #3 \rangle . \mathit{#4}}
%\newcommand{\GTI}[4]{\ptp{#1}\rightsquigarrow \ptp{#2} : \langle #3 \rangle . \mathit{#4}}
%\newcommand{\GL}[5]{\ptp{#1}\rightarrow \ptp{#2} : \{ \lab{#3} : #4 \}_{#5}}
%\newcommand{\GLI}[5]{\ptp{#1}\rightsquigarrow \ptp{#2} : \{ #3 : #4 \}_{#5}}
%\newcommand{\LS}[3]{!\langle\ptp{#1}, #2 \rangle . \mathit{#3}}
%\newcommand{\LR}[3]{?\langle\ptp{#1}, #2 \rangle . \mathit{#3}}
%\newcommand{\LSel}[4]{\oplus \langle\ptp{#1}, \{ #2 : #3\}_{#4}\rangle}
%\newcommand{\LBra}[4]{\& \langle\ptp{#1}, \{ #2 : #3\}_{#4}\rangle}
%\newcommand{\tv}{\mathtt t}
%\newcommand{\var}[1]{\mathit{\color{magenta}#1}}
%\newcommand{\lab}[1]{\mathsf{\color[RGB]{17,53,115}#1}}
%\newcommand{\trans}[1]{~~\xrightarrow{#1}~~}
%\newcommand{\proj}{\upharpoonright}
%\newcommand{\mreq}[4]{\color{black}\overline{#1}\color{black}[\ptp{#2}](#3). #4}
%\newcommand{\macc}[4]{{#1}[\ptp{#2}](#3). #4}
%\newcommand{\prcv}[4]{{#1}?(\ptp{#2},#3). #4}
%\newcommand{\pdelsend}[4]{{#1}!\langle\!\langle\ptp{#2},#3\rangle\!\rangle.  #4}
%\newcommand{\pdelrcv}[4]{{#1}?(\! (\ptp{#2},#3)\!). #4}

%\newcommand{\prcvd}[4]{{#1}?((\ptp{#2},#3)). #4}
%\newcommand{\psel}[4]{{#1}\oplus\langle\ptp{#2},#3\rangle. #4}
%\newcommand{\pbra}[5]{{#1}\&(\ptp{#2},\{#3:#4\}_{#5})}
%\newcommand{\pif}[3]{\mathsf{if}~{#1}~\mathsf{then}~{#2}~\mathsf{else}~{#3}}
%\newcommand{\pdef}[2]{\mathsf{def}~{#1}~\mathsf{in}~{#2}}
%\newcommand{\pcall}[3]{#1\langle#2,#3\rangle}
%\newcommand{\und}[1]{\color{red}#1\color{black}}
%\begin{array}{lll}
%T & ::= & \LS{p}{\mathit{S}}{T}\\ 
% & \mid & \LS{p}{\mathsf{T}}{T}\\
% & \mid & \LR{p}{\mathit{U}}{T}\\
% & \mid & \LSel{p}{l_i}{T_i}{i\in I}\\
% & \mid & \LBra{p}{l_i}{T_i}{i\in I}\\
% & \mid & \mu \tv . \mathit{T} \\
% & \mid & \tv \\
% & \mid & \mathtt{end} \\
%\end{array}

%\begin{array}{ll}
%\GT{p}{p'}{\var U}{G'} \upharpoonright \ptp q = 
%\begin{cases}
%\LS{p'}{U}{G'\upharpoonright \ptp q} & \text{if }\ptp q = \ptp p, \\
%\LR{p}{U}{G'\upharpoonright \ptp q} & \text{if }\ptp q = \ptp{p'}, \\
%G\upharpoonright \ptp q & \text{otherwise}.
%\end{cases}\\
%\GL{p}{p'}{l_i}{G_i}{i\in I} \upharpoonright \ptp q = 
%\begin{cases}
%\LSel{p'}{l_i}{G_i\upharpoonright \ptp q}{i\in I} & \text{if }\ptp q = \ptp p, \\
%\LBra{p}{l_i}{G_i\upharpoonright \ptp q}{i\in I} & \text{if }\ptp q = \ptp{p'}, \\
%G_{i0}\upharpoonright \ptp q & \text{if } \ptp p , ~\ptp{p'} \not = \ptp p,~i0\in I,~ G_i\upharpoonright \ptp q = G_j\upharpoonright \ptp q ~\text{for all }i,j\in I.
%\end{cases}
%\end{array}


==> macros/_test_sheet.tex <==
\newgeometry{left=3cm,right=3cm,top=3cm,bottom=3cm}

\begin{longtable}[t]{r c | c  l}
    %
    \texttt{Macro*}     & \mbox{} & \mbox{} & \texttt{Output} \\
    \hline
    %
    \verb|\Entails|         &         &         & \Entails*           \\
    \verb|\Par|         &         &         & \Par*           \\
    \verb|\Compat|      &         &         & \Compat*        \\
    \verb|\TypeTrue|    &         &         & \TypeTrue*      \\
    \verb|\TypeFalse|   &         &         & \TypeFalse*     \\
    \verb|\TypeEnd|     &         &         & \TypeEnd*       \\
    \verb|\PrcEnd|      &         &         & \PrcEnd*        \\
    \verb|\TypeS|       &         &         & \TypeS*         \\
    \verb|\DataType|    &         &         & \DataType*      \\
    \verb|\MsgType|     &         &         & \MsgType*       \\
    \verb|\MsgLabel|    &         &         & \MsgLabel*      \\
    \verb|\MsgData|     &         &         & \MsgData*       \\
    \verb|\Const|       &         &         & \Const*         \\
    \verb|\RSet|       &         &         & \RSet*         \\
    \verb|\RecDef|      &         &         & \RecDef*        \\
    \verb|\TypRecLabel| &         &         & \TypRecLabel*   \\
    \verb|\ProgAction|  &         &         & \ProgAction*    \\
    \verb|\SiltAction|  &         &         & \SiltAction*    \\
    \verb|\Prc|         &         &         & \Prc*           \\
    \verb|\Qrc|         &         &         & \Qrc*           \\
    \verb|\PrcP|        &         &         & \PrcP*          \\
    \verb|\PrcQ|        &         &         & \PrcQ*          \\
    \verb|\SesP|        &         &         & \SesP*          \\
    \verb|\RecVar|      &         &         & \RecVar*        \\
    \verb|\PrcScope|    &         &         & \PrcScope*      \\
    \verb|\TypComm|     &         &         & \TypComm*       \\
    \verb|\TypSend|     &         &         & \TypSend*       \\
    \verb|\TypRecv|     &         &         & \TypRecv*       \\
    \verb|\PrcRecv|     &         &         & \PrcRecv*       \\
    \verb|\PrcSend|     &         &         & \PrcSend*       \\
    \verb|\PrcTyped|    &         &         & \PrcTyped*      \\
    \verb|\TRed|        &         &         & \TRed*          \\
    \verb|\ARed|        &         &         & \ARed*          \\
    \verb|\PrcRed|      &         &         & \PrcRed*        \\
    \verb|\TypEnv|      &         &         & \TypEnv*        \\
    \verb|\RecEnv|      &         &         & \RecEnv*        \\
    \verb|\VarEnv|      &         &         & \VarEnv*        \\
    \verb|\SesEnv|      &         &         & \SesEnv*        \\
    \verb|\SesSet|      &         &         & \SesSet*        \\
    \verb|\ValClocks|   &         &         & \ValClocks*     \\
    \verb|\ValTime|     &         &         & \ValTime*       \\
    \verb|\IsoCfg|      &         &         & \IsoCfg*        \\
    \verb|\SocCfg|      &         &         & \SocCfg*        \\
    \verb|\Queue|       &         &         & \Queue*         \\
    \verb|\QHead|       &         &         & \QHead*         \\
    \verb|\Msg|         &         &         & \Msg*           \\
    \verb|\PrcMsg|      &         &         & \PrcMsg*        \\
    \verb|\QVal|        &         &         & \QVal*          \\
    \verb|\QLabel|      &         &         & \QLabel*        \\
    \verb|\SetI|        &         &         & \SetI*          \\
    \verb|\SetJ|        &         &         & \SetJ*          \\
    \verb|\RatSet|      &         &         & \RatSet*        \\
    \verb|\ClockSet|    &         &         & \ClockSet*      \\
    \verb|\GuardSet|    &         &         & \GuardSet*      \\
    \verb|\JudgeTyp|    &         &         & \JudgeTyp*      \\
    \verb|\JudgePrc|    &         &         & \JudgePrc*      \\
    \verb|\FuncDelay|   &         &         & \FuncDelay*     \\
    \verb|\FuncWait|    &         &         & \FuncWait*      \\
    \verb|\FuncNEQ|     &         &         & \FuncNEQ*       \\
    \verb|\PrcFail|     &         &         & \PrcFail*       \\
    \verb|\Const|       &         &         & \Const*         \\
    \verb|\Const|       &         &         & \Const*         \\
    \verb|\Const|       &         &         & \Const*         \\
    %
\end{longtable}

% \begin{longtable}[t]{r c l | l}
%     %
%     \texttt{Macro*}           & \hspace{1ex}
%                               & \texttt{Arguments}
%                               & \texttt{Output}                         \\ % *
%     \hline
%     %
%     % ~ base type delegate
%     \verb|\TmpTest|           &
%                               &
%                               & \TmpTest*                               \\ % *

%                               &
%                               & \verb|2{\Qrc}|
%                               & \TmpTest*2{\Qrc}                        \\ % *

%                               &
%                               & \verb|1{\text{none}}3{\emptyset}|
%                               & \TmpTest*1{\text{none}}3{\emptyset}     \\ % *
%     \hline
%     %
%     % ~ base type delegate
%     \verb|\PCalcSend|         &
%                               &
%                               & \PCalcSend*                             \\ % *

%                               &
%                               & \verb|.|
%                               & \PCalcSend*.                            \\ % *

%                               &
%                               & \verb|.[\Prc]|
%                               & \PCalcSend*.[\Prc]                      \\ % *
%     \hline
%     %
%     % ~ base type delegate
%     \verb|\PCalcRecv|         &
%                               &
%                               & \PCalcRecv*                             \\ % *

%                               &
%                               & \verb|/a|
%                               & \PCalcRecv*/a                           \\ % *
%     \hline
%     %
%     % ~ base type delegate
%     \verb|\TmpTypFutureSat|   &
%                               &
%                               & \TmpTypFutureSat*                       \\ % *

%                               &
%                               & \verb|'|
%                               & \TmpTypFutureSat*'                      \\ % *

%                               &
%                               & \verb|_j[\Resets[\Const'_i]]|
%                               & \TmpTypFutureSat*_j[\Resets[\Const'_i]] \\ % *

%                               &
%                               & \verb|[\Const']_i|
%                               & \TmpTypFutureSat*[\Const']_i            \\ % *
%     \hline
%     %
%     % ~ base type delegate
%     \verb|\TmpTypBTDelegate|  &
%                               &
%                               & \TmpTypBTDelegate*                      \\ % *

%                               &
%                               & \verb|''_i|
%                               & \TmpTypBTDelegate*''_i                  \\ % *

%                               &
%                               & \verb|'_i_j|
%                               & \TmpTypBTDelegate*'_i_j                 \\ % *
%     \hline
%     %
%     % ~ type judgement
%     \verb|\TmpTypJudge|       &
%                               &
%                               & \TmpTypJudge*                           \\ % *

%                               &
%                               & \verb|'|
%                               & \TmpTypJudge*'                          \\ % *

%                               &
%                               & \verb|'_j|
%                               & \TmpTypJudge*'_j                        \\ % *

%                               &
%                               & \verb|'_i[j]|
%                               & \TmpTypJudge*'_i[j]                     \\ % *

%                               &
%                               & \verb.|_j[k].
%                               & \TmpTypJudge*|_j[k]                     \\ % *

%                               &
%                               & \verb.|.
%                               & \TmpTypJudge*|                          \\ % *

%                               &
%                               & \verb./.
%                               & \TmpTypJudge*/                          \\ % *

%                               &
%                               & \verb./|.
%                               & \TmpTypJudge*/|                         \\ % *
%     \hline
%     %
%     % ~ template interact
%     \verb|\TmpTypSetInteract| &
%                               &
%                               & \TmpTypSetInteract*                     \\ % *

%                               &
%                               & \verb|!|
%                               & \TmpTypSetInteract*!                    \\ % *

%                               &
%                               & \verb|!?'|
%                               & \TmpTypSetInteract*!?'                  \\ % *

%                               &
%                               & \verb|?'[j][k]|
%                               & \TmpTypSetInteract*?'[j][k]             \\ % *
%     \hline
%     %
%     % ~ template interact
%     \verb|\TmpTypInteract|    &
%                               &
%                               & \TmpTypInteract*                        \\ % *

%                               &
%                               & \verb|!|
%                               & \TmpTypInteract*!                       \\ % *

%                               &
%                               & \verb|?|
%                               & \TmpTypInteract*?                       \\ % *

%                               &
%                               & \verb|!?|
%                               & \TmpTypInteract*!?                      \\ % *

%                               &
%                               & \verb|?!|
%                               & \TmpTypInteract*?!                      \\ % *

%                               &
%                               & \verb|'|
%                               & \TmpTypInteract*'                       \\ % *

%                               &
%                               & \verb|!'|
%                               & \TmpTypInteract*!'                      \\ % *

%                               &
%                               & \verb|!?'|
%                               & \TmpTypInteract*!?'                     \\ % *

%                               &
%                               & \verb|'_i|
%                               & \TmpTypInteract*'_i                     \\ % *

%                               &
%                               & \verb|!'_j|
%                               & \TmpTypInteract*!'_j                    \\ % *

%                               &
%                               & \verb|!?'_k|
%                               & \TmpTypInteract*!?'_k                   \\ % *
%     \hline
%     %
%     % ~ InSet
%     \verb|\InSet|             &
%                               &
%                               & \InSet*                                 \\ % *

%                               &
%                               & \verb|^[i]|
%                               & \InSet*^[i]                             \\ % *

%                               &
%                               & \verb|[i]'[i]|
%                               & \InSet*[i]'[i]                          \\ % *

%                               &
%                               & \verb|^[i][i]'|
%                               & \InSet*^[i][i]'                         \\ % *

%                               &
%                               & \verb|^''|
%                               & \InSet*^''                              \\ % *

%                               &
%                               & \verb|^[i][j][k]|
%                               & \InSet*^[i][j][k]                       \\ % *

%                               &
%                               & \verb|[i][j]'[k]|
%                               & \InSet*[i][j]'[k]                       \\ % *

%                               &
%                               & \verb|^[i]'[j]'[k]|
%                               & \InSet*^[i]'[j]'[k]                     \\ % *

%                               &
%                               & \verb|'''|
%                               & \InSet*'''                              \\ % *
%     \hline
%     %
%     % ~ act
%     \verb|\Act|               &
%                               &
%                               & \Act*                                   \\ % *

%                               &
%                               & \verb|/|
%                               & \Act*/                                  \\ % *

%                               &
%                               & \verb|[\TypSend\MsgLabel]|
%                               & \Act*[\TypSend\MsgLabel]                \\ % *

%                               &
%                               & \verb|/[\TypRecv\MsgLabel']|
%                               & \Act*/[\TypRecv\MsgLabel']              \\ % *
%     \hline
%     %
%     % ~ future enabled
%     \verb|\FutureEn|          &
%                               &
%                               & \FutureEn*                              \\ % *

%                               &
%                               & \verb|/|
%                               & \FutureEn*/                             \\ % *

%                               &
%                               & \verb|[\TypSend]|
%                               & \FutureEn*[\TypSend]                    \\ % *

%                               &
%                               & \verb|/[\TypRecv]|
%                               & \FutureEn*/[\TypRecv]                   \\ % *
%     \hline
%     %
%     %
% \end{longtable}


\restoregeometry
\endinput

==> macros/sessiontypes/_tools/_init.tex <==

\newcommand\IListNewLineLong{\\[2ex]}%
\newcommand\IListNewLineShort{\\[0.5ex]}%
\newcommand\IListNewLine{\\}%

\newcommand\IListInLineShort{,\;}%
\newcommand\IListInLine{,\quad\mbox{}}%

% ~ flex vars
\let\TypChoiceSep\IListNewLineShort%
\let\PrcRecvSep\IListNewLine%
\let\PrcRecvAfterSep\IListNewLine%
\let\PrcBranchAfterSep\IListNewLineLong%
\let\PrcIfSep\IListNewLine%
\let\PrcThenSep\IListNewLine%
\let\PrcElseSep\IListNewLine%

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
    \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}
    
\newcommand*\rectround[1]{\tikz[baseline=(char.base)]{
    \node[shape=rectangle,rounded corners,draw,inner sep=2pt] (char) {#1};}}
    
\newcommand*\squared[1]{\tikz[baseline=(char.base)]{
    \node[shape=rectangle,draw,inner sep=1.5pt] (char) {#1};}}


==> macros/sessiontypes/_tools/_input_all.tex <==


% \input{macros/}


% \endinput

\input{macros/sessiontypes/tools/new/_init.tex}

\input{macros/sessiontypes/tools/new/buff_queue.tex}
\input{macros/sessiontypes/tools/new/configs.tex}

\input{macros/sessiontypes/tools/new/general/general.tex}
\input{macros/sessiontypes/tools/new/general/parallel.tex}
\input{macros/sessiontypes/tools/new/general/tuple.tex}


\input{macros/sessiontypes/tools/new/types/type.tex}
\input{macros/sessiontypes/tools/new/types/choice.tex}
\input{macros/sessiontypes/tools/new/types/recursion.tex}


\input{macros/sessiontypes/tools/new/processes/general.tex}
\input{macros/sessiontypes/tools/new/processes/messages.tex}
\input{macros/sessiontypes/tools/new/processes/comm.tex}
\input{macros/sessiontypes/tools/new/processes/branch.tex}
\input{macros/sessiontypes/tools/new/processes/ifthenelse.tex}
\input{macros/sessiontypes/tools/new/processes/recursion.tex}

\input{macros/sessiontypes/tools/new/processes/calc.tex}

\input{macros/sessiontypes/tools/new/judgements/types.tex}
\input{macros/sessiontypes/tools/new/judgements/process_typing.tex}
\input{macros/sessiontypes/tools/new/judgements/eval.tex}


==> macros/sessiontypes/_tools/configs/practice/configs.tex <==

% ~ isolated configurations
% #1 : s* : math mode
% #2 : t~ : dual clock valuation
% #3 : Ov : clock valuation
% #4 : e+ : time step over clock valuations
% #5 : t; : sep
% #6 : t~ : dual type
% #7 : Os : type
% #8 : t' : prime 
% #9 : e_ : all subscript
\NewDocumentCommand{\CIso}{s t~ O{\ValClocks} e+ t; t~ O{\TypeS} t' e_}{%
    \IfBooleanT{#1}{$}%
    \IfValueTF{#9}{% * subscripted
        \Tup(\IfBooleanTF{#2}{\Dual[{#3}_{#9}\IfBooleanT{#8}{'}]\IfValueT{#4}{#4}}{{#3}_{#9}\IfBooleanT{#8}{'}\IfValueT{#4}{#4}},\IfBooleanTF{#6}{\Dual[{#7}_{#9}\IfBooleanT{#8}{'}]}{{#7}_{#9}\IfBooleanT{#8}{'}})%
    }{% * no subscript
        \Tup(\IfBooleanTF{#2}{\Dual[{#3}\IfBooleanT{#8}{'}]\IfValueT{#4}{#4}}{{#3}\IfBooleanT{#8}{'}\IfValueT{#4}{#4}},\IfBooleanTF{#6}{\Dual[{#7}\IfBooleanT{#8}{'}]}{{#7}\IfBooleanT{#8}{'}})%
    }%
    \IfBooleanT{#1}{$}%
}

% ~ social configurations
% #1 : s* : math mode
% #2 : Ov : clock valuation
% #3 : e+ : time step over clock valuations
% #4 : t; : sep
% #5 : Os : type
% #6 : E: : queue
% #7 : e+ : messages at the end of the queue
% #8 : t' : all prime
% #9 : e_ : all subscript
\NewDocumentCommand{\CSoc}{s O{\ValClocks} e+ t; O{\TypeS} E:{\Queue} e+ t' e_}{%
    \IfBooleanT{#1}{$}
    \Tup(% * valuation
    {{#2\IfValueT{#9}{_{#9}}\IfBooleanT{#8}{'}}\IfValueT{#3}{#3}},%
    % * type
    {#5\IfValueT{#9}{_{#9}}\IfBooleanT{#8}{'}},%
    % * queue
    {{#6\IfValueT{#9}{_{#9}}\IfBooleanT{#8}{'}}\IfValueT{#7}{;#7}})%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\CSys}{s O{\CSoc_1} O{\CSoc_2}}{%
    \IfBooleanT{#1}{$}%
    \Parl{{#2},{#3}}%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\VIso}{s t' e_}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#2}{% * '
        \IfValueTF{#3}{% * subscripted
            {\IsoCfg}_{#3}'%
        }{% * not sub
            {\IsoCfg'}%
        }%
    }{% * not prime 
        \IfValueTF{#3}{% * subscripted
            {\IsoCfg}_{#3}%
        }{% * not sub
            {\IsoCfg}%
        }%
    }%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\VSoc}{s t' t' e_}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#2}{% * '
        \IfBooleanTF{#3}{% * second '
            \IfValueTF{#4}{% * subscripted
                {\SocCfg}_{#4}''%
            }{% * not sub
                {\SocCfg''}%
            }%
        }{% * no second '
            \IfValueTF{#4}{% * subscripted
                {\SocCfg}_{#4}'%
            }{% * not sub
                {\SocCfg'}%
            }%
        }%
    }{% * not prime 
        \IfValueTF{#4}{% * subscripted
            {\SocCfg}_{#4}%
        }{% * not sub
            {\SocCfg}%
        }%
    }%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\VSys}{s t' e_ t' e_}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#4}{% * second prime ?
        \IfBooleanTF{#2}{% * first prime ?
            \IfValueTF{#3}{% * first subscript?
                \IfValueTF{#5}{% * second subscript?
                    \Parl{\VSoc'_{#3},\VSoc'_{#5}}%
                }{% * no second subscript
                    \Parl{\VSoc'_{#3},\VSoc'_{2}}%
                }%
            }{% * no first subscript
                \IfValueTF{#5}{% * second subscript?
                    \Parl{\VSoc'_{1},\VSoc'_{#5}}%
                }{% * no second subscript: double prime if no subscripts
                    \Parl{\VSoc''_1,\VSoc''_2}%
                }%
            }%
        }{% * no first prime
            \Parl{%
                \IfValueTF{#3}{\VSoc_{#3}}{\VSoc_1},%
                \IfValueTF{#5}{\VSoc'_{#5}}{\VSoc'_2}%
            }%
        }%
    }{% * no second prime prime
        \IfBooleanTF{#2}{% * first prime ?
            \IfValueTF{#3}{% * first subscript ?
                \Parl{%
                    \VSoc'_{#3},%
                    \IfValueTF{#5}{\VSoc_{#5}}{\VSoc_2}%
                }%
            }{% * no first subscript
                \IfValueTF{#5}{% * second subscript ?
                    \Parl{%
                        \VSoc'_1,%
                        \VSoc'_{#5}%
                    }%
                }{% * no second subscript: use first prime for both
                    \Parl{%
                        \VSoc'_1,%
                        \VSoc'_2%
                    }%
                }%
            }%
        }{% * no first prime
            \Parl{%
                \IfValueTF{#3}{\VSoc_{#3}}{\VSoc_1},%
                \IfValueTF{#5}{\VSoc_{#5}}{\VSoc_2}%
            }%
        }%
    }%
    \IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/configs/theory/configurations.tex <==


% ~ rec def def
% #1: * mm
\NewDocumentCommand{\CfgRecDef}{s O{\RecDef} O{\CfgRecLabel}}{%
    \IfBooleanT{#1}{$}% mm wrap
    {#2}{#3}
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ iso conf tuple
% #1: * mm
\NewDocumentCommand{\CfgIso}{s e_ E1{{\ValClocks}} t' E2{{\TypeS}} t'}{%
    \IfBooleanT{#1}{$}% mm wrap
    \mkTup[{\FmtMathOp{#3}{#4}_{#2}}][{\FmtMathOp{#5}{#6}_{#2}}]
    \IfBooleanT{#1}{$}% mm wrap
}


% ~ soc conf tuple
% #1: * mm
\NewDocumentCommand{\CfgSoc}{s e_ E1{{\ValClocks}} t' E2{{\TypeS}} t' E3{{\Queue}} t'}{%
    \IfBooleanT{#1}{$}% mm wrap
    \mkTup[{\FmtMathOp{#3}{#4}_{#2}}][{\FmtMathOp{#5}{#6}_{#2}}][{\FmtMathOp{#7}{#8}_{#2}}]
    \IfBooleanT{#1}{$}% mm wrap
}


% ~ sys
\NewDocumentCommand{\CfgSys}{s E1{{\SocCfg_1}} E2{{\SocCfg_2}}}{%
    \IfBooleanT{#1}{$}% mm wrap
    \Par[#2][#3]
    \IfBooleanT{#1}{$}% mm wrap
}


==> macros/sessiontypes/_tools/general/buff_queue.tex <==

% ~ 
\NewDocumentCommand\ListToBuffContents{>{\SplitList{,}}m}
{%
    {\ProcessList{#1}{\HeadBuffContents}}%
}

% ~ 
\newcommand\HeadBuffContents[1]{%
    \circled{$\mathtt{#1}$}%
    \let\HeadBuffContents\TailBuffContents%
}

% ~ inserts cdot before each subsequent par item
\newcommand\TailBuffContents[1]{%
    \!\;\cdot\,\circled{$\mathtt{#1}$}%
}

% ~ 
\NewDocumentCommand{\IBuff}{s O{\ISes} e:}{%
    \IfBooleanT{#1}{$}% mm wrap
    {#2}:%
    \IfNoValueTF{#3}{% * no buffer contents given
        \emptyset%
    }{% * use given contents
        {\ListToBuffContents{#3}}%
    }%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ 
\NewDocumentCommand\ListToQueContents{>{\SplitList{,}}m}
{%
    {\ProcessList{#1}{\HeadQueContents}}%
}

% ~ 
\newcommand\HeadQueContents[1]{%
    \squared{$\mathtt{#1}$}%
    \let\HeadQueContents\TailQueContents%
}

% ~ inserts ; before each subsequent par item
\newcommand\TailQueContents[1]{%
    \!\;;\,\squared{$\mathtt{#1}$}%
}

% ~ 
\NewDocumentCommand{\IQue}{s O{\ISes} e:}{%
    \IfBooleanT{#1}{$}% mm wrap
    {#2}:%
    \IfNoValueTF{#3}{% * no buffer contents given
        \emptyset%
    }{% * use given contents
        {\ListToQueContents{#3}}%
    }%
    \IfBooleanT{#1}{$}% mm wrap
}


==> macros/sessiontypes/_tools/general/general.tex <==

% ~ judgements
% #1 : s* : 
% #2 : t| : part of inferrule?
% #3 : m  : 
% #4 : m  : 
% #5 : o  : typing process
\NewDocumentCommand{\FmtJudgement}{s t| m m o}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{l}{#3}\end{array}%
    \IfBooleanTF{#2}{\ \\\ }{\!\;}%
    {\Entails}%
    \IfBooleanTF{#2}{\ \\\ }{\!\,}%
    \begin{array}[t]{l}{#4}\end{array}%
    \IfValueT{#5}{% * prc typing judgement
        \IfBooleanTF{#2}{\ \\\ }{\!\;}%
        {\PrcTyped}%
        \IfBooleanTF{#2}{\ \\\ }{\!\,}%
        \begin{array}[t]{l}{#5}\end{array}%
    }%
    \IfBooleanT{#1}{$}%
}

% ~ end points
% #1 : s* : math mode wrap
% #2 : t| : swap default endpoints
% #3 : Op : endpoint p
% #4 : Oq : endpoint q
\NewDocumentCommand{\ISes}{s t| O{\PrcQ} O{\PrcP}}{%
    \IfBooleanT{#1}{$}% mm wrap
    \IfBooleanTF{#2}{% * swap endpoints
        {#4}{#3}%
    }{% * default order
        {#3}{#4}%
    }%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ env items from list
\NewDocumentCommand\ListToEnvItems{>{\SplitList{,}}m}{%
    {\ProcessList{#1}{\ListEnvItem}}%
}

% ~ 
\newcommand\ListEnvItem[1]{%
    \!\,,\,{#1}%
}

% ~ for unions of constraints
\NewDocumentCommand{\IConstOr}{s t| O{\Const} E_{i} E:{\SetI}}{%
    \IfBooleanT{#1}{$}% mm wrap
    \IfBooleanTF{#2}{% * past
        \Past[{\SetOr_{\hspace{-0.5ex}\vspace{0.5ex}\scriptstyle{\AsSet[#4][#5]}}}{#3_{#4}}]%
    }{% * no past
        {\SetOr_{\hspace{-0.5ex}\vspace{0.5ex}\scriptstyle{\AsSet[#4][#5]}}}{#3_{#4}}%
    }%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ future enabled
% #1: * mm
% #2: t/
% #3: O
\NewDocumentCommand{\ActFE}{s t! t? t' m t|}{%
    \IfBooleanT{#1}{$}% mm wrap
    {#5}\!\stackrel{\IfBooleanTF{#2}{\TypSend}{\IfBooleanTF{#3}{\TypRecv}{\TypComm\IfBooleanT{#4}{'}}}}{\IfBooleanT{#6}{\not}\Rightarrow}%
    \IfBooleanT{#1}{$}% mm wrap
}

==> macros/sessiontypes/_tools/general/parallel.tex <==

% ~ smarter par
\NewDocumentCommand{\Parl}{s m}{%
    \IfBooleanT{#1}{$}%
    \ListToParl{#2}%
    \IfBooleanT{#1}{$}%
}


% ~ tex math mode spacing
\NewDocumentCommand\ListToParl{>{\SplitList{,}}m}
{%
    {\ProcessList{#1}{\HeadParlContents}}%
}

% ~ 
\newcommand\HeadParlContents[1]{%
    {#1}%
    \let\HeadParlContents\TailParlContents%
}

% ~ inserts | before each subsequent par item
\newcommand\TailParlContents[1]{%
    \!\,{\mid}\;\!{#1}%
}


==> macros/sessiontypes/_tools/general/tuple.tex <==

% #1 : s* : math mode wrap
% #2 : () : tup contents
% #3 : t| : use \left(\right)
\NewDocumentCommand{\Tup}{s D(){\emptyset} t|}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#3}{% * use strechy brackets
        \left(\ListToTupleContents{#2}\right)
    }{% * use normal ()
        (\ListToTupleContents{#2})
    }
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand\ListToTupleContents{>{\SplitList{,}}m}{%
    {\ProcessList{#1}{\HeadTupleContents}}%
}

% ~ 
\newcommand\HeadTupleContents[1]{%
    \!\;{#1}%
    \let\HeadTupleContents\TailTupleContents%
}

% ~ inserts | before each subsequent par item
\newcommand\TailTupleContents[1]{%
    \!\,,\;{#1}%
    \let\HeadTupleContents\TailTupleContents%
}


==> macros/sessiontypes/_tools/judgements/eval.tex <==
% ~ 
% #1 : s* : math mode wrap
% #2 : t< : put label on left side?
% #3 : o  : optional label
% #4 : e: : (bot) judgement
% #5 : E: : (top) premise (\Premise list)
\NewDocumentCommand{\IEval}{s t< o e: E:{\Premise}}{%
    \IfBooleanT{#1}{$}%
    \IfValueTF{#3}{% * has label
        \IfBooleanTF{#2}{% * use left side label
            {\inferrule*[Left={[#3]}]{%
                \rule{0pt}{2ex}#5%
            }{%
                {#4}%
            }}%
        }{% * use right aligned label (default)
            {\inferrule*[Right={[#3]}]{%
                \rule{0pt}{2ex}#5%
            }{%
                {#4}%
            }}%
        }%
    }{% * no label
        {\inferrule*{%
            \rule{0pt}{2ex}#5%
        }{%
            {#4}%
        }}%
    }%
    \IfBooleanT{#1}{$}%
}

% ! replaced by IT/IP Judgement macros
\NewDocumentCommand{\GenericJudgement}{s O{\emptyset\Entails\Prc\PrcTyped\SesEnv}}{%
    {\ListToInlineArgs{#2}}%
}

\NewDocumentCommand{\Premise}{s t| O{\dots}}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#2}{% * single premise
        {#3}%
    }{% * list of premises
        {\ListToInlineArgs{#3}}%
    }%
    \IfBooleanT{#1}{$}%
}


% ~ 
\NewDocumentCommand\ListToInlineArgs{>{\SplitList{,}}m}
{%
    \ProcessList{#1}{\HeadItemToInlineArgs}%
}

% ~ 
\newcommand\HeadItemToInlineArgs[1]{%
    {#1}%
    \let\HeadItemToInlineArgs\TailItemToInlineArgs%
}

\newcommand\TailItemToInlineArgs[1]{%
    \ \\\ {#1}%
    \let\HeadItemToInlineArgs\TailItemToInlineArgs% * rebinding due to outer processor being unscoped
}


==> macros/sessiontypes/_tools/judgements/process_typing.tex <==

\NewDocumentCommand{\IPJEnv}{s O{\VarEnv} e:}{%
    \IfBooleanT{#1}{$}%
    % * Gamma
    {#2}%
    \IfValueT{#3}{% * Gamma contents?
        \ListToEnvItems{#3}%
    }%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\IPJPrc}{s o}{%
    \IfBooleanT{#1}{$}%
    % * default process
    \IfNoValueTF{#2}{\Prc}{% * else list of par processes
        \Parl{#2}%
    }%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\IPJSes}{s O{\VarEnv} e:}{%
    \IfBooleanT{#1}{$}%
    % * Delta
    {#2}%
    \IfValueT{#3}{% * Delta contents?
        \ListToEnvItems{#3}%
    }%
    \IfBooleanT{#1}{$}%
}

% ~ 
% #1 : s* : 
% #2 : Og : 
% #3 : e: : 
% #4 : t< : delimiter for #6 >
% #5 : Op : 
% #6 : t> : delimiter for #4 <
% #7 : Od : 
% #8 : e: : 
\NewDocumentCommand{\IPJudgement}{s O{\VarEnv} e: t< O{\Prc} t> O{\SesEnv} e:}{%
    \IfBooleanTF{#1}{$\FmtJudgement}{\FmtJudgement|}%
    {% * Gamma
        \IfNoValueTF{#3}{\IPJEnv[#2]}{% * Gamma vars
            \IPJEnv[#2]:{#3}%
        }%
    }{% * Process
        \IPJPrc[#5]%
    }[% * Delta
        \IfNoValueTF{#8}{\IPJSes[#7]}{% * Delta roles
            \IPJSes[#7]:{#8}%
        }%
    ]%
    \IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/judgements/types.tex <==

\NewDocumentCommand{\ITJRec}{s O{\emptyset} e:}{%
    \IfBooleanT{#1}{$}%
    {#2}%
    \IfValueT{#3}{% * rec vars in A
        \ListToEnvItems{#3}%
    }%
    \IfBooleanT{#1}{$}%
}

% ~ 
% #1 : s* : mathmode wrap
% #2 : t| : is past?
% #3 : Ot : const
% #4 : e_ : subscript?
% #5 : E: : of set?
\NewDocumentCommand{\ITJCon}{s t| O{\TypeTrue} e_ E:{\SetI}}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{l}%
        \IfValueTF{#4}{% * subscript
            \IfBooleanTF{#2}{% * past
                \IConstOr|[#3]_{#4}:{#5}%
            }{% * not past
                \IConstOr[#3]_{#4}:{#5}%
            }%
        }{% * no subscript
            \IfBooleanTF{#2}{% * past
                \Past[#3]%
            }{% * not past
                {#3}%
            }%
        }%
    \end{array}%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\TypEnvCond}{s E:{\TypEnv} O{\TypeS}}{%
    \IfBooleanT{#1}{$}%
    \FmtJudgement{#2}{#3}%
    \IfBooleanT{#1}{$}%
}

\NewDocumentCommand{\ITJTyp}{s t| O{\TypeEnd} e_ E<{\SetI}}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#2}{% * do not wrap in set ?
        \ListToTupleContents{#3}%
    }{% * wrap in set
        \IfValueTF{#4}{% * use set subscript?
            {\begin{array}[t]\{{l}\}%
                \!\ListToTupleContents{#3}%
            \end{array}}_{\AsSet[#4][#5]}%
        }{% * no subscript
            \begin{array}[t]\{{l}\}%
                \!\ListToTupleContents{#3}%
            \end{array}%
        }%
    }%
    \IfBooleanT{#1}{$}%
}

% ~ 
% #1 : s* : part of infer rule?
% #2 : OA : rec environment
% #3 : e: : rec defs in A
% #4 : t| : past?
% #5 : E; : const
% #6 : o  : single type
% #7 : e- : entails interactions (only if #5 not given, default: end)
% #8 : e_ : element in set
% #9 : E< : default i in set I
\NewDocumentCommand{\ITJudgement}{s O{\RecEnv} e: t| E;{\TypeTrue} o e- e_ E<{\SetI}}{%
\IfBooleanTF{#1}{$\FmtJudgement}{\FmtJudgement|}%
{% * A
    \IfNoValueTF{#3}{% * no rec vars, A is empty
        \ITJRec%
    }{% * A rec vars
        \ITJRec[#2]:{#3}%
    }% 
    \!\,;\,%
    % * Const
    \IfBooleanTF{#4}{% * past
        \IfValueTF{#8}{% * set subscript
            \ITJCon|[#5]_{#8}:{#9}%
        }{% * no subscript
            \ITJCon|[#5]%
        }%
    }{% * not past
        \IfValueTF{#8}{% * set subscript
            \ITJCon[#5]_{#8}:{#9}%
        }{% * no subscript
            \ITJCon[#5]%
        }%
    }%
}{% * Type
    \IfNoValueTF{#7}{% * no list of interactions
        \IfValueTF{#6}{% * interaction given
            \IfValueTF{#8}{% * set subscript
                \ITJTyp|[#6]_{#8}<{#9}%
            }{% * no subscript
                \ITJTyp|[#6]%
            }%
        }{% * default interaction
            \IfValueTF{#8}{% * set subscript
                \ITJTyp|[\TypeEnd]_{#8}<{#9}%
            }{% * no subscript
                \ITJTyp|[\TypeEnd]%
            }%
        }%
    }{% * list of interactions given
        \IfValueTF{#8}{% * set subscript
            \ITJTyp[#7]_{#8}<{#9}%
        }{% * no subscript
            \ITJTyp[#7]%
        }%
    }%
}%
\IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/processes/practice/branch.tex <==

% ~ 
\NewDocumentCommand{\PBranch}{s E_{\PrcP} O{\PRecv|} e< E>{\PFail}}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{r l}%
        %
        % ~ receive
        \mathtt{on}\;{#2}\;%
        \IfValueTF{#4}{% * within
            \bm{\mathtt{recv}}^{#4}%
        }{% * forever
            \bm{\mathtt{recv}}^{\infty}%
        } & %
        %
        % ~ messages
        \begin{array}[t]\{{l}\}%
            \PrcListToArray{#3}%
        \end{array}%
        %
        % ~ timeout
        \IfValueT{#4}{% * timeout
            \PrcBranchAfterSep \rule{0pt}{3ex}{\mathtt{after}}%
            & \begin{array}[t]{l l}%
                :%
                & \!\begin{array}[t]{l}{#5}\end{array}%
            \end{array}%
        }%
        %
    \end{array}%
    \IfBooleanT{#1}{$}%
}

% ~ returns array
\NewDocumentCommand{\PrcListToArray}{>{\SplitList{,}}m}{%
    \ProcessList{#1}{\HeadPrcItemToArrayElement}%
}

% ~ returns items as line in array
\NewDocumentCommand{\HeadPrcItemToArrayElement}{m}{%
    \rule{0pt}{1.5ex}{#1}%
    \let\HeadPrcItemToArrayElement\TailPrcItemToArrayElement%
}
% ~ inserts new line before entry
\NewDocumentCommand{\TailPrcItemToArrayElement}{m}{%
    \PrcRecvSep\rule{0pt}{1.5ex}{#1}%
}


==> macros/sessiontypes/_tools/processes/practice/calc.tex <==

% ~ recv
% #1 : mm wrap
\NewDocumentCommand{\ICalcBranch}{s E1{{\SesP}} E2{{\PrcAfter}} E3{{\PrcMsg}} E4{{\Prc}} O{i} O{I} t| O{\Qrc}}{%
\IfBooleanT{#1}{$}% mm wrap
{#2}^{#3}\PrcRecv\,\InSet[{#4}_{#6}:{#5}_{#6}][#6][#7]%
\IfBooleanF{#8}{\;\TTPrcAft\,{#9}}
\IfBooleanT{#1}{$\!}% mm wrap
}

% ~ recv
% #1 : mm wrap
\NewDocumentCommand{\ICalcRecv}{s E_{\PrcP} O{\PrcMsg} E.{\Prc} e<}{%
\IfBooleanT{#1}{$}% mm wrap
{#2}^{\IfValueTF{#5}{#5}{\infty}}%
\PrcRecv\,{#3}:{#4}%
\IfBooleanT{#1}{$\!}% mm wrap
}

==> macros/sessiontypes/_tools/processes/practice/comm.tex <==

% ~ 
% #1 : s* : math mode wrap
% #2 : E_ : session role
% #3 : t| : do not format message?
% #4 : Om : message
% #5 : t/ : put proceeding on new line
% #6 : e. : proceeding process
\NewDocumentCommand{\PSend}{s E_{\PrcP} t| O{\PrcMsg} t/ e.}{%
    \IfBooleanT{#1}{$}%
    \rule{0pt}{1.5ex}%
    % \IfValueTF{#5}{% * proceeding process
    %     \IPrcFmt{%
        \begin{array}[t]{l l}%
            %
            \mathtt{on}\;{#2}\;%
            \bm{\mathtt{send}}\;%
            \IfBooleanTF{#3}{#4}{\rectround{$\mathtt{#4}$}}%
            %
            % & .%
        % }[%
            \IfBooleanTF{#5}{% * put proceeding on new line?
                \;\!\,. \\ \mbox{ }%
                \begin{array}[t]{l}%
                    \IfValueTF{#6}{#6}{\PrcEnd}%
                \end{array}%
            }{% * same line
                & .\!\,%
                \begin{array}[t]{l}%
                    \IfValueTF{#6}{#6}{\PrcEnd}%
                \end{array}%
            }
        % ]%
    % }{% * no proceeding process
    %     \IPrcFmt{%
    %     % \begin{array}[t]{r c l}%
    %         %
    %         \mathtt{on}\;{#2}\;%
    %         \bm{\mathtt{send}}\;%
    %         \IfBooleanTF{#3}{#4}{\rectround{$\mathtt{#4}$}}%
    %         %
    %         % & .%
    %         % & \!%
    %     }%
    % }%
    \end{array}%
    \IfBooleanT{#1}{$}%
}

% ~ 
% #1 : s* : math mode wrap
% #2 : E_ : session role
% #3 : t| : do not format message?
% #4 : Om : message
% #5 : t/ : put proceeding on new line
% #6 : E. : reception continuation
% #7 : e< : receive within
% #8 : E> : timeout branch
\NewDocumentCommand{\PRecv}{s E_{\PrcP} t| O{\PrcMsg} t/ E.{\PrcEnd} e< E>{\PrcFail}}{%
    \IfBooleanT{#1}{$}%
    \IfBooleanTF{#3}{% * part of branch
        \begin{array}[t]{>{\hfill$}p{3ex}<{ $} c l}%
            \rule{0pt}{1.5ex}\rectround{$\mathtt{#4}$}%
            & :%
            & \!\begin{array}[t]{l}{#5}\end{array}%
        \end{array}%
    }{% * single receive
        \begin{array}[t]{r l}%
            %
            % ~ receive
            \IfValueT{#7}{\mathllap{{\tikzmark{RecvNode}}}}%
            \mathtt{on}\;{#2}\;%
            \IfValueTF{#7}{% * within timeout
                \bm{\mathtt{recv}}^{#7}%
            }{% * forever
                \bm{\mathtt{recv}}^{\infty}%
            }%
            %
            \IfBooleanTF{#5}{% * put proceeding on new line?
                \begin{array}[t]{r c l}%
                    %
                    % ~ message
                    \rule{0pt}{1.5ex}\rectround{$\mathtt{#4}$}%
                    & \;\!\,: \\ &%
                    & \hspace{-8ex}\begin{array}[t]{l}{#6}\end{array}%
                    %
                    % ~ timeout
                    \IfValueT{#7}{% * timeout
                        \\ \mathllap{\tikzmark{AfterNode}{\mathtt{after}^{#7}}}%
                        & :%
                        & \!\begin{array}[t]{l}{#8}\end{array}%
                        \\[0.75ex]%
                    }%
                \end{array}%
            }{% * same line
                \begin{array}[t]{r c l}%
                    %
                    % ~ message
                    \rule{0pt}{1.5ex}\rectround{$\mathtt{#4}$}%
                    & :%
                    & \!\begin{array}[t]{l}{#6}\end{array}%
                    %
                    % ~ timeout
                    \IfValueT{#7}{% * timeout
                        \\ \mathllap{\tikzmark{AfterNode}{\mathtt{after}^{#7}}}%
                        & :%
                        & \!\begin{array}[t]{l}{#8}\end{array}%
                        \\[0.75ex]%
                    }%
                \end{array}%
            }%
            %
        \end{array}%
    }%
    %
    \IfValueT{#7}{%
        % \tikz[overlay,remember picture,use tikzmark]{%
        %     \draw[->,opacity=1,red,thick](pic cs:RecvNode) to (pic cs:AfterNode);%
        %     \filldraw[green] (pic cs:RecvNode) circle (2pt) node[anchor=west]{recv};%
        %     \filldraw[blue] (pic cs:AfterNode) circle (2pt) node[anchor=west]{after};%
        % }%
    }%
    \IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/processes/practice/general.tex <==

% ~ 
\NewDocumentCommand{\IScope}{s O{\ISes} e.}{%
    \IfBooleanT{#1}{$}% mm wrap
    \begin{array}[t]{l l}%
        \begin{array}[t]({l})%
            {\PrcScope}{#2}%
        \end{array}%
        & %
        % * use proceeding type if given, else end
        \begin{array}[t]({l})%
            \IfValueTF{#3}{#3}{\PrcEnd}%
        \end{array}%
    \end{array}%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ 
\NewDocumentCommand{\PDelay}{s O{0} t/ e.}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{l l}%
        \IfBooleanTF{#3}{% * new line proceeding
            \mathrlap{\FuncDelay\left({#2}\right)\;\!.} & %
            \\ \mbox{ } & {#4}%
        }{% * same line
            \FuncDelay\left({#2}\right)\;\!.\,%
            {#4}%
        }%
    \end{array}%
    \IfBooleanT{#1}{$}%
}

% ~ 
\NewDocumentCommand{\PSet}{s m t/ e.}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{l l}%
        \IfBooleanTF{#3}{% * new line proceeding
            \mathrlap{\TTPrcSet\left(\mathtt{#2}\right)\;\!.} & %
            \\ \mbox{ } & {#4}%
        }{% * same line
            \TTPrcSet\left(\mathtt{#2}\right)\;\!.\,%
            {#4}%
        }%
    \end{array}%
    \IfBooleanT{#1}{$}%
}

% ~ 
\NewDocumentCommand{\PFail}{s}{%
    \IfBooleanT{#1}{$}%
    \PrcFail%
    \IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/processes/practice/ifthenelse.tex <==

% ~ 
\NewDocumentCommand{\PIf}{s O{true} E:{\PThen} E:{\PElse}}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{l l}%
        \TTPrcIf\;\mathrlap{\mathtt{(#2)}}%
        % \hspace{\widthof{{(#2)}}}%
        \\ #3%
        \\ #4%
    \end{array}%
    \IfBooleanT{#1}{$}%
}

% ~ 
\NewDocumentCommand{\PThen}{s O{\PrcEnd}}{%
    \IfBooleanT{#1}{$}%
    % \mathllap{\TTPrcThen} & : & \begin{array}[t]{l}{#2}\end{array}%
    {\TTPrcThen} & {: \begin{array}[t]{l}{{#2}}\end{array}}%
    \IfBooleanT{#1}{$}%
}

% ~ 
\NewDocumentCommand{\PElse}{s O{\PFail}}{%
    \IfBooleanT{#1}{$}%
    % \mathllap{\TTPrcElse} & : & \begin{array}[t]{l}{#2}\end{array}%
    {\TTPrcElse} & {: \begin{array}[t]{l}{{#2}}\end{array}}%
    \IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/processes/practice/messages.tex <==

% ~ message judgement
% #1 : s* : 
% #2 : OG : var env
% #3 : m  : messages (IMsg)
\NewDocumentCommand{\IMJudgement}{s O{\VarEnv} m}{%
    \IfBooleanTF{#1}{$\FmtJudgement}{\FmtJudgement|}%
    {% * Gamma
        {#2}%
    }{% * Messages
        {\ListToTupleContents{#3}}%
    }%
    \IfBooleanT{#1}{$}%
}

% ~ message
\NewDocumentCommand{\IMsg}{s m E:{\DataType}}{%
    \IfBooleanT{#1}{$}%
    {#2}:{#3}%
    \IfBooleanT{#1}{$}%
}



==> macros/sessiontypes/_tools/processes/practice/recursion.tex <==

% ~ 
% #1 : s* : math mode wrap
% #2 : E: : process variable
% #3 : o  : recursion label script
% #4 : E= : recursion label
% #5 : e. : proceeding process
\NewDocumentCommand{\PDefRec}{s E:{\PCalcRecVar} o E={\TypRecLabel} e.}{%
    \IfBooleanT{#1}{$}%
    \begin{array}[t]{l l}%
        \TTPrcDef & %
        \IfValueTF{#3}{{#2}^{#3}={#4}^{#3}}{{#2}={#4}}\;%
        \TTPrcDefIn:%
        \\ & %
        \rule{0pt}{1ex}%
        % \hspace{6ex}%
        \IfValueTF{#5}{% * proceeding process
            {#5}
        }{\PrcEnd}%
        \;%
    \end{array}%
    \IfBooleanT{#1}{$}%
}

% ~ 
% #1 : s* : math mode wrap
% #2 : E: : recursion label
% #3 : o : recursion label script
\NewDocumentCommand{\PRec}{s E:{\TypRecLabel} o}{%
    \IfBooleanT{#1}{$}%
    \IfValueTF{#3}{{#2}^{#3}}{{#2}}%
    \IfBooleanT{#1}{$}%
}


==> macros/sessiontypes/_tools/types/practice/choice.tex <==

% ~ creates choices of types
% #1 : s* : serialised for text mode
% #2 : t^ : top or center align for choices (^ -> top)
% #3 : t| : only one option
% #4 : O  : list of types (default single type)
\NewDocumentCommand{\IChoice}{s t^ t| O{\IType}}{%
   \IfBooleanT{#1}{$}% mm wrap
   \IfBooleanTF{#3}{% * single action
      \begin{array}[\IfBooleanTF{#2}{t}{c}]\{{l}\}{#4}\end{array}%
   }{% * choice
      \begin{array}[\IfBooleanTF{#2}{t}{c}]\{{l}\}%
         \ListToArray{#4}%
      \end{array}%
   }%
   \IfBooleanT{#1}{$}% mm wrap
}

% ~ returns array
\NewDocumentCommand{\ListToArray}{>{\SplitList{,}}m}{%
   \ProcessList{#1}{\HeadItemToArrayElement}%
}

% ~ returns items as line in array
\NewDocumentCommand{\HeadItemToArrayElement}{m}{%
   \rule{0pt}{1.5ex}{#1}%
   \let\HeadItemToArrayElement\TailItemToArrayElement%
}
% ~ inserts new line before entry
\NewDocumentCommand{\TailItemToArrayElement}{m}{%
   \TypChoiceSep\rule{0pt}{1.5ex}{#1}%
   \let\HeadItemToArrayElement\TailItemToArrayElement%
}


==> macros/sessiontypes/_tools/types/practice/recursion.tex <==

% ~ creates recursive definition
% #1 : s* : math mode wrap
% #2 : o  : rec label identifier
% #3 : E: : default recursive label
% #4 : e. : proceeding type
\NewDocumentCommand{\IRecDef}{s o E:{\TypRecLabel} e.}{%
    \IfBooleanT{#1}{$}% mm wrap
    {{#3}\IfValueT{#2}{^{#2}}}%
    % * use proceeding type if given, else end
    \IfValueTF{#4}{.\,{#4}}{.\TypeEnd}%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ creates recursive call
% #1 : s* : math mode wrap
% #2 : o  : label identifier
% #3 : E:  : default recursive label
\NewDocumentCommand{\IRecCall}{s o E:{\TypRecLabel}}{%
    \IfBooleanT{#1}{$}% mm wrap
    {{#3}\IfValueT{#2}{^{#2}}}%
    \IfBooleanT{#1}{$}% mm wrap
}


==> macros/sessiontypes/_tools/types/practice/type.tex <==

% ~ message type
\NewDocumentCommand{\IMsgType}{s o d<> t' e_}{%
    \IfBooleanT{#1}{$}% mm wrap
    \IfValueTF{#2}{% * label provided
        {#2\IfBooleanT{#4}{'}\IfValueT{#5}{_{#5}}}%
    }{% * use default label
        {\MsgLabel\IfBooleanT{#4}{'}\IfValueT{#5}{_{#5}}}%
    }%
    \left\langle%
    \IfValueTF{#3}{% * data type provided
        {#3\IfBooleanT{#4}{'}\IfValueT{#5}{_{#5}}}%
    }{% * use default data type
        {\DataType\IfBooleanT{#4}{'}\IfValueT{#5}{_{#5}}}%
    }%
    \right\rangle%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ delegation type
\NewDocumentCommand{\DelType}{s o t' e_}{%
    \IfBooleanT{#1}{$}% mm wrap
    \IfValueTF{#2}{% * value provided
        \Tup(#2)%
    }{% * use default delegation
        \Tup({{\Const\IfBooleanT{#3}{'}}\IfValueT{#4}{_{#4}}},{{\TypeS\IfBooleanT{#3}{'}}\IfValueT{#4}{_{#4}}})%
    }%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ creates type actions
% #1 : s* : math mode wrap
% #2 : t! : token !
% #3 : t? : token ? 
% #4 : t! : token !
% #5 : t| : don't tt the message (or square)
% #6 : O  : message shared
% #7 : e_ : subscript
% ~ token given in #2 and #3 determines action.
% ~ together they yield comm square. #4 allows reordering.
\NewDocumentCommand{\ITypeAct}{s t! t? t! t| O{\MsgType} e_}{%
    \IfBooleanT{#1}{$}% mm wrap
    \begin{array}[t]{>{\hfill$}p{1ex}<{$\hfill} c}%
        % ~ handling action !?!
        \IfBooleanTF{#2}{% * !
            \IfBooleanTF{#3}{% * both !?
                \mathllap{\TypComm\IfValueT{#7}{_{#7}}}%
            }{% * no ? only !
                \mathllap{\TypSend\IfValueT{#7}{_{#7}}}%
            }%
        }{% * no !
            \IfBooleanTF{#3}{% * ?
                \IfBooleanTF{#4}{% * both ?!
                    \mathllap{\TypComm\IfValueT{#7}{_{#7}}}%
                }{% * only ?
                    \mathllap{\TypRecv\IfValueT{#7}{_{#7}}}%
                }%
            }{% * no !?
                \mathllap{\TypComm\IfValueT{#7}{_{#7}}}%
            }%
        }\!\,& %
        % ~ message
        \begin{array}[t]{l}%
            {#6}\IfValueT{#7}{_{#7}}%
        \end{array}%
    \end{array}%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ creates type conditions
% #1 : s* : math mode wrap
% #2 : O  : constraint (default: true)
% #3 : t| : reset indicator
% #4 : o  : resets
% #5 : e_ : subscript
% ~ reset indicator only has effect when #4 not provided.
% ~ instead true is used for constraint and #2 used for resets.
\NewDocumentCommand{\ITypeCond}{s O{\mathtt{true}} t| o e_}{%
    \IfBooleanT{#1}{$}% mm wrap
    \IfBooleanTF{#3}{% * if t|
        \IfNoValueTF{#4}{% * and #4 is null, use #2 as #4
            \Tup(\mathtt{true}\IfValueT{#5}{_{#5}},{#2}\IfValueT{#5}{_{#5}})%
        }{% * if #4 value, proceed as normal
            \Tup({#2}\IfValueT{#5}{_{#5}},{#4}\IfValueT{#5}{_{#5}})%
        }%
    }{% * no t|, proceed as normal
        \IfNoValueTF{#4}{% * omit from type
            \Tup({#2}\IfValueT{#5}{_{#5}})%
        }{% * reset given, proceed as normal
            \Tup({#2}\IfValueT{#5}{_{#5}},{#4}\IfValueT{#5}{_{#5}})%
        }%
    }%
    \IfBooleanT{#1}{$}% mm wrap
}

% ~ creates types automatically
% #1 : s* : math mode wrap
% #2 : e! : send action 
% #3 : e? : recv action  
% #4 : O  : type condition 
% #5 : t| : use #4 for resets, and true for #4
% #6 : o  : resets if no #5 
% #7 : e. : proceeding type (if false, default: end)
% #8 : e_ : subscript
% ~ #4 indicates if only a "." should be returned, else assumes ".end".
\NewDocumentCommand{\IType}{s e! e? O{\TypeTrue} t| o e. e_}{%
    \IfBooleanT{#1}{$}% mm wrap
    \!\rule{0pt}{1.5ex}%
    % ~ type action
    \IfValueTF{#2}{% * if !
        \IfValueTF{#8}{\ITypeAct![#2]_{#8}}{\ITypeAct![#2]}%
    }{% * no !
        \IfValueTF{#3}{% * if ?
            \IfValueTF{#8}{\ITypeAct?[#3]_{#8}}{\ITypeAct?[#3]}%
        }{% * no !?, syntax mode
            \!\hspace{1ex}%
            \IfValueTF{#8}{\ITypeAct|[\MsgType]_{#8}}{\ITypeAct|[\MsgType]}%
        }%
    }\!\,%
    % ~ type condition
    \IfValueTF{#6}{% * if resets
        \IfBooleanTF{#5}{% * if t|
            \IfValueTF{#8}{\ITypeCond[#4]|[#6]_{#8}}{\ITypeCond[#4]|[#6]}%
        }{% * no t|
            \IfValueTF{#8}{\ITypeCond[#4][#6]_{#8}}{\ITypeCond[#4][#6]}%
        }%
    }{% * no resets
        \IfBooleanTF{#5}{% * if t|
            \IfValueTF{#8}{\ITypeCond[#4]|_{#8}}{\ITypeCond[#4]|}%
        }{% * no t|
            \IfValueTF{#8}{\ITypeCond[#4]_{#8}}{\ITypeCond[#4]}%
        }%
    }%
    \,%
    % ~ proceeding type
    \IfValueTF{#7}{.\,{#7}\IfValueT{#8}{_{#8}}}{.\TypeEnd\IfValueT{#8}{_{#8}}}%
    \IfBooleanT{#1}{$}% mm wrap
}


==> tex/defs/configs/iso/future_en.tex <==
\begin{definition}[Future-enabled Configurations (\isFE*)]\label{def:configs_fe}
   A configuration \VIso*\ is \emph{future-enabled (\isFE*)} if\ %
   $\exists\ValTime$ such that \Trans*{\VIso}:{\ValTime,\CommMsg}[\VIso'].
   The same applies for \VSoc*.
 \end{definition}

==> tex/defs/configs/iso/latest_en.tex <==
\begin{definition}[Latest-enabled Action (\isLE*)]\label{def:configs_le}
    %
    A configuration \CIso*, that is future-enabled, has a \emph{latest-enabled send} (resp. \emph{latest-enabled receive}), or \isLE*!\ for short (resp. \isLE*?), 
    if $\forall t$ such that $\CIso+{+t}\isFE~\Implies~\exists t'\geq t: \Trans{\VIso}:{\ValTime',\SendMsg}$.
\end{definition}

==> tex/defs/configs/iso/live.tex <==
\begin{definition}[Live Configurations]\label{def:configs_live}
    \CIso*\ is \emph{live} if
    $\TypeS=\TypeEnd$ or if \VIso*\ is \isFE*.
\end{definition}

==> tex/defs/configs/iso/well_formed.tex <==
\begin{definition}[Well-formed Configurations]\label{def:configs_wf}
    %
    \CIso*\ is \emph{well-formed} if \TypeS*\ is \emph{well-formed} against \ValClocks*\ (see~\Cref{def:types_wf}).
    %
\end{definition}

==> tex/defs/configs/sys/progress.tex <==
%
% \begin{restatable}[System Progress]{definition}{DefConfigsSysProgress}
    \begin{definition}[System Progress]\label{def:configs_sys_progress}
    %
    A system \VSys*\ \emph{satisfies progress} if:
    \begin{minieq}*
        \Trans{\VSys}:{\VSys'}*
        %
        \implies
        \begin{array}[c]{l}
            %
            \VSoc'_1
            \;\text{and\ }
            \VSoc'_2
            \;\text{are both a \emph{success} (see~\cref{def:types_progress})};
            %
            \\[0ex]
            \text{or\ } \exists\ValTime:
            \Trans{\VSys'}:{\ValTime\,\SiltAction}
            %
        \end{array}
        %
    \end{minieq}
    %
% \end{restatable}
\end{definition}
%

==> tex/defs/processes/domain_clocks.tex <==
%
\begin{restatable}[Clock Domains]{definition}{DefPrcTypClockDomains}\label{def:prc_typ_clock_domains}
   %
   \TODO[need clarity on implications]
   % \begin{equation*}
   %    \emptyset
   % \end{equation*}
   %
\end{restatable}
%

==> tex/defs/processes/fail_free.tex <==
%
\begin{definition}[Fail-Free Process]\label{def:prc_fail_free}
    %
    When $\Prc=\PrcFail$, \Prc*\ is \emph{not} fail-free.%
    For all other valuations of \Prc*\ below, \Prc*\ is \emph{fail-free} if its corresponding condition holds:
    \par\noindent
    \begin{minipage}{\textwidth}\centering
        \begin{tabular}{l p{2ex} l}
            %
            \PCalcSend*            &  & %
            is \emph{fail-free} if \Prc*\ is \emph{fail-free},%
            %
            \\
            \PCalcRecv*            &  & %
            is \emph{fail-free} if \Prc*_{i}\ is \emph{fail-free}, for all $i\in\SetI$,%
            %
            \\
            \PCalcScope*           &  & %
            is \emph{fail-free} if \Prc*\ is \emph{fail-free},%
            %
            \\
            \Par*[\Prc][\Qrc]      &  & %
            is \emph{fail-free} if both \Prc*\ and \Qrc*\ are \emph{fail-free},%
            %
            \\
            \PCalcBuffer*          &  & %
            is \emph{fail-free},%
            %
            \\
            \PrcRecDef*          &  & %
            is \emph{fail-free} if \Qrc*\ is \emph{fail-free},%
            %
            \\
            \PCalcSetTimer*        &  & %
            is \emph{fail-free} if \Prc*\ is \emph{fail-free},%
            %
            % \\
            % \PCalcRecVar*|         &  & %
            % is \emph{fail-free} if \Prc*\ is \emph{fail-free},%
            %
            \\
            \PFuncDelay*           &  & %
            is \emph{fail-free} if \Prc*\ is \emph{fail-free},%
            %
            \\
            \PCalcIf*              &  & %
            is \emph{fail-free} if both \Prc*\ and \Qrc*\ are \emph{fail-free},%
            %
            \\
            \PFuncDelay*[\ValTime] &  & %
            is \emph{fail-free} if \Prc*\ is \emph{fail-free},%
            %
            \\
            \PrcEnd*               &  & %
            is \emph{fail-free}.%
            %
        \end{tabular}
    \end{minipage}
    %
\end{definition}
% %
% \begin{restatable}[Fail-Free Process]{definition}{DefPrcFailFree}\label{def:prc_fail_free}
%     %
%     A process \Prc*\ is \emph{fail-free} if:
%     \begin{tabular}{l p{2ex} l}
%         %
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcRecv*4{\Qrc} & & %
%         is \emph{fail-free} if \Qrc*_{i}\ is \emph{fail-free}, for all $i\in\SetI$%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%         \\
%         \PCalcSend*.\Qrc* & & %
%         is \emph{fail-free} if \Qrc*\ is \emph{fail-free}%
%         %
%     \end{tabular}
%     %
%  \end{restatable}
%  %

==> tex/defs/processes/free_queues.tex <==
%
\begin{definition}[Free Queues of Processes]\label{def:prc_free_queues}
    %
    The set of \emph{free queues} \PFuncFQ*[\Prc]\ of a process \Prc*\ is defined inductively as follows:
    \begin{minieq}*%
        \begin{array}[t]{l}%
            \begin{array}[c]{l p{4ex} l p{4ex} l}
                \begin{array}[c]{l c p{0ex} l}
                    \begin{array}[t]{l}%
                        \PFuncFQ[\RecVar], %
                        \mbox{}~\PFuncFQ[\PrcEnd]%
                    \end{array}%
                     & = &  & %
                    \emptyset %
                \end{array}
                %
                 &  &
                \begin{array}[c]{l c p{0ex} l}
                    \PFuncFQ[\PCfgQueue]%
                     & = &  & %
                    \PCalcEndPoints %
                \end{array}
                %
                 &  &
                \begin{array}[c]{l c p{0ex} l}
                    \PFuncFQ[\PCalcScope]%
                     & = &  & %
                    \PFuncFQ[\Prc]\backslash\mkSet[\PrcP\PrcQ,\PrcQ\PrcP] %
                \end{array}
            \end{array}
            %
            \\[-1ex]\\
            \begin{array}[c]{l c p{0ex} l}
                \PFuncFQ[\PCalcRecv] %
                 & = &  & %
                \SetUnion_{i\in\SetI} \PFuncFQ[\Prc_i]
            \end{array}
            %
            \\[-1ex]\\
            \begin{array}[c]{l c p{0ex} l}
                \begin{array}[t]{l}%
                    \PFuncFQ[\PCalcIf], %
                    \mbox{}~\PFuncFQ[\Par[\Prc][\Qrc]]%
                \end{array}%
                 & = &  & %
                \PFuncFQ[\Prc]~\cup~\PFuncFQ[\Qrc]
            \end{array}
            %
            \\[-1ex]\\
            \begin{array}[c]{l c p{0ex} l}
                \begin{array}[t]{l}%
                    \PFuncFQ[\PCalcSend],      %
                    \mbox{}~\PFuncFQ[\PCalcSetTimer],  %
                    \mbox{}~\PFuncFQ[\PFuncDelay[\Const]], %
                    \mbox{}~\PFuncFQ[\PFuncDelay[\ValTime]], \\
                    \mbox{}~\PFuncFQ[\PrcRecDef]             %
                \end{array}%
                 & = &  & %
                \PFuncFQ[\Prc] %
            \end{array}
            %
        \end{array}
    \end{minieq}
    %
\end{definition}
% 

==> tex/defs/processes/session/balanced.tex <==
%
\begin{definition}[Balanced \SesEnv*]\label{def:session_balanced}
   %
   Let \BalSes*\ be the set containing all session environments \SesEnv*\ that adhere to the following:
   \begin{enumerate}
      \item $\SesEnv=\SesEnv',%
               ~{\PrcP:\CIso},%
               ~{\PrcQ\PrcP:\Msg;\Queue}%
               ~\implies~%
               \exists\ValClocks',\TypeS':%
               \Trans{\CIso}:{\RecvMsg}[\CIso']$
            and $\SesEnv',
               ~{\PrcP:\mkTup[\ValClocks'][\TypeS']},%
               ~{\PrcP\PrcQ:\Queue}$
            and $\SesEnv'\in\BalSes$.
            %
      \item $\SesEnv=\SesEnv',%
               ~{\PrcP:\CIso_1},
               ~{\PrcQ\PrcP:\Queue_1},%
               ~{\PrcQ:\CIso_2},%
               ~{\PrcP\PrcQ:\Queue_2}%
               ~\implies~%
               \Compat$.
   \end{enumerate}
   A session environment \SesEnv*\ is said to be \emph{balanced} if $\SesEnv\in\BalSes$.
   %
\end{definition}
%

==> tex/defs/processes/session/delayable.tex <==
%
\begin{definition}[Delayable Session Environment (\SesEnv*)]\label{def:prc_typ_sesenv_delayable}
    %
    \SesEnv*\ is \emph{delayable} if $\forall\ISes\in\SesDomain$ such that $\SesEnv(\ISes)\neq\emptyset%
    \Implies%
    \PrcQ\not\in\SesDomain$
    %
\end{definition}
% 
\endinput
a session environment is delayable if for non-empty channel there does not exist a role able to receive from it

==> tex/defs/processes/session/free_queues.tex <==
%
\begin{definition}[Free Queues of \SesEnv*]\label{def:session_free_queues}
    %
    The function \PFuncFQ* is defined inductively as follows:
    \begin{minieq}
        \begin{array}[t]{c p{0.1\textwidth} c}
            \begin{array}[t]{r c l}%
                %
                \PFuncFQ[\emptyset]                        & = & \emptyset %
                %
                \\[1ex]%
                \PFuncFQ[\PrcP:\mkTup[\ValClocks][\TypeS]] & = & \emptyset %
            \end{array}
            &  & %
            \begin{array}[t]{r c l}%
                %
                \PFuncFQ[\PrcP\PrcQ:\Queue]   & = & \PrcP\PrcQ                                 %
                %
                \\[1ex]%
                \PFuncFQ[\SesEnv_1,\SesEnv_2] & = & \PFuncFQ[\SesEnv_1]\cup\PFuncFQ[\SesEnv_2] %
                %
            \end{array}
        \end{array}
    \end{minieq}
    %
\end{definition}
% 

==> tex/defs/processes/session/fully_balanced.tex <==
%
\begin{definition}[Fully Balanced \SesEnv*]\label{def:session_fully_balanced}
   %
   A session environment \SesEnv*\ is said to be \emph{fully balanced} if \SesEnv*\ is \emph{balanced} and:
   \begin{enumerate}
      \item $\SesEnv=\SesEnv',\PrcP:\mkTup[\ValClocks_1][\TypeS_1]%
               ~\implies~\begin{array}[t]{rl}%
               \exists\PrcQ,\Queue_1,\ValClocks_2,\TypeS_2,\Queue_2,{\SesEnv}'' & \\%
               \text{such that} & \SesEnv'={\SesEnv}'',%
               ~{\PrcQ\PrcP:\Queue_1},%
               ~{\PrcQ:\CIso_2},%
               ~{\PrcP\PrcQ:\Queue_2}\end{array}$
            %
      \item $\SesEnv=\SesEnv',\PrcQ\PrcP:\Queue_1%
               ~\implies~\begin{array}[t]{rl}%
               \exists\ValClocks_1,\TypeS_1,\ValClocks_2,\TypeS_2,\Queue_2,{\SesEnv}'' & \\%
               \text{such that} & \SesEnv'={\SesEnv}'',%
               ~{\PrcP:\CIso_1},%
               ~{\PrcQ:\CIso_2},%
               ~{\PrcP\PrcQ:\Queue_2}\end{array}$
   \end{enumerate}
   %
\end{definition}
% 

==> tex/defs/processes/t_reading.tex <==
%
% \begin{restatable}[\ValTime*-Reading \SesEnv*]{definition}{DefPrcTypTReading}
    \begin{definition}[\ValTime*-Reading \SesEnv*]\label{def:prc_typ_t_reading}
    %
    A session environment \SesEnv*\ is \ValTime*-reading if there exists
    \begin{inline}*+
        \item a role $\PrcP\in\SesDomain$
        %
        \item a message \Msg*\
        %
        \item a $\ValTime'<\ValTime$, such that
        %
    \end{inline}:
    \hfill\ $
        \SesEnv\left(\PrcP\right)=\CfgIso
        \;\land\;
        \CfgIso1{\ValClocks+\ValTime'}\Act[\TypAct1{\TypRecv}2{\Msg}]
    $
    %
% \end{restatable}
\end{definition}
%

==> tex/defs/processes/well_formed.tex <==
%
\begin{definition}[Well-formed Processes]\label{def:prc_well_formed}
    %
    The \emph{well-formedness} of a process \Prc*\ is given by \PFuncWF*[\Prc], which is inductively defined as follows:
    \begin{minieq}*%
        \begin{array}[t]{l}%
            \begin{array}[c]{l p{8ex} l}%
                \begin{array}[c]{l c p{0ex} l}%
                    \begin{array}[t]{l}%
                        \PFuncWF[\RecVar], %
                        \mbox{}~\PFuncWF[\PCfgQueue],%
                        \mbox{}~\PFuncWF[\PrcEnd]%
                    \end{array}%
                     & = &  & %
                    \TypeTrue %
                \end{array}%
                %
                 &  & %
                \begin{array}[c]{l c p{0ex} l}%
                    \PFuncWF[\PCalcScope]%
                     & = &  & %
                    \PFuncWF[\Prc] %
                \end{array}%
            \end{array}%
            %
            \\[-1ex]\\%
            \begin{array}[c]{l c p{0ex} l}%
                \PFuncWF[\PCalcRecv] %
                 & = &  & %
                \bigwedge\limits_{i\in\SetI}~\PFuncWF[\Prc_i]%
                \land%
                \left(\PFuncFQ[\Prc_i]=\emptyset\right)%
            \end{array}%
            %
            \\[-1ex]\\%
            \begin{array}[c]{l c p{0ex} l}%
                \begin{array}[t]{l}%
                    \PFuncWF[\PCalcIf], %
                    \mbox{}~\PFuncWF[\Par[\Prc][\Qrc]]%
                \end{array}%
                 & = &  & %
                \PFuncWF[\Prc]~\land~\PFuncWF[\Qrc]%
            \end{array}%
            %
            \\[-1ex]\\%
            \begin{array}[c]{l c p{0ex} l}%
                \begin{array}[t]{l}%
                    \PFuncWF[\PCalcSend],      %
                    \mbox{}~\PFuncWF[\PCalcSetTimer],  %
                    \mbox{}~\PFuncWF[\PFuncDelay[\Const]], %
                    \mbox{}~\PFuncWF[\PFuncDelay[\ValTime]], \\%
                    \mbox{}~\PFuncWF[\PrcRecDef]             %
                \end{array}%
                 & = &  & %
                \PFuncWF[\Prc]%
                \land%
                \left(\PFuncFQ[\Prc]=\emptyset\right) %
            \end{array}%
            %
        \end{array}%
    \end{minieq}%
    %
\end{definition}
% 

==> tex/defs/types/progress.tex <==
\begin{definition}[Type Progress]\label{def:types_progress}
    %
    A configuration with queues $\SocCfg$ is \emph{final} if $\VSoc=\CSoc;[\TypeEnd]:{\emptyset}$.
    A system \VSys*\ \emph{satisfies progress} for all \VSys*'\ reachable from \VSys*, either \VSoc*'_1\ and \VSoc*'_2\ are \emph{final}, or $\exists\ValTime$ such that \Trans*{\VSys'}:{\ValTime,\SiltAction}.
  \end{definition}

==> tex/defs/types/weak_past.tex <==
%
\begin{restatable}[Weak Past (\Past*)]{definition}{DefWeakPast}\label{def:weak_past}
    %
    It may hold that \Sat*[\ValClocks]:[\Past]\ if $\exists\ValTime$ such that \Sat*[\ValClocks+\ValTime]:[\Const].
    %
\end{restatable}
%

==> tex/defs/types/well_formed.tex <==
\begin{definition}[Well-formedness]\label{def:types_wf}
   %
   A type $\TypeS$ is well-formed with respect to $\nu$ if there exists $\delta$ such that $\nu\models \delta$ and $\emptyset;\delta\vdash \TypeS$. A type $\TypeS$ is well-formed if it is well-formed with respect to $\nu_0$.
 \end{definition}

==> tex/examples/_input_all.tex <==

\paragraph*{message throttling}\label{par:example_message_throttling}
\input{tex/examples/message_throttling/diagram.tex}
\input{tex/examples/message_throttling/type.tex}
\input{tex/examples/message_throttling/process.tex}

\paragraph*{producer consumer}\label{par:example_producer_consumer}
\NOTE[incoming recursive edges that require a reset in the diagram are not able to be described by types (?retry or ?data -> A) the clocks instead are the same as when A was first reached]
\input{tex/examples/producer_consumer/diagram.tex}
\NOTE[therefore in types, we must acknowledge that \IRecCall*[A]\ is the inital state, where all clocks are 0, but that diagrams that either require a value to be preserved over loops can not be described.]
\input{tex/examples/producer_consumer/type.tex}
\input{tex/examples/producer_consumer/process.tex}

\subsection{typing processes}
% \input{tex/examples/outdated/example_process_typing.tex}

% \subsection{other}
% \subsubsection{const diag reset sat}
% \input{tex/examples/const_diag_reset_sat.tex}
% \subsubsection{const mixed-choice}
% \input{tex/examples/const_mixed_choice.tex}


% \paragraph*{unnamed 1}
% \begin{equation}
%     \begin{array}[c]{r c l}
%         %
%         \TypeS & = & %
%         \IChoice[%
%             \IType?{a}[x\leq 1][x].{%
%                 \IType!{c}.{%
%                     \IRecDef[a].{%
%                         \IChoice[%
%                             \IType?{d}[x\leq 1],%
%                             \IType!{e}[1<x].{\IRecCall[a]}%
%                         ]%
%                     }%
%                 }%
%             },%
%             \IType!{b}[2<x<3]%
%         ]%
%         %
%         \\[2ex]%
%         \\[2ex]%
%         \Prc & = & %
%         \PSet{x}.{%
%             \PRecv[a]:{% * recv
%                 \PSet{x}.{%
%                     \PSend[c].{%
%                         \PDefRec:{%
%                             \PRecv[d]<{1}>{% * after
%                                 \PRec%
%                             }%
%                         }%
%                     }%
%                 }%
%             }<{1}>{% * after 1
%                 \PDelay[t=1].{%
%                     \PIf[2<x<3]% * use defaults (then end, else fail)
%                 }%
%             }%
%         }%
%         %
%     \end{array}
% \end{equation}

% \begin{equation}
%     \begin{array}[c]{r c l}
%         %
%         \Dual[\TypeS] & = & %
%         \IChoice[%
%             \IType!{a}[y\leq 1][y].{%
%                 \IType?{c}.{%
%                     \IRecDef[b].{%
%                         \IChoice[%
%                             \IType!{d}[y\leq 1],%
%                             \IType?{e}[1<y].{\IRecCall[b]}%
%                         ]%
%                     }%
%                 }%
%             },%
%             \IType?{b}[2<y<3]%
%         ]%
%         %
%         \\[2ex]%
%         \\[2ex]%
%         \Qrc & = & %
%         \PSet{y}.{%
%             \PIf[y\leq 1]:{\PThen[%
%                 \PSend_{q}[a].{%
%                     \PSet{y}.{%
%                         \PRecv_{q}[c]:{%
%                             \PDefRec:{%
%                                 \PIf[y\leq 1]:{\PThen[%
%                                     \PSend_{q}[d]%
%                                 ]}:{\PElse[%
%                                     \PRecv_{q}[e]:{%
%                                         \PRec%
%                                     }%
%                                 ]}%
%                             }%
%                         }%
%                     }%
%                 }%
%             ]}:{\PElse[%
%                 \PDelay[t=1].{%
%                     \PRecv[b]<{1}% * after: failed
%                 }%
%             ]}%
%         }%
%         %
%     \end{array}
% \end{equation}

\paragraph*{unnamed 2 (types)}

\begin{equation}
    %
    \begin{array}[t]{l c l}%
        %
        \TypeS & = & %
        \IChoice[%
            \IType?{a}[x\leq 1][x].{%
                \IType!{c}.{%
                    \IRecDef[a].{%
                        \IChoice[%
                            \IType?{d}[x\leq 1],%
                            \IType!{e}[1<x].{\IRecCall[a]}%
                        ]%
                    }%
                }%
            },%
            \IType!{b}[2<x<3]%
        ]%
        %
        \\[2ex]%
        \\[2ex]%
        \Dual[\TypeS] & = & %
        \IChoice[%
            \IType!{a}[y\leq 1][y].{%
                \IType?{c}.{%
                    \IRecDef[b].{%
                        \IChoice[%
                            \IType!{d}[y\leq 1],%
                            \IType?{e}[1<y].{\IRecCall[b]}%
                        ]%
                    }%
                }%
            },%
            \IType?{b}[2<y<3]%
        ]%
        %
    \end{array}%
    %
\end{equation}

\def\typeslz{\TypeS_{0}}
\def\typesli{\TypeS_{1}}
\def\typeslii{\TypeS_{2}}
\def\typesliii{\TypeS_{3}}
\def\typesliv{\TypeS_{4}}
\def\typeslv{\TypeS_{5}}
\def\typeslvi{\TypeS_{6}}
\def\typeslvii{\TypeS_{7}}

\def\typetlz{\Dual[\TypeS]_{0}}
\def\typetli{\Dual[\TypeS]_{1}}
\def\typetlii{\Dual[\TypeS]_{2}}
\def\typetliii{\Dual[\TypeS]_{3}}
\def\typetliv{\Dual[\TypeS]_{4}}
\def\typetlv{\Dual[\TypeS]_{5}}
\def\typetlvi{\Dual[\TypeS]_{6}}
\def\typetlvii{\Dual[\TypeS]_{7}}

\def\typesz{\IChoice|[\typesli,\typeslvii]}
\def\typesi{\IType?{a}[x\leq 1][x].{\typeslii}}
\def\typesii{\IType!{c}.{\typesliii}}
\def\typesiii{\IRecDef[a].{\typesliv}}
\def\typesiv{\IChoice|[\typeslv,\typeslvi]}
\def\typesv{\IType?{d}[x\leq 1]}
\def\typesvi{\IType!{e}[1<x].{\IRecCall[a]}}
\def\typesvii{\IType!{b}[2<x<3]}

\def\typetz{\IChoice|[\typetli,\typetlvii]}
\def\typeti{\IType!{a}[y\leq 1][y].{\typetlii}}
\def\typetii{\IType?{c}.{\typetliii}}
\def\typetiii{\IRecDef[b].{\typetliv}}
\def\typetiv{\IChoice|[\typetlv,\typetlvi]}
\def\typetv{\IType!{d}[y\leq 1]}
\def\typetvi{\IType?{e}[1<y].{\IRecCall[b]}}
\def\typetvii{\IType?{b}[2<y<3]}

\begin{equation}
    %
    \begin{array}[t]{l c l c l p{2ex} l c l c l }%
        %
        \TypeS & ::= & \typeslz & = & \typesz & &%
        \Dual[\TypeS] & ::= & \typetlz & = & \typetz \\%
        %
        & \mid & \typesli & = & \typesi & &%
        & \mid & \typetli & = & \typeti \\%
        %
        & \mid & \typeslii & = & \typesii & &%
        & \mid & \typetlii & = & \typetii \\%
        %
        & \mid & \typesliii & = & \typesiii & &%
        & \mid & \typetliii & = & \typetiii \\%
        %
        & \mid & \typesliv & = & \typesiv & &%
        & \mid & \typetliv & = & \typetiv \\%
        %
        & \mid & \typeslv & = & \typesv & &%
        & \mid & \typetlv & = & \typetv \\%
        %
        & \mid & \typeslvi & = & \typesvi & &%
        & \mid & \typetlvi & = & \typetvi \\%
        %
        & \mid & \typeslvii & = & \typesvii & &%
        & \mid & \typetlvii & = & \typetvii%
        %
    \end{array}%
    %
\end{equation}

\paragraph*{unnamed 2 (processes)}

\begin{equation}
    %
    \begin{array}[t]{l c l}%
        %
        \Prc & = & %
        \PSet{x}/.{%
            \PRecv[a].{% * recv
                \PSet{x}/.{%
                    \PSend[c]/.{%
                        \PDefRec[A].{%
                            \PRecv[d]<{1}>{% * after
                                \PRec[A]%
                            }%
                        }%
                    }%
                }%
            }<{1}>{% * after 1
                \PDelay[t=1]/.{%
                    \PIf[2<x<3]% * use defaults (then end, else fail)
                }%
            }%
        }%
        %
        \\[2ex]%
        \\[2ex]%
        \Qrc & = & %
        \PSet{y}.{%
            \PIf[y\leq 1]:{\PThen[%
                \PSend_{q}[a]/.{%
                    \PSet{y}/.{%
                        \PRecv_{q}[c].{%
                            \PDefRec[B].{%
                                \PIf[y\leq 1]:{\PThen[%
                                    \PSend_{q}[d]%
                                ]}:{\PElse[%
                                    \PRecv_{q}[e].{%
                                        \PRec[B]%
                                    }%
                                ]}%
                            }%
                        }%
                    }%
                }%
            ]}:{\PElse[%
                \PDelay[t=1]/.{%
                    \PRecv[b]<{1}% * after: failed
                }%
            ]}%
        }%
        %
    \end{array}%
    %
\end{equation}

\def\prclz{\Prc_{0}}
\def\prcli{\Prc_{1}}
\def\prclii{\Prc_{2}}
\def\prcliii{\Prc_{3}}
\def\prcliv{\Prc_{4}}
\def\prclv{\Prc_{5}}
\def\prclvi{\Prc_{6}}
\def\prclvii{\Prc_{7}}

\def\qrclz{\Qrc_{0}}
\def\qrcli{\Qrc_{1}}
\def\qrclii{\Qrc_{2}}
\def\qrcliii{\Qrc_{3}}
\def\qrcliv{\Qrc_{4}}
\def\qrclv{\Qrc_{5}}
\def\qrclvi{\Qrc_{6}}
\def\qrclvii{\Qrc_{7}}
\def\qrclviii{\Qrc_{8}}
\def\qrclix{\Qrc_{9}}
\def\qrclx{\Qrc_{10}}
\def\qrclxi{\Qrc_{11}}

\def\prcz{\PSet{x}.{\prcli}}
\def\prci{\PRecv[a].{\prclii}<{1}>{\prclvi}}
\def\prcii{\PSet{x}.{\prcliii}}
\def\prciii{\PSend[c].{\prcliv}}
\def\prciv{\PDefRec[A].{\prclv}}
\def\prcv{\PRecv[d]<{1}>{\PRec[A]}}
\def\prcvi{\PDelay[t=1].{\prclvii}}
\def\prcvii{\PIf[2<x<3]}

\def\qrcz{\PSet{y}.{\qrcli}}
\def\qrci{\PDelay[y\leq 1].{\qrclii}}% ~ delay inserted
\def\qrcia{\PDelay{y}.{\qrclii}}% ~ delay resolved
\def\qrcib{\PDelay{y}.{\qrclii}}% ~ delay resolved
\def\qrcic{\PDelay{y}.{\qrclii}}% ~ delay resolved
\def\qrcii{\PIf[y\leq 1]:{\PThen[\qrcliii]}:{\PElse[\qrclx]}}
\def\qrciii{\PSend_{q}[a].{\qrcliv}}
\def\qrciv{\PSet{y}.{\qrclv}}
\def\qrcv{\PRecv_{q}[c].{\qrclvi}}
\def\qrcvi{\PDefRec[B].{\qrclvii}}
\def\qrcvii{\PIf[y\leq 1]:{\PThen[\qrclviii]}:{\PElse[\qrclix]}}
\def\qrcviii{\PSend_{q}[d]}
\def\qrcix{\PRecv_{q}[e].{\PRec_{b}}}
\def\qrcx{\PDelay[t=1].{\qrclxi}}
\def\qrcxi{\PRecv[b]<{1}}

\begin{equation}
    %
    \begin{array}[t]{c p{2ex} c}%
        \begin{array}[t]{l c l c l}%
            %
            \Prc & ::= & \prclz & = & \prcz \\% 
            & \mid & \prcli & = & \prci \\%
            & \mid & \prclii & = & \prcii \\%
            & \mid & \prcliii & = & \prciii \\%
            & \mid & \prcliv & = & \prciv \\%
            & \mid & \prclv & = & \prcv \\%
            & \mid & \prclvi & = & \prcvi \\%
            & \mid & \prclvii & = & \prcvii %
            %
        \end{array}%
        & & %
        \begin{array}[t]{l c l c l}%
            %
            \Qrc & ::= & \qrclz & = & \qrcz \\% 
            & \mid & \qrcli & = & \qrci \\%
            & \mid & \qrclii & = & \qrcii \\%  
            & \mid & \qrcliii & = & \qrciii \\%
            & \mid & \qrcliv & = & \qrciv \\%
            & \mid & \qrclv & = & \qrcv \\%
            & \mid & \qrclvi & = & \qrcvi \\%
            & \mid & \qrclvii & = & \qrcvii \\%
            & \mid & \qrclviii & = & \qrcviii \\%
            & \mid & \qrclix & = & \qrcix \\%
            & \mid & \qrclx & = & \qrcx \\%
            & \mid & \qrclxi & = & \qrcxi %
            %
        \end{array}%
    \end{array}%
    %
\end{equation}


==> tex/examples/const_diag_reset_sat.tex <==
\vspace{-4ex}%
\resizebox{0.3\textwidth}{!}{%
   \begin{tikzpicture}%
      % ~ grid
      % draw horizontal
      \foreach \y in {0,...,6}%
         {%
            \draw[gray] (0,\y) -- (6,\y);%
            \node[left] at (0,\y) {\y};
         }%
      % draw vertical
      \foreach \x in {0,...,6}%
         {%
            \draw[gray] (\x,0) -- (\x,6);%
            \node[below] at (\x,0) {\x};
         }%
        % ~ axies
      \draw (0,0) -- (6,0);%
      \draw (0,0) -- (0,6);%
         %
   \end{tikzpicture}%
   }%
\endinput   

      % complete trace
      \filldraw [gray, opacity = 0.25, line width = 2pt]%
      (0,0) -- (2.5,2.5);%
      \filldraw [blue, opacity = 1, line width = 2pt]% ready
      (2,2) -- (1,1);%
      \filldraw [yellow, opacity = 0.25, line width = 0pt]% reset
      (0,1) -- (0,2) -- (2,2) -- (1,1);%
      \filldraw [gray, opacity = 0.25, line width = 0pt]%
      (0,1) -- (0,2) -- (1,3) -- (2,3);%
      \filldraw [red, opacity = 1, line width = 2pt]% latency
      (0,2) -- (8,10);%

      \filldraw [yellow, opacity = 0.25, line width = 0pt]% reset
      (0,3) -- (0,4) -- (2,4) -- (2,3);%
      \filldraw [red, opacity = 0.25, line width = 0pt]% cancel
      (0,3) -- (0,4) -- (2,6) -- (2,5);%
      \filldraw [blue, opacity = 0.25, line width = 0pt]% done
      (2,5) -- (2,6) -- (5,9) -- (5,8);%
      \filldraw [blue, opacity = 0.25, line width = 0pt]% data
      (2,5) -- (2,6) -- (5,9) -- (5,8);%
      \filldraw [blue, opacity = 0.25, line width = 0pt]% error
      (2,5) -- (2,6) -- (6,10) -- (6,9);%
      \filldraw [red, opacity = 0.25, line width = 0pt]% timeout
      (6,9) -- (6,10) -- (7,10);%

      % def z
      \draw[fill, cyan] (0,0) circle (4pt);
      \node[right] at (0.2, 0.5) {\Large $\TypRecDef\,{{\TypRecCall}^{Z}}$};

      % def a
      \draw[fill, cyan] (2,3) circle (4pt);
      \draw[fill, cyan] (2,4) circle (4pt);
      \filldraw [cyan, line width = 8pt] (2,3) -- (2,4);
      \node[right] at (2.2,3.5) {\Large $\TypRecDef\,{{\TypRecCall}^{A}}$};

      % send start
      \filldraw [red, opacity = 1, line width = 2pt]% start
      (2,4) -- (2,3);%

      % send close
      \filldraw [red, opacity = 1, line width = 2pt]%
      (2.5,2.5) circle (4pt);

      % axis labels
      \node[below] at (7.5,-0.5) {\Large $x,y,z\in\ClockSet$};
      \node[left] at (-0.5, 9.5) {\Large $g$};

      % % table of clock values: g
      % \node at (9, 10.5) {\Large $g$};
      % \node at (9, 10) {$10$};
      % \node at (9, 9) {$9$};
      % \node at (9, 8) {$8$};
      % \node at (9, 7) {$7$};
      % \node at (9, 6) {$6$};
      % \node at (9, 5) {$5$};
      % \node at (9, 4) {$4$};
      % \node at (9, 3) {$3$};
      % \node at (9, 2) {$2$};
      % \node at (9, 1) {$1$};
      % \node at (9, 0) {$0$};
      % % table of clock values: x
      % \node at (10, 10.5) {\Large $x$};
      % \node at (10, 10) {$(6,7)$};
      % \node at (10, 9) {$(5,6)$};
      % \node at (10, 8) {$(4,5)$};
      % \node at (10, 7) {$(3,4)$};
      % \node at (10, 6) {$(2,3)$};
      % \node at (10, 5) {$(1,2)$};
      % \node at (10, 4) {$2\mapsto 0$};
      % \node at (10, 3) {$\begin{array}{c}(1,2)\\2\mapsto 0\end{array}$};
      % \node at (10, 2) {$\begin{array}{c}(1,2)\\2\mapsto 0\end{array}$};
      % \node at (10, 1) {$1\mapsto 0$};
      % \node at (10, 0) {$0$};
      % % table of clock values: y
      % \node at (11, 10.5) {\Large $y$};
      % \node at (11, 10) {$10$};
      % \node at (11, 9) {$9$};
      % \node at (11, 8) {$8$};
      % \node at (11, 7) {$7$};
      % \node at (11, 6) {$6$};
      % \node at (11, 5) {$5$};
      % \node at (11, 4) {$4$};
      % \node at (11, 3) {$3$};
      % \node at (11, 2) {$2$};
      % \node at (11, 1) {$1$};
      % \node at (11, 0) {$0$};
   \end{tikzpicture}
}


==> tex/examples/const_mixed_choice.tex <==
\vspace{-4ex}%
\resizebox{0.15\textwidth}{!}{%
	\begin{tikzpicture}%
		% ~ grid
		% draw horizontal
		\foreach \y in {0,...,4}%
			{%
				\draw[gray] (0.75,\y) -- (1.25,\y);%
				\draw[gray] (1.75,\y) -- (2.25,\y);%
                % ~ axis
				\draw[gray] (0.15,\y) -- (0.35,\y);%
                % \node at (-0.25,\y) {\y};%
                % \node at (-0.75,\y) {\pgfmathtruncatemacro\result{\y+1}\result};%
			}%
		% draw vertical
		\foreach \x in {1,...,2}%
			{%
				\draw[gray] (\x,0) -- (\x,4);%
			}%
        % ~ axis
        \draw (0.25,0) -- (0.25,4);%
		% ~ labels
		% \node[above] at (-0.75,4) {\Clx*};%
		% \node[above] at (-0.25,4) {\Cly*};%
		\node[above] at (0.25,4) {\Const*};%
		\node[above] at (1,4) {\TypSend*};%
		\node[above] at (2,4) {\TypRecv*};%
        % ~ clock values
		% \node[right] at (0,4) {\Clx*};
		% \node[right] at (0,4) {\Cly*};
		%
	\end{tikzpicture}%
}%
\endinput

==> tex/examples/message_throttling/process.tex <==
%
\begin{equation}
    %
    \begin{array}[t]{l c l}%
        %
        \Prc & = & %
        %
        \PDefRec[A].{%
            \PDelay[t\geq 3]/.{%
                \PSend[msg1]/.{%
                    \PDefRec[B].{%
                        \PRecv[ack1].{%
                            \PRec[A]%
                        }<{3}>{%
                            \PSend[msg2]/.{%
                                \PRecv[ack2].{%
                                    \PRec[B]%
                                }<{3}>{%
                                    \PSend[tout]%
                                }%
                            }%
                        }%
                    }%
                }%
            }%
        }%
        %
        \\ \\%
        \Qrc & = & %
        %
        \PDefRec[C].{%
            \PRecv_q[msg1].{%
                \PSet{y}/.{%
                    \PDelay[t< 5]/.{%
                        \PIf[y<3]:{\PThen[%
                            \PSend_q[ack1].{%
                                \PRec[C]%
                            }%
                        ]}:{\PElse[%
                            \PDefRec[D].{%
                                \PRecv_q[msg2].{%
                                    \PSet{y}/.{%
                                        \PDelay[t< 5]/.{%
                                            \PIf[y<3]:{\PThen[%
                                                \PSend_q[ack2].{%
                                                    \PRec[D]%
                                                }%
                                            ]}:{\PElse[%
                                                \PRecv_q[tout]%
                                            ]}%
                                        }%
                                    }%
                                }<{3}%
                            }%
                        ]}%
                    }%
                }%
            }<{3}%
        }%
        %
    \end{array}
    %
\end{equation}
%

==> tex/examples/message_throttling/type.tex <==
%
\begin{equation*}
	%
	\resizebox{\textwidth}{!}{$
        \IRecDef[A].{%
            \IType!{msg}[3\leq x][\{x\}].{%
                \IChoice[%
                    \IType?{ack}[x<3][\{x\}].{%
                        \IRecCall[A]%
                    },%
                    \IRecDef[B].{%
                        \IType!{msg}[3\leq x][\{x\}].{%
                            \IChoice[%
                                \IType?{ack}[x<3][\{x\}].{%
                                    \IRecCall[B]%
                                },%
                                \IType!{tout}[3\leq x]%
                            ]%
                        }%
                    }%
                ]%
            }%
        }%
    $}%
	%
\end{equation*}
%

==> tex/examples/producer_consumer/diagram.tex <==
%
\resizebox{5cm}{!}{%
   \begin{tikzpicture}[scale=0.2]
      %
      \tikzstyle{every node}+=[inner sep=0pt]
      %
      \draw [black] (16.3,-11.3) circle (3);
      \draw (16.3,-11.3) node {$A$};
      \draw [black] (35.9,-11.3) circle (3);
      \draw (35.9,-11.3) node {$B$};
      \draw [black] (35.9,-11.3) circle (2.4);
      \draw [black] (16.3,-20.8) circle (3);
      \draw (16.3,-20.8) node {$C$};
      %
      \draw [black] (11.3,-11.3) -- (13.3,-11.3);
      \fill [black] (13.3,-11.3) -- (12.5,-10.8) -- (12.5,-11.8);
      %
      \draw [black] (19.3,-11.3) -- (32.9,-11.3);
      \fill [black] (32.9,-11.3) -- (32.1,-10.8) -- (32.1,-11.8);
      \draw (26.1,-11.8) node [below] {$\TypSend\!\;\squared{$\mathtt{stop}$}\mbox{ }(x<1)$};
      %
      \draw [black] (16.814,-8.356) arc (197.82696:-90.17304:2.25);
      \fill [black] (18.95,-9.92) -- (19.86,-10.15) -- (19.56,-9.2);
      \draw (29.01,-5.35) node [above] {$\TypRecv\!\;\squared{$\mathtt{data}$}\mbox{ }(1\leq x\leq 5,\,x)$};
      %
      \draw [black] (14.13,-18.787) arc (-149.02088:-210.97912:5.316);
      \fill [black] (14.13,-18.79) -- (14.15,-17.84) -- (13.29,-18.36);
      \draw (12.87,-16.05) node [left] {$\TypSend\!\;\squared{$\mathtt{tout}$}\mbox{ }(6\leq x,\,x)$};
      %
      \draw [black] (18.729,-12.982) arc (38.03468:-38.03468:4.979);
      \fill [black] (18.73,-12.98) -- (18.83,-13.92) -- (19.62,-13.3);
      \draw (20.29,-16.05) node [right] {$\TypRecv\!\;\squared{$\mathtt{retry}$}\mbox{ }(1\leq x,\,x)$};
      %
   \end{tikzpicture}
}
%

==> tex/examples/producer_consumer/process.tex <==
%
\begin{equation}
    %
    \begin{array}[t]{l c l}%
        %
        \Prc & = & %
        %
        \PDefRec[A].{%
            \PSet{x}/.{%
                \PDelay[t<2]/.{%
                    \PIf[x<1]:{\PThen[%
                        \PSend[stop]%
                    ]}:{\PElse[%
                        \PRecv[data].{%
                            \PRec[A]%
                        }<{4}>{%
                            \PDelay[1].{%
                                \PSend[tout]/.{%
                                    \PDelay[1]/.{%
                                        \PRecv[retry].{%
                                            \PRec[A]%
                                        }%
                                    }%
                                }%
                            }%
                        }%
                    ]}%
                }
            }%
        }%
        %
        \\ \\%
        \Qrc & = & %
        %
        \PDefRec[B].{%
            \PSet{y}/.{%
                \PRecv_q[stop]<{1}>{%
                    \PDelay[t<10]/.{%
                        \PIf[y\leq 4]:{\PThen[%
                            \PSend_q[data].{%
                                \PRec[B]%
                            }%
                        ]}:{\PElse[%
                            \PRecv_q[tout]/.{%
                                \PDelay[1\leq t]/.{%
                                    \PSend_q[retry].{%
                                        \PRec[B]%
                                    }%
                                }%
                            }%
                        ]}%
                    }%
                }%
            }%
        }%
        %
    \end{array}
    %
\end{equation}
%

==> tex/examples/producer_consumer/type.tex <==
%
\begin{equation}
	%
	\resizebox{\textwidth}{!}{$
		\IRecDef[A].{%
			\IChoice[%
				\IType!{stop}[x<1],%
				\IType?{data}[1\leq x\leq 5].{%
					\IRecCall[A]%
				},%
				\IType!{tout}[6\leq x][x].{%
					\IType?{retry}[1\leq x].{%
						\IRecCall[A]%
					}%
				}%
			]%
		}%
	$}%
	%
\end{equation}
%

==> tex/examples/unnamed_1/diagram.tex <==
%
\resizebox{\textwidth}{!}{%
   \begin{tikzpicture}[scale=0.2]
      %
      %
   \end{tikzpicture}
}
%

==> tex/examples/unnamed_1/process.tex <==
%
\begin{equation}
    %
    %
\end{equation}
%

==> tex/examples/unnamed_1/type.tex <==
%
\begin{equation*}
	%
	\resizebox{\textwidth}{!}{$
	$}%
	%
\end{equation*}
%

==> tex/figs/configs/actions.tex <==
% 
\begin{minieq}\label{eq:configs_actions}
    \begin{array}[t]{c p{2ex} c p{2ex} c}
        %
        \ProgAction::=\TypComm\Msg
        \mid\ValTime
        \mid\SiltAction
        %
            &  & %
        %
        \Msg::=\DefMsgType
        %
            &  & %
        %
        \Queue::=\emptyset
        \mid\Msg;\Queue
        %
    \end{array}
\end{minieq}
%

==> tex/figs/processes/calculus.tex <==
%
% ~ figure
% \begin{figure}[!htb]
\begin{minieq}\label{eq:prc_calc}
    \begin{array}[t]{r c l p{2ex} r c l}
        %
        \Prc,\Qrc & ::=
                  & \PCalcSend
                  &                                                                    & %
                  & \mid
                  & \PCalcRecv
        %
        \\\Buff[2.25]%
                  & \mid
                  & \PCalcScope
                  &                                                                    & %
                  & \mid
                  & \Par[\Prc][\Qrc]
        %
        \\\Buff[2.25]%
                  & \mid
                  & \PCalcBuffer
                  &                                                                    & %
                  & \mid
                  & \PrcRecDef
        %
        \\\Buff[2.25]%
                  & \mid
                  & \PCalcSetTimer
                  &                                                                    & %
                  & \mid
                  & \RecPrcCall
        %
        \\\Buff[2.25]%
                  & \mid
                  & \PFuncDelay
                  &                                                                    & %
                  & \mid
                  & \PCalcIf
        %
        \\\Buff[2.25]%
                  & \mid
                  & \PFuncDelay[\ValTime]
                  &                                                                    & %
                  & \mid
                  & \PrcEnd
        %
        \\\Buff[3]%
        \PrcMsg   & ::=
                  & \DefMsgType
                  &                                                                    & %
        \QHead    & ::=
                  & \mathrlap{\emptyset\mid{\QHead\cdot\PrcMsg}\mid{\QHead\cdot\PrcP}}
        %
    \end{array}
\end{minieq}
% \end{figure}
%

==> tex/figs/processes/func/nonempty.tex <==
%
% \begin{restatable}[htb]{figure}{FigPrcFuncNEQ}
\begin{figure}[htb]
	\begin{equation*}
		\PFuncNEQ =
		\begin{cases}
			%
			\mkSet[\SesQ]
			 & \text{if}\,
			\Prc=\PCalcBuffer\land\QHead\neq\emptyset
			%
			\\[0ex]
			\PFuncNEQ[\Qrc]\setminus\mkSet[\PrcP,\PrcQ]
			 & \text{if}\,
			\Prc=\PCalcScope[\Qrc]
			%
			\\[0ex]
			\PFuncNEQ[\Qrc]
			 & \text{if}\,
			\Prc=\PrcRecDef
			%
			\\[0ex]
			\PFuncNEQ[\Prc]\cup\PFuncNEQ[\Qrc]
			 & \text{if}\,
			\Prc=\Parl{P,Q}
			%
			\\[0ex]
			\emptyset
			 & \text{otherwise}
			%
		\end{cases}
	\end{equation*}
	\caption[Definition of \PFuncNEQ*]{Definition of \PFuncNEQ*}
	\label{fig:prc_func_neq}
\end{figure}
% \end{restatable}
%

==> tex/figs/processes/func/time_passing.tex <==
%
\begin{figure}[p]
   \centering%$
   \resizebox{\textwidth}{!}{$%
         %
         \begin{array}[t]{l}
            %
            \begin{array}[t]{l p{4ex} l p{4ex} l p{4ex} l }
               %
               \ColBoxOld{%
                  \PFuncTime[\PrcEnd]=
                  \PrcEnd
               }
               &  & %
               \ColBoxOld{%
                  \PFuncTime[\PCalcBuffer]=
                  \PCalcBuffer
               }
               &  & %
               % \PFuncTime[\PCalcSetTimer]=
               % \PFuncTime
               %  &  & %
               \ColBoxOld{%
                  \PFuncTime[\PCalcScope]=
                  \PCalcScope|\;\PFuncTime[\Prc]
               }
               %
                &  & %
               % \PFuncTime[\PCalcSetTimer]=
               % \PFuncTime
               %  &  & %
               \ColBoxOld{%
                  \PFuncTime[\PrcErr]=
                  \PrcErr
               }
            \end{array}
            %
            \\[-1ex]\\
            % \begin{array}[t]{l p{16ex} l}
            %     \PFuncTime[\RedPrc{\Prc}]=
            %     \RedPrc[\RedTimers+\ValTime]{\PFuncTime[\Prc]}
            %     %
            %      &  & %
            \ColBoxOld{%
               \PFuncTime[\PFuncDelay[\ValTime']]=
               \PFuncDelay[\ValTime'-\ValTime]
               \qquad
               \text{if}\;
               \ValTime'\geq\ValTime
            }
            % \end{array}
            %
            \\[-1ex]\\
            \ColBoxOld{%
               \PFuncTime[\Par[\Prc_1][\Prc_2]]=
               \Par[\PFuncTime[\Prc_1]][\PFuncTime[\Prc_2]]
               \qquad
               \text{if}\;
               \PFuncWait[\Prc_i]\cap\PFuncNEQ[\Prc_j]=
               \emptyset,
               i\neq j\in\left\{1,2\right\}%
            }
            %
            \\[2.5ex]
            \ColBoxOld{%\ColBoxMod{%
            \PFuncTime[\PrcRecDef]=
            \PrcRecDef>{\PFuncTime[\Qrc]}
            }
            %
            \\[2.5ex]
            \ColBoxOld{%\ColBoxNew{%
            \PFuncTime[\PCalc{\On{p}\Recv{l}[b]:{P}_{i}[i]~\After<{n}:{Q}}]=
            \begin{cases}
               % infty
               \PCalc{\On{p}\Recv{l}[b]:{P}_{i}[i]~\After<{n}:{Q}}
                &
               { n = \infty}
               %
               \\[0.5ex]
               %
               \PCalc{\On{p}\Recv{l}[b]:{P}_{i}[i]~\After<{n-t}:{Q}}
                &
               {n\in\RatSet \textit{ and  } n \geq t}
               %
               \\[0.5ex]
               \PFuncTime_{t-n}[Q]
                &
               \text{otherwise}
               %
            \end{cases}
            }
            %
            %
         \end{array}
         %
      $}
   \caption[Definition of \PFuncTime*]{Time-passing for processes.}
   \label{fig:prc_func_time}
\end{figure}
% \footnotetext{(Used when typing processes.)}
%

==> tex/figs/processes/func/wait.tex <==
%
% \begin{restatable}[htb]{figure}{FigPrcFuncWait}
\begin{figure}[htb]
   \begin{equation*}
      \PFuncWait =
      \begin{cases}
         %
         \mkSet[\SesP]
          & \text{if}\,
         \Prc\in\begin{array}[c]\{{l}\}\PCalc{\On{p}\Recv{l}[b]:{P}_{i}[i]~\After<{e}:{Q}},%
         ~% \\[-1ex]\\
         \PCalc{\On{p}\Recv{l}[b]:{P}_{i}[i]}\end{array}
         %
         \\[0ex]
         \PFuncWait[\Qrc]\setminus\mkSet[\PrcP,\PrcQ]
          & \text{if}\,
         \Prc=\PCalcScope[\Qrc]
         %
         \\[0ex]
         \PFuncWait[\Qrc]
          & \text{if}\,
         \Prc=\PrcRecDef
         %
         \\[0ex]
         \PFuncWait[\Prc]\cup\PFuncWait[\Qrc]
          & \text{if}\,
         \Prc=\Par[\Prc][\Qrc]
         %
         \\[0ex]
         \emptyset
          & \text{otherwise}
         %
      \end{cases}
   \end{equation*}
   \caption[Definition of \PFuncWait*]{Definition of \PFuncWait*}
   \label{fig:prc_func_wait}
   % \end{restatable}
\end{figure}
%

==> tex/figs/processes/rule_typing.tex <==
%%
\begin{figure}[htbp]
    \centering
    \resizebox{\textwidth}{!}{$%
            \begin{array}[c]{c}
                % ~ 
                \begin{array}[c]{c p{0ex} c p{0ex} c}
                    \begin{array}[c]{c c}
                        \ColBoxOld{\PTypRuleEnd} & \LblPrcTypEnd\end{array}
                    &  &
                    \begin{array}[c]{c c} \ColBoxOld{\PTypRuleEmptyQ} & \LblPrcTypEmptQ \end{array}
                    &  &
                    \begin{array}[c]{c c} \ColBoxOld{\PTypRulePar} & \LblPrcTypPar \end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxOld{\PTypRuleRes} & \LblPrcTypRes\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c p{0ex} c}
                    \begin{array}[c]{c c} \ColBoxMod{\PTypRuleVQue} & \LblPrcTypVQue \end{array}
                    &  &
                    \begin{array}[c]{c c} \ColBoxOld{\PTypRuleWeak} & \LblPrcTypWeak \end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c p{0ex} c}
                    \begin{array}[c]{c c} \ColBoxMod{\PTypRuleDQue} & \LblPrcTypDQue \end{array}
                    &  &
                    \begin{array}[c]{c c} \ColBoxNew{\PTypRuleTimer} & \LblPrcTypTimer \end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c p{0ex} c}
                    \begin{array}[c]{c c}
                        \ColBoxOld{\PTypRuleDelDelta} & \LblPrcTypDelDelta\end{array}
                    &  &
                    \begin{array}[c]{c c} \ColBoxMod{\PTypRuleDelTime} & \LblPrcTypDelTime \end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxNew{\PTypRuleBranch} & \LblPrcTypBranch\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxMod{\PTypRuleVRecv} & \LblPrcTypVRecv\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxMod{\PTypRuleDRecv} & \LblPrcTypDRecv\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c p{0ex} c}
                    \begin{array}[c]{c c}
                        \ColBoxNew{\PTypRuleIfTrue} & \LblPrcTypIfTrue\end{array}
                    &  &
                    \begin{array}[c]{c c}
                        \ColBoxNew{\PTypRuleIfFalse} & \LblPrcTypIfFalse\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxMod{\PTypRuleVSend} & \LblPrcTypVSend\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxMod{\PTypRuleDSend} & \LblPrcTypDSend\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c}
                        \ColBoxMod{\PTypRuleVar} & \LblPrcTypVar\end{array}
                \end{array}
                \\[1ex]\\%
                % ~ 
                \begin{array}[c]{c}
                    \begin{array}[c]{c c} \ColBoxMod{\PTypRuleRec} & \LblPrcTypRec \end{array}
                \end{array}
            \end{array}
        $}%
    \caption[Typing Processes Rules]{Rules for Typing Processes}
    \label{fig:prc_typ_rule}
\end{figure}
%
\endinput
\begin{sidewaysfigure}[htbp]
    \centering
    $% \begin{minieq}*
        % \resizebox{\textwidth}{!}{$%
        \begin{array}[c]{c}
            % ~ 
            % \begin{array}[c]{c p{0ex} c p{0ex} c}
            % 	\begin{array}[c]{c c}
            % 		\ColBoxOld{\PTypRuleEnd} & \LblPrcTypEnd\end{array}
            % 	 &  &
            % 	\begin{array}[c]{c c} \ColBoxOld{\PTypRuleEmptyQ} & \LblPrcTypEmptQ \end{array}
            % 	 &  &
            % 	\begin{array}[c]{c c} \ColBoxOld{\PTypRulePar} & \LblPrcTypPar \end{array}
            % \end{array}
            % \\[1ex]\\%
            % % ~ 
            % \begin{array}[c]{c}
            % 	\begin{array}[c]{c c}
            % 		\ColBoxOld{\PTypRuleRes} & \LblPrcTypRes\end{array}
            % \end{array}
            % \\[1ex]\\%
            % % ~ 
            % \begin{array}[c]{c p{0ex} c}
            % 	\begin{array}[c]{c c}
            % 		\ColBoxOld{\PTypRuleDelDelta} & \LblPrcTypDelDelta\end{array}
            % 	 &  &
            % 	\begin{array}[c]{c c} \ColBoxNew{\PTypRuleDelTime} & \LblPrcTypDelTime \end{array}
            % \end{array}
            % \\[1ex]\\%
            % % ~ 
            % \begin{array}[c]{c p{0ex} c}
            % 	\begin{array}[c]{c c} \ColBoxMod{\PTypRuleVQue} & \LblPrcTypVQue \end{array}
            % 	 &  &
            % 	\begin{array}[c]{c c} \ColBoxOld{\PTypRuleWeak} & \LblPrcTypWeak \end{array}
            % \end{array}
            % \\[1ex]\\%
            % % ~ 
            % \begin{array}[c]{c p{0ex} c}
            % 	\begin{array}[c]{c c} \ColBoxMod{\PTypRuleDQue} & \LblPrcTypDQue \end{array}
            % 	 &  &
            % 	\begin{array}[c]{c c} \ColBoxNew{\PTypRuleTimer} & \LblPrcTypTimer \end{array}
            % \end{array}
            % \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxNew{\PTypRuleBranch} & \LblPrcTypBranch\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleVRecv} & \LblPrcTypVRecv\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleDRecv} & \LblPrcTypDRecv\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            % \begin{array}[c]{c p{0ex} c}
            % 	\begin{array}[c]{c c}
            % 		\ColBoxNew{\PTypRuleIfTrue} & \LblPrcTypIfTrue\end{array}
            % 	 &  &
            % 	 \begin{array}[c]{c c}
            % 		 \ColBoxNew{\PTypRuleIfFalse} & \LblPrcTypIfFalse\end{array}
            % \end{array}
            % \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleVSend} & \LblPrcTypVSend\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleDSend} & \LblPrcTypDSend\end{array}
            \end{array}
            % \\[1ex]\\%
            % % ~ 
            % \begin{array}[c]{c}
            % 	\begin{array}[c]{c c}
            % 		\ColBoxNew{\PTypRuleVar} & \LblPrcTypVar\end{array}
            % \end{array}
            % \\[1ex]\\%
            % % ~ 
            % \begin{array}[c]{c}
            % 	\begin{array}[c]{c c} \ColBoxMod{\PTypRuleRec} & \LblPrcTypRec \end{array}
            % \end{array}
        \end{array}
        % $}%
    $% \end{minieq}
    \caption[Typing Processes Rules]{Rules for Typing Processes}
    \label{fig:prc_typ_rule}
\end{sidewaysfigure}
%
\endinput
%
%~figure
\begin{figure}[hp]
    \begin{minieq}*
        % \resizebox{\textwidth}{!}{$%
        \begin{array}[c]{c}
            % ~ 
            \begin{array}[c]{c p{0ex} c p{0ex} c}
                \begin{array}[c]{c c}
                    \ColBoxOld{\PTypRuleEnd} & \LblPrcTypEnd\end{array}
                &  &
                \begin{array}[c]{c c} \ColBoxOld{\PTypRuleEmptyQ} & \LblPrcTypEmptQ \end{array}
                &  &
                \begin{array}[c]{c c} \ColBoxOld{\PTypRulePar} & \LblPrcTypPar \end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxOld{\PTypRuleRes} & \LblPrcTypRes\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c p{0ex} c}
                \begin{array}[c]{c c}
                    \ColBoxOld{\PTypRuleDelDelta} & \LblPrcTypDelDelta\end{array}
                &  &
                \begin{array}[c]{c c} \ColBoxNew{\PTypRuleDelTime} & \LblPrcTypDelTime \end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c p{0ex} c}
                \begin{array}[c]{c c} \ColBoxMod{\PTypRuleVQue} & \LblPrcTypVQue \end{array}
                &  &
                \begin{array}[c]{c c} \ColBoxOld{\PTypRuleWeak} & \LblPrcTypWeak \end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c p{0ex} c}
                \begin{array}[c]{c c} \ColBoxMod{\PTypRuleDQue} & \LblPrcTypDQue \end{array}
                &  &
                \begin{array}[c]{c c} \ColBoxNew{\PTypRuleTimer} & \LblPrcTypTimer \end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxNew{\PTypRuleBranch} & \LblPrcTypBranch\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleVRecv} & \LblPrcTypVRecv\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleDRecv} & \LblPrcTypDRecv\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c p{0ex} c}
                \begin{array}[c]{c c}
                    \ColBoxNew{\PTypRuleIfTrue} & \LblPrcTypIfTrue\end{array}
                &  &
                \begin{array}[c]{c c}
                    \ColBoxNew{\PTypRuleIfFalse} & \LblPrcTypIfFalse\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleVSend} & \LblPrcTypVSend\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxMod{\PTypRuleDSend} & \LblPrcTypDSend\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c}
                    \ColBoxNew{\PTypRuleVar} & \LblPrcTypVar\end{array}
            \end{array}
            \\[1ex]\\%
            % ~ 
            \begin{array}[c]{c}
                \begin{array}[c]{c c} \ColBoxMod{\PTypRuleRec} & \LblPrcTypRec \end{array}
            \end{array}
        \end{array}
        % $}%
    \end{minieq}
    \caption[Typing Processes Rules]{Rules for Typing Processes}
    \label{fig:prc_typ_rule}
\end{figure}
%

==> tex/figs/processes/session_reduction.tex <==
%
% ~ figure
\begin{figure}[!htb]
    \begin{minieq}*
        \begin{array}[t]{c}
        \begin{array}[t]{c p{4ex} c}
            %
            \infer[\LblSesRedRed]{% * judgement
                \SesEnv_1,\SesEnv_2
                \PrcRed
                \SesEnv_1',\SesEnv_2
            }{% * premise
                \SesEnv_1
                \PrcRed
                \SesEnv_1'
            }
            %
            % \\\\[0.5ex]%
            & & %
            %
            \infer[\LblSesRedSend]{% * judgement
                \PrcP:\CIso,\ISes|:\Queue
                \PrcRed
                \PrcP:\CIso',\ISes|:\Queue;\Msg
            }{% * premise
                \Trans{\CSoc}:{\SendMsg}[\CSoc']
            }
            %
            % \\\\[0.5ex]%
        \end{array}
        \\\\[0.5ex]%
        \begin{array}[t]{c}
            %
            \infer[\LblSesRedSilent]{% * judgement
                \PrcP:\CIso,\ISes:\Msg;\Queue
                \PrcRed
                \PrcP:\CIso',\ISes:\Queue
            }{% * premise
                \Trans{\CSoc}:{\SiltAction}[\CSoc']
            }
            %
        \end{array}
    \end{array}
    \end{minieq}
    \caption[Reduction relation for session environments \SesEnv*]{Reduction relation for session environments \SesEnv*, building upon~\cref{fig:typesemantics}.}
    \label{fig:session_reduction}
\end{figure}
%

==> tex/figs/processes/typing.tex <==
%
% \begin{figure}[!htb]
\begin{minieq}\label{eq:prc_typ_env}
   \begin{array}[t]{r c l p{2ex} r c l p{2ex} r c l}
      %
      \SesEnv & ::=                     %
              & \emptyset               %
              &                       & %
      \VarEnv & ::=                     %
              & \emptyset               %
              &                       & %
      \SesSet & ::=                     %
              & \emptyset               %
      %
      \\\Buff[2.25]%
              & \mid                    %
              & \PSesEnvTypeSession     %
              &                       & %
              & \mid                    %
              & \VarEnv,~\PrcVal:\DataType   %
              &                       & %
              & \mid                    %
              & \PSesSetTypeEnvs        %
      %
      \\\Buff[2.25]%
              & \mid                    %
              & \PSesEnvTypeBuffer      %
              &                       & %
              & \mid                    %
              & \VarEnv,~x:n            %
              &                       & %
              &                         %
              &                         %
      %
      \\\Buff[2.25]%
              &                         %
              &                         %
              &                       & %
              & \mid                    %
              & \VarEnv,~\RecVar:\EnvPrcVar     %
              &                       & %
              &                         %
              &                         %
      %
   \end{array}
\end{minieq}
% \end{figure}
%

==> tex/figs/types/predicates.tex <==
%
\begin{minieq}\label{eq:types_predicates}
    \begin{array}[c]{>{$} p{0.65\textwidth} <{$} r}
        \Const ::= \TypeTrue%
        \mid \Clx>\ValTime%
        \mid \Clx=\ValTime%
        \mid \Clx-\Cly>\ValTime%
        \mid \Clx-\Cly=\ValTime%
        \mid \neg\Const%
        \mid \Const_1\land\Const_2%
        %
            & \text{where\ }\Clx,\Cly\in\ClockSet %
    \end{array}
\end{minieq}
%

==> tex/main/_restatable/_all_defs.tex <==

\subsection{Types}
\FigTypesPredicates*
\FigTypesSyntax*
% ~ types
\DefTypesWellFormed*

\DefTypesDual*

\subsection{Configurations}
% ~ configs
\FigConfigsActions*

% ~ iso configs
\DefConfigsIsoFutureEn*

\DefConfigsIsoLive*

\DefConfigsIsoWellFormed*

% ~ sys configs
\DefConfigsCompat*

\DefConfigsSysProgress*

\subsection{Processes}
% ~ process calc
\FigPrcCalc*
\FigPrcTyp*

% ~ process typing
\DefPrcTypClockDomains*

\DefPrcTypTReading*


==> tex/main/_restatable/_all_figs.tex <==

% ~ types
\FigTypesRule*

% ~ configs
% ~ iso configs
\FigConfigsIsoRule*

% ~ soc configs
\FigConfigsSocRule*

% ~ sys configs
\FigConfigsSysRule*

% ~ process calc
\FigPrcReduc*

\FigPrcFuncTime*

% ~ process typing
\FigPrcRuleTyp*


==> tex/main/configs/configs.tex <==

This section presents a compositional semantics for timeout session types in the form of labelled transition systems (LTS) over configurations.
In this work, configurations refer to a tuple (or triple) used in the evaluation of a types behaviour; comprised of a type \TypeS*\ and a valuation of clocks \ValClocks*. 

This section explores different collections of semantics in a structured manner, in order to better provide an understanding of the overarching control flow of a system.
This work considers three kinds of configurations
\begin{inline}*+;
   \item \emph{isolated} configurations capture the behaviour of a type uninfluenced by anything beyond itself
   \item \emph{social} configurations capture the behaviour a type exhibits in order to communicate with others
   \item \emph{system} configurations capture the behaviour of a system comprised of multiple \emph{social} configurations, that run in parallel and communicate with each other
\end{inline}
Hereafter, configurations may be referred to as \emph{configs}.

Configurations are layered, building upon and encapsulating the layers below
\begin{inline}>[\;$\subset$\,]
   \item an isolated config
   \item a social config
   \item a system config
\end{inline}
In practice, a system makes a transition comprised of one or more social transitions, which is in turn comprised of some isolated transitions.

\paragraph*{Configuration Transitions}
Configurations may perform actions corresponding transition on a given LTS
(for isolated see~\cref{fig:configs_iso_rule}; social see~\cref{fig:configs_soc_rule}, and for system see:~\cref{fig:configs_sys_rule}).
Let \ProgAction*\ be any action that a configuration can take. Configuration transitions may be more specific than \ProgAction*.
\input{tex/figs/configs/actions.tex}
Let \Msg*\ be a message used in a communication between two configurations, comprised of a message label \MsgLabel*\ and some real data of type \DataType*. The symbol \TypComm*\ is defined with the same meaning as in the types.
Let \Queue*\ be a queue where messages \Msg*\ are to be received.

The transition \TypComm*\Msg*\ describes a message \Msg*\ being either being sent or received.
A transition of \ValTime*\ describes a time step occurring, with the value of \ValTime*\ passing over the configuration.
A \SiltAction*\ transition describes an action beyond the scope of its use.
\begin{note}
    Sequences of actions, such as \Act*\Act*, yield the same meaning as \Act*[\ProgAction\,\ProgAction].
\end{note}

\endinput


\subsection{Configurations of Isolated Types}
\TODO % TODO: 

\begin{note}
   A configuration of isolated types \isoconfig{}\ can also be written: \iso{}.
\end{note}

\subsubsection{Semantics of Isolated Configurations}\label{ssec:configs_iso_lts}
The semantics of social configurations are presented in~\cref{fig:configs_iso_lts}, followed by an explanation for each.

\begin{figure}[h]\centering%
   \input{tex/figs/configs_iso_lts.tex}
   %
   \caption[Semantics of Isolated Configurations]{{Semantics of Isolated Configurations}.}
   \label{fig:configs_iso_lts}
\end{figure}\vspace{-4ex}
\begin{description}[itemsep=1.25ex,parsep=1.25ex]
   \item[Rule \isorInteract\;] Describes an interaction being performed; having sent some data \msglabel, the relevant clocks are reset to 0 and the configuration progresses to the next type.

      The premise enforces that the current valuation of clocks must satisfy the constraint; and, using the same condition as \formChoice\ of the formation rules, ensures that only interactions of the same communication direction (sending or receiving) are considered together.

   \item[Rule \isorRec] Unfolds recursive types.

   \item[Rule \isorTime] Allows time to pass, adding \tval\ to the valuation of all clocks.

\end{description}

\input{tex/defs/configs_iso_future_enabled.tex}

\input{tex/defs/configs_iso_live.tex}
\begin{lemma}
   Given a well-formed \st, \isoinit{}\ is \emph{live}.
\end{lemma}
\begin{proof}
   As $\of{\mval}{0}\models\mpast$ holds for any possible \constr.
\end{proof}

\input{tex/defs/configs_iso_well_formed.tex}

\subsection{Social Configurations}
\TODO % TODO: 

A sent message $\mmsg$ must first be enqueued into the recipients queue, before it can be received.

\begin{note}
   A configuration of social types \socconfig{}\ can also be written: \soc{}.
\end{note}

\subsubsection{Semantics of Social Configurations}\label{ssec:configs_soc_lts}
The semantics of social configurations are presented in~\cref{fig:configs_soc_lts}, followed by an explanation for each.
\begin{figure}[h]\centering%
   \input{tex/figs/configs_soc_lts.tex}
   %
   \caption[Semantics of Social Configurations]{{Semantics of Social Configurations}.}
   \label{fig:configs_soc_lts}
\end{figure}\vspace{-4ex}
\begin{description}[itemsep=1.25ex,parsep=1.25ex]
   \item[Rule \socrSend] Sends a message $\mmsg$ representing some labelled data as defined by the types, given that this action adheres to the premise of \isorInteract, meaning that the constraint is satisfied and this is considered to be a safe mixed-choice. The resulting configuration has a new current type and updated valuation of clocks.

   \item[Rule \socrRecv] Retrieves a message $\mmsg$ from the queue, given that there is a corresponding receiving action, and, similarly \socrSend, that this receiving action adheres to the premise of \isorInteract. On a successful evaluation, the message received is removed from the queue, and the configuration has a new current type and updated valuation of clocks.

   \item[Rule \socrEnqu] Receives a message $\mmsg$ and enqueues it to the end of the queue.

   \item[Rule \socrTime] Allows a time step \tval\ over the valuation of clocks given that both of the following hold
      \begin{inlineEnum}
         \item the viability of any sending actions are still possible after the step (their constraints remain either satisfied or unsatisfied)
         \item that there is no smaller time step possible that would allow a message to be received from the queue sooner
      \end{inlineEnum}
      It is not enough that there is a message in the queue, but that the message in the queue corresponds to a receiving action, and will result in a new type and updated valuation of clocks (by \socrRecv).

\end{description}


==> tex/main/configs/isolated.tex <==

Isolated configurations capture the behaviour of types without any influences beyond itself. All transitions reflect local actions, hidden to anything but itself.
An isolated configuration \CfgIso*\ is a tuple comprised of a valuation of clocks \ValClocks*\ and type \TypeS*, and may be written as \IsoCfg*.
\begin{note}
    Any configuration with a transition $\IsoCfg\Act\IsoCfg'$ may be written as $\IsoCfg\Act$, to mean that there exists some possible transition \ProgAction*\ such that a new configuration \IsoCfg*'\ can be reached.
\end{note}
The semantics of isolated configurations is presented in~\cref{fig:configs_iso_rule}.
\input{tex/figs/configs/rule_iso.tex}
Rule \LblCfgIsoUnfold*\ handles recursive types, unfolding them by substituting any occurrence of the corresponding call \CfgRecDef*, in the proceeding type \TypeS*, with the sequence of types between \TypeS*\ and any recursive call \CfgRecDef*. The resulting type \TypeS*'\ may be some intermediate type between the recursive definition and a corresponding call.
Rule \LblCfgIsoTick*\ allows time to pass over the clocks.

The \LblCfgIsoInteract*\ rule allows a configuration to perform any interaction with constraints satisfied by the current valuation of clocks. The resulting configuration has the type \TypeS*_j\ corresponding to the interaction performed, along with any conditional resets being applied to \ValClocks*.


==> tex/main/configs/social.tex <==

The behaviour of communication between types can be captured using social configuration. A social configuration \CfgSoc*\ is a triple with a similar composition as an isolated configuration, but with the addition of a queue \Queue*. A social configuration \CfgSoc*\ may be written as \SocCfg*\ just as \CfgIso*\ can be written as \IsoCfg*.
The transitions for social configurations, shown in~\cref{fig:configs_soc_rule}, often depend on a corresponding isolated configuration transition, comprised of the same \ValClocks*\ and \TypeS*.
\input{tex/figs/configs/rule_soc.tex}
Rule \LblCfgSocSend*\ depends on \LblCfgIsoInteract*, requiring that the message \Msg*\ being sent corresponds to an interaction within \TypeS*, that has its constraints satisfied by \ValClocks*. The resulting configuration, as defined in \LblCfgIsoInteract*, has any resets applied to \ValClocks*'\ and continues as the proceeding type \TypeS*'. The queue is unaffected by this behaviour.

Message reception is handled by two rules, \LblCfgSocEnqu*\ and \LblCfgSocRecv*. The former allows messages to be enqueued into \Queue*, and describes the abstraction of how messages are received over a network.
The latter, \LblCfgSocRecv*, requires a message \Msg*\ to have already been enqueued into \Queue*, so that the system can receive it. Just as with \LblCfgSocSend*, this rule is dependant on \LblCfgIsoInteract*, and yields the same results; with one exception: the message \Msg*\ must be removed from the queue \Queue*. This is described by the silent \SiltAction*, which in this instance describes both of the actions taking place.
Only the message at the head of the queue is received as, following \emph{communication safety}, all messages are expected and able to be received.

The rule \LblCfgSocTime*\ allows an amount of time \ValTime*\ to pass, requiring the following premises hold
\begin{inline}*+
    \item the value of \ValTime*\ is added to all valuations of clocks, by rule \LblCfgIsoTick*
    \item no sending opportunities are missed by the time step
    \item that there exists no smaller time step that would allow a message to be received sooner
\end{inline}
Together, these ensure that as few and as small time steps are taken so that interactions are performed as soon as possible; this is explored further in~\cref{sssec:configs_sys_compatibility}.
\begin{note}
    The notion of \emph{liveness} (see~\cref{def:configs_iso_live}) can be applied to social configurations.
\end{note}


==> tex/main/configs/systems.tex <==

%\subsubsection{Progress of Systems}\label{sssec:configs_sys_progress}
\input{tex/defs/types/progress.tex}
\input{tex/defs/configs/sys/progress.tex}

\input{tex/proofs/progress/thm.tex}

\endinput
System configurations are composed of two distinct social configurations, \SocCfg*_1\ and \SocCfg*_2, running in parallel: \CfgSys*. The rules given in~\cref{fig:configs_sys_rule} reveal the following high-level control flow of a system
\begin{inline}>
	\item \dots
	\item \LblCfgSysWait*
	\item \LblCfgSysLComm*
	\item \LblCfgSysLPar*
	\item \dots
\end{inline}\etc\ .
Describing there being some time to wait \ValTime*\ until a communication between the two parties can occur, which results in the message being received by a queue; at which point the message can be retrieved from the queue and received by the configuration. This cycle continues indefinitely until either both types terminate or a deadlock is reached.
\input{tex/figs/configs/rule_sys.tex}
Rule \LblCfgSysLComm*\ specifies that both configurations can make transitions to new configurations when one performs a transition via \LblCfgSocSend*\ and the other by \LblCfgSocEnqu*; for example:
\begin{minieq}
	\Par[\CfgSoc_1][\CfgSoc_2]
	\;\Act[\SiltAction]\,
	\Par[\CfgSoc_{1}''][\CfgSoc1{\ValClocks_2}2{\TypeS_2}3{\Queue_2;\Msg}]
\end{minieq}
While rule \LblCfgSysLPar*\ describes one party successfully receiving a message from their queue by a transition via \LblCfgSocRecv*.

Rule \LblCfgSysWait*\ allows time to pass evenly over the entire system, requiring both participants to make a transition via \LblCfgSocTime*\ of the same value of \ValTime*. The amount of time \ValTime*\ is restricted to the greatest value shared by both parties by the premise of their respective \LblCfgSocTime*\ transitions. This ensures that time passes evenly for separate participants, effectively halting time for the whole system once a participant has no choice but to perform an action.

\subsubsection{Ensuring System Compatibility}\label{sssec:configs_sys_compatibility}
Given a system composed of configurations with dual well-formed types, there is the potential for the system to exhibit \emph{communication safety} and deadlock freedom.
However, this is not guaranteed just by types being well-formed, but must be ensured by their defined behaviour.

Naturally, the rules of~\cref{fig:configs_iso_rule,fig:configs_soc_rule,fig:configs_sys_rule} specify that messages must be sent my one party before being received by another.
Furthermore, sending actions exhibit a \emph{relaxed} notion of urgency, by the premise of \LblCfgSocTime*, which specifies that a value of time may pass, delaying the sending of messages in order to accumulate as many viable actions as possible, so long as no opportunities for sending a message are missed.
Given that a receiving party is composed of dual types, a message that is delayed will still be successfully received.

Conversely, receiving actions \emph{must} exhibit urgency, as a message existing in a queue indicates that the sender has already progressed to some later type. Consider the trace of a type in~\cref{eq:example_configs_sys_compatability}.
\begin{minieq}\label{eq:example_configs_sys_compatability}
	\TypAct1{\TypSend}2{\mathtt{e}}
	\TypCond1{\Clx<3}2{\Clx}
	.
	\TypAct1{\TypRecv}2{\mathtt{f}}
	\TypCond1{\Clx=0}2{\emptyset}
	\dots
\end{minieq}
In the instance where the sending of \texttt{e} is delayed until the last possible moment $\Clx=2.9$, any delay of its dual counterpart would result in \texttt{f} being send too late. \TODO[note cite?]
\begin{note}
	In this work latency over a network is not considered, but may be accounted for in implementations.
\end{note}

For this reason, \LblCfgSocTime*\ does not allow time to pass for a configuration if there is a message waiting to be received. Additionally, receive urgency ensures that the clocks of each participant are kept synchronised as they progress.
This notion of compatibility is formally defined in~\cref{def:configs_compat}; an explanation of each condition is as follows
\begin{inline}*+;
	\item only one participant may receive messages at any time
	\item compatibility is preserved as messages are received
	\item both initial configurations of a system and systems in waiting are compatible, with both having matching clock valuations and dual types
\end{inline}
\input{tex/defs/configs/sys/compat.tex}
In practice conditions 2 and 3 are of interest, as it reflects the control flow of a system described at the beginning of~\cref{ssec:configs_sys} where a system has either
\begin{inline}|;
	\item performed a \LblCfgSysLComm*\ leading to a subsequent \LblCfgSysLPar*, following condition 2
	\item no interactions are possible, meaning only time may pass via \LblCfgSysWait*, following condition 3
\end{inline}
Additionally, condition 2 of compatibility supports situations where one participant sends several messages in succession without the other participant receiving them. This is valid behaviour.



==> tex/main/configs/well_formed.tex <==

Building upon the notion of well-formed types (\cref{def:types_well_formed}), a well-formed configuration exhibits behaviour without deadlocks, where there is always some action able to be performed in the future, until the termination type is reached.
This behaviour is referred to as \emph{liveness}, and is given in~\cref{def:configs_iso_live}, and depends on \emph{future enabled} actions.
\input{tex/defs/configs/iso/future_en.tex}
\input{tex/defs/configs/iso/live.tex}
The liveness of a configuration indicates whether a deadlock has been reached. There must either be an action immediately viable, some future enabled actions, or the type must have reached termination.
\input{tex/defs/configs/iso/well_formed.tex}
Given a type \TypeS*\ well-formed against \ValClocks*, it holds that a configuration of \IsoCfg*\ will have future enabled actions, and therefore be live.
\begin{note}
    For a \emph{well-formed} \TypeS*, \CfgIso*1{\ValClocks_{0}} is \emph{live}.
\end{note}


==> tex/main/extra/dnf.tex <==
Let $\Pi$ be a fixed, finite set of non-strict inequalities over the set of variables $X$.  We suppose that $\Pi$ is closed under binding variables to zero, that is, 
if $\pi \in \Pi$ then $\pi[x/0] \in \Pi$. (This is needed to support the $d[\lambda/0]$ calculation in the snd and rcv rules.) It follows that $true, false \in \Pi$.

Let $\delta = \pi | \neg \delta | \delta_1 \wedge \delta_2$.

To demonstrate that $\delta_1 \rightarrow \delta_2$ is computable we need to find a symbolic representation of $\delta_i$ that allows $\delta_1 \rightarrow \delta_2$ to be expressed in the same representation.   
We elect to represent $\delta_i$ as a disjunct of prime implicants where each prime implicant is a (non-redundant) conjunct of non-strict inequalities (positive literals) and negated inequalities (negative literals). This gives a compact and intuitive representation which is amenable to derivation using an SMT solver supporting difference logic or linear arithmetic.

To see this, first recall that $\delta_1$ and $\delta_2$ can be transformed to equi-satisfiable SMT formulae $f_1$ and $f_2$, with only a polynomial increase in space, by introducing fresh propositional (Tseytin) variables such that if $f_i$ holds then $t_i$ is true iff $\delta_i$ holds. Then the formula $f = (t_1 \rightarrow t_2) \wedge f_1 \wedge f_2$ is equi-satisfiable with $\delta_1 \rightarrow \delta_2$.

Now solve the SMT instance $f$. Suppose that $f$ is satisfiable with an assignment 
$\theta = \{ x_1 \mapsto c_1, \ldots, x_n \mapsto c_n \}$ where $X = \{ x_1, \ldots, x_n \}$ and $c_i \in \mathbb{Q}$.

Given the assignment $\theta$, construct the cube $c = q_1 \wedge \ldots q_n$ where
$q_i = \pi_i$ if $\pi_i$ holds for $\theta$ and $q_i = \neg \pi_i$ otherwise.
Observe that $c \models f$ since the truth or falsity of $f$ is defined only by the truth or falsity of inequalities of $\Pi$.  Now find a minimal subcube $c_1$ of $c$ such that $c_1 \models f$. To do so, consider eliminating $q_i$ and put $c’ = c \setminus q_i$.
If $c’ \wedge \neg f$ is unsatisfiable then $c’ \models f$ hence $q_i$ is redundant, else $q_i$ must be retained. Consider each $q_i$ in turn to derive a minimal subcube $c_1$.  Such a minimal subcube is called a prime implicant.

Now repeat the process with $f’ = f \wedge (\neg c_1)$ to give another minimal cube $c_2$, continuing until $f \wedge (\neg c_1) \ldots (\neg c_m)$ is unsatisfiable.  Then $\delta_1 \rightarrow \delta_2 \equiv f \equiv \vee_{j = 1}^{m} c_j$.

\begin{example}
Suppose $\Pi = \{  p, q, r \}$ and let $p = (x \leq y)$, $q = (y – z \leq -2)$
and $r = (z – y \leq 1)$. Now consider computing a representation for $f_0 = \delta_1 \rightarrow \delta_2$ where $\delta_1 = p$ and $\delta_2 = (q \vee r)$.
\begin{itemize}

\item
Consider the assignment $\theta_0 = \{  x \mapsto 1, y \mapsto 0, z \mapsto 0 \}$ of $f_0$.
Then $c = (\neg p) \wedge (\neg q) \wedge r$ and $c_0 = (\neg p)$.
Put $f_1 = f_0 \wedge (\neg c_0) = f_0 \wedge p$.

\item
Now consider the assignment $\theta_1 = \{  x \mapsto 0, y \mapsto 1, z \mapsto 0 \}$ of $f_1$.
Then $c = p \wedge (\neg q) \wedge r$ and $c_1 = (p \wedge r)$.

Put $f_2 = f_1 \wedge (\neg c_1) = f_0 \wedge p \wedge (\neg p \vee \neg r) \equiv f_0 \wedge p \wedge (\neg r)$.

\item
Now consider the assignment $\theta_2 = \{  x \mapsto 0, y \mapsto 1, z \mapsto 4 \}$ of $f_2$.
Then $c = p \wedge q \wedge (\neg r)$ and $c_2 = (p \wedge q)$.

Put $f_3 = f_1 \wedge (\neg c_1) = f_0 \wedge p \wedge (\neg p \vee \neg r) \wedge (\neg p \vee \neg q) \equiv f_0 \wedge p \wedge (\neg r) \wedge (\neg q)$.

\item
But $f_3$ is unsatiable hence $f_0 = c_1 \vee c_2 \vee c_3$.

\end{itemize}
\end{example}

Note that we could work in disjunctive normal form (DNF) and calculate $\delta_1 \rightarrow \delta_2 = (\neg \delta_1) \vee \delta_2$ but applying de Morgan's and a distribution law to place $\neg \delta_1$ is DNF. However, we would still need to check that each disjunct is satisfiable (which follows immediately in the above since the cube $c$ is derived from an assignment) and there is no guarantee that the disjuncts will be short (prime) or few in number.

==> tex/main/extra/subtyping.tex <==
% !TEX root = main.tex

%\subsection{Subtyping}

\def\myend{\texttt{end}}

\begin{lemma}\label{lemma-zero}
    $\delta[x/0] = \vee \{ \delta' \mid \delta'[x \mapsto 0] \models \delta \}$
\end{lemma}

\begin{proof}[For Lemma~\ref{lemma-zero}] \mbox{}
    \begin{itemize}
        \item Observe
              \[
                  \begin{array}{rcl}
                      \delta[x/0][x \mapsto 0] & =      & \exists_x(\delta[x/0]) \wedge (x = 0) \\
                                               & =      & \delta[x/0] \wedge (x = 0)            \\
                                               & \equiv & \delta \wedge (x = 0) \models \delta
                  \end{array}
              \]
        \item Let $\delta'[x \mapsto 0] \models \delta$.
              Then
              \[
                  \begin{array}{rcl}
                      \delta' \models \exists_x(\delta') & = & \exists_x(\delta') \wedge true                  \\
                                                         & = & (\exists_x(\delta') \wedge (x = 0))[x/0]        \\
                                                         & = & (\delta'[x \mapsto 0])[x/0] \models \delta[x/0]
                  \end{array}
              \]

    \end{itemize}
\end{proof}

%\begin{definition}
%$\delta_1 \multimap \delta_2 = 
%\vee \{ \delta \mid \delta \wedge \delta_1 \models \delta_2, (\delta \wedge \delta_1) \not\models %false \}$
%\end{definition}

\begin{figure}[t!]
    \begin{center}
        \begin{tabular}{ccc}
            \resizebox{0.3\textwidth}{!}{
                \begin{tikzpicture}
                    \draw (0,0) -- (7,0);
                    \draw (0,0) -- (0,7);

                    \foreach \x in {1,...,7}
                        {
                            \draw [gray] (\x,0) -- (\x,7);
                            \draw [gray] (0,\x) -- (7,\x);
                        }

                    \filldraw [red, opacity = 0.25] (0,2) -- (3,5) -- (5, 5) -- (5, 2) -- (0, 2);
                    %\filldraw [red, opacity = 0.25] (4,2) -- (4, 4) -- (7, 7) -- (7, 5) -- (4, 2);
                    
                    \filldraw [red, line width = 2pt] (0,0) -- (2, 2);
                    \draw[fill, red] (0,0) circle (4pt);
                    
                    \filldraw [red, line width = 2pt] (4,4) -- (7, 7);
                    \draw[fill, red] (4,4) circle (4pt);
                    \draw[fill, red] (7,7) circle (4pt);

                    \node at (3,3) {\Large $\delta_1$};
                    \node[below] at (7,0) {\Large $x_1$};
                    \node[left] at (0, 7) {\Large $x_2$};
                \end{tikzpicture}}
             &
            \resizebox{0.3\textwidth}{!}{
                \begin{tikzpicture}
                    \draw (0,0) -- (7,0);
                    \draw (0,0) -- (0,7);

                    \foreach \x in {1,...,7}
                        {
                            \draw [gray] (\x,0) -- (\x,7);
                            \draw [gray] (0,\x) -- (7,\x);
                        }

                    %\filldraw [red, opacity = 0.25] (0,2) -- (3,5) -- (5, 5) -- (5, 2) -- (0, 2);
                    \filldraw [red, opacity = 0.25] (4,2) -- (4, 4) -- (7, 7) -- (7, 5) -- (4, 2);
                    
                    \filldraw [red, line width = 2pt] (0,0) -- (2, 2);
                    \draw[fill, red] (0,0) circle (4pt);
                    
                    \filldraw [red, line width = 2pt] (4,4) -- (7, 7);
                    \draw[fill, red] (4,4) circle (4pt);
                    \draw[fill, red] (7,7) circle (4pt);

                    %\node at (3,3) {\Large $\delta_1$};
                    \node at (6,5) {\Large $\delta_2$};
                    \node[below] at (7,0) {\Large $y_1$};
                    \node[left] at (0, 7) {\Large $y_2$};
                \end{tikzpicture}}
             &
            \resizebox{0.3\textwidth}{!}{
                \begin{tikzpicture}
                    \draw (0,0) -- (7,0);
                    \draw (0,0) -- (0,7);

                    \foreach \x in {1,...,7}
                        {
                            \draw [gray] (\x,0) -- (\x,7);
                            \draw [gray] (0,\x) -- (7,\x);
                        }

                    \filldraw [orange, opacity = 0.5] (0,0) -- (2,0) -- (2, 7) -- (0, 7) -- (0, 0);
                    \filldraw [orange, opacity = 0.5] (4,0) -- (7,0) -- (7, 7) -- (4, 7) -- (4, 0);
                    \filldraw [orange] (0,0) -- (7, 7);
                    \filldraw [orange, line width = 2pt] (0,0) -- (2, 2);
                    \filldraw [orange, line width = 2pt] (4,4) -- (7, 7);
                    \draw[fill, orange] (0,0) circle (4pt);
                    \draw[fill, orange] (4,4) circle (4pt);
                    \draw[fill, orange] (7,7) circle (4pt);

                    \node at (6,5) {\Large $\delta_1 \multimap \delta_2$};
                    \node[below] at (7,0) {\Large $x_1$};
                    \node[left] at (0, 7) {\Large $x_2$};
                \end{tikzpicture}}
            \\
        \end{tabular}
    \end{center}
    \caption{Exploiting the vector of time}
\end{figure}

\begin{definition}
Suppose $vars(\delta_1) \subseteq vars(\vec{x})$,
$vars(\delta_2) \subseteq vars(\vec{y})$
and
$vars(\vec{x}) \cap vars(\vec{y}) = \emptyset$.
Then
\[
\delta_1 \multimap \delta_2 = 
\vee \{ \vec{x} = \vec{x_1} \wedge \vec{y} = \vec{x_1} \wedge x_1 \in I \mid I \in C^{*} \}
\]
where
\[
T = \{ t \in \mathbb{Q}^{+} \mid \vec{x} = \vec{t} \wedge \vec{y} = \vec{t} \wedge \delta_1 \models \delta_2 \}
\]
\[
C = \{ I \in Int \mid I \subseteq T \}
\qquad
C^{*} = \{ I \in C \mid \forall J \in C . I \subseteq J \rightarrow I = J \}
\]

\end{definition}

\begin{lemma}
Let $\nu \in \llbracket \delta_1 \multimap \delta_2 \rrbracket$.
Then 
$\nu + t \in \llbracket \delta_1 \multimap \delta_2 \rrbracket$
iff
$\nu + t \in \llbracket \delta_1 \rightarrow \delta_2 \rrbracket$.
\end{lemma}

\begin{proposition}[soundness and optimality]\label{lemma-implication} \mbox{}
    \begin{itemize}
        \item $\delta_1 \wedge (\delta_1 \multimap \delta_2) \models \delta_2$
        \item Let $\delta = \vee_{i=1}^n \pi_i$. If $\delta_1 \wedge \delta \models \delta_2$ then $\delta_1 \wedge \delta \models \delta_1 \wedge (\delta_1 \multimap \delta_2)$
    \end{itemize}
\end{proposition}

\begin{proof}[for proposition~\ref{lemma-implication}] \mbox{}
    \begin{itemize}
        \item
              %Let $\nu \in \llbracket \delta_1 \wedge (\delta_1 \multimap \delta_2) \rrbracket$.
              Observe $\delta_1 \wedge \neg \delta_2 \models ch(\delta_1 \wedge \neg \delta_2) \models core(ch(\delta_1 \wedge \neg \delta_2), \delta_2)$
              and therefore $\delta_1 \multimap \delta_2 = \neg core(ch(\delta_1 \wedge \delta_2), \delta_2) \models \neg (\delta_1 \wedge \neg \delta_2) \equiv (\neg \delta_1) \vee \delta_2$.
              It thus follows $\delta_1 \wedge (\delta_1 \multimap \delta_2) \models \delta_1 \wedge ((\neg \delta_1) \vee \delta_2) \equiv false \vee (\delta_1 \wedge \delta_2) \equiv \delta_1 \wedge \delta_2 \models \delta_2$.

        \item Let $\delta_1 \wedge \delta \models \delta_2$.
              Then
              $\delta_1 \wedge \pi_i \models \delta_2$ for all $i \in \{ 1, \ldots, n \}$.
              \begin{itemize}
                  \item Suppose $\delta_1 \wedge \pi_i \models false$. Then $\delta_1 \wedge \pi_i \models \delta_1 \wedge (\delta_1 \multimap \delta_2)$.

                  \item Suppose $\delta_1 \wedge \pi_i \not\models false$.
                        Let $\nu \in \llbracket \delta_1 \wedge \pi_i \rrbracket$.
                        Since $\delta_1 \wedge \pi \models \delta_2$ it follows that $\nu \in \llbracket \delta_2 \rrbracket$ but
                        $\nu \not\in \llbracket \neg \pi_i \rrbracket$.
                        Thus $\delta_2 \not\models \neg \pi_i$ and $core(\{ \neg \pi_i \}, \delta_2) = \{ \neg \pi_i \}$.
                        Observe $(\delta_1 \wedge \neg \delta_2) \wedge \pi_i \models false$
                        thus $\delta_1 \wedge \neg \delta_2 \models \neg \pi_i$.
                        Therefore
                        $\neg \pi_i \in ch(\delta_1 \wedge \neg \delta_2)$
                        and by Lemma~\label{lemma-mono}
                        $\wedge core(ch(\delta_1 \wedge \neg \delta_2), \delta_2) \models \neg \pi_i$.
                        It follows that
                        $\pi_i \models \neg \wedge core(ch(\delta_1 \wedge \neg \delta_2), \delta_2) \equiv \delta_1 \multimap \delta_2$ and
                        $\delta_1 \wedge \pi_i \models \delta_1 \wedge (\delta_1 \multimap \delta_2)$.
              \end{itemize}
              Therefore $\delta_1 \wedge \delta \models \delta_1 \wedge (\delta_1 \multimap \delta_2)$
    \end{itemize}
\end{proof}

\begin{figure}[t]
    \[
        \begin{array}{c}
            \infer[\text{end}]{
                true \vdash \myend \leq \myend
            }
            {
            }
            \\\\
            \infer[\text{snd}]{
                \delta_1 \multimap \delta_2 \wedge d[\lambda_1 \cup \lambda_2 / 0] \vdash ! \; m_1 (\delta_1, \lambda_1) . S_1 \leq ! \; m_2 (\delta_2, \lambda_2) . S_2
            }
            {
                m_2 \sqsubseteq m_1 \qquad 
                d \vdash S_1 \leq S_2 
            }
            \\\\
            \infer[\text{rcv}]{
                \delta_2 \multimap \delta_1 \wedge d[\lambda_1 \cup \lambda_2 / 0] \vdash ? \; m_1 (\delta_1, \lambda_1) . S_1 \leq ? \; m_2 (\delta_2, \lambda_2) . S_2
            }
            {
                m_1 \sqsubseteq m_2 \qquad 
                d \vdash S_1 \leq S_2 
            }
            \\\\
            \infer[\text{mix}]
            {
            d
            \vdash
            \{ \square_i m_i(\delta_i, \lambda_i) . S_i \}_{i \in I}
            \leq
            \{ \square_j m'_j(\delta'_j, \lambda'_j) . S_j \}_{j \in J}
            }
            {\begin{array}{c}
                 \forall i \in I, j \in J \; . \; \square_i = \square_j \rightarrow
                 d_{i, j} \vdash \square_i m_i (\delta_i, \lambda_i) . S_i \leq \square_j m'_j (\delta'_j, \lambda'_j) . S_j \\
                 d =
                 (\wedge_{i \in I \downarrow !} \vee_{j \in J \downarrow !} d_{i, j})
                 \wedge
                 (\wedge_{j \in J \downarrow ?} \vee_{i \in I \downarrow !} d_{i, j})
             \end{array}
            }
        \end{array}
    \]
    \caption{Subtyping rules}
\end{figure}

\begin{example}\label{exam-snd}
    Consider $S_i = ! t(\delta_i, \lambda_i) . \myend$
    where
    \[
        \delta_1 = (2 \leq x) \wedge (x \leq 4)
        \qquad
        \delta_2 = (3 \leq x) \wedge (x \leq 5)
        \qquad
        \lambda_1 = \lambda_2 = \emptyset
    \]
    Then $d \wedge true[\emptyset /0] \wedge true[\emptyset / 0] =
        d \vdash S_1 \leq S_2$ where
    \[
        \begin{array}{rcl}
            d & = & \delta_1 \rightarrow \delta_2                                        \\
              & = & \neg (2 \leq x) \vee \neg (x \leq 4) \vee (3 \leq x \wedge x \leq 5) \\
              & = & (x < 2) \vee (4 < x) \vee (3 \leq x \wedge x \leq 5)                 \\
              & = & (x < 2) \vee (3 \leq x)
        \end{array}
    \]
    Observe
    $d \wedge \delta_1 = (3 \leq x \wedge x \leq 4) \models \delta_2$
    hence
    $d \wedge \delta_1 \models d \wedge \delta_2$.  Note that hand-cranking the algorithm at the back gives the above simplification.  But maybe it could also give $(x < 2) \vee (4 < x) \vee (3 \leq x)$ depending on selection of the truth assignment.
\end{example}

\begin{example}\label{exam-rcv}
    Now consider $S_i = ? t(\delta_i, \lambda_i) . \myend$
    where
    \[
        \delta_1 = (2 \leq x \wedge 2 \leq y)
        \qquad
        \delta_2 = (3 \leq x \wedge 1 \leq y)
        \qquad
        \lambda_1 = \lambda_2 = \emptyset
    \]
    Then $d' \wedge true[\emptyset /0] \wedge true[\emptyset / 0] =
        d' \vdash S_1 \leq S_2$ where
    \[
        \begin{array}{rcl}
            d' & = & \delta_2 \rightarrow \delta_1                      \\
               & = & (\neg \delta_2) \vee \delta_1                      \\
               & = & (x < 3 \vee y < 1) \vee (2 \leq x \wedge 2 \leq y) \\
               & = & \ldots                                             \\
               & = & 2 \leq y
        \end{array}
    \]
    Observe
    $d' \wedge \delta_2 = (3 \leq x \wedge 2 \leq y) \models \delta_1$
    hence $d' \wedge \delta_2 \models d' \wedge \delta_1$.
\end{example}

\begin{example}
    Now suppose $\square = \; !$ and
    $\lambda_1 = \lambda_2 = \{ x \}$.
    Then $true[\{ x \} /0]$ = $true$,
    hence $\lambda_i$ has no impact when
    $S_1 \leq S_2$ holds. Likewise for $\square = \; ?$.
\end{example}

\begin{example}
    Continuing with example~\ref{exam-snd}, now consider
    $S'_i = ! t'(\delta'_i, \lambda'_i) . S_i$ where
    \[
        \delta'_1 = (2 \leq x)
        \qquad
        \delta'_2 = (x \leq 1)
        \qquad
        \lambda'_1 = \lambda'_2 = \{ x \}
    \]
    Then
    \[
        \begin{array}{rcl}
            d' & = & \delta_1 \rightarrow \delta_2 \\
               & = & (\neg \delta_1) \vee \delta_2 \\
               & = & (x < 2) \vee (x \leq 1)       \\
               & = & (x \leq 1)
        \end{array}
        \qquad
        \begin{array}{rcl}
            d' \wedge d[\{ x \} / 0] \wedge d[\{ x \} / 0] & = & d' \wedge d[\{ x \} / 0]            \\
                                                           & = & d' \wedge ((0 < 2) \vee (3 \leq 0)) \\
                                                           & = & d' \wedge (true \vee false) =       \\
                                                           & = & d'
        \end{array}
    \]
    thus $d' \vdash S'_1 \leq S'_2$.
\end{example}

\begin{example}
    Developing the examples further, now suppose
    $\lambda'_1 = \lambda'_2 = \emptyset$.
    Then
    \[
        \begin{array}{rcl}
            d' \wedge d[\emptyset / 0] \wedge d[\emptyset / 0] & = & d' \wedge d[\emptyset / 0]              \\
                                                               & = & (x \leq 1) \wedge (x < 2 \vee 3 \leq x) \\
                                                               & = & (x \leq 1)
        \end{array}
    \]
    thus again $d' \vdash S'_1 \leq S'_2$.
\end{example}

\begin{example} Consider
    \[
        \begin{array}{rcllll}
            S                                & = & \{ !t(\delta_1, \emptyset) . \myend,  &
            !t(\delta_2, \emptyset). \myend, &
            !t(\delta_3, \emptyset). \myend \}
            \\
            S'                               & = & \{ !t(\delta'_1, \emptyset) . \myend, &
            !t(\delta'_2, \emptyset). \myend \}
        \end{array}
    \]
    where
    %\[
    %\begin{array}{rrr}
    %\delta_1 = (x \leq 1) & \delta_2 = (x \leq 1) \\ 
    %\delta'_1 = (x \leq 1) & \delta'_2 = (x \leq 1) & \delta_1 = (x \leq 1) & \delta_2 = (x \leq 1) \\
    %\]
\end{example}

\begin{proposition}[soundness]\label{prop-soundness}
Suppose $vars(S_1) \subseteq vars(\vec{x})$,
$vars(S_2) \subseteq vars(\vec{y})$ and $vars(\vec{x}) \cap vars(\vec{y}) = \emptyset$.
%Suppose $vars(S_1) \cap vars(S_2) = \emptyset$. 
The relation
\[
{\cal R}^{*} = \{  ((\nu \downarrow \vec{x}, S_1), (\nu \downarrow \vec{y}, S_2)) \mid d \vdash S_1 \leq S_2 \wedge 
\nu \in \llbracket d \rrbracket 
\}
\]
is a timed type simulation.
\end{proposition}


\begin{proof}[for proposition~\ref{prop-soundness}]
Let $((\nu \downarrow \vec{x}, S_1), (\nu \downarrow \vec{y}, S_2)) \in {\cal R}^{*}$.
\begin{itemize}

\item
Suppose $S_1 = \myend$.  Then $S_2 = \myend$ as required.

\item 
Suppose $(\nu \downarrow \vec{x}, S_1) \xrightarrow{t!m_1} (\nu_1, S'_1)$.
Put $\mu = \nu + t$.
Then 
$\mu \in \llbracket d \rrbracket$
where $d \vdash S_1 \leq S_2$.

Then $(\mu \downarrow \vec{x}, S_1) \xrightarrow{!m_1} ((\mu \downarrow \vec{x})[\lambda_1 \mapsto 0], S'_1)$
where $S_1 = !m_1(\delta_1, \lambda_1).S'_1$
and
$\mu \downarrow \vec{x} \in \llbracket \delta_1 \rrbracket$.

Since $d \vdash S_1 \leq S_2$ it follows
$S_2 = !m_2(\delta_2, \lambda_2).S'_2$
where $m_2 \sqsubseteq m_1$.

Furthermore $d = (\delta_1 \multimap \delta_2) \wedge d'[\lambda_1 \cup \lambda_2 / 0]$
where $d' \vdash S'_1 \leq S'_2$.

Since $vars(\delta_1) \subseteq vars(\vec{x})$
it follows $\mu \in \llbracket \delta_1 \rrbracket$.

Moreover, $d \models \delta_1 \multimap \delta_2 \models \delta_1 \rightarrow \delta_2$
hence $\mu \in \llbracket \delta_1 \wedge (\delta_1 \rightarrow \delta_2) \rrbracket$
whence $\mu \in \llbracket \delta_2 \rrbracket$
and $\mu \downarrow \vec{y} \in \llbracket \delta_2 \rrbracket$
because $vars(\delta_2) \subseteq vars(\vec{y})$.

Therefore $(\mu \downarrow \vec{y}, S_2) \xrightarrow{m_2} ((\mu \downarrow \vec{y})[\lambda_2 \mapsto 0], S'_2)$.

Put $\theta = \mu[\lambda_1 \cup \lambda_2 \mapsto 0]$
and observe
$\theta \downarrow \vec{x} = (\mu \downarrow \vec{x})[\lambda_1 \mapsto 0]$
and
$\theta \downarrow \vec{y} = (\mu \downarrow \vec{y})[\lambda_2 \mapsto 0]$.

Since $d \models d'[\lambda_1 \cup \lambda_2/0]$ it follows
$\mu \in \llbracket d'[\lambda_1 \cup \lambda_2/0] \rrbracket$
hence $\theta \in \llbracket d' \rrbracket$.

Therefore
$((\theta \downarrow \vec{x}, S'_1), (\theta \downarrow \vec{y}, S'_2)) \in {\cal R}^{*}$ as required.

\item 
Suppose $(\nu \downarrow \vec{x}, S_1) \xrightarrow{t?m_1} (\nu_1, S'_1)$.
Analogous to the previous case.
\end{itemize}
\end{proof}

Note that ${\cal R} = \emptyset$ is a timed type simulation.

\newpage

\begin{proposition}[completeness]\label{prop-completeness}
${\cal R}^{*}$ is the greatest timed type simulation.
\end{proposition}

\begin{proof}[for proposition~\ref{prop-completeness}]
Let ${\cal R}$ be a timed type simulation
and $((\nu_1, S_1), (\nu_2, S_2)) \in {\cal R}$.
\begin{itemize}

\item Suppose $S_1 = \myend$. Then $S_2 = \myend$
hence $true \vdash S_1 \leq S_2$.

Put $\nu = \lambda v . \nu_1(v)$ else $\nu_2(v)$ 
so that $\nu_1 = \nu \downarrow \vec{x}$,
$\nu_2 = \nu \downarrow \vec{y}$.
Since $\nu \in \llbracket true \rrbracket$ it follows
$((\nu_1, S_1), (\nu_2, S_2)) \in {\cal R}^{*}$ as required.

\item Suppose $(\nu_1, S_1) \xrightarrow{t!m_1} (\nu'_1, S'_1)$.
Then $(\nu_2, S_2) \xrightarrow{t!m_2} (\nu'_2, S'_2)$ and moreover
$((\nu'_1, S'_1), (\nu'_2, S'_2)) \in {\cal R}$.

Put $\nu = \lambda v . \nu_1(v)$ else $\nu_2(v)$ and $\mu = \nu + t$.

It follows that 
$S_1 = !m_1(\delta_1, \lambda_1) . S'_1$
and
$S_2 = !m_2(\delta_2, \lambda_2) . S'_2$
where
$\mu \downarrow \vec{x} \in \llbracket \delta_1 \rrbracket$
and
$\mu \downarrow \vec{y} \in \llbracket \delta_2 \rrbracket$.

Now suppose $((\nu_1, S_1), (\nu_2, S_2)) \in {\cal R}^{*}$.

Then $\nu + t' \in \llbracket d \rrbracket$
for some $t' \geq 0$
where $d = (\delta_1 \multimap \delta_2) \wedge d'[\lambda_1 \cup \lambda_2 / 0]$
and $d' \vdash S'_1 \leq S'_2$.

Since $\delta_1 \wedge \delta_2 \wedge diagonal \models \delta_1 \multimap \delta_2$ it follows $\mu \in \llbracket
\delta_1 \multimap \delta_2 \rrbracket$.

To show $\mu \in \llbracket d \rrbracket$.

Since $d \models d'[\lambda_1 \cup \lambda_2 / 0]$
it follows $\mu \in \llbracket d'[\lambda_1 \cup \lambda_2 / 0] \rrbracket$.

Therefore $\nu' = \mu[\lambda_1 \cup \lambda_2 \mapsto 0] \in \llbracket d' \rrbracket$.
It follows that $((\nu'_1, S'_1), (\nu'_2, S'_2)) \in {\cal R}^{*}$ as required.
    
\item Analogous to the previous case.

\end{itemize}
It follows ${\cal R} \subseteq {\cal R}^{*}$.
\end{proof}

Conspicuous by its absence is any [\text{rec}] rule but it is not clear how the timing constraints can generate an infinite decending chain of constraints.



==> tex/main/intro/contribution.tex <==

\endinput

This work builds directly on~\cite{Bocchi2019} and provides a new typing system that allows \emph{mixed-choice} to be described by types, and therefore enabling processes to perform timeouts.
These new types are proven to be exhibit progress (deadlock freedom), and the extension to the process calculus is proven to fully reduce.


==> tex/main/intro/existing_work.tex <==

\subsection{Session Types \& Mixed-Choices}
While mixed-choice have been successfully introduced in the synchronous scenario~\cite{Vasconcelos2020}, asynchronous mixed-choice have largely remained partially, if not wholly disallowed by most definitions.
%
The work of~\cite{Denielou2012a} is able to model a subset of mixed-choice which allow the ordering of messages to be interleaved, when communication is not half-duplex, by \emph{forking} a process into various subprocesses which may perform their actions independently before \emph{joining} together and continuing as one process.
%
In work adjacent to session types~\cite{Berger2007}, timers have been used timers to model mixed-choice, by allowing a silent internal transition to another state after a certain amount of time.
%
Other approaches to modelling mixed-choice are often similar, requiring a silent transition between internal states without mixed-choice.


==> tex/main/intro/motivation.tex <==

\subsection{Impact \& Applications}
While session types provide a means of designing a system guaranteed to enjoy progress via tools such as Scribble~\cite{Scribble,Yoshida2013}, or assisting with code generation~\cite{Neykova2013,Neykova2018,Miu2020}, they also have been shown to be an effective means of verifying the behaviour of existing systems~\cite{Neykova2013a,Lange2019}, and even generating runtime monitors~\cite{Neykova2014a}.



Large scale concurrent systems that consist of smaller systems communicating asynchronously with each other, such as web and cloud-services, often depend on runtime monitors for their reliability.
%
Unintended behaviour, such as deadlocks, becomes inevitable at such scales~\cite{Huang2017}\TODO[reread this paper~\cite{Huang2017}].
Such systems commonly follow the \emph{let is crash model}, where crashed nodes are simply restarted once detected (with any nodes dependant on the now restarted node often restarted too).
%
Session types have been used to improve this method~\cite{Neykova2017}, by automatically recovering all of the states that the crashed node depends on, and is a dependency of, to an earlier point in the process.
%
This method uses session types to ensure that the recovered process is sound, able to continue from a point before the error occurred.
%
However, methods such as these can only provide a benefit to those systems which can be modelled by session types.



However, reliability is still not guaranteed, and deadlocks can still occur in systems that utilise these techniques.
%
\emph{Gray failures} are instances where a system is unable to recover due to the failure of its monitors, or their detectors.
%
Gray failures appear to resist detection, and are often unrecoverable due to being detected far too late, requiring a total system restart.
%
Such large systems cannot be verified, and fall outside the scope of decidable \CFSM, and therefore are currently unable to be completely modelled by session types.
%
By expanding session types to include mixed-choice, a greater range of asynchronous communicating systems will be able to benefit from the guaranteed progress session types provide.



\endinput



A system that \emph{enjoys progress} describes a system free from deadlocks.
%
A system that is not in deadlock is called \emph{live}, and has either terminated successfuly or may still peform an action.
%
System compatibility specifies that for every sending action, there exists a corresponding receiving action (and vice versa).
%
Communication safety requires freefom from orphaned messages and unspecified receptions.
%
Together, \emph{liveness}, \emph{compatibility} and \emph{communication safety} have been proven to guarantee progress~\cite{Honda2008,Denielou2012a}.





\TODO[SMTP, producer/consumer, ring protocol (message throttling)]

% ~ examples

\paragraph*{Simple Mail Transfer Protocol}
The Internet Standards specify in {RFC 5321}~{\cite[Section~4.5.3.2]{RFC5321}}:
\begin{quote}
    An \SMTP\ client MUST provide a timeout mechanism
\end{quote}
and proceed to detail various cases and their minimum required timeout duration for each (ranging from 2 to 10 minutes).

\paragraph*{Producers \& Consumers} (shown in~\cref{par:example_producer_consumer})
As in~\cite{Vasconcelos2020}

\paragraph*{Message Throttling} (shown in~\cref{par:example_message_throttling})
Referred to as \emph{ring protocol} in~\cite{Lagaillardie2022}






==> tex/main/processes/subject_reduction.tex <==

In this section we discuss the properties of our typing system, most importantly \emph{time safety}, building on the usual property of subject reduction. 

Time safety without mixed choices in Timed Session Types~\cite{Bocchi2019} relies on a property called receive-liveness. Receive-liveness is defined on untimed counterpart of a timed process $P$, obtained by removing all timing aspect from $P$. Intuitively, receive-liveness ensures that if a process is waiting to receive a message, the other (parallel) processes will provide with that message. This property, on the untimed counterpart of the processes in~\cite{Bocchi2019} can be checked with the techniques for global progress in~\cite{Bettini2008} that can prevent deadlocks due to circular dependencies in interleaved sessions. 
%
It might seem that receive-liveness is an unusually strong requirements for error-freedom, compared with untimed formulation of session types which use it only to prove progress. We argue that, when considering time and punctuality, the distinction between progress and safety is not clear-cut, since deadlocks may cause violation of time constraints. 

Unfortunately, since out processes feature mixed choice, techniques similar to the ones in~\cite{Bettini2008} are not available to us. We rely on a simplifying assumption that each process in a system is \emph{single session}, namely that it implements a single session at a time. This constraint was introduced in~\cite{Honda2008} in the context of Multiparty Session Types. 


%

%
%This provides the guarantee that a process that is both \emph{well-typed} and \emph{live} was also free from circular dependencies of interleaved sessions.

%We are unable to define \emph{untimed processes}, due to the unique structuring of our \texttt{receive\text{-}after} process, and therefore unable to follow the approach of~\cite{Bocchi2019}.
%, and therefore take a different approach when defining \emph{receive liveness}.
%
%Instead, we define receive liveness over tuples ${(\RedTimers,~P)}$ and utilise skip reductions (defined below) to filter out any immediate delays such that a process can reduce instantly.
%We apply this to the non-waiting process in a waiting binary session such that some reduction can be made instantly to provide the message being waited upon, which is analogous to the underlying mechanism for receive liveness in~\cite{Bocchi2019}.
%
%We define $\mathtt{skip}(P)=\mathtt{skip}(P')$ if $P=\mathtt{delay}(t).P'$ else $P$.
%
%We define ${(\RedTimers,~P)}~{{\ARed}_{\scriptstyle \mathtt{skip}}}~{(\RedTimers',~P')}$ which is equivalent to ${(\RedTimers,~\mathtt{skip}(P))}~{\ARed}~{(\RedTimers',~P')}$.
%
% Receive liveness is defined as follows:
%
%\begin{definition}[Receive Liveness]\label{def:receive_liveness}
    %
%    ${(\RedTimers,~P)}$ is said to be \emph{live} if for all $\RedTimers',P'$ such that ${(\RedTimers,~P)}~{\PrcRed}^{*}~{(\RedTimers',~P')}:
    %
    % \begin{minieq}*
        %
        % \begin{array}[t]{l}
 %       {P'}\equiv%
  %      {(\nu pq){(\Parl{P'',Q})}}%
   %     ~\land~%
    %    {p\in\PFuncWait[P'']}%
     %   ~\implies~%
        %
        % \\[0.5ex]\qquad\qquad\qquad%
      %  \exists {\RedTimers}',{Q'}:%
       % {(\RedTimers,~Q)}~{{\ARed}_{\mathtt{skip}}^{*}}~{(\RedTimers',~Q')}%
        % \\[0.5ex]\qquad\qquad\qquad\qquad\qquad\qquad%
        %~\land~%
        %{p\in\PFuncNEQ[{(\nu pq){(\Parl{P'',Q'})}}]}%
        %
        % \end{array}
        %
    $.% \end{minieq}
    %
%\end{definition}
%
%A process is said to be \emph{live} if a non-waiting sub-process %can provide another that is waiting with a suitable message by %only making instant reductions.

Subject reduction,~\cref{thm:subject_reduction}, proves if a process \emph{well-typed} and \emph{single-session}, then any reduction of that process is also \emph{well-typed}.
%
Time safety,~\cref{thm:time_safety}, builds upon Subject Reduction, specifying that any reduction reached by a well-typed process is not the \PrcErr*\ process; that all reductions are \emph{error-free}.



\input{tex/proofs/reduction/thm.tex}

%\subsubsection*{Time Safety}
Building upon the proof of subject reduction,~\cref{thm:time_safety} states that for a \emph{well-typed} process that is \emph{single-session}, any reduction is \emph{error-free}.

\begin{theorem}[Time-Safety]\label{thm:time_safety}
    %
    If ${\Prc}$ is \emph{single-session}
    and $\emptyset~\Entails~\Prc~\PrcTyped~\emptyset$
    and \Trans*{\Prc}*[\Prc'],
    then \Prc*'\ is \emph{error-free}.
    %
\end{theorem}




\endinput
We follow the approach in~\cite{Bocchi2019}. First we define \emph{untimed processes} (by erasing all time-related information) and define an assumption on the interaction structures, called \emph{receive liveness}~\cref{def:receive_liveness}, which is easily attainable by existing techniques and simplifies our theory.  
%
%Receive liveness is restricted to processes at the outer scope of a binary session.
A process is said to be \emph{live} if their \emph{untimed} counterpart can provide any process waiting to receive with a suitable message in the queue. 
%
Subject Reduction,~\cref{thm:subject_reduction}, proves if a process \emph{well-typed}, and its untimed counterpart is \emph{live}, then any reduction of that process is also \emph{well-typed}.
% Formally given in~\cref{thm:subject_reduction}.
%
Time Safety,~\cref{thm:time_safety}, builds upon Subject Reduction, specifying that any reduction reached by a well-typed process is not the \PrcErr*\ process; that all reductions are \emph{error-free}.

% Formally given in~\cref{thm:time_safety}.
%
%Following~\cite{Bocchi2019,Honda2008,Bettini2008,Bocchi2014}, cyclic dependencies of interleaved sessions in malformed processes are not checked by our typing system.

%\subsubsection*{Untimed Calculus}
%Following~\cite{Bocchi2019}, 
We define the untimed calculus by \emph{erasing} any error, delays or timing constraints in a process.
%
Given a timed process \Prc*\ we its untimed counterpart $\hat{\Prc}$ is obtained from $\mathtt{erase}(P)$.
%
Naturally, an untimed process can only reduce instantaneously, and not via any \emph{time-consuming} reductions.

\begin{definition}[Receive Liveness]%\label{def:receive_liveness}
    %
    $\hat{\Prc}$ is said to be \emph{live} if for all $\hat{\Prc'}$ such that $\Trans{\hat{\Prc}}*[\hat{\Prc'}]:
    %
    % \begin{minieq}*
        %
        \hat{\Prc}%
        \equiv%
        {(\nu pq)\hat{\Qrc}}%
        ~\land~%
        {p\in\PFuncWait[\hat{\Qrc}]}%
        \implies%
        {\exists {\hat{\Qrc'}}:%
        \Trans{\hat{\Qrc}}*[\hat{\Qrc'}]%
        ~\land~%
        {p\in\PFuncNEQ[\hat{\Qrc'}]}%
        }%
        %
    $.% \end{minieq}
    %
\end{definition}

\input{tex/proofs/reduction/thm.tex}

\subsubsection*{Time Safety}
Building upon the proof of subject reduction,~\cref{thm:time_safety} states that for a \emph{well-typed} process that is \emph{live}, any reduction is \emph{error-free}.

\begin{theorem}\label{thm:time_safety}
    %
    If $\hat{\Prc}$ is \emph{live}
    and $\emptyset~\Entails~\Prc~\PrcTyped~\emptyset$
    and \Trans*{\Prc}*[\Prc'],
    then \Prc*'\ is \emph{error-free}.
    %
\end{theorem}



==> tex/main/processes/time_passing.tex <==

The time passing function \PFuncTime*\ is defined in~\cref{fig:prc_func_time} for each valid case of \Prc*\ and is undefined for any other.
%
%
\input{tex/figs/processes/func/time_passing.tex}

The auxiliary functions that \PFuncTime*\ depend on are largely unchanged from~\cite{Bocchi2019} and can be found in~\cref{fig:prc_func_wait,fig:prc_func_neq}.
Together they are used to ensure that time does not pass while a process is waiting to receive a message already in their queue.
% The function \PFuncWait*\ recursively unfolds processes until returning either
% \begin{inline}+
%     %
%     \item a message \PrcMsg*\ that is waiting to be received within the given \ValTime*\ specified by the outer \PFuncTime*\ call
%     %
%     \item the emptyset, signifying no messages are waiting to be received within the given time frame
%     %
% \end{inline}
% In short, \PFuncWait*\ returning something other than the empty set indicates that there exists a process currently trying to receive a message from the returned channel.
% The function \PFuncNEQ*\ is similar returning either the empty set or a non-empty channel buffer.
%
% Together, as used in~\cref{fig:prc_func_time} for the passing time over parallel processes, the intersection of two distinct processes yielding nothing indicates that there does not exist a message in a buffer that is able to be received by a process.


==> tex/main/processes/typing_env.tex <==

Processes are validated against types using judgements of the form: $\VarEnv~\Entails~{P}~\PrcTyped~\SesEnv$
% using the environments as defined in~\Cref{eq:prc_typ_env}.
%
% \input{tex/figs/processes/typing.tex}
\begin{minieq}*%\label{eq:prc_typ_env}
    \begin{array}[t]{lcl p{8ex} lcl}
        %
        \VarEnv & ::= & \mathrlap{\emptyset%
        ~\mid~{\VarEnv,~{\pl:T}}
        ~\mid~{\VarEnv,~{x:n}}
        ~\mid~{\VarEnv,~{\RecVar:{(\RecPrcMsg;\RecPrcTimers;\SesSet)}}}}
        %
        \\[-1ex]\\
        \SesEnv & ::= & \emptyset%
        ~\mid~{\SesEnv,~{p:\CIso}}
        ~\mid~{\SesEnv,~{pq:\Queue}}
        %
        & & %
        \SesSet & ::= & \emptyset%
        ~\mid~{\SesSet\cup\left\{\SesEnv\right\}}
        %
    \end{array}
\end{minieq}
%
\emph{Session Environments} \SesEnv* map roles \PrcP*\ to configurations and session endpoints $\PrcQ\PrcP$ to queues \Queue*.
%
\emph{Variable Environments} \VarEnv* map values $\pl$ to data types \DataType*, process timers $x$ to values $n$, and process variables \RecVar*\ to triples \EnvPrcVar*, where
\begin{inline}+
    \item \RecPrcMsg*\ is a vector of messages (consisting of labels and data types)
    \item \RecPrcTimers*\ is a vector of process timers valuations
    \item \SesSet*\ is a set of session environments used for typing recursive processes
\end{inline}
With respect to usual formulations of session types, we use the mapping of timers as a virtual state to correctly type check time-sensitive conditional statements.  

\subsubsection*{Auxiliary definitions \& notation}
%The following definitions are largely unchanged from~\cite{Bocchi2019}.
%We only include those relevant to this work, while definitions such as ``disjoint union of clocks'' still carry over but are omitted for brevity.
%\marginpar{I've tried to only include the bits important for this work/proof without plagiarising Laura. There isn't anything new to add. --Jonah}
%
We write $\mathtt{dom}(\SesEnv)$ for the domain of \SesEnv*, and $\SesEnv_1,\SesEnv_2$ for $\SesEnv_1 \cup \SesEnv_2$ when $\mathtt{dom}(\SesEnv_1)\cap\mathtt{dom}(\SesEnv_2)=\emptyset$.
%
%Given a role $p$, a configuration \CIso*\ and a session environment \SesEnv*, 
We define $\SesEnv(p)=\CIso$ iff $p\in\SesEnv$ and $\exists \SesEnv'$ such that $\SesEnv=\SesEnv',~{p:{\CIso}}$, and define $\mathtt{val}(p)=\ValClocks$ and $\mathtt{type}(p)=\TypeS$.
%
Given a time offset $t\in\RatSet$, we define: 
(1) ${p+t}={({\mathtt{val}(p)+t},~{\mathtt{type}(p)})}$, (2) 
$\SesEnv+t=\{ {p+t} \mid {p\in\mathtt{dom}(\SesEnv)} \}$, (3) $\VarEnv+\ValTime=\{ x+\ValTime \mid x\in\VarEnv\}$. 
%
We say that $\Delta$ is \emph{$t$-reading} iff there exist
$p\in\mathtt{dom}(\Delta)$ and $t'<t$ such that $\Delta+t'(p)$ can make a reading action. 
%
We define $\Gamma [x\mapsto 0]$ similarly to $\RedTimers{}{} [x\mapsto0]$. 

Given a role $p$, $\mathtt{wf}(p)$ holds iff $\exists\delta: \mathtt{val}(p)\models\delta$ and $\emptyset;~\delta~\Entails~\mathtt{type}(p)$.
%
Given a role $p$ and $t\in\RatSet$, we define $\mathtt{AE}(p,t)=\mathtt{true}$ iff $\exists{t'}>t:\mathtt{wf}(p+{t'})$.
% We write $\mathtt{LE}(\mathtt{}p)=$.
%
\endinput
In a given session, a processes performs a single role; roles specify the different actions able to be performed by a process, and are defined by a configuration. Two processes performing different roles exchange data via asynchronous channels, each with a \texttt{FIFO} buffer. The session environment \SesEnv*\ contains all of the information relevant to the ongoing session, accumulating any roles received through delegated sessions.

\paragraph*{Variable Environment (\VarEnv*)}
All of the variables available during the runtime execution of a process is contained within the variable environment \VarEnv*; including:
\begin{inline}+
    \item received messages \PrcMsg*\ against a type \DataType*
    \item set timers \Tix*\ with their known values \Const*
    \item recursive variables, a triple comprised of the following sets
    \begin{inline}*+.{}
        \item \PrcSorts*\ containing all \PrcMsg*\ against types \DataType*
        \item \RecPrcTimers*\ containing all timers \Tix*\ and valuations \Const*
        \item \SesSet*\ containing all session environments \SesEnv*\ possible given that this point is recalled back to via recursion
    \end{inline}
\end{inline}

\paragraph*{Set of Session Environments (\SesSet*)}
Contains all of the possible entry points to a recursive definition, which is necessary for ensuring that all possible instances of a recursive call on a given recursive definition are considered and evaluated.

% \subsection{Notions and Assumptions}
\paragraph*{Session Domains}
\TODO[session domains etc]
% \input{tex/defs/processes/domain_clocks.tex}
%
\input{tex/defs/processes/t_reading.tex}
\begin{note}
    \ValTime*-reading \SesEnv*\ can be denoted by \PSesEnvTRead*, and non-\ValTime*-reading \SesEnv*\ by \PSesEnvTRead*|.
\end{note}


==> tex/main/processes/typing_rule.tex <==

The rules for typing processes are given in~\Cref{fig:prc_typ_rule}.
%
\input{tex/figs/processes/rule_typing.tex}
%
%Rules \begin{inline}/+.
%    \item \LblPrcTypEnd*
%    \item \LblPrcTypEmptQ*
%    \item \LblPrcTypPar*
%    \item \LblPrcTypRes*
%    \item \LblPrcTypWeak*
%    \item \LblPrcTypVQue*
%    \item \LblPrcTypDQue*
%    \item \LblPrcTypDelDelta*
%\end{inline} are unchanged from~\cite{Bocchi2019}.
%
We have highlighted the rules that were changed (orange) or added (green) with respect to~\cite{Bocchi2019}.
%
Terminated processes and empty channel buffers are typed using axioms \LblPrcTypEnd*\ and \LblPrcTypEmptQ*, respectively. Rule \LblPrcTypPar*\ divides the session environment in two, $\Delta_1$ and $\Delta_2$, so that each session is carried by only one of $P$ and $Q$. 
%
Rule \LblPrcTypRes*\ ensures scoped processes are well-typed against binary sessions composed of compatible configurations. Compatibility $\bot$ has been discussed after \Cref{thm:progress}.
%
Non-empty buffers and queues are typed by \LblPrcTypVQue*\ or rule \LblPrcTypDQue*. The former is for payloads containing \emph{base types}, while the latter is for delegated sessions.
%
%
Rule \LblPrcTypTimer*\ adds or resets timer $x$ in \VarEnv*.
%
Rule \LblPrcTypDelDelta*\ checks that $P$ is well-typed against all solutions of \Const*.
%
Rule \LblPrcTypDelTime*\ reflects time passing  on  \VarEnv*\ and the session \SesEnv*. The left-hand side premise enforces \emph{receive urgency} (see rule \LblCfgSocTime*\ in~\Cref{fig:typesemantics}) in processes.

Rule \LblPrcTypBranch*\ is checks that a \texttt{receive\text{-}after} process is well-typed against a choice type.
%
The first line in the premise checks that other ongoing sessions in $\Delta$ allow time passing (i.e., that the process can wait $n$ time units to receive). If this is not the case, rules for checking other sessions should be applied first. The second line in the premise checks that all actions $j$ that are viable in $\nu$: (1) are receiving actions, (2) are viable until the timeout of $n$ expires, (3) have a corresponding branch $i$ can be well-typed against option $j$. In (3) we use an intermediate process (used only for typing) of the form \PCalc*{\On{p}\Recv*<{n}{l}[\pl]:{P}_{i}}\ that allows for modular typing of each single branch via \LblPrcTypVRecv*\ or \LblPrcTypDRecv*.
%
The final line of the premise checks if the type has (send or receive) future-enabled actions in $\nu+n$ and, if so, checks that these are correctly implemented by timeout process $Q$.  
%
Rule \LblPrcTypVRecv*\ is applied when evaluating individual base-type receptions.
The premise ensures a process adheres to the types timing constraints and maps the received message $b$ to \DataType*\ within \VarEnv*, and checks that the continuation process $P$ is well-typed against the continuation type $S$, with any clock resets applied, for the entire duration of $n$.
%
Rule \LblPrcTypDRecv*\ is similar, but for reception of delegated sessions, which is added to the session environment.

Rule \LblPrcTypVSend*\ and \LblPrcTypDSend*\ are for typing processes that send messages against a choice type, by finding a matching pair of labels in the process and type.
%
Rule \LblPrcTypVSend*\ applies for sending base-types, requiring that $v$ is well-typed against \DataType*, and the continuation process $P$ is well-typed against the continuation $S$, with any clock resets applied.
%
Rule \LblPrcTypDSend*\ is similar, but for sending session delegations, and removes role $d$ from the session environment.

Rule \LblPrcTypIfTrue*\ is for typing time-sensitive conditional statements. If the timers in $\Gamma$ satisfy the condition $\delta$, then the evaluation continues with $P$.
%
Likewise, if $\delta$ is not met by the contents of \VarEnv*\ the evaluation continues with $Q$, by rule \LblPrcTypIfFalse*.
%
%In other works where processes cannot branch using time, both $P$ and $Q$ can be typed against the same environment.
%However, by branching depending on values of time, we can encode richer processes more tightly aligned to the types, by ensuring that processes are well-typed against session environments with a certain range of clock valuations.
%


Rules \LblPrcTypRec*\ and \LblPrcTypVar*\ are essentially unchanged from~\cite{Bocchi2019}, only extended to accommodate process timers.
%
Rule \LblPrcTypRec*\ handles recursive definitions by first exploring all of $P$, collecting within the triple $(\RecPrcMsg;\RecPrcTimers;\SesSet)$ all messages, timers and session environments which lead to a recursive corresponding call.
%
This triple containing the ``valid traces'' is mapped to a process variable assigned to $P$, and added to \VarEnv*\ as the evaluation continues with $Q$.
%
Rule \LblPrcTypVar*\ determines if a call is well-typed by checking that the provided messages, timers and channels correspond to those in the process variable.
%
\marginpar{This needs to be reworded. More punch and precision. --Jonah}

\endinput
Rule \LblPrcTypRec*\ handles recursive processes \Prc*\ by first unfolding the remainder of the process before continuing as \Qrc*.
%
During this unfolding \SesSet*\ collects all of the \SesEnv*\ that \Prc*\ and its continuation are typed against until reaching a recursive call \RecPrcCall*.
%
Additionally, both \RecSetMsg*\ and \RecSetTimers*\ are added to the environment \VarEnv*\ to ensure that any recursive calls encountered provide the necessary messages and process timers, as specified by \RecPrcVar*.
%
Rule \LblPrcTypVar*\ handles recursive calls, requiring that it has been defined and that all of the expected messages and clocks are present.
%
\subsubsection{Handling Receptions}
Rule \LblPrcTypBranch*\ first collects all of the viable receiving actions defined by the type in the set $K$, and enforces \emph{receive urgency} by requiring that there are no messages currently waiting to be received.
%
Next, every reception in the type and process are individually matched together to be evaluated and typed by either \LblPrcTypVRecv*\ or \LblPrcTypDRecv*.
%
The \TTPrcAft*\ branch (timeout branch) is evaluated against a session environment and process timers which have been incremented by \PrcAfter*.

\emph{Rule} \LblPrcTypVRecv*\ handles the reception of non-delegation messages. The type must specify that the message can be received for the entire duration of \PrcAfter*.
For every possible reception within \PrcAfter*, the continuation \Prc*\ is typed against the proceeding \TypeS*, with the received message added to \VarEnv*.

\emph{Rule} \LblPrcTypDRecv*\ handles the reception of delegations, and is similar to \LblPrcTypVRecv*, but instead of the received message being added to \VarEnv*, a new role is created within \SesEnv*\ for the received delegation.

\subsubsection{Outgoing Messages}
Rule \LblPrcTypVSend*\ and \LblPrcTypDSend*\ handle outgoing messages.

\endinput
Due to the number of rules, they will be discussed in groups.
\begin{note}
    Message labels \MsgLabel*\ and data-types \DataType*\ are distinguished as pertaining to a \emph{type} or a \emph{process} by writing either
    \begin{inline}|
        \item \MsgLabel*_{\MsgType}\ and \DataType*_{\MsgType}\ to indicate those corresponding to \emph{types}
        \item \MsgLabel*_{\PrcMsg}\ and \DataType*_{\PrcMsg}\ correspond \emph{processes}
    \end{inline}
\end{note}
\input{tex/figs/processes/rule_typing.tex}

\subsubsection{Handing Receptions}\hfill\ \LblPrcTypBranch*\ \par%
The \LblPrcTypBranch*\ rule does not explicitly evaluate that the given process is well-typed against the given type itself.
Instead, a set \mkSet*[k]\ collects all viable receiving actions specified by the type within the time frame \PrcAfter*.
The final condition requires that \SesEnv*\ is not \ValTime*-reading, which ensures that there is not a message already waiting to be received. This is to ensure that all messages are received before the evaluation continues.
The second line of the premise requires that every reception specified by the types within \mkSet*[k]\ has a corresponding reception defined in the process. This is achieved with $\PrcMsg_i=\MsgType_k$ on the second line of the premise. Given that this holds, the evaluation of each pair of process reception and type is passed onto either \LblPrcTypVRecv*\ or \LblPrcTypDRecv*, to be evaluated depending on the message type.

Additionally, in the case that no message is received within \PrcAfter*\ units of time, the final line of the premise for \LblPrcTypBranch*\ initiates the evaluation of the \TTPrcAft*\ branch (timeout branch) against a session environment and process timers which have been incremented by \PrcAfter*.

\paragraph*{Receiving Messages}\hfill\ \LblPrcTypVRecv*\ \par%
The premise ensures that this particular interaction type is not a delegation.
It is required that the message expected by the process \PrcMsg*\ adheres to the data-type specified by the type \DataType*_{\MsgType}.
Continuing, the evaluation of the proceeding process \Prc*\ against the continuation type \TypeS*\ ensues, for each possible time \ValTime*\ permitted within the limit of \PrcAfter*.
For each instance of evaluation, the value of \ValTime*\ is incremented over the timers previously set within the processes, along with the clocks within the session environment \SesEnv*. Any clocks declared to be reset by the type are also enacted within \SesEnv*.

\paragraph*{Receiving Delegations}\hfill\ \LblPrcTypDRecv*\ \par%
Similarly to \LblPrcTypVRecv*\, but conversely the premise requires that the data-type \DataType*_{\MsgType}\ specified by the types is a delegation type \TmpTypBTDelegate*.
Given that this is true, a new role \PrcMsg*\ is added to the session environment \SesEnv*, comprised of a new valuation of clocks that adheres to the constraints specified in the delegation message, and the corresponded delegated session type.

\subsubsection{Ordering Transmissions}\hfill\ \LblPrcTypIfTrue*\ \par%
Given the absence of a \emph{selection} construct in the calculus, outgoing transmissions are deterministic, and it is always known what has been communicated.
Instead, outgoing transmissions are to be structured using the \TTIf*\ structure included in the calculus. The conditions of these \TTIff*\ statements differs from other work by only permitting constraints on timers within the process to be used. This is for simplicity, but should be somewhat straightforward to implement this approach with other work that allows for the traditional approach of using any (non-delegation) data received for conditional control flow of the process.
Similarly to receptions, sending messages are handled separately to sending delegations.
\begin{note}
    Once a given evaluation branch is known to take either the \Prc*\ branch pertaining to a given sending action, any opportunities for reception after this point, given in the type, do not need to be evaluated as it is known this sending action will always occur here.
\end{note}

\paragraph*{Sending Messages}\hfill\ \LblPrcTypVSend*\ \par%
The first line of the premise ensures that there exists a viable sending action which corresponds to the message the process will send. This rule only handles the evaluation of \emph{non-delegating} sending actions.
The second line ensures that the message \PrcMsg*\ is well-typed against \DataType*_{a_{i}}, and initiates the evaluation of the continuation process \Prc*\ being well-typed against the proceeding type \TypeS*.

\paragraph*{Sending Delegations}\hfill\ \LblPrcTypDSend*\ \par%
The first line of the premise is identical to \LblPrcTypVSend*, except that the message being sent \emph{must} be a delegation.
An additional role \PrcMsg*\ must exist within the session environment \SesEnv*, which corresponds to the message to be sent, and that will subsequently be removed from \SesEnv*\ once it has been sent.

\subsubsection{Timers, Delays and Variables}\hfill\ \ \par%

\endinput


==> tex/main/types/mixed_choices.tex <==

Communication safety
%

\endinput

In the asynchronous setting, at a given point of an execution, deciding which choices to take from a set of options is typically achieved by a \emph{selection} and a corresponding \emph{branch}; where one participant decides which option to take, sends it to another participant, which then continues with the corresponding branch.
% \begin{wrapfigure}[16]{r}{0.15\textwidth}\centering%
%     \input{tex/figs/examples/const_mixed_choice.tex}
%     \caption{}
%     \label{fig:example_const_mixed_choice}
% \end{wrapfigure}
A \emph{mixed-choice} is a point in execution where either party has the opportunity to send the next message, deciding the direction of the overall system. 
Mixed-choice are often disallowed from the asynchronous scenario as it can lead to a breakdown of \emph{communication safety}; which namely refers to freedom from
\begin{inline}+
    \item unspecified receptions
    \item orphan messages
    \item deadlocks
\end{inline}; (see~\cite{Denielou2013,Padovani2016}).
For these reasons, it has become standard to only allow one participant to send a message at any time, as this ensures that both parties take the same choices.
mixed-choice allow for either participant to send a message at within the same choice, and due to the "fire and forget" nature of asynchronous communication, each could send their messages before receiving the others message, and not know how to correctly receive it.
This breakdown leads to incompatible states, and ultimately deadlock.

However, Timeout Session Types \emph{allow} for mixed-choice, where either participant can send the next message, by ensuring that only one may do so at any point in time. 
Time can be used to schedule the interactions between participants within the same choice. The scheduling of interactions is achieved using the \emph{logical clocks} local to each participant, which are kept relatively synchronised as the system progresses (this is guaranteed by \emph{duality}. see~\cref{def:types_dual}). This builds on the work of~\cite{Bocchi2019}, which establishes that progress can be guaranteed for systems within the asynchronous setting, by adhering to \emph{communication safety}. 


==> tex/main/types/well_formed_duality.tex <==

%Given a system composed of configurations with dual well-formed types, there is the potential for the system to exhibit \emph{communication safety} and deadlock freedom.
%However, this is not guaranteed just by types being well-formed, but must be ensured by their defined behaviour.

%Naturally, the rules of~\cref{fig:configs_iso_rule,fig:configs_soc_rule,fig:configs_sys_rule} specify that messages must be sent my one party before being received by another.
%Furthermore, sending actions exhibit a \emph{relaxed} notion of urgency, by the premise of \LblCfgSocTime*, which specifies that a value of time may pass, delaying the sending of messages in order to accumulate as many viable actions as possible, so long as no opportunities for sending a message are missed.
%Given that a receiving party is composed of dual types, a message that is delayed will still be successfully received.

%Conversely, receiving actions \emph{must} exhibit urgency, as a message existing in a queue indicates that the sender has already progressed to some later type. Consider the trace of a type in~\cref{eq:example_configs_sys_compatability}.
%\begin{minieq}\label{eq:example_configs_sys_compatability}
%   \TypAct1{\TypSend}2{\mathtt{e}}
%   \TypCond1{\Clx<3}2{\Clx}
%   .
%   \TypAct1{\TypRecv}2{\mathtt{f}}
%   \TypCond1{\Clx=0}2{\emptyset}
%   \dots
%\end{minieq}
%In the instance where the sending of \texttt{e} is delayed until the last possible moment $\Clx=2.9$, any delay of its dual counterpart would result in \texttt{f} being send too late. \TODO[note cite?]
%\begin{note}
 %  In this work latency over a network is not considered, but may be accounted for in implementations.
%\end{note}


\endinput
The notion of \emph{well-formedness}, in the context of session types, is a supplement to valid types. It is not enough that a type is syntactically correct, it is also required that they are practically functional and usable.
In the context of timed session types, well-formedness asserts that the constraints of a valid type are also satisfiable given a specific set of clock valuations \ValClocks*.
Hereafter, all types adhere to~\cref{def:types_well_formed} unless otherwise stated.
\input{tex/defs/types/well_formed.tex}

The notion of \emph{duality} refers to a binary setting where each half of a system is an opposes and complements the other. In the context of communicating systems, for every sending action appearing in one type, there must exist a corresponding receiving type in its \emph{dual}. Building on this notion for session types~\cite{Bernardi2014}, and its extension for timed types~\cite{Bocchi2019}, the duality of timeout session types is defined in~\cref{def:types_dual}.
\input{tex/defs/types/duality.tex}
In the binary setting, it is possible to construct a whole system from only one participant, as it is straightforward to derive its co-party.
In other contexts, such as the multiparty setting, the equivalent of \emph{dual types} would be \emph{co-types}; where every sending action has a corresponding reception, but only between the two participants that participate.



==> tex/proofs/progress/lem/configs_compat_wf_fe.tex <==
%
% ! (lemma 16) : compat wf, end or future enabled
\begin{lemma}\label{lem:configs_compat_wf_fe}
	%
	If both \VIso*_1\ and \VIso*_2\ are \emph{well-formed} 
    and \Compat*[\VSoc_1][\VSoc_2],
	then both \VSoc*_1\ and \VSoc*_2\ are \emph{final} 
	or $\exists\ValTime$ such that \Trans*{\VSys}:{\ValTime,\SiltAction}[\Parl{\VSoc'_1,\VSoc'_2}].%
	%
\end{lemma}
\begin{proof}
	%
	By~\Cref{lem:cfgs_trans_wf_pres} \VIso*'_1\ and \VIso*'_2\ are \emph{well-formed} and by~\Cref{lem:cfg_wf_then_live} are \emph{live}.
	%
	By~\Cref{def:types_progress} if \VSoc*_2\ is \emph{final} then $\VSoc_2=\CSoc[\ValClocks_2];[\TypeEnd]:{\emptyset}$.
    %
    We proceed with the assumption that at least one participant is \emph{not final}, and hereafter only consider \VSoc*'_1.
	%
	The transition is given below:
 %in~\Cref{eq:configs_compat_wf_fe_trans}.
	%
	\begin{minieq}*\label{eq:configs_compat_wf_fe_trans}
		\Trans{\VSys}:{\ValTime}[\Trans{\Parl{\CSoc+{+\ValTime}_1,\CSoc+{+\ValTime}_2}}:{\SiltAction}[\Parl{\CSoc'_1,\CSoc'_2}]]
	\end{minieq}
	%
	We proceed only considering each case of \VSoc*_1\ not being \emph{final}.
	By induction on the cases of \TypeS*_1:
	%
	\begin{inductivecase}
		%
		%
		% ~ choice
		\item\NewCase[$\TypeS=\simplechoice$] 
		% Then by judgement of \LblTypChoice*\ $\exists\Const_i$ such that $\ValClocks\models\Past[\Const_i]$ and $\emptyset;\Past[\Const_i]~\Entails\simplechoice$.
		%
		As described in~\Cref{sec:types} we write $\Past$ if $\exists\ValTime$ such that $\ValClocks+\ValTime\models\Const$.
		Therefore, if $\ValClocks\not\models\Const$ and $\emptyset;\Const~\Entails\TypeS$ for a \emph{well-formed} \CIso*\ then $\ValClocks\models\Past[\Const]$.
		%
		By~\Cref{lem:cfgs_trans_wf_pres} the only possible values of \ValTime*\ ensure that the latest system-wide sending action is never missed and messages are received as soon as they arrive in a queue by rule \LblCfgSocTime*.
		
		Therefore, the hypothesis holds for systems composed where one participant is known to be a \emph{non-final} choice type.
		%
		%
		% ~ rec def
		\item\NewCase[$\TypeS=\mu\alpha.\TypeS'$]
		It follows~\Cref{lem:cfgs_trans_wf_pres} that \TypeS*'\ is \emph{well-formed} against $\ValClocks+\ValTime$.
		%
	\end{inductivecase}
	
	\noindent Therefore, if a \emph{well-formed} and compatible system \Parl*{\VSoc_1,\VSoc_2}\ that is not \emph{final}, then there is some value of time $\ValTime\geq 0$ that will enable a future action, which will result in a \emph{well-formed} and compatible system \Parl*{\VSoc'_1,\VSoc'_2}, which may or may not be \emph{final}, and to which this behaviour still applies.
	%
\end{proof}
% 

==> tex/proofs/progress/lem/configs_iso_trans.tex <==
%
% ! (lemma 12) : iso cfg trans
\begin{lemma}\label{lem:configs_iso_trans}
   %
   The following holds for transitions of configurations:
   \begin{minieq}*
      \begin{array}[c]{c c l}
         %
         \Trans{\CIso}:{\ValTime}[\CIso']%
         & \implies & %
         \begin{array}[c]{lcl}
            %
            \ValClocks'=\ValClocks+\ValTime & %
            \land & %
            \TypeS'=\TypeS%
            %
         \end{array}
         %
         \\[-1ex]\\%
         \Trans{\CIso}:{\CommAction}[\CIso']%
         & \implies & %
         \begin{array}[t]{lcl c lcl c lcl}
            %
            \ValClocks & \models & \Const & %
            \land & %
            \ValClocks' & = & \ReSet[\ValClocks] & %
            \land & %
            \Const' & = & \ReSet[\Const]%
            %
            \\[-1ex]\\%
            \mathllap{\land\;}\ValClocks' & \models & \Const' & %
            \land & %
            \Const' & \subseteq & \TypEnvCond[\TypeS'] %
            %
         \end{array}%
         %
      \end{array}%
   \end{minieq}
   %
\end{lemma}
\begin{proof}
   %
   By inspection of the formation and transition rules in~\Cref{fig:types_rule,fig:typesemantics_tuple}.
   %
\end{proof}
%

==> tex/proofs/progress/lem/configs_soc_trans.tex <==
%
% ! (lemma 11) : soc cfg trans
\begin{lemma}\label{lem:configs_soc_trans}
   %
   The following holds for transitions of configurations with queues:
   \begin{minieq}*
      \begin{array}[c]{c c lcl c lcl c l}
         %
         \Trans{\CSoc}:{\ValTime}[\CSoc']%
         & \implies & %
            %
            \TypeS' & = & \TypeS & \land & %
            \Queue' & = & \Queue & \land & %
            \ValClocks'=\ValClocks+\ValTime%
            %
         \\[1ex]%
         \Trans{\CSoc}:{\RecvMsg}[\CSoc']%
         & \implies & %
            %
            \TypeS' & = & \TypeS & \land & %
            \Queue' & = & \Queue;\Msg & \land & %
            \ValClocks'=\ValClocks
            %
         \\[1ex]%
         \Trans{\CSoc}:{\SendMsg}[\CSoc']%
         & \implies & %
            %
            \MsgType & = & \Msg & \land & %
            \Queue' & = & \Queue & \land & %
            \Trans{\CIso}:{\SendAction}[\CIso'] %
            %
         \\[1ex]%
         \Trans{\CSoc}:{\SiltAction}[\CSoc']%
         & \implies & %
            % 
            \MsgType & = & \Msg & \land & %
            \Queue' & = & \Msg;\Queue & \land & %
            \Trans{\CIso}:{\RecvAction}[\CIso']%
            %
      \end{array}
   \end{minieq}
   %
\end{lemma}
\begin{proof}
   %
   By inspection of the transitions in~\Cref{fig:typesemantics_triple}, supported by~\Cref{lem:configs_iso_trans}.
   %
\end{proof}
%

==> tex/proofs/progress/lem/configs_sys_progress.tex <==
%
% ! (lemma 20) : sys cfg progress
\begin{lemma}\label{lem:configs_sys_progress}
    %
    For all \TypeS*, \ValClocks* such that \ITJudgement*[\emptyset];{\Const}[\TypeS]\ and \Sat*\ :\par\noindent
    \hfill\ \Parl*{\CSoc:{\emptyset},\CSoc;[\Dual]:{\emptyset}}\ satisfies progress.\hfill\ \ %
    %
\end{lemma}
\begin{proof}
    %
    By the hypothesis the system is compatible and composed of well-formed dual types. 
    %
    By~\Cref{lem:configs_trans_compat_wf_pres} any configurations reachable by such a system will be compatible and \emph{well-formed}.
    %
    By~\Cref{lem:configs_compat_wf_fe} such a system adheres to~\Cref{def:types_progress} and \emph{satisfies progress}.
    %
\end{proof}
% 

==> tex/proofs/progress/lem/configs_trans_compat_preserved.tex <==
%
% ! (lemma 15) : compat, single transition -> compat
\begin{lemma}\label{lem:configs_trans_compat_pres}
	%
	If \VIso*_1\ and \VIso*_2\ are both \emph{well-formed} 
    and \Compat*[\VSoc_1][\VSoc_2]\ 
    and \Trans*{\Parl{\VSoc_1,\VSoc_2}}[\Parl{\VSoc'_1,\VSoc'_2}], 
	then \Compat*[\VSoc'_1][\VSoc'_2].
	%
\end{lemma}
\begin{proof}
	%
	We proceed by induction on the depth of the derivation tree, analysing each case of the last rule applied for the transition \Trans*{\Parl{\VSoc_1,\VSoc_2}}[\Parl{\VSoc'_1,\VSoc'_2}]:
	% \begin{inline}+
	% 	\item \LblCfgSysWait*
	% 	\item \LblCfgSysLComm*
	% 	\item \LblCfgSysLPar*
	% \end{inline}
	%
	\begin{inductivecase}
		%
		%
		%
		%
		%
		% ~ wait
		\item\NewCase[\LblCfgSysWait*]\label{case:configs_trans_compat_pres_wait}
		Then both \VSoc*_1\ and \VSoc*_2\ make a \ValTime*\ transition via \LblCfgSocTime*\ as shown in~\Cref{eq:configs_trans_compat_pres_wait_trans}.
		%
        If $\ValTime=0$ then by~\Cref{lem:configs_iso_trans,lem:configs_soc_trans} $\VSoc_1=\VSoc'_1$ and $\VSoc_2=\VSoc'_2$ and the hypothesis holds; \Compat*[\VSoc'_1][\VSoc'_2].
        %
        \begin{minieq}\label{eq:configs_trans_compat_pres_wait_trans}
            \infer[\LblCfgSysWait]{%
                \Trans{\Parl{\VSoc_1,\VSoc_2}}:{\ValTime}[\Parl{\VSoc'_1,\VSoc'_2}]
            }{%
                \infer[\LblCfgSocTime]{%
                    \Trans{\VSoc_1}:{\ValTime}[\VSoc'_1]
                }{\dots}
                & %
                \infer[\LblCfgSocTime]{%
                    \Trans{\VSoc_2}:{\ValTime}[\VSoc'_2]
                }{\dots}
            }
        \end{minieq}
        
        \noindent If $\ValTime>0$ then by~\Cref{lem:configs_iso_trans,lem:configs_soc_trans} $\ValClocks'_1=\ValClocks_1+\ValTime$ and $\TypeS'_1=\TypeS_1$ and $\Queue'_1=\Queue_1$ (and the same for \ValClocks*'_2, \TypeS*'_2\ and \Queue*'_2).
		%
        By~\Cref{lem:cfgs_trans_wf_pres} \VIso*'_1\ and \VIso*'_2\ are both \emph{well-formed}.
		%
		By~\Cref{lem:sys_compat_time_trans} $\Queue_1=\emptyset=\Queue_2$ and by~\Cref{itm:configs_compat_dual_types} of~\Cref{def:configs_compat} $\ValClocks_1=\ValClocks_2$ and $\TypeS_1=\Dual[\TypeS_2]$.
		%
		Therefore \Compat*[\CSoc[\ValClocks_1]+{+\ValTime};[\TypeS_1]:{\emptyset}][\CSoc[\ValClocks_2]+{+\ValTime};[\Dual[\TypeS_2]]:{\emptyset}].
		%
		%
		%
		%
		%
		% ~ comm
		\item\NewCase[\LblCfgSysLComm*]\label{case:configs_trans_compat_pres_comm}
		By~\cref{lem:cfgs_trans_wf_pres} both \VIso*'_1\ and \VIso*'_2\ are \emph{well-formed}.
        The transition is as shown below: %in~\cref{eq:configs_trans_compat_pres_comm_trans}.
		%
		\begin{minieq}*\label{eq:configs_trans_compat_pres_comm_trans}
			% \begin{array}{c}%\mathllap{%
			\resizebox{\linewidth}{!}{$%
				\infer[\LblCfgSysLComm]{%
					\Trans{\Parl{\CSoc[\ValClocks_1];[\TypeS_1]:{\emptyset},\CSoc[\ValClocks_2];[\TypeS_2]:{\Queue_2}}}:{\SiltAction}[\Parl{\CSoc[\ValClocks'_1];[\TypeS'_1]:{\emptyset},\CSoc[\ValClocks_2];[\TypeS_2]:{\Queue_2;\Msg}}]
				}{%
					\infer[\LblCfgSocSend]{%
						\Trans{\CSoc[\ValClocks_1];[\TypeS_1]:{\emptyset}}:{\SendMsg}[\CSoc[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]:{\emptyset}]
					}{%
						\infer[\LblCfgIsoInteract]{%
							\Trans{\CIso[\ValClocks_1];[\TypInteract]}:{\SendMsg}[\CIso[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]]
						}{%
                        \ValClocks_1\models\Const_j
                        & %
                        {m}={l_j\left\langle T_j \right\rangle}
                        & % 
                        {\TypSend=\TypComm_j}
                        & % 
                        j\in I
						}
					}
					& %
					% \infer[\LblCfgSocEnqu]{%
						\Trans{\VSoc_2}:{\RecvMsg}[\CSoc[\ValClocks_2];[\TypeS_2]:{\Queue_2;\Msg}]
						\quad \LblCfgSocEnqu
					% }{\dots}
				}
			$}%
	%	}\end{array}
		\end{minieq}
		
        \noindent We proceed by inner induction on each combination of the contents of queues:
		\begin{inductivecase}
			%
			%
			% ~ comm -> e e
			\item\NewCase[$\Queue_1=\emptyset$, $\Queue_2=\emptyset$]\label{case:configs_trans_compat_pres_comm_ee}
			By~\Cref{itm:configs_compat_dual_types} of~\Cref{def:configs_compat} $\ValClocks_1=\ValClocks_2$ and $\TypeS_1=\Dual[\TypeS_2]$.
			%
			The resulting system is no longer \emph{dual}.
			%
			By~\cref{lem:cfgs_trans_wf_pres,lem:sys_compat_time_trans} time cannot pass if $\Queue_2\neq\emptyset$.
			%
			By~\Cref{def:types_dual} the message \Msg*\ sent by \VSoc*_1\ must have a corresponding receiving action in \VSoc*_2\ as in~\Cref{itm:configs_compat_expected_receive} of~\Cref{def:configs_compat}.
			%
			Therefore \Compat*[\CSoc[\ValClocks'_1];[{\TypeS}'_1]:{\emptyset}][\CSoc;+{\Msg}_2].
			%
			%
			%
			% ~ comm -> e m
			\item\NewCase[$\Queue_1=\emptyset$, $\Queue_2\neq\emptyset$]\label{case:configs_trans_compat_pres_comm_en}
			By~\Cref{itm:configs_compat_expected_receive} of~\Cref{def:configs_compat} $\exists\Msg',{\ValClocks}'',{\TypeS}''$ such that $\Queue_2=\Msg';\Queue_2$ and \Trans*{\CIso_2}:{\TypRecv,\Msg'}[\CIso[{\ValClocks}''_2];[{\TypeS}''_2]]\ and \Compat*[\CSoc[\ValClocks'_1];[{\TypeS}'_1]:{\emptyset}][\CSoc[{\ValClocks}''_2];[{\TypeS}''_2]:{{\Queue}_2}]\ and by \LblCfgSocTime*\ (urgency) time cannot pass.
			%
			If a system has a configuration with sequence of outgoing sending actions and each has constraints that are satisfiable immediately after the other, then the system can both receive the messages as they arrive, or accumulate the messages and instantly receive each in succession and become \emph{dual} again (by inspection of~\Cref{def:types_dual,def:configs_compat} and~\Cref{fig:types_rule,fig:typesemantics_tuple,fig:typesemantics_triple}).
			%
			Therefore \Compat*[\CSoc[\ValClocks'_1];[{\TypeS}'_1]:{\emptyset}][\CSoc[{\ValClocks}''_2];[{\TypeS}''_2]:{\Msg';{\Queue}_2;\Msg}].
			%
			%
			% ~ comm -> m e
			\item\NewCase[$\Queue_1\neq\emptyset$, $\Queue_2=\emptyset$]\label{case:configs_trans_compat_pres_comm_ne}
			Contradicts the hypothesis by~\Cref{itm:configs_compat_expected_receive} of~\Cref{def:configs_compat} as by \LblCfgSocTime*\ (urgency) messages must be removed from a queue immediately, and by \LblTypChoice*\ of~\Cref{fig:types_rule} sending and receiving actions cannot be performed at the same time.
			%
			%
			% ~ comm -> m m
			\item\NewCase[$\Queue_1\neq\emptyset$, $\Queue_2\neq\emptyset$]\label{case:configs_trans_compat_pres_comm_nn}
			Contradicts the hypothesis by~\Cref{itm:configs_compat_non_empty_queues} of~\Cref{def:configs_compat}.
			%
		\end{inductivecase}

		\noindent Therefore, compatibility is preserved across \LblCfgSysLComm*\ transitions.
		%
		%
		%
		%
		%
		% ~ dequ
		\item\NewCase[\LblCfgSysLPar*]\label{case:configs_trans_compat_pres_dequ}
		By~\Cref{lem:configs_soc_trans} $\Queue_2=\Msg;\Queue_2$ and by~\Cref{itm:configs_compat_expected_receive} of~\Cref{def:configs_compat} \Compat*[\VSoc'_1][\VSoc'_2], the hypothesis holds.
		%
	\end{inductivecase}

	\noindent Therefore, it holds that any transition made by a compatible system composed of well-formed types will result in configurations that are \emph{compatible}.
	%
\end{proof}
% 

==> tex/proofs/progress/lem/configs_trans_compat_wf_preserved.tex <==
%
% ! (lemma 18) : compat wf, any amount of transitions -> compat wf
\begin{lemma}\label{lem:configs_trans_compat_wf_pres}
    %
    If both \VIso*_1 and \VIso*_2 are \emph{well-formed}
    and \Compat*[\VSoc_1][\VSoc_2]\ 
    and $\Trans{\Parl{\VSoc_1\!,\VSoc_2}}*[\Parl{\VSoc'_1\!,\VSoc'_2}]$, 
    then \Compat*[\VSoc'_1][\VSoc'_2]\ 
    and both \VIso*'_1\ and \VIso*'_2\ are \emph{well-formed}.%
    %
\end{lemma}
\begin{proof}
    %
    By~\Cref{lem:cfgs_trans_wf_pres,lem:configs_trans_compat_pres} the hypothesis holds for single transitions and that the resulting configurations are \emph{live}, and either \emph{final} or \emph{satisfies progress} by~\Cref{lem:cfg_wf_then_live,lem:configs_compat_wf_fe}.
    %
    Therefore it holds that \Compat*[\VSoc'_1][\VSoc'_2]\ 
    and both \VIso*'_1\ and \VIso*'_2\ are \emph{well-formed} across an arbitrary number of transitions, as each single transition preserves compatibility and well-formedness.
    %
\end{proof}
% 

==> tex/proofs/progress/lem/configs_trans_wf_preserved.tex <==
%
% ! (lemma 17) : compat wf, single transition -> wf
\begin{lemma}\label{lem:cfgs_trans_wf_pres}
    %
    If \VIso*_1\ and \VIso*_2\ are both \emph{well-formed} 
    and \Compat*[\VSoc_1][\VSoc_2]\ 
    and \Trans*{\Parl{\VSoc_1,\VSoc_2}}[\Parl{\VSoc'_1,\VSoc'_2}], 
    then both \VIso*'_1\ and \VIso*'_2\ are \emph{well-formed}.
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the depth of the derivation tree, analysing each case of the last rule applied for the transition \Trans*{\Parl{\VSoc_1,\VSoc_2}}[\Parl{\VSoc'_1,\VSoc'_2}].
    % \begin{inline}+
    %     \item \LblCfgSysWait*
    %     \item \LblCfgSysLComm*
    %     \item \LblCfgSysLPar*
    % \end{inline}
    %
    \begin{inductivecase}
        %
        %
        %
        %
        %
        % ~ wait
        \item\NewCase[\LblCfgSysWait*]\label{case:cfgs_trans_wf_pres_wait} 
        As shown in~\Cref{eq:cfgs_trans_wf_pres_wait_trans}, both \VSoc*_1\ and \VSoc*_2\ make a rule \LblCfgSocTime*\ transition with the same valuation of \ValTime*.
        If $\ValTime=0$ then by~\Cref{lem:configs_iso_trans,lem:configs_soc_trans} $\VIso_1=\VIso'_1$ and $\VIso_2=\VIso'_2$ and both \VIso*'_1\ and \VIso*'_2\ are \emph{well-formed}.
        %
        \begin{minieq}\label{eq:cfgs_trans_wf_pres_wait_trans}
        \begin{array}[c]{l}
            \infer[\LblCfgSysWait]{%
                \Trans{\Parl{\VSoc_1,\VSoc_2}}:{\ValTime}[\Parl{\VSoc'_1,\VSoc'_2}]
            }{%
                \infer[\LblCfgSocTime]{%
                    \Trans{\VSoc_1}:{\ValTime}[\VSoc'_1]
                }{\dots}
                & %
                \infer[\LblCfgSocTime]{%
                    \Trans{\VSoc_2}:{\ValTime}[\VSoc'_2]
                }{\dots}
            }
            \end{array}
        \end{minieq}
            
        \noindent We proceed with only \VSoc*_1\ as the analysis covers \VSoc*_2.
        If $\ValTime>0$ then by~\Cref{lem:configs_iso_trans,lem:configs_soc_trans} $\ValClocks'_1=\ValClocks_1+\ValTime$ and $\TypeS'_1=\TypeS_1$.
        %
        By induction on the depth of the derivation tree, analysing the last rule applied for the transition \Trans*{\VIso_1}:{\ValTime}[\VIso'_1]:
        \begin{inductivecase}
            %
            %
            % ~ wait -> tick
            \item\NewCase[\LblCfgIsoTick*]\label{case:cfgs_trans_wf_pres_wait_tgtz_tick} 
            Then \Trans*{\CIso_1}:{\ValTime}[\CIso+{+\ValTime}_1].
            We proceed by inner induction on the different cases of \TypeS*_1:
            \begin{inductivecase}
                %
                % ~ wait -> tick -> choice
                \item\NewCase[$\TypeS_1=\simplechoice$]\label{case:cfgs_trans_wf_pres_wait_tgtz_tick_choice} 
                By rule \LblCfgIsoInteract*\ $\exists\Const_i$ such that $\ValClocks_1\models\Past[\Const_i]$ and $\emptyset;\Past[\Const_i]~\Entails\FullChoice$, as in~\Cref{itm:cfg_wf_then_live_choice} of~\Cref{lem:cfg_wf_then_live}.
                %
                By induction hypothesis $\exists\Const'_i$ such that $\ValClocks_1+\ValTime\models\Past[\Const'_i]$ and $\emptyset;\Past[\Const'_i]~\Entails\FullChoice$, which is assured by the (persistency) premise of rule \LblCfgSocTime*.
                %
                Therefore, it holds that \CIso*[\ValClocks_1]+{+\ValTime};[\simplechoice]\ is \emph{well-formed}.
                % By~\Cref{def:configs_fe} \CIso*_1\ is \emph{future-enabled} and by rule \LblCfgSocTime*\ $\text{(persistency)}$ it holds that \CIso*+{+\ValTime}_1\ is also \emph{future-enabled}.
                % %
                % Therefore the hypothesis holds, \CIso*[\ValClocks_1]+{+\ValTime};[\simplechoice]\ is \emph{well-formed}; by~\Cref{def:types_wf} and rule \LblTypChoice*\ $\exists\Const'_i$ such that $\ValClocks_1+\ValTime\models\Past[\Const'_i]$ and $\emptyset;\Past[\Const'_i]~\Entails\simplechoice$.
                %
                %
                % ~ wait -> tick -> recursion
                \item\NewCase[$\TypeS_1=\mu\alpha.{\TypeS}''_1$]\label{case:cfgs_trans_wf_pres_wait_tgtz_tick_recursion} 
                By~\Cref{def:types_wf} $\exists\Const$ such that $\ValClocks_1\models\Const$ and $\emptyset;\Const~\Entails\mu\alpha.{\TypeS}''_1$, and (by rule \LblTypRec*) $\alpha:\Const;\Const~\Entails{\TypeS}''_1$ and \CIso*[\ValClocks_1];[{\TypeS}''_1]\ is \emph{well-formed}.
                %
                Therefore, the well-formedness of \CIso*[\ValClocks_1]+{+\ValTime};[\mu\alpha.{\TypeS}''_1]\ is dependant on the well-formedness of \CIso*[\ValClocks_1]+{+\ValTime};[{\TypeS}''_1]. (See other cases, as in~\Cref{itm:wf_then_live_recdef} of~\Cref{lem:cfg_wf_then_live}.)
                %
                %
                % ~ wait -> tick -> end
                \item\NewCase[$\TypeS_1=\TypeEnd$]\label{case:cfgs_trans_wf_pres_wait_tgtz_tick_end} 
                By~\Cref{lem:cfg_wf_end} \CIso*+{+\ValTime};[\TypeEnd]\ is \emph{well-formed}.
                %
                %
                % ~ wait -> tick -> rec call
                \item\label{case:cfgs_trans_wf_pres_wait_tgtz_tick_reccal} ${\TypeS}_1$ cannot equal $\alpha$ by~\Cref{lem:cfg_wf_neq_alpha}.
                %
            \end{inductivecase}
            %
            %
            % ~ wait -> unfold
            \item\NewCase[\LblCfgIsoUnfold*]\label{case:cfgs_trans_wf_pres_wait_tgtz_unfold} 
            Then $\TypeS_1=\mu\alpha.{\TypeS}''_1$ and by the hypothesis $\exists\Const$ such that $\ValClocks_1\models\Const$ and $\emptyset;\Const~\Entails\TypRecDef$, and by rule \LblTypRec*\ $\alpha:\Const;\Const~\Entails{\TypeS}''_1$.
            The transition is as shown below:
            %
            \begin{minieq}*%\label{eq:cfgs_trans_wf_pres_wait_tgtz_unfold_trans}
        \begin{array}[c]{l}
                \infer[\LblCfgIsoUnfold]{%
                    \Trans{\CIso[\ValClocks_1];[\mu\alpha.{\TypeS}''_1]}:{\ProgAction}[\CIso'_1]
                }{%
                    \Trans{\CIso[\ValClocks_1];[{\TypeS}''_1\Subst[\mu\alpha.{\TypeS}''_1][\alpha]]}:{\ValTime}[\CIso'_1]
                }
                \end{array}
            \end{minieq}
            
            \noindent By inner induction on the different cases of ${\TypeS}''_1$:
            \begin{inductivecase}
                %
                % ~ wait -> unfold -> choice
                \item\NewCase[${\TypeS}''_1=\simplechoice$]\label{case:cfgs_trans_wf_pres_wait_tgtz_unfold_choice} 
                Then, by rule \LblCfgIsoTick*:
                \[\Trans{\CIso[\ValClocks_1];[{\simplechoice}\Subst[\mu\alpha.{\simplechoice}][\alpha]]}:{\ValTime}[\CIso[\ValClocks_1]+{+\ValTime};[\simplechoice]]\]
                
                \noindent By the rules \LblTypRec*\ and \LblTypChoice*\ the following holds:
                \[
                \infer[\LblTypRec]{%
                \emptyset;\Const_i~\Entails\mu\alpha.{\FullChoice}
                }{%
                \infer[\LblTypChoice]{%
                    \alpha:\Const_i;\Past_i~\Entails\FullChoice
                }{%
                \dots
                }
                }
                \]
                
                % \noindent It holds that \CIso*[\ValClocks_1];[{\simplechoice}\Subst[\mu\alpha.{\simplechoice}][\alpha]]\ is \emph{well-formed} and \emph{future-enabled}.
                %
                \noindent By induction hypothesis: \[\exists\Const'_i:\ValClocks_1+\ValTime\models\Past[\Const'_i] ~\land~ \emptyset;\Past[\Const'_i]~\Entails\FullChoice\] which is assured by the (persistency) premise of rule \LblCfgSocTime*, as in~\Cref{case:cfgs_trans_wf_pres_wait_tgtz_tick_choice} of~\Cref{lem:cfgs_trans_wf_pres}.
% 
                Therefore, \CIso*[\ValClocks_1]+{+\ValTime};[\mu\alpha.{\simplechoice}]\ is \emph{well-formed} as \CIso*[\ValClocks_1]+{+\ValTime};[{\simplechoice}\Subst[\mu\alpha.{\simplechoice}][\alpha]]\ the following is \emph{well-formed}.
                %
                %
                % ~ wait -> unfold -> recursion
                \item\NewCase[${\TypeS}''_1=\mu\alpha'.{\TypeS}'''_1$]\label{case:cfgs_trans_wf_pres_wait_tgtz_unfold_recursion} 
                % By the hypothesis $\exists\Const$ such that $\ValClocks_1\models\Const$ and $\emptyset;\Const~\Entails\mu\alpha.\mu\alpha'.{\TypeS}'''_1$, by the premise of rule \LblTypRec*\ $\alpha:\Const;\Const~\Entails\mu\alpha'.{\TypeS}'''_1$ and $\alpha:\Const,\alpha':\Const;\Const~\Entails{\TypeS}'''_1$, and \CIso*[\ValClocks_1];[{\TypeS}'''_1]\ is \emph{well-formed}.
                % 
                The well-formedness of \CIso*[\ValClocks_1]+{+\ValTime};[\mu\alpha'.{\TypeS}'''_1]\ depends on the well-formedness of \CIso*[\ValClocks_1]+{+\ValTime};[{\TypeS}'''_1]. (See other cases of $S$.) %, as in~\Cref{itm:wf_then_live_recdef} of~\Cref{lem:cfg_wf_then_live}.)
                %
                %
                % ~ wait -> unfold -> end
                \item\NewCase[${\TypeS}''_1=\TypeEnd$]\label{case:cfgs_trans_wf_pres_wait_tgtz_unfold_end} 
                By~\Cref{lem:cfg_wf_end} \CIso*+{+\ValTime};[\TypeEnd]\ is \emph{well-formed}.
                %
                %
                % ~ wait -> unfold -> rec call
                \item\label{case:cfgs_trans_wf_pres_wait_tgtz_unfold_reccall} ${\TypeS}''_1$ cannot equal $\alpha$ by~\Cref{lem:cfg_wf_neq_alpha}.
                %
            \end{inductivecase}
            %
        \end{inductivecase}

        \noindent Therefore, it holds that well-formedness is preserved by transition made by \emph{well-formed} configurations via rule \LblCfgSysWait*.
        %
        %
        %
        %
        %
        % ~ comm
        \item\NewCase[\LblCfgSysLComm*]\label{case:cfgs_trans_wf_pres_comm} 
        % Then by~\cref{case:configs_trans_compat_pres_comm} of~\cref{lem:configs_trans_compat_pres} $\Queue_1=\Queue'_1=\emptyset$.
        The transition is as shown below:
        %
        \begin{minieq}*%\label{eq:cfgs_trans_wf_pres_comm_trans}
        \begin{array}[c]{l}
            \infer[\LblCfgSysLComm]{%
                \Trans{\Parl{\VSoc_1,\VSoc_2}}:{\SiltAction}[\Parl{\VSoc'_1,\VSoc'_2}]
            }{%
                \infer[\LblCfgSocSend]{%
                    \Trans{\VSoc_1}:{\SendMsg}[\VSoc'_1]
                }{\dots}
                & %
                % \infer[\LblCfgSocEnqu]{%
                    \Trans{\VSoc_2}:{\RecvMsg}[\VSoc'_2]
					\quad \LblCfgSocEnqu
                % }{\dots}
            }
            \end{array}
        \end{minieq}
        
        % ~ comm-l s1
        \noindent Focusing first on \VSoc*_1, we proceed by induction on the depth of the derivation tree, analysing the last rule applied for the transition \Trans*{\VIso_1}:{\SendMsg}[\VIso'_1]:
        \begin{inductivecase}
            %
            %
            % ~ comm-l s1 -> act
            \item\NewCase[\LblCfgIsoInteract*]\label{case:cfgs_trans_wf_pres_comm_act} 
            Then $\TypeS_1=\simplechoice$, and the evaluation is shown below:
            %
            \begin{minieq}*\label{eq:cfgs_trans_wf_pres_comm_act_trans}
        \begin{array}[c]{l}
                \infer[\LblCfgSocSend]{%
                    \Trans{\CSoc[\ValClocks_1];[\simplechoice]:{\Queue_1}}:{\SendMsg}[\CSoc[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]:{\Queue_1}]
                }{%
                    \infer[\LblCfgIsoInteract]{%
                        \Trans{\CIso[\ValClocks_1];[\TypInteract]}:{\SendMsg}[\CIso[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]]
                    }{%
                        \ValClocks_1\models\Const_j
                        & %
                        {m}={l_j\left\langle T_j \right\rangle}
                        & % 
                        {\TypSend=\TypComm_j}
                        & % 
                        j\in I
                    }
                }
                \end{array}
            \end{minieq}
            
            \noindent By rule \LblTypChoice*\ $\exists\Const_i:\ValClocks_1\models\Past[\Const_i]$ and $\emptyset;\Past[\Const_i]~\Entails\FullChoice$, and by the premise of rule \LblTypChoice*\ it holds that $\Const_i\ReSet[]_i\subseteq\gamma$ and $\emptyset;\gamma~\Entails\TypeS_i$.
            %
            Combined with~\Cref{lem:configs_iso_trans} it holds that $\ValClocks_1\models\Const_j$ and $\emptyset;\Const_j\ReSet[]_j~\Entails\TypeS_j$ and $\ValClocks_1\ReSet[]_j\models\Const_j\ReSet[]_j$.
            
            Therefore, \CIso*[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]\ is \emph{well-formed}.
            %
            %
            % ~ comm-l s1 -> unfold
            \item\NewCase[\LblCfgIsoUnfold*]\label{case:cfgs_trans_wf_pres_comm_unfold} 
            Then $\TypeS_1=\mu\alpha.{\TypeS}''_1$.
            The transition is as shown below:
            %
            \begin{minieq}*\label{eq:cfgs_trans_wf_pres_comm_unfold_trans}
        \begin{array}[c]{l}
                \infer[\LblCfgIsoUnfold]{%
                    \Trans{\CIso[\ValClocks_1];[\mu\alpha.{\TypeS}''_1]}:{\ProgAction}[\CIso'_1]
                }{%
                    \Trans{\CIso[\ValClocks_1];[{\TypeS}''_1\Subst[\mu\alpha.{\TypeS}''_1][\alpha]]}:{\SendMsg}[\CIso'_1]
                }
                \end{array}
            \end{minieq}
            
            \noindent By the hypothesis $\exists\Const$ such that $\ValClocks_1\models\Const$ and $\emptyset;\Const~\Entails\TypRecDef$, and by the premise of rule \LblTypRec*\ $\alpha:\Const;\Const~\Entails{\TypeS}''_1$, and \CIso*[\ValClocks_1];[{\TypeS}''_1\Subst[\mu\alpha.{\TypeS}''_1][\alpha]]\ is \emph{well-formed}.
            %
            The well-formendess of \CIso*'_1\ is dependant on the state of ${\TypeS}''_1$, which for the transition \Trans*{\CIso[\ValClocks_1];[{\TypeS}''_1\Subst[\mu\alpha.{\TypeS}''_1][\alpha]]}:{\SendMsg}[\CIso'_1]\ must be either $\simplechoice$ or $\mu\alpha'.{\TypeS}'''_1$ (see other cases, as in~\Cref{lem:cfg_wf_then_live}).
            %
        \end{inductivecase}
        %
        % ~ comm-l s1
        Now, focusing on \VSoc*_2, the transition \Trans*{\CSoc_2}:{\RecvMsg}[\CSoc'_2]\ via rule \LblCfgSocEnqu*\ yields $\ValClocks_2'=\ValClocks_2$ and $\TypeS_2'=\TypeS_2$ and $\Queue_2'=\Queue_2;\Msg$ by~\Cref{lem:configs_soc_trans}.
        %
        Therefore \CIso*'_2\ is \emph{well-formed} as $\VIso_2=\VIso'_2$.
        %
        Transitions via rule \LblCfgSysRComm*\ are symmetric and omitted.
        %
        %
        %
        %
        %
        % ~ par-l
        \item\NewCase[\LblCfgSysLPar*]\label{case:cfgs_trans_wf_pres_par} 
        By~\Cref{lem:configs_soc_trans} $\Queue'_1=\Msg;\Queue_1$.
        The transition is as shown below: %in~\Cref{eq:cfgs_trans_wf_pres_par_trans}.
        %
        \begin{minieq}*\label{eq:cfgs_trans_wf_pres_par_trans}
        \begin{array}[c]{l}
            \infer[\LblCfgSysLPar]{%
                \Trans{\Parl{\VSoc_1,\VSoc_2}}:{\SiltAction}[\Parl{\VSoc'_1,\VSoc'_2}]
            }{%
                \infer[\LblCfgSocRecv]{%
                    \Trans{\VSoc_1}:{\SiltAction}[\VSoc'_1]
                }{\dots}
            }
            \end{array}
        \end{minieq}
        
        \noindent We proceed by induction on the depth of the derivation tree, analysing the last rule applied for the transition \Trans*{\VIso_1}:{\RecvMsg}[\VIso'_1]\ via the premise of rule \LblCfgSocRecv*:
        \begin{inductivecase}
            %
            %
            % ~ par-l -> act
            \item\NewCase[\LblCfgIsoInteract*]\label{case:cfgs_trans_wf_pres_par_act} 
            Then $\TypeS_1=\simplechoice$.
            The transition is as shown below: %in~\Cref{eq:cfgs_trans_wf_pres_par_act_trans}.
            %
            \begin{minieq}*\label{eq:cfgs_trans_wf_pres_par_act_trans}
        \begin{array}[c]{l}
                \infer[\LblCfgSocRecv]{%
                    \Trans{\CSoc[\ValClocks_1];[\simplechoice]:{\Msg;\Queue_1}}:{\SiltAction}[\CSoc[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]:{\Queue_1}]
                }{%
                    \infer[\LblCfgIsoInteract]{%
                        \Trans{\CIso[\ValClocks_1];[\TypInteract]}:{\RecvMsg}[\CIso[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]]
                    }{%
                        \ValClocks_1\models\Const_j
                        & %
                        {m}={l_j\left\langle T_j \right\rangle}
                        & % 
                        {\TypRecv=\TypComm_j}
                        & % 
                        j\in I
                    }
                }
                \end{array}
            \end{minieq}
            
            \noindent By the hypothesis and the judgement of rule \LblTypChoice*\ $\exists\Const_i$ such that $\emptyset;\Past[\Const_i]~\Entails\simplechoice$ and $\ValClocks_1\models\Past[\Const_i]$, and by the premise of rule \LblTypChoice*\ $\Const_i\ReSet[]_i\subseteq\gamma$ and $\emptyset;\gamma~\Entails\TypeS_i$.
            
            It follows~\Cref{case:cfgs_trans_wf_pres_comm_act} of~\Cref{lem:cfgs_trans_wf_pres} that \CIso*[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]\ is \emph{well-formed}.
            % Therefore \CIso*[\ValClocks_1]+{\ReSet[]_j};[\TypeS_j]\ is \emph{well-formed} as $\ValClocks_1\models\Const_j$ and $\emptyset;\Const_j\ReSet[]_j~\Entails\TypeS_j$ and $\ValClocks_1\ReSet[]_j\models\Const_j\ReSet[]_j$ (as in~\Cref{case:cfgs_trans_wf_pres_comm_act} of~\Cref{lem:cfgs_trans_wf_pres}).
            %
            %
            % ~ par-l -> unfold
            \item\NewCase[\LblCfgIsoUnfold*]\label{case:cfgs_trans_wf_pres_par_unfold} 
            Then $\TypeS_1=\mu\alpha.{\TypeS}''_1$.
            The transition shown below, and is analogous to the one in~\Cref{eq:cfgs_trans_wf_pres_comm_unfold_trans} of~\Cref{lem:cfgs_trans_wf_pres}:
            % in~\Cref{eq:cfgs_trans_wf_pres_par_unfold_trans} and is analogous to the one in~\Cref{eq:cfgs_trans_wf_pres_comm_unfold_trans}.
            %
            \begin{minieq}\label{eq:cfgs_trans_wf_pres_par_unfold_trans}
        \begin{array}[c]{l}
                \infer[\LblCfgIsoUnfold]{%
                    \Trans{\CIso[\ValClocks_1];[\mu\alpha.{\TypeS}''_1]}:{\ProgAction}[\CIso'_1]
                }{%
                    \Trans{\CIso[\ValClocks_1];[{\TypeS}''_1\Subst[\mu\alpha.{\TypeS}''_1][\alpha]]}:{\RecvMsg}[\CIso'_1]
                }
                \end{array}
            \end{minieq}
            
            \noindent By the hypothesis $\exists\Const$ such that $\ValClocks_1\models\Const$ and $\emptyset;\Const~\Entails\TypRecDef$, and by the premise of rule \LblTypRec*\ $\alpha:\Const;\Const~\Entails{\TypeS}''_1$, and \CIso*[\ValClocks_1];[{\TypeS}''_1\Subst[\mu\alpha.{\TypeS}''_1][\alpha]]\ is \emph{well-formed}.
            %
            The well-formendess of \CIso*'_1\ is dependant on ${\TypeS}''_1$, which for the transition by the premise of rule \LblCfgIsoUnfold*\ must be either $\simplechoice$ or $\mu\alpha'.{\TypeS}'''_1$ (see other cases, as in~\Cref{lem:cfg_wf_then_live}).
            %
        \end{inductivecase}
        %
    \end{inductivecase}

    \noindent Therefore, it holds that any transition made by a system composed of compatible and \emph{well-formed} configurations will result in configurations that are \emph{well-formed}.
    %
\end{proof}
% 

==> tex/proofs/progress/lem/prog_sys.tex <==
\begin{lemma}\label{lem:prog_sys}
   \REDO[The following holds:]
   \begin{equation*}\begin{array}{l}
         \begin{array}{l}
            \forall\mst,\mval:\quad%
            \emptyset;\,\mconstr\imp\mst%
            \quad\land\quad%
            \mval\models\mconstr:%
         \end{array} \\\qquad\qquad%
         \begin{array}{r}
            (\of{\mval}{0},\,\mst,\emptyset)%
            \,\mid\,%
            (\of{\mval}{0},\,\mdual[\mst],\emptyset)%
            \quad\text{satisfies progress (\cref{def:type_progress})}
         \end{array}
      \end{array}
   \end{equation*}
\end{lemma}
\begin{proof}
   Combination of~\cref{lem:prog_trans_iso_wf,lem:prog_trans_soc_compat,lem:prog_trans_compat_wf}.
\end{proof}

==> tex/proofs/progress/lem/prog_trans_compat_wf.tex <==
\begin{lemma}\label{lem:prog_trans_compat_wf}
   Given two participants that are compatible \compconfig{}{1}{}{2}, and, both \isoconfig{1}\ and \isoconfig{2} are \emph{well-formed}:\par
   %
   If \;$\mparconfig{}{1}{}{2} {\transition{}}^{*} \mparconfig{'}{1}{'}{2}$,\par\noindent
   \hspace{7ex}\rule{0pt}{2.5ex} then \compconfig{'}{1}{'}{2},\par\noindent
   \hspace{9ex}\rule{0pt}{2.5ex}and, both \isoconfig[']{1}\ and \isoconfig[']{2} are \emph{well-formed}.
   %
\end{lemma}
\begin{proof}
   \REDO By~\cref{lem:prog_trans_iso_wf,lem:prog_trans_soc_compat}, it is shown that any transition taken by a system composed of a configurations \soc{1}\ and \soc{2}\ running in parallel, preserves the properties of \emph{well-formedness} and \emph{compatibility}.
\end{proof}

==> tex/proofs/progress/lem/prog_trans_iso_wf.tex <==
\begin{lemma}\label{lem:prog_trans_iso_wf}
   Two compatible participants \compconfig{}{1}{}{2}, where \isoconfig{1}\ and \isoconfig{2} are \emph{well-formed}, that take a transition \action:
   \par\noindent\hspace{5ex}\rule{0pt}{2.5ex}\configtrans[\maction]{\mparconfig{}{1}{}{2}}{\mparconfig{'}{1}{'}{2}},
   \par\noindent\hspace{11ex}\rule{0pt}{2.5ex}result with \isoconfig[']{1}\ and \isoconfig[']{2} that are well-formed.
   %
\end{lemma}
\begin{proof}
   This proof proceeds by induction on the depth of the derivation tree, proceeding by analysing the last rule applied
   \begin{inline}
      \item \sysrWait
      \item \sysrComm
      \item \sysrDequ
   \end{inline}
   \begin{description}[itemsep=1.75ex,parsep=1.25ex]
      % ! Wait
      \item[{Rule \sysrWait}]
         Then $\maction=\mtval$, and by the premise of \sysrWait, the transition of \tval\ is a time stepping transition only possible via \socrTime\ for social configurations:
         \begin{equation*}
            \msocconfig{1}%
            \transition{\mtval}%
            \msocconfig[']{1}%
            %
            \qquad\text{and}\qquad
            %
            \msocconfig{2}%
            \transition{\mtval}%
            \msocconfig[']{2}%
         \end{equation*}
         and via \isorTime\ for isolated configurations:
         \begin{equation*}
            \misoconfig{1}%
            \transition{\mtval}%
            \misoconfig[']{1}%
            %
            \qquad\text{and}\qquad
            %
            \misoconfig{2}%
            \transition{\mtval}%
            \misoconfig[']{2}%
         \end{equation*}
         By~\cref{lem:configs_iso_trans,lem:configs_soc_trans} it is known that
         \begin{inline}
            \item $\of{\mst}{1}'=\of{\mst}{1}$
            \item $\of{\mval}{1}'=\of{\mval}{1}+\mtval$
            \item $\of{\queue}{1}'=\of{\queue}{1}$
         \end{inline}
         The same applies for
         \begin{inline}
            \item $\of{\mst}{2}'$
            \item $\of{\mval}{2}'$
            \item $\of{\queue}{2}'$
         \end{inline}
         Therefore, for the hypothesis to hold, $(\of{\mval}{1}+\mtval,\,\of{\mst}{1})\quad\text{and}\quad(\of{\mval}{2}+\mtval,\,\of{\mst}{2})$ must be well-formed.

         When $\mtval=0$, there are no changes, indicating that this is either the last opportunity for a viable sending action, or, that there is a message ready to be received in the queue. By~\cref{lem:configs_iso_trans,lem:configs_soc_trans}, $\miso[']{}=\miso{}$ and $\msoc[']{}=\msoc{}$.
         The premise of \socrTime\ has the following additional items:
         \begin{enumerate}
            \item $\mactFE{(\mval,\,\mst)}{\msend}\implies\mactFE{(\mval',\,\mst)}{\msend}$
                  ensuring that as sending actions become viable, time is allowed to pass across the clocks up until the soonest constraint would be come unsatisfied, at which point one action must be taken. It is important to note that a \emph{future-enabled} sending action is not necessarily viable, but has the potential to be viable in the future.
                  %
            \item $\forall\mtval'<\mtval:(\mval+\mtval',\,\mst,\,\queue)\ntransition{\tau}$
                  ensuring that messages are received as soon as they become available in the queue.
                  %
         \end{enumerate}
         Whenever a transition of \tval\ is performed, it must be valued so that both of the conditions above are met by reducing its valuation.

         By inner induction of the derivation of
         $\miso{1}:\menvempty\,\of{\mconstr}{1}\imp\of{\mst}{1}$ and $\of{\mval}{1}\models\of{\mconstr}{1}$,
         by case analysis of the last rule applied is as follows (with \iso{2} being the same)
         \begin{inline}
            \item \formEnd
            \item \formChoice
            \item \formRec
         \end{inline}
         In the scenarios that follow, it is assumed that \iso{1}\ is next to perform an action, and therefore the focus as it is responsible for reducing the value of \tval.
         \begin{description}[parsep=0.75ex,listparindent=4ex]
            \item[{Rule \formEnd}]
               Then $\of{\mst}{1}=\mend$. \iso{1}\ is always well-formed as $\mtrue\imp\mend$ and $\of{\mval}{1}\models\mtrue$ always holds.
               Therefore, $(\of{\mval}{1}+\mtval,\,\mend)$ is well-formed as $\menvempty\,\mtrue\imp\of{\mst}{1}$ and $\of{\mval}{1}+\mtval\models\mtrue$.
               %
            \item[{Rule \formChoice}]
               Then $\of{\mst}{1}=\msetinteract{i}$.
               By~\cref{def:types_well_formed,def:configs_iso_well_formed} and the hypothesis, the following holds for \iso{1}:
               \begin{equation*}
                  \menvempty\,\mpast[\of{\bigvee}{\elemofset{i}{i}}\,\of{\mconstr}{i}]\imp\msetinteract[i]{i}
                  %
                  \qquad\text{and}\qquad
                  %
                  \of{\mval}{1}\models\of{\mconstr}{i}
                  %
               \end{equation*}
               The premise of \formChoice\ enforces that constraints on actions of one kind (sending or receiving) are only satisfiable when the constraints on actions of the other kind (receiving or sending) are not satisfied:
               \begin{equation*}
                  \forall\elemofset{i \neq j}{i}\quad%
                  \of{\mconstr}{i}\cap\of{\mconstr}{j}=\emptyset%
                  \quad\lor\quad%
                  \of{\mcomm}{i}=\of{\mcomm}{j}%
               \end{equation*}
               Therefore interactions with different actions (sending or receiving) \emph{cannot} compete to be taken at the same time.
               Combined with the premises of \socrTime\ discussed earlier in this Lemma, \tval\ is valued so that $\of{\mval}{1}+t\models\of{\mconstr}{i}$ and $\menvempty\,\of{\mconstr}{i}\imp\of{\mst}{1}$ where $\elemofset{i}{i}=\lvert\of{\mst}{1}\rvert$.
               %
            \item[{Rule \formRec}]
               Then $\of{\mst}{1}=\mrec\mathtt{t}.\of{\mst}{1}'$. By the hypothesis and~\cref{def:types_well_formed,def:configs_iso_well_formed}, the following is known of \iso{1}:
               \begin{equation*}
                  \menvempty\,\mconstr\imp\mrec\mathtt{t}.\of{\mst}{1}'
                  %
                  \qquad\text{and}\qquad
                  %
                  \of{\mval}{1}\models\mconstr
                  %
               \end{equation*}
               By induction on the depth of the derivation tree, the analysis of \isorRec\ premised by \isorTime, is as follows:
               \begin{equation*}
                  \infer[\begin{array}{l}\raisebox{1ex}{$\rulem{iso-time}$}\\\raisebox{2.5ex}{$\rulem{recursion}$}\end{array}]%
                  {%
                  (\of{\mval}{1},\,\mrec\mathtt{t}.\of{\mst}{1}')
                  \transition{\mtval}
                  (\of{\mval}{1}+\mtval,\,\of{\mst}{1}')
                  }{%
                  (\of{\mval}{1},\,\of{\mst}{1}' [\mrec\mathtt{t}.\of{\mst}{1}'/\mathtt{t}])
                  \transition{\mtval}
                  (\of{\mval}{1}+\mtval,\,\of{\mst}{1}')
                  }%
               \end{equation*}
               The rule \isorRec\ only unfolds recursive types, and by the premise of the rule \formRec, it is shown that the constraints on clocks is unchanged as it progresses to the proceeding type $\of{\mst}{1}'$:
               \begin{equation*}
                  \menvempty[,\,\mathtt{t}:\mconstr]\,\mconstr\imp\of{\mst}{1}'
                  %
                  \qquad\text{and}\qquad
                  %
                  \of{\mval}{1}+\mtval\models\mconstr
                  %
               \end{equation*}
               Therefore, whether $(\of{\mval}{1}+t,\,\of{\mst}{1}')$ is well-formed depends on $\of{\mst}{1}'$. Each possibility is discussed in each of the cases of this inner induction of \sysrWait.
               %
         \end{description}

         % ! Comm
      \item[{Rule \sysrComm}]
         The following only considers the scenario where \soc{1}\ sends the message $\mmsg$, and \soc{2}\ enqueues it. The evaluation is as follows:
         \begin{equation*}\label{eqn:prog_trans_iso_wf_comm}
            \infer[\begin{array}{l}\raisebox{1ex}{$\rulem{enqu}$}\\\raisebox{2.5ex}{$\rulem{comm}$}\end{array}]%
            {%
               \msocconfig{1}\mid\msocconfig{2}%
               \transition{\tau}%
               \msocconfig[']{1}\mid\msocconfig[']{2}%
            }%
            {%
               \infer[\rulem{send}]%
               {%
                  \msocconfig{1}%
                  \transition{\msend\,\mmsg}%
                  (\of{\mval}{1}',\,\of{\mst}{1}',\,\of{\queue}{1})%
               }%
               {%
                  \misoconfig{1}%
                  \transition{\msend\,\mlabel}%
                  \misoconfig[']{1}
                  %
                  &%
                  \mlabel=\mmsg%
                  &%
                  \mcomm=\msend
               }%
               %
               &%
               %
               (\of{\mval}{2},\,\of{\mst}{2},\,\of{\queue}{2})%
               \transition{\mrecv\,\mmsg}%
               (\of{\mval}{2},\,\of{\mst}{2},\,\of{\queue}{2};\mmsg)%
               %
            }%
         \end{equation*}
         By~\cref{lem:configs_soc_trans}, $\miso{2}=\miso[']{2}$, therefore \iso[']{2}\ is well-formed.
         By induction of the derivation of
         $\miso{1}:\menvempty\,\of{\mconstr}{1}\imp\of{\mst}{1}$ and $\of{\mval}{1}\models\of{\mconstr}{1}$,
         the case analysis of the last rule applied is as follows:
         \begin{inline}
            \item \formEnd
            \item \formChoice
            \item \formRec
         \end{inline}
         \begin{description}[parsep=0.75ex,listparindent=4ex]
            \item[{Rule \formEnd}]
               \REDO[As with the previous case \sysrWait.] Then $\of{\mst}{1}=\mend$. \iso{1} is always well-formed as $\mtrue\imp\mend$ and $\of{\mval}{1}\models\mtrue$ always holds.
               Therefore, $(\of{\mval}{1}+\mtval,\,\mend)$ is well-formed as $\menvempty\,\mtrue\imp\of{\mst}{1}$ and $\of{\mval}{1}+\mtval\models\mtrue$.
               %
            \item[{Rule \formChoice}]
               Then $\of{\mst}{1}=\msetinteract{i}$.
               By the induction hypothesis, and the premise of \formChoice, \iso{1}\ being well-formed requires that the following must hold, following~\cref{def:types_well_formed,def:configs_iso_well_formed}:
               \begin{equation}
                  \menvempty\,\mpast[\of{\mconstr}{i}]\imp\of{\mst}{1}
                  \quad\text{and}\quad
                  \of{\mval}{1}\models\mpast[\of{\mconstr}{i}]
               \end{equation}
               For the above, $\mpast[\of{\mconstr}{i}]$ is used by following the judgement of \formChoice, to indicate that there is still a viable action.

               Proceeding by induction on the depth of the derivation tree, the analysis of \socrSend\ premised by \isorInteract, is as follows, beginning with its evaluation:
               \begin{equation*}
                  \infer[\rulem{send}]%
                  {%
                     (\of{\mval}{1},\,\msetinteract{i},\,\of{\queue}{1})
                     \transition{\msend\,\mmsg}
                     (\of{\mval}{1}',\,\of{\mst}{j},\,\of{\queue}{1})
                  }{%
                     \infer[\rulem{interact}]%
                     {%
                        (\of{\mval}{1},\msetinteract[i]{i})%
                        \transition{\of{\mcomm}{j}\,\of{\mlabel}{j}}%
                        (\of{\mval}{1}\actReset[\of{\mresets}{j}],\of{\mst}{j})%
                        %
                        \quad%
                        %
                        \of{\mlabel}{j}=\mmsg%
                        \quad%
                        \of{\mcomm}{j}=\msend
                     }%
                     {%
                        \of{\mval}{1}\models\of{\mconstr}{j}&%
                        (\of{\mconstr}{j}\cap\of{\mconstr}{k}=\emptyset%
                        \,\vee\,%
                        \of{\mcomm}{j}=\of{\mcomm}{k})&%
                        \elemofset{j\neq k}{i}%
                     }%
                  }%
               \end{equation*}
               The premise of \isorInteract\ coincides with the induction hypothesis, indicating that \iso{1}\ is well-formed (note that the premise of \isorInteract\ does not use $\of{\mval}{1}\models\mpast[\of{\mconstr}{j}]$, indicating that the constraints are currently satisfied with the valuation of clocks). In order fo $\miso[']{1}=(\of{\mval}{1}',\,\of{\mst}{j},\,\of{\queue}{1})$ to be well-formed, the following must hold:
               \begin{equation}
                  \menvempty\,\mpast[\mconstr']\imp\of{\mst}{1}'
                  \quad\text{and}\quad
                  \of{\mval}{1}'\models\mpast[\mconstr']
               \end{equation}
               Where $\mconstr'=\of{\mconstr}{k}$, and, $\elemofset{k}{k}=\lvert\of{\mst}{1}'\rvert$, and
               \begin{inline}
                  \item the new type corresponds to the action taken $\of{\mst}{1}'=\of{\mst}{j}$
                  %
                  \item the relevant clocks are reset in the new valuation $\of{\mval}{1}'=\of{\mval}{1}\actReset[\of{\mresets}{j}]$
                  %
                  \item the new type is a set of interactions $\of{\mst}{j}=\msetinteract[k]{k}$
                  %
               \end{inline}

               It must be that the current evaluation of clocks satisfies an actions constraints $\of{\mval}{1}\models\of{\mconstr}{j}$ by the premise of \isorInteract.
               It follows that the same clock resets imposed on both the valuation and constraints of clocks yields the similarly equivalent: $\of{\mval}{1}\actReset[\of{\mresets}{j}]\models\of{\mconstr}{j}\actReset[\of{\mresets}{j}]$.

               By the induction hypothesis, the initial configuration being well-formed requires that the types adhere to the formation rules, and by \formChoice, subsequent types must have at least one interaction with constraints that are satisfiable given the last constraints imposed on the clocks: $\of{\mconstr}{j}\actReset[\of{\mresets}{j}]\subseteq\mconstr'$; and, a satisfiable constraint allows types to be reached: $\of{\mconstr}{j}\imp\of{\mst}{j}$.

               Therefore, it holds that the new valuation of clocks must be able to satisfy the constraints of the proceeding type, either immediately or in the future $\of{\mval}{1}'\models\mpast[\mconstr']$, and that when this constraint is satisfied an interaction can be taken $\menvempty\,\mconstr'\imp\of{\mst}{1}'$. Therefore, \isoconfig[']{1}\ is well-formed.
               \TODO[need to do case of $\of{\mst}{1}'$ being a recursive type?]
               % 
            \item[{Rule \formRec}]
               Then $\of{\mst}{1}=\mrec\mathtt{t}.\of{\mst}{1}'$.
               \TODO[same as with case \rulet{wait}?]
               %
         \end{description}

         % ! Dequ
      \item[{Rule \sysrDequ}]
         The following only considers the scenario where \soc{2}\ is receiving a message $\mmsg$ from its queue. The evaluation is as follows:
         \begin{equation*}
            \infer[\rulem{dequ}]%
            {%
               \msocconfig{1}\mid\msocconfig{2}%
               \transition{\tau}%
               \msocconfig{1}\mid\msocconfig[']{2}%
            }%
            {%
               \infer[\rulem{recv}]%
               {%
                  (\of{\mval}{2},\,\of{\mst}{2},\,\mmsg;\of{\queue}{2})%
                  \transition{\mrecv\,\mmsg}%
                  (\of{\mval}{2}',\,\of{\mst}{2}',\,\of{\queue}{2})%
               }%
               {%
                  \infer[\rulem{interact}]%
                  {%
                     (\of{\mval}{2},\msetinteract[i]{i})%
                     \transition{\of{\mcomm}{j}\,\of{\mlabel}{j}}%
                     (\of{\mval}{2}\actReset[\of{\mresets}{j}],\of{\mst}{j})%
                     %
                     \quad%
                     %
                     \of{\mlabel}{j}=\mmsg%
                     \quad%
                     \of{\mcomm}{j}=\mrecv
                  }%
                  {%
                     \of{\mval}{2}\models\of{\mconstr}{j}\quad%
                     (\of{\mconstr}{j}\cap\of{\mconstr}{k}=\emptyset%
                     \,\vee\,%
                     \of{\mcomm}{j}=\of{\mcomm}{k})\quad%
                     \elemofset{j\neq k}{i}%
                  }%
               }%
            }%
         \end{equation*}
         By~\cref{lem:configs_soc_trans}, $\miso{1}=\miso[']{1}$, therefore \iso[']{1}\ is well-formed.
         By induction of the derivation of
         $\miso{2}:\menvempty\,\of{\mconstr}{2}\imp\of{\mst}{2}$ and $\of{\mval}{2}\models\of{\mconstr}{2}$,
         the case analysis of the last rule applied is as follows:
         \begin{inline}
            \item \formEnd
            \item \formChoice
            \item \formRec
         \end{inline}
         \begin{description}[parsep=0.75ex,listparindent=4ex]
            \item[{Rule \formEnd}]
               \REDO[As with the previous case \sysrWait.] Then $\of{\mst}{2}=\mend$. \iso{2} is always well-formed as $\mtrue\imp\mend$ and $\of{\mval}{2}\models\mtrue$ always holds.
               Therefore, $(\of{\mval}{2}+\mtval,\,\mend)$ is well-formed as $\menvempty\,\mtrue\imp\of{\mst}{2}$ and $\of{\mval}{2}+\mtval\models\mtrue$.
               %
            \item[{Rule \formChoice}]
               Then $\of{\mst}{2}=\msetinteract{i}$.
               By the induction hypothesis, and following the premise of \formChoice, \iso{2}\ being well-formed requires that the following must hold, following~\cref{def:types_well_formed,def:configs_iso_well_formed}:
               \begin{equation}
                  \menvempty\,\mpast[\of{\mconstr}{i}]\imp\of{\mst}{2}
                  \quad\text{and}\quad
                  \of{\mval}{2}\models\mpast[\of{\mconstr}{i}]
               \end{equation}
               \REDO[The rest of the proof is analogous to the one found in case \rulet{comm} of this Lemma.]
               %
            \item[{Rule \formRec}]
               \REDO[The rest of the proof is analogous to the one found in case \rulet{comm} of this Lemma.]
               %
         \end{description}
   \end{description}
\end{proof}

\endinput

==> tex/proofs/progress/lem/prog_trans_soc_compat.tex <==
\begin{lemma}\label{lem:prog_trans_soc_compat}
   Given two participants that are compatible \compconfig{}{1}{}{2}, and, both \isoconfig{1}\ and \isoconfig{2} are \emph{well-formed}:\par
   %
   If \;\configtrans[\maction]{\mparconfig{}{1}{}{2}}{\mparconfig{'}{1}{'}{2}}, \par\noindent
   \hspace{7ex}\rule{0pt}{2.5ex} then \compconfig{'}{1}{'}{2}.
   %
\end{lemma}
\begin{proof}
   This proof proceeds by induction on the depth of the derivation tree, proceeding by analysing the last rule applied
   \begin{inline}
      \item \sysrWait
      \item \sysrComm
      \item \sysrDequ
   \end{inline}
   \begin{description}[itemsep=1.25ex,parsep=1.25ex]
      % ! Wait
      \item[{Rule \sysrWait}]
         then $\maction=\mtval$. The evaluation is the same as in~\cref{lem:prog_trans_iso_wf}, {Rule \rulet{wait}}:
         \begin{equation*}
            \infer[\rulem{wait}]%
            {%
               (\of{\mval}{1},\,\of{\mst}{1},\,\of{\queue}{1})
               \,\mid\,
               (\of{\mval}{2},\,\of{\mst}{2},\,\of{\queue}{2})
               %
               \transition{\mtval}
               %
               (\of{\mval}{1}',\,\of{\mst}{1},\,\of{\queue}{1})
               \,\mid\,
               (\of{\mval}{2}',\,\of{\mst}{2},\,\of{\queue}{2})
            }{%
               \infer[\rulem{time}]%
               {%
                  (\of{\mval}{1},\,\of{\mst}{1},\,\of{\queue}{1})
                  \transition{\mtval}
                  (\of{\mval}{1}',\,\of{\mst}{1},\,\of{\queue}{1})
               }{%
                  \dots
               }%
               &
               \infer[\rulem{time}]%
               {%
                  (\of{\mval}{2},\,\of{\mst}{2},\,\of{\queue}{2})
                  \transition{\mtval}
                  (\of{\mval}{2}',\,\of{\mst}{2},\,\of{\queue}{2})
               }{%
                  \dots
               }%
            }%
         \end{equation*}
         By~\cref{lem:configs_iso_trans,lem:configs_soc_trans} it is known that
         \begin{inline}
            \item $\of{\mst}{1}'=\of{\mst}{1}$
            \item $\of{\mval}{1}'=\of{\mval}{1}+\mtval$
            \item $\of{\queue}{1}'=\of{\queue}{1}$
         \end{inline}
         The same applies for
         \begin{inline}
            \item $\of{\mst}{2}'$
            \item $\of{\mval}{2}'$
            \item $\of{\queue}{2}'$
         \end{inline}

         Regardless of the value of \mtval, the compatibility of the configurations will remain the same. Below the evaluation of \soc{1}\ is continued (with the evaluation of \soc{2}\ being analogous):
         \begin{equation*}
            \infer[\rulem{time}]%
            {%
               (\of{\mval}{1},\,\of{\mst}{1},\,\of{\queue}{1})%
               \transition{\mtval}%
               (\of{\mval}{1}',\,\of{\mst}{1},\,\of{\queue}{1})%
            }{%
               (\of{\mval}{1},\,\of{\mst}{1})%
               \transition{\mtval}%
               (\of{\mval}{1}+\mtval,\,\of{\mst}{1})%
               &
               \mactFE{(\of{\mval}{1},\,\of{\mst}{1})}{\msend}%
               \implies%
               \mactFE{(\of{\mval}{1}',\,\of{\mst}{1})}{\msend}%
               &
               \forall\mtval'<\mtval:(\of{\mval}{1}+\mtval',\,\of{\mst}{1},\,\of{\queue}{1})%
               \ntransition{\tau}%
            }%
         \end{equation*}
         By the premise of \isorTime, as in~\cref{lem:prog_trans_iso_wf}, $\mtval=0$ indicates that there is either a message in the queue or a sending action must be performed. Again, by~\cref{lem:configs_iso_trans,lem:configs_soc_trans} it is known that, for $\mtval=0$ it must be that $\msoc[']{1}\,\bot\,\msoc[']{2}$.

         $\mtval>0$ indicates that the queues are empty $\of{\queue}{1}=\emptyset=\of{\queue}{2}$ until at least $\mval+\mtval$; by~\cref{itm:configs_soc_compat_duality} of~\cref{def:configs_soc_compat}, the types are dual $\of{\mst}{1}=\mdual[\of{\mst}{2}]$ and have matching clock valuations $\of{\mval}{1}=\of{\mval}{2}$. Hereafter, the analysis of \sysrWait\ continues with only focusing on \soc{1}\ as by duality, \soc{2}\ \REDO[is analogous.]

         The inner induction of the derivation of $\of{\mst}{1}$ and $\of{\mst}{2}$ for a time stepping transition \tval, is the same as shown in~\cref{lem:prog_trans_iso_wf}. As the initial configurations queues are empty, they are dual, and time will progress equally. Therefore the resulting configurations \socconfig[']{1}\ and \socconfig[']{2}\ are also compatible by adhereing to the conditions specified in~\cref{def:configs_soc_compat}.

         % ! Comm
      \item[{Rule \sysrComm}]
         The following only considers the scenario where \soc{1}\ sends the message $\mmsg$, and \soc{2}\ enqueues it. The evaluation is as follows:
         \begin{equation*}
            \infer[\begin{array}{l}\raisebox{1ex}{$\rulem{enqu}$}\\\raisebox{2.5ex}{$\rulem{comm}$}\end{array}]%
            {%
               \msocconfig{1}\,\mid\,\msocconfig{2}%
               \transition{\tau}%
               \msocconfig[']{1}\,\mid\,\msocconfig[']{2}%
            }%
            {%
               \infer[\rulem{send}]%
               {%
                  \msocconfig{1}%
                  \transition{\msend\,\mmsg}%
                  (\of{\mval}{1}',\,\of{\mst}{1}',\,\of{\queue}{1})%
               }%
               {%
                  \misoconfig{1}%
                  \transition{\msend\,\mlabel}%
                  \misoconfig[']{1}
                  %
                  &%
                  \mlabel=\mmsg%
                  &%
                  \mcomm=\msend
               }%
               %
               &%
               %
               (\of{\mval}{2},\,\of{\mst}{2},\,\of{\queue}{2})%
               \transition{\mrecv\,\mmsg}%
               (\of{\mval}{2},\,\of{\mst}{2},\,\of{\queue}{2};\mmsg)%
               %
            }%
         \end{equation*}
         Proceeding by inner induction on the queue contents $\of{\queue}{1}$ and $\of{\queue}{2}$, analysing the possible configurations by the induction hypothesis
         \begin{inlineEnum}
            \item $\of{\queue}{1}=\emptyset\;\mid\;\of{\queue}{2}=\emptyset$\;
            %
            \item $\of{\queue}{1}=\emptyset\;\mid\;\of{\queue}{2}=\mmsg';\of{\queue}{2}$\;
            %
            \item $\of{\queue}{1}=\mmsg';\of{\queue}{1}\;\mid\;\of{\queue}{2}'=\emptyset$\;
            %
         \end{inlineEnum}
         \begin{description}[parsep=0.75ex,listparindent=4ex]
            \item[{Case $\of{\queue}{1}=\emptyset\;\mid\;\of{\queue}{2}=\emptyset$}]
               Both queues are empty, by~\cref{itm:configs_soc_compat_duality} of~\cref{def:configs_soc_compat}, the types are dual $\of{\mst}{1}=\mdual[\of{\mst}{2}]$.
               The resulting configurations $\msoc[']{1}\,\mid\,\msoc[']{2}$ are as follows:
               \begin{equation*}
                  (\of{\mval}{1}',\,\of{\mst}{1}',\,\emptyset)%
                  \,\mid\,%
                  (\of{\mval}{2},\,\of{\mst}{2},\,\mmsg;\emptyset)%
               \end{equation*}
               As~\cref{def:types_duality} specifies, dual types have a corresponding receiving action for every sending action; both types sharing the same constraints and resets over their respective local and equivalent clocks.

               Therefore, it is guaranteed that the message will be received by \soc[']{2}, which by adhering to~\cref{itm:configs_soc_compat_expected_receive} of~\cref{def:configs_soc_compat}, means that $\msoc[']{1}\,\mid\,\msoc[']{2}$ are compatible.
               %
            \item[Case $\of{\queue}{1}=\emptyset\;\mid\;\of{\queue}{2}=\mmsg';\of{\queue}{2}$]
               There is a message $\mmsg'$ already in the recipients queue $\of{\queue}{2}$, waiting to be received.
               By the hypothesis, and~\cref{itm:configs_soc_compat_expected_receive} of~\cref{def:configs_soc_compat}, the message $\mmsg'$ is expected, and will lead to a new configuration \soc['']{2}\ that is compatible with the sender \soc{1}.
               The resulting configurations $\msoc[']{1}\,\mid\,\msoc[']{2}$ are as follows:
               \begin{equation*}
                  (\of{\mval}{1}',\,\of{\mst}{1}',\,\emptyset)%
                  \,\mid\,%
                  (\of{\mval}{2},\,\of{\mst}{2},\,\mmsg';\mmsg;\emptyset)%
               \end{equation*}
               If, instead of \soc{1}\ sending the second message $\mmsg$, \soc{2}\ were to have received the message $\mmsg'$ that is already in its queue, the resulting configurations would have empty queues queues. By~\cref{itm:configs_soc_compat_duality} of~\cref{def:configs_soc_compat}, types would be dual $\of{\mst}{1}=\mdual[\of{\mst}{2}'']$, and clock valuations would match $\of{\mval}{1}=\of{\mval}{2}''$. Afterwards, if \soc{1}\ were to continue sending the message $\mmsg$, by the notion of duality in~\cref{def:types_duality}, any sending action must have a corresponding receiing action, as shown in the previous case, {Rule $\of{\queue}{1}=\emptyset,\;\of{\queue}{2}=\emptyset$}.

               Therefore, it holds that, for compatible and well-formed configurations, enqueuing subsequent messages into a non-empty queue will result in compatible configurations.
               %
            \item[Case $\of{\queue}{1}=\mmsg;\of{\queue}{1}\;\mid\;\of{\queue}{2}=\emptyset$]
               The resulting configurations $\msoc[']{1}\,\mid\,\msoc[']{2}$ are \emph{not compatible} by~\cref{itm:configs_soc_compat_empty_queues} of~\cref{def:configs_soc_compat}, as shown below:
               \begin{equation*}
                  (\of{\mval}{1}',\,\of{\mst}{1}',\,\mmsg';\emptyset)%
                  \,\mid\,%
                  (\of{\mval}{2},\,\of{\mst}{2},\,\mmsg;\emptyset)%
               \end{equation*}
               However, the initial configurations \soc{1}\ and \soc{2}\ do not coincide with the hypothesis, as well-formed configurations should not have a viable sending action while there is a message waiting to be received.

               As shown in~\cref{lem:prog_trans_iso_wf}, case {Rule \rulet{wait}}, time cannot pass over the clocks while there is a message waiting to be received.
               By induction hypothesis, the message $\mmsg'$ in the queue of \soc{1}\ is known to be an expected and viable receiving action, by~\cref{itm:configs_soc_compat_expected_receive} of~\cref{def:configs_soc_compat}.

               By induction hypothesis, \iso{1}\ and \iso{2}\ are well-formed, and must adhere to the formation rules. By inner induction on the derivation of $\of{\mst}{1}:(\of{\mval}{1},\,\of{\mst}{1},\,\mmsg';\emptyset)\transition{\msend\,\mmsg}$, analysing the last rule applied: \REDO[add recursive?]
               \begin{description}[parsep=0.75ex,listparindent=4ex]
                  \item[Rule \formChoice]
                     Then $\of{\mst}{1}=\msetinteract{i}$.
                     The premise of \formChoice\ ensures that sending and receiving actions cannot happen at the same time.

                     Therefore, it holds that it is not possible for a message to be sent while the senders queue is not empty, for the following reasons
                     \begin{inlineEnum}
                        \item By induction hypothesis, the message $\mmsg'$ in the queue of \soc{1}\ is able to be received
                        %
                        \item By~\cref{lem:prog_trans_iso_wf}, case {Rule \rulet{wait}}, time cannot pass while any message can be received
                        %
                        \item By the premise of \formChoice, it is not possible for a sending action to be viable while a receiving action waits for the message
                        %
                     \end{inlineEnum}
                     %
               \end{description}
         \end{description}

         % ! Dequ
      \item[{Rule \sysrDequ}]
         The following only considers the scenario where \soc{2}\ is receiving a message $\mmsg$ from its queue. The evaluation is as follows:
         \begin{equation*}
            \infer[\rulem{dequ}]%
            {%
               \msocconfig{1}\,\mid\,\msocconfig{2}%
               \transition{\tau}%
               \msocconfig[']{1}\,\mid\,\msocconfig[']{2}%
            }{%
               \infer[\rulem{recv}]%
               {%
                  \msocconfig{2}%
                  \transition{\tau}%
                  \msocconfig[']{2}%
               }{%
                  (\of{\mval}{2},\,\of{\mst}{2})%
                  \transition{\mrecv\,\mlabel}%
                  (\of{\mval}{2}',\,\of{\mst}{2}')%
                  &
                  \mlabel=\mmsg%
               }%
            }%
         \end{equation*}
         Proceeding by inner induction on the derivation of $\of{\mst}{2}:(\of{\mval}{2},\,\of{\mst}{2},\,\emptyset)\transition{\mrecv\,\mmsg}$, analysing the last rule applied:
         \begin{description}[parsep=0.75ex,listparindent=4ex]
            \item[Rule \formChoice]
               Then $\of{\mst}{2}=\msetinteract{i}$.
               The evaluation continues as follows:
               \begin{equation*}
                  \infer[\rulem{dequ}]%
                  {%
                     \msocconfig{1}\,\mid\,\msocconfig{2}%
                     \transition{\tau}%
                     \msocconfig[']{1}\,\mid\,\msocconfig[']{2}%
                  }{%
                     \infer[\rulem{recv}]%
                     {%
                        \msocconfig{2}%
                        \transition{\tau}%
                        \msocconfig[']{2}%
                     }{%
                        \infer[\rulem{interact}]%
                        {%
                           (\of{\mval}{2},\msetinteract[i]{i})%
                           \transition{\of{\mcomm}{j}\,\of{\mlabel}{j}}%
                           (\of{\mval}{2}\actReset[\of{\mresets}{j}],\of{\mst}{j})%
                           %
                           \quad%
                           %
                           \of{\mlabel}{j}=\mmsg%
                           \quad%
                           \of{\mcomm}{j}=\mrecv
                        }{%
                           \of{\mval}{2}\models\of{\mconstr}{j}&%
                           (\of{\mconstr}{j}\cap\of{\mconstr}{k}=\emptyset%
                           \,\vee\,%
                           \of{\mcomm}{j}=\of{\mcomm}{k})&%
                           \elemofset{j\neq k}{i}%
                        }%
                     }%
                  }%
               \end{equation*}
               By the induction hypothesis, \soc{1}\ and \soc{2}\ being compatible requires that the message $\mmsg$ in the queue of \soc{2}\ is guaranteed to be a viable receiving action, which will lead to another compatible configuration. Therefore, \soc[']{1}\ and \soc[']{2}\ are compatible.
               %
            \item[Rule \formRec]
               Then $\of{\mst}{2}=\mrec\mathtt{t}.\of{\mst}{2}''$.
               The evaluation continues as follows:
               \begin{equation*}
                  \infer[\rulem{dequ}]%
                  {%
                  \msocconfig{1}\,\mid\,\msocconfig{2}%
                  \transition{\tau}%
                  \msocconfig[']{1}\,\mid\,\msocconfig[']{2}%
                  }{%
                  \infer[\rulem{recv}]%
                  {%
                  \msocconfig{2}%
                  \transition{\tau}%
                  \msocconfig[']{2}%
                  }{%
                  \infer[\rulem{recursion}]%
                  {%
                  (\of{\mval}{2},\mrec\mathtt{t}.\of{\mst}{2}'')%
                  \transition{\mrecv\,\mlabel}%
                  (\of{\mval}{2}',\of{\mst}{2}')%
                  }{%
                  (\of{\mval}{2},\of{\mst}{2}''[\mrec\mathtt{t}.\of{\mst}{2}''/\mathtt{t}])%
                  \transition{\mrecv\,\mlabel}%
                  (\of{\mval}{2}',\of{\mst}{2}')%
                  }%
                  }%
                  }%
               \end{equation*}
               \REDO[continue, redirecting to other cases depending on the value of ]$\of{\mst}{2}''$?
               %
         \end{description}
   \end{description}
\end{proof}

\endinput


==> tex/proofs/progress/lem/sys_compat_time_trans.tex <==
%
% ! (lemma 13) : time passing implies empty queues
\begin{lemma}\label{lem:sys_compat_time_trans}
   %
   If \Compat*[\VSoc_1][\VSoc_2]\ and \Trans*{\Parl{\VSoc_1,\VSoc_2}}:{\ValTime}\ and $\ValTime>0$ then $\Queue_1=\emptyset=\Queue_2$.
   %
\end{lemma}
\begin{proof}
   %
   Such a transition is only specified by \LblCfgSysWait*, which by its premise requires a \LblCfgSocTime*\ transition of \ValTime*\ for each \VSoc*_1\ and \VSoc*_2.
   %
   By contradiction, if one queue were \emph{non-empty}, say $\Queue_1=\Msg;\Queue_1$, then by~\Cref{itm:configs_compat_expected_receive} of~\Cref{def:configs_compat} message \Msg*\ must be able to be received immediately.
   %
   The premise of \LblCfgSocTime*\ (urgency) ensures that \ValTime*\ must be valued such that no time passes while a message is able to be received.
   %
   % It holds that $t$ must equal 0 when there is a non-empty queue.
   
   Therefore the hypothesis holds.
   %if a system makes a $t$ transition where $t>0$ then all queues in the system must be empty.
   % Therefore, \ValTime*\ must equal $0$ when there is a message in any queue in a system composed of compatible configurations.
   %
 \end{proof}
 % 

==> tex/proofs/progress/lem/typ_rec_capture_avoiding.tex <==
%
\begin{lemma}\label{lem:typ_rec_capture_avoiding}
    %
    recursion capture avoiding substitution \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}
%

==> tex/proofs/progress/lem/wf_then_live.tex <==
%
\begin{lemma}\label{lem:cfg_wf_then_live}
    %
    If \CIso*\ is \emph{well-formed}, then \CIso*\ is \emph{live}.
    %
\end{lemma}
\begin{proof}
    %
    By the hypothesis, there must $\exists\Const$ such that $\emptyset;\Const~\Entails\TypeS$ and $\ValClocks\models\Const$.
    %
    We proceed by induction on each case of \TypeS*:
    \begin{inductivecase}
        %
        %
        %
        % ~ choice
        \item\NewCase[$\TypeS=\simplechoice$]\label{itm:cfg_wf_then_live_choice} 
        By the hypothesis and the judgement of rule \LblTypChoice*\ $\exists\Const_i$ such that $\ValClocks\models\Past[\Const_i]$ and $\emptyset;\Past[\Const_i]~\Entails\FullChoice$.
        %
        By~\Cref{def:configs_wf,def:configs_fe} \CIso*\ is \isFE*, and therefore, by~\Cref{def:configs_live} \CIso*\ is \emph{live}.
        %
        %
        %
        % ~ rec def
        \item\NewCase[$\TypeS=\mu\alpha.{\TypeS}'$]\label{itm:wf_then_live_recdef} 
        By the hypothesis $\exists\Const$ such that $\ValClocks\models\Const$ and $\emptyset;\Const~\Entails\TypRecDef$, and by the premise of rule \LblTypRec*\ $\alpha:\Const;\Const~\Entails{\TypeS}'$ and \CIso*;[\TypeS']\ is \emph{well-formed}.
        
        We proceed by inner induction on each case of \TypeS*':
        \begin{inductivecase}
            %
            %
            % ~ rec def -> choice
            \item\NewCase[$\TypeS'=\simplechoice$] 
            By the judgement of rule \LblTypChoice*\ and the premise of rule \LblTypRec*, $\exists\Const_i$ such that $\ValClocks\models\Const_i$ and $\emptyset;\Const_i~\Entails\TypRecDef$ and $\alpha:\Const_i;\Past[\Const_i]~\Entails\FullChoice$.
            %
            It follows~\Cref{itm:cfg_wf_then_live_choice} of~\Cref{lem:cfg_wf_then_live} that, by~\Cref{def:configs_wf,def:configs_fe,def:configs_live}, \CIso*;[\simplechoice]\ is \isFE*, \emph{well-formed} and \emph{live}.
            Therefore, it holds that \CIso*\ is \emph{live}.
            % Then by the judgement of \LblTypChoice*\ and the premise of \LblTypRec*\ $\exists\Const_i$ such that $\ValClocks\models\Const_i$ and $\emptyset;\Const_i~\Entails\TypRecDef$ and $\alpha:\Const_i;\Past[\Const_i]~\Entails\simplechoice$ and \CIso*;[\simplechoice]\ is \emph{well-formed} and \emph{future-enabled} by~\cref{def:configs_fe}.
            %
            % Therefore \CIso*;[\simplechoice]\ is \emph{live} by definition.
            %
            %
            % ~ rec def -> rec def
            \item\NewCase[$\TypeS'=\mu\alpha'.{\TypeS}''$] 
            Then $\alpha:\Const;\Const~\Entails\mu\alpha'.{\TypeS}''$ and $\alpha:\Const,\alpha':\Const;\Const~\Entails{\TypeS}''$ and \CIso*;[{\TypeS}'']\ is \emph{well-formed}.
            %
            Therefore, \CIso*\ is \emph{live} if \CIso*;[{\TypeS}'']\ is \emph{live} (see other cases).
            %
            %
            % ~ rec def -> end
            \item $\TypeS'=\TypeEnd$ is \emph{live} by~\Cref{def:configs_live}.
            %
            %
            % ~ rec def -> alpha
            \item ${\TypeS'}$ cannot equal $\alpha$ by~\Cref{lem:cfg_wf_neq_alpha}.
            %
        \end{inductivecase}
        %
        %
        %
        % ~ end
        \item\NewCase[$\TypeS=\TypeEnd$]\label{itm:wf_then_live_end} 
        By~\Cref{def:configs_live} it holds that \CIso*;[\TypeEnd]\ is live.
        %
        %
        %
        % ~ alpha
        \item\NewCase[$\TypeS\neq\alpha$] By~\Cref{lem:cfg_wf_neq_alpha}.
        %
    \end{inductivecase}

    \noindent Therefore, it holds that for any $S$ that \CIso*\ is \emph{well-formed}, \CIso*\ is \emph{live}.
    %
\end{proof}
%
%

%

==> tex/proofs/progress/progress.tex <==

% \input{tex/defs/configs/iso/well_formed.tex}

\newcommand{\FullChoice}[0]{\left\{\TypComm_i \,\MsgLabel_i\left\langle T_i\right\rangle \left(\delta_i,\lambda_i\right).\TypeS_i\right\}_{i\in I}}

\begin{lemma}\label{lem:cfg_wf_neq_alpha}
   %
   If \CIso*\ is \emph{well-formed} then $\TypeS\neq\alpha$.
   %
\end{lemma}
\begin{proof}
   %
   By the hypothesis \CIso*\ is \emph{well-formed} meaning $\exists\Const$ such that $\ValClocks\models\Const$ and  $\emptyset;\Const~\Entails\TypeS$.

   Consider by contradiction of the hypothesis that $\TypeS=\alpha$.
   If \CIso*;[\alpha]\ is \emph{well-formed} then, by the judgement of rule \LblTypVar*\ $\alpha:\Const;\Const~\Entails\alpha$ and the evaluation shown in~\Cref{eq:cfg_wf_neq_alpha_eval} must hold, where there must be some recursive definition earlier in the derivation tree $\mu\alpha.\TypeS'$ corresponding to $\alpha$.
   %
   \begin{minieq}\label{eq:cfg_wf_neq_alpha_eval}
   \begin{array}[c]{l}
      \infer[\LblTypRec]{%
         \emptyset;\Const~\Entails\mu\alpha.\TypeS'%
      }{%   
         \infer{\alpha:\Const;\Const~\Entails\TypeS'}{%
            \infer[\vdots]{}{%
               \infer[\LblTypVar]{%
                  \alpha:\Const;\Const~\Entails\alpha%
               }{}%
            }%
         }%
      }
    \end{array}
   \end{minieq}
   
   \noindent If $\exists\ValClocks',\mu\alpha.\TypeS'$ such that \CIso*[\ValClocks'];[\mu\alpha.\TypeS']\ is \emph{well-formed} and \Trans*{\CIso[\ValClocks'];[\mu\alpha.\TypeS']}*[\CIso;[\alpha]], then the immediate transition must be via rule \LblCfgIsoUnfold*\ as shown in~\Cref{eq:cfg_wf_neq_alpha_unfold}; where either $\CIso[{\ValClocks}''];[{\TypeS}'']=\CIso;[\alpha]$ or \Trans*{\CIso[{\ValClocks}''];[{\TypeS}'']}*[\CIso;[\alpha]].
   %
   By the premise of rule \LblCfgIsoUnfold*\ any recursive calls following their definition are replaced by the definition of their next unfolding denoted by $\TypeS'\Subst[\mu\alpha.\TypeS'][\alpha]$.
   %
   \begin{minieq}\label{eq:cfg_wf_neq_alpha_unfold}
   \begin{array}[c]{l}
      \infer[\LblCfgIsoUnfold]{%
      \Trans{\CIso[\ValClocks'];[\mu\alpha.\TypeS']}:{\ProgAction}[\CIso[{\ValClocks}''];[{\TypeS}'']]
      }{%
      \Trans{\CIso[\ValClocks'];[{\TypeS}'\Subst[\mu\alpha.\TypeS'][\alpha]]}:{\ProgAction}[\CIso[{\ValClocks}''];[{\TypeS}'']]
      }
    \end{array}
   \end{minieq}
   
   \noindent Therefore, if \CIso*\ is \emph{well-formed} then $\TypeS\neq\alpha$.
   %
\end{proof}

% \input{tex/defs/configs/iso/live.tex}

\begin{lemma}\label{lem:cfg_wf_end}
   %
   \CIso*;[\TypeEnd]\ is always \emph{well-formed}.
   %
\end{lemma}
\begin{proof}
   %
   By the hypothesis $\exists\Const$ such that $\ValClocks\models\Const$ and $\emptyset;\Const~\Entails\TypeS$, and by rule \LblTypEnd*\ $\emptyset;\TypeTrue~\Entails\TypeEnd$.
%   
   Therefore the hypothesis holds as $\ValClocks\models\TypeTrue$ always holds.
   %
\end{proof}

\input{tex/proofs/progress/lem/wf_then_live.tex}

\begin{lemma}\label{lem:init_wf_then_live}
   %
   Given a \emph{well-formed} \TypeS*, \CIso*[\ValClocks_0]\ is \emph{live}.
   %
\end{lemma}
\begin{proof}
   %
   By~\Cref{def:types_wf}, \Sat*[\ValClocks_0]:[\Past]\ holds for any valid \Const*.
   %
\end{proof}

% ~ configuration transitions
% ! 
\input{tex/proofs/progress/lem/configs_iso_trans.tex}
\input{tex/proofs/progress/lem/configs_soc_trans.tex}

% ~ preservation of wf and compat
% \input{tex/defs/configs/sys/compat.tex}
% \input{tex/defs/configs/iso/latest_en.tex}

% ! 
\input{tex/proofs/progress/lem/configs_trans_wf_preserved.tex}

% ~ time passing
% ! 
% \newpage
\input{tex/proofs/progress/lem/sys_compat_time_trans.tex}

\input{tex/proofs/progress/lem/configs_trans_compat_preserved.tex}

% ~ preservation is preserved 
% ! 
\input{tex/proofs/progress/lem/configs_compat_wf_fe.tex}
\input{tex/proofs/progress/lem/configs_trans_compat_wf_preserved.tex}

% ~ system progress
% ! 
\input{tex/proofs/progress/lem/configs_sys_progress.tex}

% ! thm proof
\ThmProgress*
\begin{proof}
   %
   By~\Cref{def:types_wf}, types \TypeS*\ and \Dual*\ are always \emph{well-formed} against \ValClocks*_0.
   %
   By \Cref{lem:init_wf_then_live} and~\Cref{itm:configs_compat_dual_types} of~\Cref{def:configs_compat}, both \CSoc*[\ValClocks_0]:{\emptyset}\ and \CSoc*[\ValClocks_0];[\Dual]:{\emptyset} are \emph{live} and \emph{compatible}.
   %
   It follows~\Cref{lem:configs_compat_wf_fe,lem:configs_trans_compat_wf_pres} that such as system will always perform actions when possible, waiting if necessary (never missing the \emph{latest-enabled} action), until reaching a \emph{final} configuration, and any \emph{non-final} configuration is guaranteed to be \emph{well-formed}, \emph{compatible} and \emph{live}.

   Therefore, it holds that an initial system composed of dual types that are well-formed is compatible, and guaranteed to \emph{satisfy progress}.
   %
\end{proof}


==> tex/proofs/progress/thm.tex <==
\begin{restatable}[Progress of Systems]{theorem}{ThmProgress}\label{thm:progress}
    %
    If $\TypeS$ is \emph{well-formed} then \CSys*[\CSoc[\ValClocks_0]:{\emptyset}][\CSoc[\ValClocks_0];[\Dual]:{\emptyset}]\ \emph{satisfies progress}.
  \end{restatable}

==> tex/proofs/reduction/lem/configs_viable_actions.tex <==
%
% ! (lemma 23) : only send or recv viable (changed from fe)
\begin{lemma}\label{lem:typing_configs_viable_actions}
    %
    Given a \VIso*\ that is both \emph{well-formed} and \isFE*, both of the following hold:
    \begin{enumerate}
        \item\label{itm:typing_configs_viable_actions_lem_i} If $\exists\Msg$ such that \Trans*{\VIso}:{\SendMsg}\ then $\nexists\Msg'$ such that \Trans*{\VIso}:{\RecvMsg}.
        %
        \item\label{itm:typing_configs_viable_actions_lem_ii} Similarly, if $\exists\Msg$ such that \Trans*{\VIso}:{\RecvMsg}\ then $\nexists\Msg'$ such that \Trans*{\VIso}:{\SendMsg}.
    \end{enumerate}
    %
\end{lemma}
\begin{proof}
    %
    By the hypothesis, the judgement \ITJudgement*;{\Const}[\TypeS]\ holds against the formation rules given in~\cref{fig:types_rule}.
    %
    The proof proceeds considering~\cref{itm:typing_configs_viable_actions_lem_i} of the hypothesis, as~\cref{itm:typing_configs_viable_actions_lem_ii} is similar.
    % $\Trans{\VIso}:{\CommAction}\Implies\Trans{\VIso}:{\CommAction'}$ where $\CommAction\neq\CommAction'$, which are 
    The transition \Trans*{\VIso}:{\SendMsg}\ only possible via either
    \begin{inline}|.
        \item \LblCfgIsoInteract*
        \item \LblCfgIsoUnfold*
    \end{inline} of~\cref{fig:typesemantics}.
    %
    By induction on the depth of the derivation tree, analysing the last rule applied:
    \begin{inductivecase}
        %
        % ~ interact
        \item\NewCase[\LblCfgIsoInteract*]\label{case:typing_configs_viable_actions_interact} Then $\TypeS=\TypInteract$ and $\exists\AsSet[j][i]$ such that \Sat*:[\Const_j]\ and $\TypComm_j=\TypSend$.
        %
        By the hypothesis \TypeS*\ must adhere to the formation rules in~\cref{fig:types_rule}; in particular with \LblTypChoice*.

        Suppose $\exists\AsSet[k][i]$ such that \Sat*:[\Const_k]\ %
        and $\TypComm_k=\TypRecv$,
        and both \Trans*{\CIso}:{\SendMsg_j}\
        and \Trans*{\CIso}:{\RecvMsg_k}\ hold;
        by the premise of \LblTypChoice*, as $\TypComm_j\neq\TypComm_k$ then $\Const_j\cap\Const_k=\emptyset$ must hold.
        and both \Sat*:[\Const_j]\
        and \Sat*:[\Const_k] cannot hold.
        %
        Therefore the hypothesis holds for~\cref{itm:typing_configs_viable_actions_lem_i}, and similarly for~\cref{itm:typing_configs_viable_actions_lem_ii}.
        %
        % ~ recursion
        \item\NewCase[\LblCfgIsoUnfold*]\label{case:typing_configs_viable_actions_recursion} \TODO[recusive case].
        %
    \end{inductivecase}
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/configs_wf_timestep_fe.tex <==
%
% ! (lemma 31) : if iso cfg is fe, and time step wf, then time step fe
\begin{lemma}\label{lem:configs_wf_timestep_fe}
    %
    If \CIso*\ is \isFE*\ %
    and \Trans*{\CSoc}:{\ValTime}[\CSoc+{+\ValTime}]\ %
    and \CIso*+{+\ValTime}\ is \emph{well-formed}, %
    \hfill\ \linebreak%
    then \CIso*+{+\ValTime}\ is \isFE*.
    %
\end{lemma}
\begin{proof}
    %
    By~\cref{def:types_wf,def:configs_wf}, a \emph{well-formed} \TypeS*\ is

    has a \emph{future-enabled} action (see~\cref{def:configs_fe}).
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/delay_defined.tex <==
%
% ! (lemma 35) : delay process defined => no msg waiting ot be received
\begin{lemma}\label{lem:delay_defined}
    %
    If \PFuncTime*\ is defined then $\PFuncWait\cap\PFuncNEQ=\emptyset$.
    %
\end{lemma}
\begin{proof}
    %
    By inspection of~\cref{fig:prc_func_time} the hypothesis holds for any \Prc*\ where \PFuncTime*\ is defined.
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/delayable/defined_delayable.tex <==
%
% ! (lemma 41) : delay defined, fail free, balanced => delayable
\begin{lemma}\label{lem:defined_delayable}
    %
    If \IPJudgement*\ %
    and \PFuncTime*\ is defined and \emph{fail-free}
    and \SesEnv*\ is \emph{balanced},
    then \SesEnv*\ is \emph{delayable}.
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/delayable/delayed_balanced.tex <==
%
% ! (lemma 40) : balanced and delayable => timestep is balanced
\begin{lemma}\label{lem:delayed_balanced}
    %
    If \SesEnv*\ is \emph{balanced} 
    and \emph{delayable}
    and $\SesEnv+\ValTime$ is \emph{well-formed},
    then $\SesEnv+\ValTime$ is \emph{balanced}.
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/delayable/typing_delayed_prc.tex <==
%
% ? (lemma 42) : neq prc, delay defined prc and sesenv => sesenv types delayed prc
\begin{lemma}\label{lem:typing_delayed_prc}
    %
    If \IPJudgement*\ %
    and $\PFuncTime=\Prc'$ is defined and \emph{fail-free}
    and $\PFuncNEQ=\emptyset$
    and $\SesEnv+\ValTime$ is \emph{well-formed},
    then \IPJudgement*<[\Prc']>[\SesEnv+\ValTime].
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/prctyping_inversion.tex <==
%
% ? (lemma 30) : typing a process requirements
\begin{lemma}\label{lem:prc_typ_claims}
    %
    The following claims hold:
    %
\end{lemma}
% ~ (1) typing comm send prc
\begin{claim}\label{claim:prc_typ_claim_comm_send_prc}
    %
    If \IPJudgement*<[\PCalcSend]\ 
    then $\exists\PrcP,\SesEnv'$ such that 
    % \par%
    $\SesEnv=\SesEnv',\PrcP:\CIso;[\TypInteract]$ 
    and $\exists\AsSet[i][\SetI]$ such that
    \Sat*:[\Const_i]\ 
    and $\TypComm_i=\TypSend$ 
    and $\PrcMsg=\MsgType_i$
    and $\PFuncNEQ[\SesEnv]=\emptyset$ 
    and at least one of the following holds:
    \begin{itemize}
        %
        \item %\IMJudgement*{\DataType_\PrcMsg:\DataType_i}\ 
        %and 
        \IPJudgement*>[\SesEnv']:{\PrcP:\CIso+{\ReSet[]}}
        %
        \item $\DataType_i=\TmpTypBTDelegate''$ 
        and \Sat*'\ 
        and $\SesEnv'={\SesEnv}'',\PrcMsg:\CIso'$
        and \IPJudgement*>[{\SesEnv}'']:{\PrcP:\CIso+{\ReSet[]}}
        %
    \end{itemize}
    %
\end{claim}
% ~ typing comm branch prc
\begin{claim}\label{claim:prc_typ_claim_comm_branch_prc}
    %
    If \IPJudgement*<[\PCalcRecv]\ 
    then $\exists\PrcP,\SesEnv'$ such that 
    % \par%
    $\SesEnv=\SesEnv',\PrcP:\CIso;[\TypInteract[j][j]]$ 
    and $\forall\AsSet[j][j]%
    \forall\ValTime<\PrcAfter%
    \forall\ValTime'<\ValTime:$
    $\Trans{\SesEnv'+\ValTime'}|:{\RecvMsg}$
    and $\Sat[\ValClocks+\ValTime']:[\Const_j]$
    and $\exists i,j$ such that
    $\TypComm_j=\TypRecv$ 
    and $\PrcMsg_i=\MsgType_j$
    and $\AsSet[j][k]$
    and $\AsSet[k]\neq\emptyset$
    and $\PFuncNEQ[\SesEnv]=\emptyset$
    %
    and if $\PrcAfter\neq\infty$ 
    then \IPJudgement*<[\Qrc]>[\SesEnv'+\PrcAfter]:{\PrcP:\CIso+{+\PrcAfter};[\TypInteract[j][j]]}.
    %
\end{claim}
% ~ (8) typing comm recv prc
\begin{claim}\label{claim:prc_typ_claim_comm_recv_prc}
    %
    If \IPJudgement*<[\PCalcRecvSingle]\ 
    then $\exists\PrcP,\SesEnv'$ such that
    % \par%
    $\SesEnv=\SesEnv',\PrcP:\CIso;[\TypInteract|]$ 
    and \Sat*\ 
    and $\TypComm=\TypRecv$ 
    and $\PrcMsg=\MsgType$
    and $\PFuncNEQ[\SesEnv]=\emptyset$ 
    and at least one of the following holds for all $\ValTime'<\ValTime$:
    \begin{itemize}
        %
        \item \IPJudgement*:{\PrcMsg:\MsgType}>[\SesEnv'+\ValTime']:{\PrcP:\CIso+{+\ValTime'\ReSet[]}}
        %
        \item $\DataType_\MsgType=\TmpTypBTDelegate''$ 
        and for all \ValClocks*'\ such that \Sat*'\ 
        and \IPJudgement*>[\SesEnv'+\ValTime']:{\PrcP:\CIso+{+\ValTime'\ReSet[]},\PrcMsg:\CIso'}
        %
    \end{itemize}
    %
\end{claim}
% ~ (2) sesenv captures all par prc
\begin{claim}\label{claim:prc_typ_claim_sesenv_par}
    %
    \TODO
    %
\end{claim}
% ~ (5) sesenv scope compat
\begin{claim}\label{claim:prc_typ_claim_sesenv_scope_compat}
    %
    \TODO
    %
\end{claim}
% ~ (6) empty buffers/queues
\begin{claim}\label{claim:prc_typ_claim_empty_buff}
    %
    \TODO[why end only in~\cite{Bocchi2019}?]
    %
\end{claim}
% ~ (7) typing buffers/queues
\begin{claim}\label{claim:prc_typ_claim_buff_queue}
    %
    \TODO[why $ab\PrcTyped ba$ in~\cite{Bocchi2019}?]
    %
\end{claim}
% ~ (9) delay
\begin{claim}\label{claim:prc_typ_claim_delay}
    %
    \TODO
    %
\end{claim}
% ~ (3) prc rec typ
\begin{claim}\label{claim:prc_typ_claim_rec_call}
    %
    \TODO
    %
\end{claim}
% ~ (4) rec prc def 
\begin{claim}\label{claim:prc_typ_claim_rec_def}
    %
    \TODO
    %
\end{claim}
% ! proof
\begin{proof}
    %
    By inspection on the structure of \Prc*\ as in~\cref{sec:prc_calc} typed using the rules in~\cref{fig:prc_typ_rule} using the environments as defined in~\cref{sec:prc_typ_env}.
    %
\end{proof}
%

==> tex/proofs/reduction/lem/typing/delay_defined.tex <==
%
% ! (lemma 37) : delay prc defined => sesenv roles have empty queues
\begin{lemma}\label{lem:typing_delay_defined}
    %
    If \IPJudgement*>:{%
    \PrcP:\CIso_1,%
    \PrcQ:\CIso_2,%
    \ISes:\Queue_2,%
    \ISes|:\Queue_1%
    }\ and \SesEnv*\ is \emph{balanced}
    and \PFuncTime*\ is defined and \emph{fail-free}
    and \Compat*, 
    then $\PrcP\not\in\PFuncNEQ$ 
    and $\PrcQ\not\in\PFuncNEQ$.
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/typing/delayed_fe.tex <==
%
% ! (lemma 39) : balanced and delayable => fe
\begin{lemma}\label{lem:typing_delayed_fe}
    %
    If \IPJudgement*>:{\PrcP:\CIso}\ %
    and \ActFE*!{\CIso}\ %
    and $\PFuncNEQ=\emptyset$
    and \PFuncTime*\ is defined and \emph{fail-free},
    then \ActFE*!{\CIso+{+\ValTime}}.
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/typing/inversion.tex <==
%
% ? (lemma 30) : typing a process requirements
\begin{lemma}\label{lem:prc_typ_claims}
    %
    The following claims hold:
    %
\end{lemma}
%
% ~ (1) typing comm send prc
\begin{claim}\label{claim:prc_typ_claim_comm_send_prc}
    %
    If \IPJudgement*<[\PCalcSend]\ %
    then $\exists\PrcP,\SesEnv'$ such that 
    %
    $\SesEnv=\SesEnv',\PrcP:\CIso;[\TypInteract]$ 
    and $\exists\AsSet[i][\SetI]$ such that
    \Sat*:[\Const_i]\ %
    and $\TypComm_i=\TypSend$ 
    and $\PrcMsg=\MsgType_i$
    and $\PFuncNEQ[\SesEnv]=\emptyset$ 
    and at least one of the following holds:
    \begin{itemize}
        %
        \item \IPJudgement*>[\SesEnv']:{\PrcP:\CIso+{\ReSet[]_i};[\TypeS_i]}
        %
        \item $\DataType_i=\TmpTypBTDelegate''$ 
        and \Sat*'\ %
        and $\SesEnv'={\SesEnv}'',\PrcMsg:\CIso'$
        and \IPJudgement*>[{\SesEnv}'']:{\PrcP:\CIso+{\ReSet[]}}
        %
    \end{itemize}
    %
\end{claim}
%
% ~ typing comm branch prc
\begin{claim}\label{claim:prc_typ_claim_comm_branch_prc}
    %
    If \IPJudgement*<[\PCalcRecv]\ %
    then $\PFuncNEQ[\SesEnv]=\emptyset$
    and $\exists\PrcP,\SesEnv'$ such that
    %
    $\SesEnv=\SesEnv',\PrcP:\CIso;$
    and $\TypeS=\TypInteract[j][j]$ 
    and $\forall\AsSet[j][j]%
    \forall\ValTime<\PrcAfter%
    \forall\ValTime'<\ValTime:$
    $\Trans{\SesEnv'+\ValTime'}|:{\RecvMsg}$
    and $\Sat[\ValClocks+\ValTime']:[\Const_j]$
    and $\exists i,j:\TypComm_j=\TypRecv$ 
    and $\PrcMsg_i=\MsgType_j$
    and $\AsSet[j][k]$
    %
    and $\forall\AsSet[i][i],\AsSet[k][k]$ such that
    $\PrcMsg_i=\MsgType_k:$
    \IPJudgement*<[\ICalcRecv[\PrcMsg_i].{\Prc_i}<{\PrcAfter}]>:{\PrcP:\CIso;[\TypInteract|_[k]]}\ %
    %
    and if $\PrcAfter\neq\infty$ 
    then \IPJudgement*<[\Qrc]>[\SesEnv'+\PrcAfter]:{\PrcP:\CIso+{+\PrcAfter}}.
    %
\end{claim}
%
% ~ (8) typing comm recv prc
\begin{claim}\label{claim:prc_typ_claim_comm_recv_prc}
    %
    If \IPJudgement*<[\PCalcRecvSingle]\ %
    then $\exists\PrcP,\SesEnv'$ such that
    %
    $\SesEnv=\SesEnv',\PrcP:\CIso;[\TypInteract|]$ 
    and \Sat*\ %
    and $\TypComm=\TypRecv$ 
    and $\PrcMsg=\MsgType$
    and $\PFuncNEQ[\SesEnv]=\emptyset$ 
    and at least one of the following holds for all $\ValTime'<\ValTime$:
    \begin{itemize}\vskip-\baselineskip%
        %
        \item \IPJudgement*:{\PrcMsg:\MsgType}>[\SesEnv'+\ValTime']:{\PrcP:\CIso+{+\ValTime'\ReSet[]}}
        %
        \item $\DataType_\MsgType=\TmpTypBTDelegate''$ 
        and $\forall\ValClocks'$ such that ${\Sat'}:$ 
        \IPJudgement*>[\SesEnv'+\ValTime']:{\PrcP:\CIso+{+\ValTime'\ReSet[]},\PrcMsg:\CIso'}
        %
    \end{itemize}
    %
\end{claim}
%
% ~ (2) sesenv captures all par prc
\begin{claim}\label{claim:prc_typ_claim_sesenv_par}
    %
    \TODO
    %
\end{claim}
%
% ~ (5) sesenv scope compat
\begin{claim}\label{claim:prc_typ_claim_sesenv_scope_compat}
    %
    \TODO
    %
\end{claim}
%
% ~ (6) empty buffers/queues
\begin{claim}\label{claim:prc_typ_claim_empty_buff}
    %
    \TODO[why end only in~\cite{Bocchi2019}?]
    %
\end{claim}
%
% ~ (7) typing buffers/queues
\begin{claim}\label{claim:prc_typ_claim_buff_queue}
    %
    \TODO[why $ab\PrcTyped ba$ in~\cite{Bocchi2019}?]
    %
\end{claim}
%
% ~ (9) delay
\begin{claim}\label{claim:prc_typ_claim_delay}
    %
    \TODO
    %
\end{claim}
%
% ~ (3) prc rec typ
\begin{claim}\label{claim:prc_typ_claim_rec_call}
    %
    \TODO
    %
\end{claim}
%
% ~ (4) rec prc def 
\begin{claim}\label{claim:prc_typ_claim_rec_def}
    %
    \TODO
    %
\end{claim}
%
% ! proof
\begin{proof}
    %
    By inspection on the structure of \Prc*\ as in~\cref{sec:prc_calc} typed using the rules in~\cref{fig:prc_typ_rule} using the environments as defined in~\cref{sec:prc_typ_env}.
    %
\end{proof}
%

==> tex/proofs/reduction/lem/typing/iso_wf.tex <==
%
% ! (lemma 36) : roles in sesenv are wf
\begin{lemma}\label{lem:typing_iso_wf}
    %
    If \IPJudgement*>:{\PrcP:\CIso}\ then \CIso*\ is \emph{well-formed}.%
\end{lemma}
\begin{proof}
    %
    By the hypothesis and inspection the rules for typing processes in~\cref{fig:prc_typ_rule}, the last rule applied must be one of the following
    \begin{inline}|
        \item \LblPrcTypBranch*
        \item \LblPrcTypDRecv*
        \item \LblPrcTypVRecv*
        \item \LblPrcTypDSend*
        \item \LblPrcTypVSend*
    \end{inline}
    %
    Each of these rules require \Sat*\ holds as part of their premise.
    %
    By~\cref{def:configs_wf} the hypothesis holds.
    %
\end{proof}
%

==> tex/proofs/reduction/lem/typing/prc_buff_nonempty.tex <==
%
% ! (lemma 33) : queue in sesenv has corresponding prc buffer
\begin{lemma}\label{lem:typing_prc_buff_nonempty}
    %
    If \IPJudgement*>:{\ISes:\Msg;\Queue}\ then $\PrcP\in\PFuncNEQ$.
    %
\end{lemma}
\begin{proof}
    %
    By the hypothesis it must be that $\Prc=\ISes:\Msg\cdot\QHead$.
    By~\cref{fig:prc_func_neq} the hypothesis holds.
    %
\end{proof}
% 

==> tex/proofs/reduction/lem/typing/prc_role_waiting.tex <==
%
% ! (lemma 32) : delay prc and fe recv sesenv role => role is waiting
\begin{lemma}\label{lem:typing_prc_role_waiting}
    %
    If \IPJudgement*>:{\PrcP:\CIso}\ %
    and \PFuncTime*\ is defined 
    and \emph{fail-free} 
    and \Trans*{\CIso}:{\RecvMsg}, 
    then $\PrcP\in\PFuncWait$.
    %
\end{lemma}
\begin{proof}
    %
    By the hypothesis it must be that $\Prc=\PCalcRecv$ (where $\PrcAfter=\infty\Implies\Qrc=\PrcFail$). 
    %
    \Prc*\ cannot be anything else as it is typed against \CIso*, which is able to make a transition via \LblCfgIsoInteract* (where $\TypComm=\TypRecv$).
    %
    Additionally, \PFuncTime*\ being defined ensures that \Prc*\ is not a parallel composition of processes.
    Combined with~\cref{fig:prc_func_wait} the hypothesis holds.
    %
\end{proof}
%
\endinput
if a process typed against a configuration that is currently able to receive and able to let time pass, then the role is currently being waited upon.

==> tex/proofs/reduction/reduction.tex <==

\ThmSubjectReduction*

% ~ wf config actions

% * 23
\begin{lemma}
    %
    If \CIso*\ is \emph{well-formed}
    and $\exists\TypComm,\Msg,\Const$ such that $\ValClocks\models\Const$
    and \Trans*{\CIso}:{\CommMsg},
    then $\forall\TypComm',\Const':
        \TypComm\neq\TypComm'
        ~\implies~
        \ValClocks\not\models\Const'$.
    %
\end{lemma}
\begin{proof}
    %
    By~\cref{lem:cfg_wf_then_live} \CIso*\ is \emph{live}.
    We proceed by induction on the transition \Trans*{\CIso}:{\CommMsg}, analysing the last rule applied:
    \begin{inductivecase}
        %
        %
        % ~ act
        \item\NewCase[\LblCfgIsoInteract*]
        then $\TypeS=\simplechoice$. By the premise of \LblTypChoice*\ the hypothesis holds.
        %
        %
        % ~ unfold
        \item\NewCase[\LblCfgIsoUnfold*]
        then $\TypeS=\mu\alpha.\TypeS'$ and \Trans*{\CIso;[\TypeS']}:{\CommMsg}. The hypothesis holds depending on \TypeS*'; similar to~\cref{itm:cfg_wf_then_live_choice} of~\cref{lem:cfg_wf_then_live} and in~\cref{lem:cfgs_trans_wf_pres,lem:configs_trans_compat_pres}.
        %
    \end{inductivecase}
    %
\end{proof}

% * 31
\begin{lemma}\label{lem:cfg_fe_timepass_wf_fe}
    %
    If \VIso*\ is \isFE*\
    and \Trans*{\VSoc}:{\ValTime}[\VSoc']\
    and \VIso*'\ is \emph{well-formed}
    then \VIso*'\ is \isFE*.
    %
\end{lemma}
\begin{proof}
    %
    By~\cref{lem:cfg_wf_then_live} \VIso*'\ is \emph{live} and either $\TypeS=\TypeEnd$ or \VIso*'\ is \isFE*.
    By induction hypothesis $\exists\ValTime,\TypComm,\Msg$ such that \Trans*{\VSoc}:{\ValTime,\CommMsg}[\VSoc']\ and therefore by the premise of \LblCfgSocTime*\ (persistency) $\exists\ValTime',\TypComm',\Msg'$ such that \Trans*{\VSoc'}:{\ValTime',\TypComm',\Msg'}[\VSoc''].
    %
\end{proof}

% ~ delayed processes
% * 35
\begin{lemma}
    %
    If \PFuncTime*\ is defined
    then $\PFuncWait~\cap~\PFuncNEQ=\emptyset$.
    %
\end{lemma}
\begin{proof}
    %
    Suppose by contradiction that $\PFuncWait~\cap~\PFuncNEQ\neq\emptyset$, then \Prc*\ must be structured such that $\Prc\equiv{\PCalcRecv~\mid~\ISes:\QHead~\mid~\Prc'}$, and by~\cref{fig:prc_func_time} \PFuncTime*\ cannot be defined which contradicts with they hypothesis.
    Therefore $\PFuncWait~\cap~\PFuncNEQ=\emptyset$.
    %
\end{proof}

% * 53
\begin{lemma}\label{lem:timepass_func_defined_t}
    %
    For all \Prc*:
    \begin{enumerate}
        \item\label{itm:timepass_func_defined_t_forall} either \PCalc*{\TimePass_{\ValTime}{\Prc}}\ is defined for all \ValTime*,
        \item\label{itm:timepass_func_defined_t_exists} or, $\exists\ValTime'<\ValTime$ such that \PCalc*{\TimePass_{\ValTime'}{\Prc}}\ is defined for.
    \end{enumerate}
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the structure of \Prc*\ such that \PCalc*{\TimePass_{\ValTime'}{\Prc}}\ being defined is determined by the value of \ValTime*.
    \begin{inductivecase}
        %
        \item\NewCase[\PCalc*{\TimePass_{\ValTime}{\mathtt{delay}({\ValTime}''').\Prc'}}] then $\ValTime\leq{\ValTime}'''$ and~\cref{itm:timepass_func_defined_t_exists} holds.
        %
        \item\NewCase[\PCalc*{\TimePass_{\ValTime}{\PCalcRecv}}] if $\PrcAfter=\infty$ then~\cref{itm:timepass_func_defined_t_forall} holds;
        else $\ValTime\leq\PrcAfter$~\cref{itm:timepass_func_defined_t_exists} holds.
        %
    \end{inductivecase}
    %
\end{proof}

% * 52
\begin{lemma}
    %
    If \PCalc*{\TimePass_{\ValTime}{\Prc}}\ is defined then \PCalc*{\TimePass_{\ValTime+\ValTime'}{\Prc}=\TimePass_{\ValTime}{\TimePass_{\ValTime'}{\Prc}}}.
    %
\end{lemma}
\begin{proof}
    %
    \TODO[check?]
    %
\end{proof}

% ~ typing processes
% * 36
\begin{lemma}\label{lem:typ_prc_role_wf}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,~\ISes:\CIso$
    then \CIso*\ is \emph{well-formed}.
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the typing derivation analysing the last rule applied
    \begin{inline}|
        \item \LblPrcTypDQue*\
        \item \LblPrcTypBranch*\
        \item \LblPrcTypVRecv*\
        \item \LblPrcTypDRecv*\
        \item \LblPrcTypVSend*\
        \item \LblPrcTypDSend*\
    \end{inline}
    Each requires as a premise that $\ValClocks\models\Const$.
    By~\cref{def:types_wf} it follows that \CIso*\ is \emph{well-formed}.
    %
\end{proof}

% * 48
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    and $\Prc\equiv\Qrc$
    then $\VarEnv~\Entails~\Qrc~\PrcTyped~\SesEnv$.
    %
\end{lemma}
\begin{proof}
    %
    It follows as standard, with the addition that $\mathtt{delay}(0).P\equiv\Prc$.
    %
\end{proof}

% * 58
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,\ISes:\Queue$
    then $\exists\QHead,\Prc'$ such that $\Prc\equiv\ISes:\QHead~\mid~\Prc'$.
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the typing derivation of \Prc*, analysing the last rule applied
    \begin{inline}|
        \item \LblPrcTypEmptQ*\
        \item \LblPrcTypVQue*\
        \item \LblPrcTypDQue*\
    \end{inline}
    The hypothesis holds for each, and by the \emph{well-formedness} of processes \Prc*'\ does not contain any other \emph{free-queues}.
    \TODO[check]
    %
\end{proof}

% ~ well-formed processes
\input{tex/defs/processes/free_queues.tex}
\input{tex/defs/processes/well_formed.tex}

% ~ inversion lemma
% * 30
\begin{lemma}[Inversion Lemma]\label{lem:typ_prc_inversion}
    %
    The following claims hold:
    %
    % ~ send
    \begin{claim}
        %
        If $\VarEnv~\Entails~\PCalcSend~\PrcTyped~\SesEnv$
        then $\exists p, \SesEnv'$
        such that $\SesEnv=\SesEnv',~{p:\CIso;[\TypInteract[i][i]]}$
        and $\exists i\in I$
        such that $\ValClocks\models\Const_i$
        and $\TypComm_i=\TypSend$
        and $\PrcLabel=\MsgLabel_i$
        and $\PFuncNEQ[\SesEnv]=\emptyset$
        and either:
        \begin{enumerate}
            %
            % ~ value
            \item $\DataType_i\neq\CIso[\Const]'$
                  and $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv',~{p:\CIso+{\ReSet[]_i};[\TypeS_i]}$.
                  %
                  % ~ delegation
            \item $\DataType_i=\CIso[\Const]'$
                  and $\ValClocks'\models\Const'$
                  and $\exists{\SesEnv}''$ \begin{tabular}[t]{rl}
                      such that & $\SesEnv'={\SesEnv}'',\PrcVal:\CIso'$                                             \\
                      and       & $\VarEnv~\Entails~\Prc~\PrcTyped~{\SesEnv}'',~{p:\CIso+{\ReSet[]_i};[\TypeS_i]}$.
                  \end{tabular}
                  %
        \end{enumerate}
        %
    \end{claim}
    %
    % ~ branch
    \begin{claim}
        %
        If $\VarEnv~\Entails~\PCalcRecv~\PrcTyped~\SesEnv$
        then $\PFuncNEQ[\SesEnv]=\emptyset$
        and $\exists p, \SesEnv'$
        such that $\SesEnv=\SesEnv',~{p:\CIso;[\TypInteract[j][j]]}$
        and $\forall i \in I, \exists j\in j$
        such that $\TypComm_j=\TypRecv$
        and $\PrcLabel_i=\MsgLabel_j$
        and $\forall\ValTime\leq\PrcAfter$
        such that $\ValClocks+\ValTime\models\Const_j$
        and \Trans*{\SesEnv'+\ValTime}|:{\RecvMsg}\
        and:
        \begin{itemize}
            %
            % ~ typing
            \item $\VarEnv+\ValTime~\Entails~\PCalcRecvSingle2{\PrcAfter-\ValTime}_{i}~\PrcTyped~\SesEnv'+\ValTime,~{p:\CIso+{+\ValTime};[\TypInteract|_[j][j]]}$.
                  %
                  % ~ after
            \item $\PrcAfter\neq\infty~\Implies~\VarEnv+\PrcAfter~\Entails~\Qrc~\PrcTyped~\SesEnv'+\PrcAfter,~{p:\CIso+{+\PrcAfter};[\TypInteract[j][j]]}$.
                  %
                  % ~ error
            \item $\Qrc=\PrcErr$ if $\CIso+{+\PrcAfter};[\TypInteract[i][i]]$ is not \emph{well-formed}.
                  %
        \end{itemize}
        %
    \end{claim}
    %
    % ~ recv
    \begin{claim}
        %
        If $\VarEnv~\Entails~\PCalcRecvSingle~\PrcTyped~\SesEnv$
        then $\exists p, \SesEnv'$
        such that $\SesEnv=\SesEnv',~{p:\CIso;[\TypInteract|]}$
        and $\TypComm=\TypRecv$
        and $\PrcLabel=\MsgLabel$
        and $\forall\ValTime\leq\PrcAfter$
        such that $\ValClocks\models\Const$
        and \Trans*{\SesEnv'+\ValTime}|:{\RecvMsg}\
        and $\PFuncNEQ[\SesEnv]=\emptyset$
        and either:
        \begin{enumerate}
            %
            % ~ value
            \item $\DataType\neq\CIso[\Const]'$
                  and $\VarEnv+\ValTime~\Entails~\Prc~\PrcTyped~\SesEnv'+\ValTime,~\PrcMsg:\DataType,~{p:\CIso+{+\ValTime\ReSet[]};[\TypeS]}$.
                  %
                  % ~ delegation
            \item $\DataType=\CIso[\Const]'$
                  and $\ValClocks'\models\Const'$
                  and $\VarEnv+\ValTime~\Entails~\Prc~\PrcTyped~\SesEnv'+\ValTime,~{p:\CIso+{+\ValTime\ReSet[]};[\TypeS]},~\PrcMsg:\CIso'$.
                  %
        \end{enumerate}
        %
    \end{claim}
    %
    % ~ parl
    \begin{claim}
        %
        If $\VarEnv~\Entails~\Parl{\Prc,\Qrc}~\PrcTyped~\SesEnv$
        then $\SesEnv=\SesEnv_1,\SesEnv_2$
        and $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv_1$
        and $\VarEnv~\Entails~\Qrc~\PrcTyped~\SesEnv_2$.
        %
    \end{claim}
    %
    % ~ scope
    \begin{claim}
        %
        If $\VarEnv~\Entails~{(\nu q p)\Prc}~\PrcTyped~\SesEnv$
        then $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,
            ~{p:\VIso_1},
            ~{q:\VIso_2},
            ~{qp:\Queue_1},
            ~{pq:\Queue_2}$
        and \Compat*.
        %
    \end{claim}
    %
    % ~ rec var
    \begin{claim}
        %
        If $\VarEnv~\Entails~\RecPrcCall~\PrcTyped~\SesEnv$
        then $\exists\VarEnv'$
        such that $\VarEnv=\VarEnv',~\EnvPrcVar$
        and $\SesEnv\in\RecSetRoles$
        \linebreak
        and $\forall \DataType\in\RecPrcMsg,\exists \PrcMsg\in\RecSetMsg$
        such that $\VarEnv~\Entails~\PrcMsg:\DataType$
        and $\forall \Const\in\RecPrcTimers,\exists x\in\RecSetTimers$
        such that $x\models\Const$.
        %
    \end{claim}
    %
    % ~ rec def
    \begin{claim}
        %
        If $\VarEnv~\Entails~\PrcRecDef~\PrcTyped~\SesEnv$
        then $\forall \PSesSetCfgs\in\SesSet$
        such that
        \linebreak
        $\VarEnv,~\RecSetMsg:\RecPrcMsg,~\RecSetTimers:\RecPrcTimers,~\RecVar:\EnvPrcVar%
            ~\Entails~%
            \Prc%
            ~\PrcTyped~%
            \RecSetRoles:\PSesSetCfgs$
        and $\VarEnv,~\RecVar:\EnvPrcVar%
            ~\Entails~%
            \Qrc%
            ~\PrcTyped~%
            \SesEnv$.
        %
    \end{claim}
    %
    % ~ par rec
    \begin{claim}
        %
        If $\VarEnv~\Entails~\PrcRecDef>{\Parl{\Qrc,\Qrc'}}~\PrcTyped~\SesEnv$
        then $\SesEnv=\SesEnv_1,\SesEnv_2$
        and $\VarEnv,~\EnvPrcVar~\Entails~\Qrc~\PrcTyped~\SesEnv_1$
        and $\VarEnv,~\EnvPrcVar~\Entails~\Qrc'~\PrcTyped~\SesEnv_2$.
        %
    \end{claim}
    %
    % ~ empty buffer
    \begin{claim}
        %
        If $\VarEnv~\Entails~{qp:\emptyset}~\PrcTyped~\SesEnv$
        then $\exists \SesEnv'$
        such that $\SesEnv=\SesEnv',~{qp:\emptyset}$
        %
    \end{claim}
    %
    % ~ buffer
    \begin{claim}
        %
        If $\VarEnv~\Entails~{qp:\PrcLabel\PrcMsg\cdot\QHead}~\PrcTyped~\SesEnv$
        then $\exists \SesEnv'$
        such that $\SesEnv=\SesEnv',~{qp:\IMsgType[\MsgLabel'];\Queue}$
        and $\PrcLabel=\MsgLabel'$
        then $\PFuncNEQ[\SesEnv]=\emptyset$
        and either:
        \begin{enumerate}
            %
            % ~ value
            \item $\DataType\neq\CIso[\Const]'$
                  and $\VarEnv~\Entails~{\PrcMsg:\DataType}$
                  and $\VarEnv~\Entails~{qp:\QHead}~\PrcTyped~\SesEnv',~{qp:\Queue}$.
                  %
                  % ~ delegation
            \item $\DataType=\CIso[\Const]'$
                  and $\ValClocks'\models\Const'$
                  and $\PrcMsg=q$
                  and $\exists {\SesEnv}''$
                  such that $\SesEnv'={\SesEnv}'',~{q:\CIso'}$
                  and $\VarEnv~\Entails~{qp:\QHead}~\PrcTyped~\SesEnv',~{qp:\Queue}$.
                  %
        \end{enumerate}
        %
    \end{claim}
    %
    % ~ delay
    \begin{claim}
        %
        If $\VarEnv~\Entails~{\mathtt{delay}(\ValTime).\Prc}~\PrcTyped~\SesEnv$
        then $\PFuncNEQ[\SesEnv]=\emptyset$
        and $\forall \ValTime'<\ValTime$
        such that \Trans*{\SesEnv+\ValTime}|:{\RecvMsg}\
        and $\VarEnv+\ValTime~\Entails~\Prc~\PrcTyped~\SesEnv+\ValTime$.
        %
    \end{claim}
    %
\end{lemma}
\begin{proof}
    %
    By inspection of the typing rules for processes in~\cref{fig:prc_typ_rule}, given the structure of \Prc*\ each claim holds.
    %
\end{proof}

% ~ fail free processes
\input{tex/defs/processes/fail_free.tex}

% ~ balanced sessions
In~\cref{def:session_balanced} the notion of compatibility (\cref{def:configs_compat}) is extended from individual system configurations, across all \SesEnv*\ in the balanced set \BalSes*.
%
\input{tex/defs/processes/session/balanced.tex}
\input{tex/defs/processes/session/fully_balanced.tex}

% ~ free queues of session
\input{tex/defs/processes/session/free_queues.tex}

% ~ typing environmental variables
% * 45
\begin{lemma}
    %
    The following hold:
    \begin{enumerate}
        %
        % ~ DRecv
        \item If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,~{p:\CIso}$
              and $\PrcMsg\not\in\SesDomain$
              then $\VarEnv~\Entails~\Prc\Subst[\PrcMsg][p]~\PrcTyped~\SesEnv,~\PrcMsg:\CIso$.
              %
              % ~ VRecv
        \item If $\VarEnv_1,~{\PrcMsg:\DataType}~\Entails~\Prc~\PrcTyped~\SesEnv$
              and $\VarEnv_2~\Entails~{\PrcVal:\DataType}$
              and $\SesDomain[\VarEnv_1]\cap\SesDomain[\VarEnv_2]=\emptyset$
              then \hspace*{\fill}\begin{tabular}[t]{l}\\\llap{$\VarEnv_1,\VarEnv_2~\Entails~\Prc\Subst[\PrcVal][\PrcMsg]~\PrcTyped~\SesEnv$}.\end{tabular}
              %
              % ~ Var
        \item If $\VarEnv_1,~{x:n}~\Entails~\Prc~\PrcTyped~\SesEnv$
              and $\VarEnv_2~\Entails~{y\models\Const}$
              and $\SesDomain[\VarEnv_1]\cap\SesDomain[\VarEnv_2]=\emptyset$
              then \hspace*{\fill}\begin{tabular}[t]{l}\\\llap{$\VarEnv_1,\VarEnv_2~\Entails~\Prc\Subst[y][x]~\PrcTyped~\SesEnv$}.\end{tabular}
              %
    \end{enumerate}
    %
\end{lemma}
\begin{proof}
    %
    By the premise of the relevant typing rule in~\cref{fig:prc_typ_rule}
    \begin{inline}|
        \item \LblPrcTypDRecv*\
        \item \LblPrcTypVRecv*\
        \item \LblPrcTypVar*\
    \end{inline}
    %
\end{proof}

% * 46
\begin{lemma}
    %
    If $\VarEnv~\Entails~{\PrcVal:\DataType}$
    then \DataType*\ is a \emph{base type}.
    %
\end{lemma}
\begin{proof}
    %
    Follows~\cref{fig:prc_typ_rule} that \DataType*\ is not a \emph{delegation type} by inspecting the premise of the relevant typing rule
    \begin{inline}|
        \item \LblPrcTypVSend*\
        \item \LblPrcTypVQue*\
    \end{inline}
    %
\end{proof}

% * 47
\begin{lemma}
    %
    Let $\VarEnv~\Entails~{qp:\QHead}~\PrcTyped~\SesEnv,~{qp:\Queue}$.
    The following hold:
    \begin{itemize}
        %
        % ~ val
        \item If $\VarEnv~\Entails~{\PrcVal:\DataType}$
              then $\VarEnv~\Entails~{qp:\QHead\cdot\PrcVal}~\PrcTyped~\SesEnv,~{qp:\Queue;\DataType}$.
              %
              % ~ delegation
        \item If $\DataType=\CIso[\Const]$
              and $\ValClocks\models\Const$
              and $p\not\in\SesDomain$
              then $\VarEnv~\Entails~{qp:\QHead\cdot p}~\PrcTyped~\SesEnv,~{qp:\Queue;\DataType},~{p:\CIso}$.
              %
    \end{itemize}

    %
\end{lemma}
\begin{proof}
    %
    Follows~\cref{fig:prc_typ_rule} by inspecting the premise of the relevant typing rule
    \begin{inline}|
        \item \LblPrcTypDQue*\
        \item \LblPrcTypVQue*\
    \end{inline}
    %
\end{proof}

% ~ typing receptions
% * 32
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,~{p:\CIso}$
    and \PCalc*{\TimePass{\Prc}}\ is defined and \emph{error-free}
    and $\exists \Msg$
    such that \Trans*{\CIso}:{\RecvMsg}\
    then $p\in\PFuncWait$.
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the transition \Trans*{\CIso}:{\RecvMsg}\ via either
    \begin{inline}|
        \item \LblCfgIsoInteract*\
        \item \LblCfgIsoUnfold*\
    \end{inline}
    \begin{inductivecase}
        %
        % ~ choice
        \item\NewCase[\LblCfgIsoInteract*] then $\TypeS=\simplechoice$.
        By~\cref{lem:typ_prc_role_wf} \CIso*\ is \emph{well-formed} and by~\cref{lem:cfg_wf_then_live} is also \isFE*.
        By inner induction on the typing derivation of the hypothesis.
        \begin{inductivecase}
            %
            % ~ branch
            \item\NewCase[\LblPrcTypBranch*] then $\Prc=\PCalcRecv$ and the hypothesis holds.
            %
            % ~ d recv
            \item\NewCase[\LblPrcTypDRecv*] then $\Prc=\PCalcRecvSingle$ and the hypothesis holds. \LblPrcTypVRecv*\ is similar.
            %
            % ~ rec
            \item\NewCase[\LblPrcTypRec*] then $\Prc=\PrcRecDef$ and the hypothesis depends on the structure of \Qrc*\ (see other cases).
            %
        \end{inductivecase}
        % Cases \LblPrcTypRes*\ and \LblPrcTypPar*\ are straightforward.
        %
    \end{inductivecase}
    We omit case \LblCfgIsoUnfold*\ as $\TypeS=\mu\alpha.\TypeS'$ as it follows~\cref{lem:cfg_wf_then_live,lem:cfgs_trans_wf_pres,lem:configs_trans_compat_pres} that there exist some continuation of \TypeS*\ such that case \LblCfgIsoInteract*\ applies.
    %
\end{proof}

% * 33
\begin{lemma}\label{typ_prc_ses_que_then_neq}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,~{qp:\Msg;\Queue}$
    then $p\in\PFuncNEQ$.
    %
\end{lemma}
\begin{proof}
    %
    By induction on the typing derivation the last rule applied is either
    \begin{inline}|
        \item \LblPrcTypVQue*\
        \item \LblPrcTypDQue*\
    \end{inline}
    \Prc*\ must be structured such that $\VarEnv~\Entails~{qp:\PrcMsg\cdot\QHead}~\PrcTyped~\SesEnv,~{qp:\Msg;\Queue}$ and $\PFuncNEQ[qp:\PrcMsg\cdot\QHead]=\{p\}$.
    %
\end{proof}

% * 34
\begin{lemma}\label{typ_prc_neq_then_ses_que}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    and $p\in\PFuncNEQ$
    then $\exists \SesEnv'$
    such that $\SesEnv=\SesEnv',~{qp:\Msg;\Queue}$.
    %
\end{lemma}
\begin{proof}
    %
    \Prc*\ must be structured such that $\Prc\equiv\Parl{qp:\PrcMsg\cdot\QHead,\Qrc}$.
    The hypothesis follows~\cref{typ_prc_ses_que_then_neq}.
    %
\end{proof}

% ~ delaying processes
% * 37
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,
        ~{p:\VIso_1},
        ~{q:\VIso_2},
        ~{qp:\Queue_1},
        ~{pq:\Queue_2}$
    and \Compat*\
    and \SesEnv*\ is \emph{balanced}
    and \PCalc*{\TimePass{\Prc}}\ is defined and \emph{error-free}
    then $p\not\in\PFuncNEQ$
    and $q\not\in\PFuncNEQ$.
    %
\end{lemma}
\begin{proof}
    %
    We only show the case of $p:\CIso_1$.
    By~\cref{lem:typ_prc_inversion} and \LblPrcTypRes*\ the structure of \Prc*\ must be such that $\Prc\equiv\Parl{\Prc',\Qrc,{qp:\QHead},{pq:\QHead'}}$.
    By the induction hypothesis \PCalc*{\TimePass{\Parl{\Prc',\Qrc,{qp:\QHead},{pq:\QHead'}}}}\ is defined and therefore $p\not\in\PFuncNEQ$.
    %
\end{proof}

% * 39
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv,~{p:\CIso}$
    and \CIso*\ is \isFE*\
    and $\PFuncNEQ=\emptyset$
    and \PCalc*{\TimePass{\Prc}}\ is defined and \emph{error-free}
    then \CIso*+{+\ValTime}\ is \isFE*.
    %
\end{lemma}
\begin{proof}
    %
    By~\cref{lem:cfg_wf_then_live} $\TypeS=\simplechoice$
    and $\exists \Const_i$
    such that $\ValClocks\models\Past[\Const_i]$
    and $\emptyset;\Past[\Const_i]~\Entails~\TypInteract[i][i]$.
    We proceed by induction on the structure of \Prc*\ such that \PCalc*{\TimePass{\Prc}}\ is defined and the value of \ValTime*\ is relevant.
    \begin{inductivecase}
        %
        %
        % ~ delay
        \item\NewCase[$\Prc=\mathtt{delay}(\ValTime').\Prc'$] then $\ValTime\leq\ValTime'$.
        By~\cref{lem:typ_prc_inversion} $\VarEnv+\ValTime'~\Entails~\Prc'~\PrcTyped~\SesEnv+\ValTime',~{p:\CIso+{+\ValTime'}}$ and by~\cref{lem:typ_prc_role_wf} \CIso*+{+\ValTime'}\ is \emph{well-formed}. It follows~\cref{lem:cfg_fe_timepass_wf_fe} that the hypothesis holds.
        %
        %
        % ~ receive
        \item\NewCase[$\Prc=\PCalcRecv$] By~\cref{lem:typ_prc_inversion} and \LblPrcTypBranch*\ $\forall\ValTime'\leq\PrcAfter$ it holds that $\VarEnv+\ValTime'~\Entails~\Prc~\PrcTyped~\SesEnv+\ValTime',~{p:\CIso+{+\ValTime'}}$.
        If $\ValTime>\PrcAfter$ then \PCalc*{\TimePass{\Prc}=\TimePass{\Qrc}}\ and by the hypothesis $\Qrc\neq\PrcErr$.
        By~\cref{lem:typ_prc_role_wf,lem:timepass_func_defined_t} the hypothesis holds.
        Case $\Prc=\PCalcRecvSingle$ is similar.
        %
    \end{inductivecase}
    %
\end{proof}

% ~ delayable sessions
\input{tex/defs/processes/session/delayable.tex}
% * 40
\begin{lemma}
    %
    If \SesEnv*\ is \emph{balanced} and \emph{delayable}
    and $\SesEnv+\ValTime$ is \emph{well-formed}
    then $\SesEnv+\ValTime$ is \emph{balanced}.
    %
\end{lemma}
\begin{proof}
    %
    By~\cref{def:session_balanced} $\SesEnv=\SesEnv',%
        ~{\PrcP:\VIso_1},
        ~{\PrcQ\PrcP:\Queue_1},%
        ~{\PrcQ:\VIso_2},%
        ~{\PrcP\PrcQ:\Queue_2}$
    and \Compat*\ and by~\cref{def:prc_typ_sesenv_delayable} $\Queue_1=\emptyset=\Queue_2$.
    By~\cref{lem:cfgs_trans_wf_pres,lem:configs_trans_compat_pres} if \Compat*\ and \Trans*{\VSoc_1}:{\ValTime}[\VSoc'_1]\ and \Trans*{\VSoc_2}:{\ValTime}[\VSoc'_2]\ then \Compat*'.
    %
\end{proof}

% * 41
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    and \PCalc*{\TimePass{\Prc}}\ is defined
    and \SesEnv*\ is \emph{balanced}
    then \SesEnv*\ is \emph{delayable}.
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the structure of \Prc*\ such that \PCalc*{\TimePass{\Prc}}\ is defined and \emph{well-typed} against a \emph{balanced} \SesEnv*.
    % ~ parl
    If $\Prc=\Parl{\Prc',\Qrc}$ then \PCalc*{\TimePass{\Prc'}}\ and \PCalc*{\TimePass{\Qrc}}\ are defined.
    Suppose by contradiction that \PCalc*{\TimePass{\Prc}}\ is \emph{not} defined. \Prc*'\ and \Qrc*\ must be structured such that $\PFuncWait[\Prc']\cup\PFuncNEQ[\Qrc]\neq\emptyset$ and it must be that $\Prc'=\PCalcRecv[i][i][\Qrc']$ and $\Qrc={qp:\PrcMsg\cdot\QHead}$.
    By~\cref{def:session_balanced} $\exists \SesEnv'$ such that $\SesEnv=\SesEnv',~{p:\CIso_1},~{qp:\Msg;\Queue_1}$ and $\exists \Msg:\Trans{\CIso_1}:{\RecvMsg}$. However as \PCalc*{\TimePass{\Prc}}\ is defined, there are no messages able to be received by \Prc*\ which is \emph{well-typed} against \SesEnv*. Therefore follows that \SesEnv*\ is \emph{delayable} by~\cref{def:prc_typ_sesenv_delayable}.
    %
\end{proof}

% * 42
\begin{lemma}\label{lem:well_typed_delayed_prc}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    and \PCalc*{\TimePass{\Prc}}\ is defined and \emph{error-free}
    and $\PFuncNEQ=\emptyset$
    and $\SesEnv+\ValTime$ is \emph{well-formed}
    then $\VarEnv+\ValTime~\Entails~\PCalc{\TimePass{\Prc}}~\PrcTyped~\SesEnv+\ValTime$.
    %
\end{lemma}
\begin{proof}
    %
    We proceed by induction on the structure of \Prc*\ such that \PCalc*{\TimePass{\Prc}}\ is defined and \emph{error-free}.
    \begin{inductivecase}
        %
        %
        % ~ recv
        \item\NewCase[$\Prc=\PCalcRecv$] By~\cref{lem:typ_prc_inversion} $\SesEnv=\SesEnv',~{p:\CIso;[\simplechoice_{j}]}$.
        By inner induction on the typing derivation analysing the last rule applied: \LblPrcTypBranch*\ %(and \LblPrcTypDRecv*, \LblPrcTypVRecv*)
        \begin{inductivecase}
            %
            % ~ t <= n
            \item\NewCase[If $\ValTime\leq\PrcAfter$ then] $\forall \ValTime'\leq\PrcAfter-\ValTime$~\cref{eq:well_typed_delayed_prc_branch} holds and $\forall {\ValTime}''\leq\ValTime:\Trans{\SesEnv+\ValTime'+{\ValTime}''}|:{\RecvMsg}$ and $\forall j\in J$ such that $\ValClocks+\ValTime+\ValTime'\models\Const_j~\implies~\TypComm_j=\TypRecv$ and $\exists i\in I$ such that $\PrcLabel_i=\MsgLabel_j$ and:
            \begin{itemize}
                %
                % ~ val
                \item$\DataType_j\neq\CIso[\Const]~\implies~\VarEnv+\ValTime+\ValTime',\PrcMsg_i:\DataType_j~\Entails~\Prc_i~\PrcTyped~\SesEnv+\ValTime+\ValTime',~{p:\CIso+{+\ValTime+\ValTime'\ReSet[]_j};[\TypeS_j]}$.
                %
                % ~ delegation
                \item$\DataType_j=\CIso[\Const]~\implies~\VarEnv+\ValTime+\ValTime'~\Entails~\Prc_i~\PrcTyped~\SesEnv+\ValTime+\ValTime',~{p:\CIso+{+\ValTime+\ValTime'\ReSet[]_j};[\TypeS_j]},~{\PrcMsg_i:\CIso'}$ %\linebreak \hspace*{\fill} 
                and $\ValClocks'\models\Const'$.
                %
            \end{itemize}
            \begin{minieq}\label{eq:well_typed_delayed_prc_branch}
                \VarEnv+\ValTime+\ValTime'~\Entails~\PCalcRecv2{\PrcAfter-(\ValTime+\ValTime')}~\PrcTyped~\SesEnv+\ValTime+\ValTime',~{p:\CIso+{+\ValTime+\ValTime'};[\simplechoice_{j}]}
            \end{minieq}\vspace{-4ex}%
            %
            % ~ t > n
            \item\NewCase[If $\ValTime>\PrcAfter$ then] \PCalc*{\TimePass{\Prc}=\TimePass_{\ValTime-\PrcAfter}{\Qrc}}\ and $\Qrc\neq\PrcErr$ and $\VarEnv+\PrcAfter~\Entails~{\Qrc}~\PrcTyped~\SesEnv+\PrcAfter$. It follows by induction hypothesis $\VarEnv+\ValTime~\Entails~\PCalc{\TimePass_{\ValTime-\PrcAfter}{\Qrc}}~\PrcTyped~\SesEnv+\ValTime$.
            %
        \end{inductivecase}
        %
        %
        % ~ delay
        \item\NewCase[$\Prc=\mathtt{delay}(\ValTime').\Prc'$] then $\ValTime\leq\ValTime'$ and $\forall {\ValTime}''\leq\ValTime':\Trans{\SesEnv+{\ValTime}''}|:{\RecvMsg}$. By induction hypothesis $\VarEnv+\ValTime~\Entails~{\mathtt{delay}(\ValTime'-\ValTime).\Prc'}~\PrcTyped~\SesEnv+\ValTime$.
        %
        %
        % ~ parl
        \item\NewCase[$\Prc=\Parl{\Prc',\Qrc}$] By~\cref{lem:typ_prc_inversion} $\SesEnv=\SesEnv_1,\SesEnv_2$.
        %
        %
        % ~ scope
        \item\NewCase[$\Prc=(\nu qp)\Prc'$] By~\cref{lem:typ_prc_inversion} $\SesEnv=\SesEnv',~{p:\CIso;[\simplechoice_{j}]}$.
        %
    \end{inductivecase}
    %
\end{proof}

% ~ typing delayed processes
% * 43
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    then
    %
\end{proof}

% * 44
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    then
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% ~ typing reduction steps
% * 49
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    then
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 50
\begin{lemma}
    %
    If $\VarEnv~\Entails~\Prc~\PrcTyped~\SesEnv$
    then
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% ~ fail-free processes
% * 51
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 52
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 54
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% ~ fail free reduction
% * 55
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 56
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 57
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 62
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 61
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% ~ untimed processes
% * 60
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% * 63
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

% ~ subject reduction
% * 64
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

\endinput

% * 
\begin{lemma}
    %
    %
\end{lemma}
\begin{proof}
    %
    %
\end{proof}

\begin{definition}[Future-enabled Actions (\isFE*$\TypSend/\TypRecv$)]\label{def:fe_actions}
    %
    A configuration \VIso*\
    is \isFE*\
    if $\exists\ValTime,\TypComm,\Msg$
    such that \Trans*{\VIso}:{\ValTime,\CommMsg}[\VIso'];
    \VIso*\ is \isFE*!\ if $\TypComm=\TypSend$,
    and is \isFE*?\ if $\TypComm=\TypRecv$.
    %
\end{definition}

\input{tex/defs/processes/fail_free.tex}

In~\cref{def:session_balanced} the notion of compatibility (\cref{def:configs_compat}) is extended from individual system configurations, across all \SesEnv*\ in the balanced set \BalSes*.
%
\input{tex/defs/processes/session/balanced.tex}
\input{tex/defs/processes/session/fully_balanced.tex}

\input{tex/defs/processes/session/free_queues.tex}

% ~ future enabled
\input{tex/proofs/reduction/lem/configs_viable_actions.tex} % 23
\input{tex/proofs/reduction/lem/configs_wf_timestep_fe.tex} % 31

% ~ typing judgements
\input{tex/proofs/reduction/lem/typing/inversion.tex} % 30
\input{tex/proofs/reduction/lem/typing/iso_wf.tex} % 36
% 48

% ~ substitution lemma
% 45
% 46

% ~ delaying processes
\input{tex/proofs/reduction/lem/typing/prc_role_waiting.tex} % 32
\input{tex/proofs/reduction/lem/typing/prc_buff_nonempty.tex} % 33
\input{tex/proofs/reduction/lem/delay_defined.tex} % 35

% ~ typing delayed processes
\input{tex/proofs/reduction/lem/typing/delay_defined.tex} % 37
\input{tex/proofs/reduction/lem/typing/delayed_fe.tex} % 39

% * time passing sesenv
% A \SesEnv*\ is delayable given that for every non-empty queue, there does not exist a role capable of receiving from it.
\input{tex/defs/processes/session/delayable.tex}

\input{tex/proofs/reduction/lem/delayable/delayed_balanced.tex} % 40
\input{tex/proofs/reduction/lem/delayable/defined_delayable.tex} % 41
\input{tex/proofs/reduction/lem/delayable/typing_delayed_prc.tex} % 42

% 43
% 44

% 47

% ~ typing preserved across session reduction
\input{tex/figs/processes/session_reduction.tex}
% 49
% 50

% ~ fail free delay
% 51
% 52
% 53
% 54

% ~ fail free session
% 55

% ! TODO: untimed ? ? ? ? ?

% ! (lemma 43) : timestep preserve balanced sesenv
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ? (lemma 44) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 45) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 46) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 47) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 49) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 50) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 52) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 54) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 55) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 56) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 57) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 58) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 59) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 60) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 61) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 62) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 63) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ! (lemma 64) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

\endinput

% ! (lemma ) : 
\begin{lemma}%\label{lem:}
    %
    \TODO
    %
\end{lemma}
\begin{proof}
    %
    \TODO
    %
\end{proof}

% ~ () 
\begin{claim}
    %
    \TODO
    %
\end{claim}


==> tex/proofs/reduction/thm.tex <==
%
% ~
\begin{restatable}[Subject Reduction of Processes]{theorem}{ThmSubjectReduction}\label{thm:subject_reduction}
    %
    Let ${(\RedTimers,~P)}$ be \emph{live}.
    If $\emptyset\;\Entails\,\Prc\;\PrcTyped\,\emptyset$ and ${(\RedTimers,~P)}~\longrightarrow~{(\RedTimers',~P')}$, then $\emptyset\;\Entails\,\Prc'\;\PrcTyped\,\emptyset$.
    %
\end{restatable}
%

==> tex/workings/prc_typ_timer_recursion.tex <==

% \endinput

\subsection{Example Types \& Processes}

\begin{equation}
    \begin{array}[c]{r c l}
        %
        \TypeS & = & %
        \IChoice[%
            \IType?{a}[x\leq 1][x].{%
                \IType!{c}.{%
                    \IRecDef[a].{%
                        \IChoice[%
                            \IType?{d}[x\leq 1],%
                            \IType!{e}[1<x].{\IRecCall[a]}%
                        ]%
                    }%
                }%
            },%
            \IType!{b}[2<x<3]%
        ]%
        %
        \\[2ex]%
        \\[2ex]%
        \Prc & = & %
        \PSet{x}.{%
            \PRecv[a]:{% * recv
                \PSet{x}.{%
                    \PSend[c].{%
                        \PDefRec:{%
                            \PRecv[d]<{1}>{% * after
                                \PRec%
                            }%
                        }%
                    }%
                }%
            }<{1}>{% * after 1
                \PDelay[t=1].{%
                    \PIf[2<x<3]% * use defaults (then end, else fail)
                }%
            }%
        }%
        %
    \end{array}
\end{equation}

\begin{equation}
    \begin{array}[c]{r c l}
        %
        \Dual[\TypeS] & = & %
        \IChoice[%
            \IType!{a}[y\leq 1][y].{%
                \IType?{c}.{%
                    \IRecDef[b].{%
                        \IChoice[%
                            \IType!{d}[y\leq 1],%
                            \IType?{e}[1<y].{\IRecCall[b]}%
                        ]%
                    }%
                }%
            },%
            \IType?{b}[2<y<3]%
        ]%
        %
        \\[2ex]%
        \\[2ex]%
        \Qrc & = & %
        \PSet{y}.{%
            \PIf[y\leq 1]:{\PThen[%
                \PSend_{q}[a].{%
                    \PSet{y}.{%
                        \PRecv_{q}[c]:{%
                            \PDefRec:{%
                                \PIf[y\leq 1]:{\PThen[%
                                    \PSend_{q}[d]%
                                ]}:{\PElse[%
                                    \PRecv_{q}[e]:{%
                                        \PRec%
                                    }%
                                ]}%
                            }%
                        }%
                    }%
                }%
            ]}:{\PElse[%
                \PDelay[t=1].{%
                    \PRecv[b]<{1}% * after: failed
                }%
            ]}%
        }%
        %
    \end{array}
\end{equation}

\subsection{Experiments}

\begin{equation}
    %
    \Tup(1,2,3 ,5, 3)%
    %
\end{equation}

\begin{equation}
    %
    \Tup(\ValClocks, \IType)%
    %
\end{equation}


\begin{equation}
    %
    \ITypeAct%
    \ITypeAct!%
    \ITypeAct?%
    %
\end{equation}

\subsubsection{Configs}


\subsection{judgements}


\begin{itemize}
    \item \IPJudgement*
    \item \IPJudgement*[\VarEnv_1]:{\PrcMsg:\DataType_\MsgType}<[\Qrc]>[\SesEnv_2]:{\PrcP\PrcQ:\emptyset}
    \item \IPJudgement*>[\SesEnv_2]:{\PrcP\PrcQ:\emptyset}
    \item \IPJudgement*<[\Qrc]>
    \item \IPJudgement*[\VarEnv_1]:{\PrcMsg:\DataType_\MsgType}
\end{itemize}

\begin{equation}
    %
    \IPJudgement<[\PCalcSend]
    %
\end{equation}

\begin{itemize}
    \item \ITJudgement*%
    \item \ITJudgement*:{\alpha:(x<3)}%
    \item \ITJudgement*[R]:{\alpha,\beta};{x\leq3}_{j}<{\SetJ}%
    \item \ITJudgement*;{y\leq3\land3\geq x}%
    \item \ITJudgement*-{\IType!{a}[x<3][x],\IType?{b}[x>3][x]}%
\end{itemize}

\begin{equation}
    %
    \ITJudgement[R]:{%
            \alpha:(x=3)%
        };{x=4}-{%
            \IType!{a}[x<3],%
            \IType?{b}[x<5],%
            \IType!{c}[x=6],%
            \dots%
        }%
    %
\end{equation}

\subsection{Process Typing}

% % ~ 
% \NewDocumentCommand\ListToInlineArgs{>{\SplitList{,}}m}
% {%
%     \ProcessList{#1}{\HeadItemToInlineArgs}%
% }

% % ~ 
% \newcommand\HeadItemToInlineArgs[1]{%
%     {#1}%
%     \let\HeadItemToInlineArgs\TailItemToInlineArgs%
% }

% % ~ inserts | before each subsequent par item
% \newcommand\TailItemToInlineArgs[1]{%
%     \ \\\ {#1}%
%     \let\HeadItemToInlineArgs\TailItemToInlineArgs% * rebinding due to outer processor being unscoped
% }

\begin{equation}
    \IEval[test]:{
        \FmtJudgement|{a}{b}
    }:{\Premise[%
        1,%
        2,%
        \IEval[test2]:{%
            \FmtJudgement|{c}{d}[e]%
        }:{\Premise[%
            \IEval<[test3]:{%
                \FmtJudgement|{f}{g}[h]%
            }:{\Premise[%
                3,4,5%
            ]},%
            6,%
            \IEval[test4]:{%
                \FmtJudgement|{i}{j}%
            }:{\Premise[%
                7,8,9%
            ]},%
            10%
        ]},%
        11%
    ]}%
\end{equation}

\subsection{actual examples}

\subsubsection{types}

\def\typeslz{\TypeS_{0}}
\def\typesli{\TypeS_{1}}
\def\typeslii{\TypeS_{2}}
\def\typesliii{\TypeS_{3}}
\def\typesliv{\TypeS_{4}}
\def\typeslv{\TypeS_{5}}
\def\typeslvi{\TypeS_{6}}
\def\typeslvii{\TypeS_{7}}

\def\typetlz{\Dual[\TypeS]_{0}}
\def\typetli{\Dual[\TypeS]_{1}}
\def\typetlii{\Dual[\TypeS]_{2}}
\def\typetliii{\Dual[\TypeS]_{3}}
\def\typetliv{\Dual[\TypeS]_{4}}
\def\typetlv{\Dual[\TypeS]_{5}}
\def\typetlvi{\Dual[\TypeS]_{6}}
\def\typetlvii{\Dual[\TypeS]_{7}}

\def\typesz{\IChoice|[\typesli,\typeslvii]}
\def\typesi{\IType?{a}[x\leq 1][x].{\typeslii}}
\def\typesii{\IType!{c}.{\typesliii}}
\def\typesiii{\IRecDef[a].{\typesliv}}
\def\typesiv{\IChoice|[\typeslv,\typeslvi]}
\def\typesv{\IType?{d}[x\leq 1]}
\def\typesvi{\IType!{e}[1<x].{\IRecCall[a]}}
\def\typesvii{\IType!{b}[2<x<3]}

\def\typetz{\IChoice|[\typetli,\typetlvii]}
\def\typeti{\IType!{a}[y\leq 1][y].{\typetlii}}
\def\typetii{\IType?{c}.{\typetliii}}
\def\typetiii{\IRecDef[b].{\typetliv}}
\def\typetiv{\IChoice|[\typetlv,\typetlvi]}
\def\typetv{\IType!{d}[y\leq 1]}
\def\typetvi{\IType?{e}[1<y].{\IRecCall[b]}}
\def\typetvii{\IType?{b}[2<y<3]}

\begin{equation}
    %
    \begin{array}[t]{l c l}%
        %
        \TypeS & = & %
        \IChoice[%
            \IType?{a}[x\leq 1][x].{%
                \IType!{c}.{%
                    \IRecDef[a].{%
                        \IChoice[%
                            \IType?{d}[x\leq 1],%
                            \IType!{e}[1<x].{\IRecCall[a]}%
                        ]%
                    }%
                }%
            },%
            \IType!{b}[2<x<3]%
        ]%
        %
        \\[2ex]%
        \\[2ex]%
        \Dual[\TypeS] & = & %
        \IChoice[%
            \IType!{a}[y\leq 1][y].{%
                \IType?{c}.{%
                    \IRecDef[b].{%
                        \IChoice[%
                            \IType!{d}[y\leq 1],%
                            \IType?{e}[1<y].{\IRecCall[b]}%
                        ]%
                    }%
                }%
            },%
            \IType?{b}[2<y<3]%
        ]%
        %
    \end{array}%
    %
\end{equation}

\begin{equation}
    %
    \begin{array}[t]{l c l c l p{2ex} l c l c l }%
        %
        \TypeS & ::= & \typeslz & = & \typesz & &%
        \Dual[\TypeS] & ::= & \typetlz & = & \typetz \\%
        %
        & \mid & \typesli & = & \typesi & &%
        & \mid & \typetli & = & \typeti \\%
        %
        & \mid & \typeslii & = & \typesii & &%
        & \mid & \typetlii & = & \typetii \\%
        %
        & \mid & \typesliii & = & \typesiii & &%
        & \mid & \typetliii & = & \typetiii \\%
        %
        & \mid & \typesliv & = & \typesiv & &%
        & \mid & \typetliv & = & \typetiv \\%
        %
        & \mid & \typeslv & = & \typesv & &%
        & \mid & \typetlv & = & \typetv \\%
        %
        & \mid & \typeslvi & = & \typesvi & &%
        & \mid & \typetlvi & = & \typetvi \\%
        %
        & \mid & \typeslvii & = & \typesvii & &%
        & \mid & \typetlvii & = & \typetvii%
        %
    \end{array}%
    %
\end{equation}

\subsubsection{processes}

\def\prclz{\Prc_{0}}
\def\prcli{\Prc_{1}}
\def\prclii{\Prc_{2}}
\def\prcliii{\Prc_{3}}
\def\prcliv{\Prc_{4}}
\def\prclv{\Prc_{5}}
\def\prclvi{\Prc_{6}}
\def\prclvii{\Prc_{7}}

\def\qrclz{\Qrc_{0}}
\def\qrcli{\Qrc_{1}}
\def\qrclii{\Qrc_{2}}
\def\qrcliii{\Qrc_{3}}
\def\qrcliv{\Qrc_{4}}
\def\qrclv{\Qrc_{5}}
\def\qrclvi{\Qrc_{6}}
\def\qrclvii{\Qrc_{7}}
\def\qrclviii{\Qrc_{8}}
\def\qrclix{\Qrc_{9}}
\def\qrclx{\Qrc_{10}}
\def\qrclxi{\Qrc_{11}}

\def\prcz{\PSet{x}.{\prcli}}
\def\prci{\PRecv[a]:{\prclii}<{1}>{\prclvi}}
\def\prcii{\PSet{x}.{\prcliii}}
\def\prciii{\PSend[c].{\prcliv}}
\def\prciv{\PDefRec_{a}={\prcliv}:{\prclv}}
\def\prcv{\PRecv[d]<{1}>{\PRec_{a}}}
\def\prcvi{\PDelay[t=1].{\prclvii}}
\def\prcvii{\PIf[2<x<3]}

\def\qrcz{\PSet{y}.{\qrcli}}
\def\qrci{\PDelay[y\leq 1].{\qrclii}}% ~ delay inserted
\def\qrcia{\PDelay{y}.{\qrclii}}% ~ delay resolved
\def\qrcib{\PDelay{y}.{\qrclii}}% ~ delay resolved
\def\qrcic{\PDelay{y}.{\qrclii}}% ~ delay resolved
\def\qrcii{\PIf[y\leq 1]:{\PThen[\qrcliii]}:{\PElse[\qrclx]}}
\def\qrciii{\PSend_{q}[a].{\qrcliv}}
\def\qrciv{\PSet{y}.{\qrclv}}
\def\qrcv{\PRecv_{q}[c]:{\qrclvi}}
\def\qrcvi{\PDefRec_{b}={\qrcliv}:{\qrclvii}}
\def\qrcvii{\PIf[y\leq 1]:{\PThen[\qrclviii]}:{\PElse[\qrclix]}}
\def\qrcviii{\PSend_{q}[d]}
\def\qrcix{\PRecv_{q}[e]:{\PRec_{b}}}
\def\qrcx{\PDelay[t=1].{\qrclxi}}
\def\qrcxi{\PRecv[b]<{1}}

\begin{equation}
    %
    \begin{array}[t]{l c l}%
        %
        \Prc & = & %
        \PSet{x}.{%
            \PRecv[a]:{% * recv
                \PSet{x}.{%
                    \PSend[c].{%
                        \PDefRec:{%
                            \PRecv[d]<{1}>{% * after
                                \PRec%
                            }%
                        }%
                    }%
                }%
            }<{1}>{% * after 1
                \PDelay[t=1].{%
                    \PIf[2<x<3]% * use defaults (then end, else fail)
                }%
            }%
        }%
        %
        \\[2ex]%
        \\[2ex]%
        \Qrc & = & %
        \PSet{y}.{%
            \PIf[y\leq 1]:{\PThen[%
                \PSend_{q}[a].{%
                    \PSet{y}.{%
                        \PRecv_{q}[c]:{%
                            \PDefRec:{%
                                \PIf[y\leq 1]:{\PThen[%
                                    \PSend_{q}[d]%
                                ]}:{\PElse[%
                                    \PRecv_{q}[e]:{%
                                        \PRec%
                                    }%
                                ]}%
                            }%
                        }%
                    }%
                }%
            ]}:{\PElse[%
                \PDelay[t=1].{%
                    \PRecv[b]<{1}% * after: failed
                }%
            ]}%
        }%
        %
    \end{array}%
    %
\end{equation}

\begin{equation}
    %
    \begin{array}[t]{c p{2ex} c}%
        \begin{array}[t]{l c l c l}%
            %
            \Prc & ::= & \prclz & = & \prcz \\% 
            & \mid & \prcli & = & \prci \\%
            & \mid & \prclii & = & \prcii \\%
            & \mid & \prcliii & = & \prciii \\%
            & \mid & \prcliv & = & \prciv \\%
            & \mid & \prclv & = & \prcv \\%
            & \mid & \prclvi & = & \prcvi \\%
            & \mid & \prclvii & = & \prcvii %
            %
        \end{array}%
        & & %
        \begin{array}[t]{l c l c l}%
            %
            \Qrc & ::= & \qrclz & = & \qrcz \\% 
            & \mid & \qrcli & = & \qrci \\%
            & \mid & \qrclii & = & \qrcii \\%  
            & \mid & \qrcliii & = & \qrciii \\%
            & \mid & \qrcliv & = & \qrciv \\%
            & \mid & \qrclv & = & \qrcv \\%
            & \mid & \qrclvi & = & \qrcvi \\%
            & \mid & \qrclvii & = & \qrcvii \\%
            & \mid & \qrclviii & = & \qrcviii \\%
            & \mid & \qrclix & = & \qrcix \\%
            & \mid & \qrclx & = & \qrcx %
            %
        \end{array}%
    \end{array}%
    %
\end{equation}

\pagebreak
\subsubsection{using compacted versions}

\begin{equation}
    %
    \begin{array}[t]{l c l c l p{2ex} l c l c l }%
        %
        \TypeS & ::= & \typeslz & = & \typesz & &%
        \Dual[\TypeS] & ::= & \typetlz & = & \typetz \\%
        %
        & \mid & \typesli & = & \typesi & &%
        & \mid & \typetli & = & \typeti \\%
        %
        & \mid & \typeslii & = & \typesii & &%
        & \mid & \typetlii & = & \typetii \\%
        %
        & \mid & \typesliii & = & \typesiii & &%
        & \mid & \typetliii & = & \typetiii \\%
        %
        & \mid & \typesliv & = & \typesiv & &%
        & \mid & \typetliv & = & \typetiv \\%
        %
        & \mid & \typeslv & = & \typesv & &%
        & \mid & \typetlv & = & \typetv \\%
        %
        & \mid & \typeslvi & = & \typesvi & &%
        & \mid & \typetlvi & = & \typetvi \\%
        %
        & \mid & \typeslvii & = & \typesvii & &%
        & \mid & \typetlvii & = & \typetvii%
        %
    \end{array}%
    %
\end{equation}

\begin{equation}
    %
    \begin{array}[t]{c p{2ex} c}%
        \begin{array}[t]{l c l c l}%
            %
            \Prc & ::= & \prclz & = & \prcz \\% 
            & \mid & \prcli & = & \prci \\%
            & \mid & \prclii & = & \prcii \\%
            & \mid & \prcliii & = & \prciii \\%
            & \mid & \prcliv & = & \prciv \\%
            & \mid & \prclv & = & \prcv \\%
            & \mid & \prclvi & = & \prcvi \\%
            & \mid & \prclvii & = & \prcvii %
            %
        \end{array}%
        & & %
        \begin{array}[t]{l c l c l}%
            %
            \Qrc & ::= & \qrclz & = & \qrcz \\% 
            & \mid & \qrcli & = & \qrci \\%
            & \mid & \qrclii & = & \qrcii \\%  
            & \mid & \qrcliii & = & \qrciii \\%
            & \mid & \qrcliv & = & \qrciv \\%
            & \mid & \qrclv & = & \qrcv \\%
            & \mid & \qrclvi & = & \qrcvi \\%
            & \mid & \qrclvii & = & \qrcvii \\%
            & \mid & \qrclviii & = & \qrcviii \\%
            & \mid & \qrclix & = & \qrcix \\%
            & \mid & \qrclx & = & \qrcx \\%
            & \mid & \qrclxi & = & \qrcxi %
            %
        \end{array}%
    \end{array}%
    %
\end{equation}

\def\sespq{\ISes[\PrcP][\PrcQ]}
\def\sesqp{\ISes[\PrcQ][\PrcP]}

\begin{equation}
    %
    \resizebox{\textwidth}{!}{$%
        \IEval[Scope]:{\IPJudgement<[% * process
            \IScope.{\Parl{%
                \prclz,\qrclz,%
                \IBuff[\sespq],%
                \IBuff[\sesqp]%
        }}]>:{% * session
            \PrcP:\CIso[\ValClocks_0];[\typeslz],%
            \PrcQ:\CIso[\ValClocks_0];[\typetlz]~,%
            \IQue[\sespq],%
            \IQue[\sesqp]%
        }}:{\Premise[%
            \IEval[Timer]:{\IPJudgement<[% * process
                \prcz,\qrcz,%
                \IBuff[\sespq],%
                \IBuff[\sesqp]%
            ]>:{% * session
                \PrcP:\CIso[\ValClocks_0];[\typesz],%
                \PrcQ:\CIso[\ValClocks_0];[\typetz]~,%
                \IQue[\sespq],%
                \IQue[\sesqp]%
            }}:{\Premise[%
                \IEval[Timer]:{\IPJudgement:{% * vars
                    x:0
                }<[% * process
                    \prci,\qrcz,%
                    \IBuff[\sespq],%
                    \IBuff[\sesqp]%
                ]>:{% * session
                    \PrcP:\CIso[\ValClocks_0];[\typesz],%
                    \PrcQ:\CIso[\ValClocks_0];[\typetz]~,%
                    \IQue[\sespq],%
                    \IQue[\sesqp]%
                }}:{\Premise[%
                    \IEval[Del\Const*]:{\IPJudgement:{% * vars
                        x:0,y:0
                    }<[% * process
                        \prci,\qrci,%
                        \IBuff[\sespq],%
                        \IBuff[\sesqp]%
                    ]>:{% * session
                        \PrcP:\CIso[\ValClocks_0];[\typesz],%
                        \PrcQ:\CIso[\ValClocks_0];[\typetz]~,%
                        \IQue[\sespq],%
                        \IQue[\sesqp]%
                    }}:{\Premise[%
                        \IEval[Del\Const*]:{\IPJudgement:{% * vars
                            x:0,y:0
                        }<[% * process
                            \prci,\qrci,%
                            \IBuff[\sespq],%
                            \IBuff[\sesqp]%
                        ]>:{% * session
                            \PrcP:\CIso[\ValClocks_0];[\typesz],%
                            \PrcQ:\CIso[\ValClocks_0];[\typetz]~,%
                            \IQue[\sespq],%
                            \IQue[\sesqp]%
                        }}:{\Premise[%
                        ]}
                    ]}
                ]}
            ]}
        ]}
    $}
    %
\end{equation}

\endinput

\begin{equation}
    %
    \resizebox{\textwidth}{!}{$%
        \IEval[Del\Const*]:{\IPJudgement<[% * process
            \PDelay[x=1].{\Prc^{*}},%
            \PDelay[y=1].{\Qrc^{*}},%
            \IBuff[\ISes[\PrcP][\PrcQ]],%
            \IBuff[\ISes[\PrcQ][\PrcP]]%
        ]>:{% * session
            \PrcP:\CIso,%
            \PrcQ:\CIso,%
            \IQue[\ISes[\PrcP][\PrcQ]],%
            \IQue[\ISes[\PrcQ][\PrcP]]%
        }}:{\Premise[%
            \IEval[Del\Const*]:{\IPJudgement<[% * process
                \PDelay[1].{\Prc^{*}},%
                \PDelay[y=1].{\Qrc^{*}},%
                \IBuff[\ISes[\PrcP][\PrcQ]],%
                \IBuff[\ISes[\PrcQ][\PrcP]]%
            ]>:{% * session
                \PrcP:\CIso,%
                \PrcQ:\CIso,%
                \IQue[\ISes[\PrcP][\PrcQ]],%
                \IQue[\ISes[\PrcQ][\PrcP]]%
            }}:{\Premise[%
                \IEval[Delt]:{\IPJudgement<[% * process
                    \PDelay[1].{\Prc^{*}},%
                    \PDelay[1].{\Qrc^{*}},%
                    \IBuff[\ISes[\PrcP][\PrcQ]],%
                    \IBuff[\ISes[\PrcQ][\PrcP]]%
                ]>:{% * session
                    \PrcP:\CIso,%
                    \PrcQ:\CIso,%
                    \IQue[\ISes[\PrcP][\PrcQ]],%
                    \IQue[\ISes[\PrcQ][\PrcP]]%
                }}:{\Premise[%
                    \IEval[Delt]:{\IPJudgement<[% * process
                        \PSend_{\PrcP}[a].{\Prc^{*}},%
                        \PDelay[0].{\Qrc^{*}},%
                        \IBuff[\ISes[\PrcP][\PrcQ]],%
                        \IBuff[\ISes[\PrcQ][\PrcP]]%
                    ]>:{% * session
                        \PrcP:\CIso,%
                        \PrcQ:\CIso,%
                        \IQue[\ISes[\PrcP][\PrcQ]],%
                        \IQue[\ISes[\PrcQ][\PrcP]]%
                    }}:{\Premise[%
                        \IEval[VSend]:{\IPJudgement<[% * process
                            \PSend_{\PrcP}[a].{\Prc^{*}},%
                            \PRecv_{q}[a]:{\Qrc^{*}}<{0}>{{\Qrc'}^{*}},%
                            \IBuff[\ISes[\PrcP][\PrcQ]],%
                            \IBuff[\ISes[\PrcQ][\PrcP]]%
                        ]>:{% * session
                            \PrcP:\CIso,%
                            \PrcQ:\CIso,%
                            \IQue[\ISes[\PrcP][\PrcQ]],%
                            \IQue[\ISes[\PrcQ][\PrcP]]%
                        }}:{\Premise[%
                            \IMJudgement{% * msg typing
                                \IMsg{b}:{\DataType_{a_{i}}}%
                            },%
                            \IEval[VRecv]:{\IPJudgement<[% * process
                                \PRecv_{p}[b]:{\Prc^{*}}<{1}>{{\Prc'}^{*}},%
                                \PRecv_{q}[a]:{\Qrc^{*}}<{0}>{{\Qrc'}^{*}},%
                                \IBuff[\ISes[\PrcP][\PrcQ]]:{a},%
                                \IBuff[\ISes[\PrcQ][\PrcP]]%
                            ]>:{% * session
                                \PrcP:\CIso,%
                                \PrcQ:\CIso,%
                                \IQue[\ISes[\PrcP][\PrcQ]]:{a},%
                                \IQue[\ISes[\PrcQ][\PrcP]]%
                            }}:{\Premise[%
                                \IEval[VRecv]:{\IPJudgement<[% * process
                                    \PRecv_{p}[b]:{\Prc^{*}}<{1}>{{\Prc'}^{*}},%
                                    \PRecv_{q}[a]:{\Qrc^{*}}<{0}>{{\Qrc'}^{*}},%
                                    \IBuff[\ISes[\PrcP][\PrcQ]]:{a},%
                                    \IBuff[\ISes[\PrcQ][\PrcP]]%
                                ]>:{% * session
                                    \PrcP:\CIso,%
                                    \PrcQ:\CIso,%
                                    \IQue[\ISes[\PrcP][\PrcQ]]:{a},%
                                    \IQue[\ISes[\PrcQ][\PrcP]]%
                                }}:{\Premise[%
                                ]}%
                            ]}%
                        ]}%
                    ]}%
                ]}%
            ]}%
        ]}%
    $}%
    %
\end{equation}
\endinput


\begin{equation}\label{eq:example_prctyp_ia_yleqi_then}%
    \resizebox{\textwidth}{!}{$%
        \infer[%
            {\begin{array}[t]{l l}%
                \RName[Timer] & x,y%
                \\[2ex]\ValClocks_1 = \ValClocks_2%
            \end{array}}%
        ]{%
            \begin{array}{c c c c c c c c c c c c c c c c c c c c c}%
                % * var env (Gamma)
                \VarEnv,\emptyset & %
                \Entails & %
                % * processes
                \PSet{x}.{\dots} & %
                \mid &%
                \PSet{y}.{\dots} & %
                \mid &%
                pq:\emptyset & %
                \mid &%
                qp:\emptyset & %
                %
                \PrcTyped & %
                %
                % * session (Delta)
                \SesEnv & %
                , & %
                % * configs
                \CfgIso_p & %
                , & % 
                \CfgIso_q2{\Dual[\TypeS]} & %
                , & % 
                pq:\emptyset & %
                , & %
                qp:\emptyset%
                %
                \\[1ex]% * for annotations
                & % var env (Gamma)
                & % imp
                \Prc & % p1
                & % |
                \Qrc & % q1
                & % |
                & % pq
                & % |
                & % qp
                & % typed by
                & % session (Delta)
                & % ,
                & % cfg p
                & % ,
                & % cfg q
                & % ,
                & % pq
                & % ,
                & % qp
            \end{array}%
        }{%
            \infer[%
                {\begin{array}[t]{l l}%
                    \RName[IfStmt] & \text{then}%
                    \\ \text{for ELSE see:}%\cref{eq:example_prctyp_ib_yleqi_else}}%
                \end{array}}%
            ]{%
                \begin{array}{c c c c c c c c c c c c c c c c c c c c c}%
                    % * var env (Gamma)
                    \VarEnv,\emptyset & %
                    \Entails & %
                    % * processes
                    \PRecv_{p}[a]:{\dots}<{1}>{\dots} %
                    & \mid &%
                    %
                    \PIf[y\leq 1]:{\PThen[%
                        \dots%
                    ]}:{\PElse[%
                        \dots%
                    ]}%
                    & \mid &%
                    %
                    pq:\emptyset & \mid &%
                    qp:\emptyset & %
                    %
                    \PrcTyped & %
                    %
                    % * session (Delta)
                    \SesEnv & , & %
                    % * configs
                    \CfgIso_p & , & % 
                    \CfgIso_q2{\Dual[\TypeS]} & , & % 
                    pq:\emptyset & , & %
                    qp:\emptyset%
                    %
                \end{array}%
            }{%
                \infer[%
                    {\begin{array}[t]{l l}%
                        \RName[VSend] & \circled{$\mathtt{a}$}%
                    \end{array}}%
                ]{%
                    \begin{array}{c c c c c c c c c c c c c c c c c c c c c}%
                        % * var env (Gamma)
                        \VarEnv,\emptyset & %
                        \Entails & %
                        % * processes
                        \PRecv_{p}[a]:{\dots}<{1}>{\dots} %
                        & \mid &%
                        %
                        \PSend_{q}[a].{\dots}%
                        & \mid &%
                        %
                        pq:\emptyset%
                         & \mid &%
                        qp:\emptyset & %
                        %
                        \PrcTyped & %
                        %
                        % * session (Delta)
                        \SesEnv & , & %
                        % * configs
                        \CfgIso_p & , & % 
                        \CfgIso_q2{\Dual[\TypeS]} & , & % 
                        pq:\emptyset & , & %
                        qp:\emptyset%
                        %
                    \end{array}%
                }{%
                    \infer[%
                        {\begin{array}[t]{l l}%
                            \RName[VRecv] & \circled{$\mathtt{a}$}%
                        \end{array}}%
                    ]{%
                        \begin{array}{c c c c c c c c c c c c c c c c c c c c c}%
                            % * var env (Gamma)
                            \VarEnv,\emptyset & %
                            \Entails & %
                            % * processes
                            \PRecv_{p}[a]:{\dots}<{1}>{\dots} %
                            & \mid &%
                            %
                            \PSet{y}.{\dots}%
                            & \mid &%
                            %
                            pq:\emptyset%
                            & \mid &%
                            qp:\circled{$\mathtt{a}$} & %
                            %
                            \PrcTyped & %
                            %
                            % * session (Delta)
                            \SesEnv & , & %
                            % * configs
                            \CfgIso_p & , & % 
                            \CfgIso_q2{\Dual[\TypeS]} & , & % 
                            pq:\emptyset & , & %
                            qp:\squared{$\mathtt{a}$}%
                            %
                        \end{array}%
                    }{%
                        \infer[%
                            {\begin{array}[t]{l l}%
                                \RName[Timer] & x,y%
                            \end{array}}%
                        ]{%
                            \begin{array}{c c c c c c c c c c c c c c c c c c c c c}%
                                % * var env (Gamma)
                                \VarEnv,\emptyset & %
                                \Entails & %
                                % * processes
                                \PSet{x}.{\dots} %
                                & \mid &%
                                %
                                \PSet{y}.{\dots}%
                                & \mid &%
                                %
                                pq:\emptyset%
                                & \mid &%
                                qp:\emptyset & %
                                %
                                \PrcTyped & %
                                %
                                % * session (Delta)
                                \SesEnv & , & %
                                % * configs
                                \CfgIso_p & , & % 
                                \CfgIso_q2{\Dual[\TypeS]} & , & % 
                                pq:\emptyset & , & %
                                qp:\emptyset%
                                %
                            \end{array}%
                        }{%
                        \dots%
                        }%
                    }%
                }%
            }%
        }%
    $}%
\end{equation}

\begin{equation}\label{eq:example_prctyp_ib_yleqi_else}%
    \resizebox{\textwidth}{!}{$%
        \infer[%
            {\begin{array}[t]{l l}%
                \RName[IfStmt] & \text{else}%
                \\ \text{for THEN see:}%~\cref{eq:example_prctyp_ia_yleqi_then}]%
            \end{array}}%
        ]{%
            \begin{array}{c c c c c c c c c c c c c c c c c c c}%
                % * var env (Gamma)
                \VarEnv,\emptyset & %
                \Entails & %
                % * processes
                \PRecv_{p}[a]:{\dots}<{1}>{\dots} %
                & \mid &%
                %
                \PIf[y\leq 1]:{\PThen[%
                    \dots%
                ]}:{\PElse[%
                    \dots%
                ]}%
                & \mid &%
                %
                pq:\emptyset & \mid &%
                qp:\emptyset & %
                %
                \PrcTyped & %
                %
                % * session (Delta)
                \SesEnv & , & %
                % * configs
                \CfgIso_p & , & % 
                \CfgIso_q2{\Dual[\TypeS]} & , & % 
                pq:\emptyset & , & %
                qp:\emptyset%
                %
            \end{array}%
        }{%
            \infer[%
                {\begin{array}[t]{l l}%
                    \RName[Timer] & x,y%
                \end{array}}%
            ]{%
                \begin{array}{c c c c c c c c c c c c c c c c c c c}%
                    % * var env (Gamma)
                    \VarEnv,\emptyset & %
                    \Entails & %
                    % * processes
                    \PRecv_{p}[a]:{\dots}<{1}>{\dots} %
                    & \mid &%
                    %
                    \PSend_{q}[a].{\dots}%
                    & \mid &%
                    %
                    pq:\emptyset & \mid &%
                    qp:\emptyset & %
                    %
                    \PrcTyped & %
                    %
                    % * session (Delta)
                    \SesEnv & , & %
                    % * configs
                    \CfgIso_p & , & % 
                    \CfgIso_q2{\Dual[\TypeS]} & , & % 
                    pq:\emptyset & , & %
                    qp:\emptyset%
                    %
                \end{array}%
            }{%
            }
        }
    $}%    
\end{equation}

\endinput


\begin{equation}
    \begin{array}[c]{r c l}
        \Prc & = & %
        \PBranch[%
            \PRecv|[b],%
            \PRecv|[d]:{%
                \PRecv[f]:{%
                    \PSend[g]%
                }<{3}>{%
                    \PSend_{q}[c]%
                }%
            },%
            \PRecv|[e]:{%
                \PSend%
            }%
        ]<{1}>{%
            \PSend.{%
                \PBranch[%
                    \PRecv|[h]:{%
                        \PSend[i]%
                    },%
                    \PRecv|[j]%
                ]%
            }%
        }%
        %
    \end{array}
\end{equation}



% ~ 
\NewDocumentCommand{\IPrcSend}{s E|{\PrcP}}{%
    \IfBooleanT{#1}{$}%
    \mathtt{to}\,{#2}%
    \mathtt{->}\,{}
    \IfBooleanT{#1}{$}%
}

\endinput

\begin{equation}
    \IChoice
\end{equation}

\begin{equation}
    \IChoice[\IType,\IType]
\end{equation}

\begin{equation}
    \IType!{a}
\end{equation}



\endinput

\begin{equation}
    \IChoice[%
        \IType?{a}[x\leq 1][x].{%
            \IType!{c}.{%
                \IRecDef[a].{%
                    \IChoice[%
                        \IType?{d}[x\leq 1],%
                        \IType!{e}[1<x].{%
                            \IChoice[%
                                \IType?{d}[x\leq 1],%
                                \IType!{e}[1<x].{%
                                    \IChoice[%
                                        \IType?{d}[x\leq 1],%
                                        \IType!{e}[1<x].{\IRecCall[a]}%
                                    ]%
                                }%
                            ]%
                        }%
                    ]%
                }%
            }%
        },%
        \IType!{b}[2<x<3]%
    ]%
\end{equation}

\endinput

